Personalized Treatment Selection using Causal Heterogeneity

Randomized experimentation (also known as A/B testing or bucket testing) is widely used in the internet industry to measure the metric impact obtained by different treatment variants. A/B tests identify the treatment variant showing the best performance, which then becomes the chosen or selected treatment for the entire population. However, the effect of a given treatment can differ across experimental units and a personalized approach for treatment selection can greatly improve upon the usual global selection strategy. In this work, we develop a framework for personalization through (i) estimation of heterogeneous treatment effect at either a cohort or member-level, followed by (ii) selection of optimal treatment variants for cohorts (or members) obtained through (deterministic or stochastic) constrained optimization. We perform a two-fold evaluation of our proposed methods. First, a simulation analysis is conducted to study the effect of personalized treatment selection under carefully controlled settings. This simulation illustrates the differences between the proposed methods and the suitability of each with increasing uncertainty. We also demonstrate the effectiveness of the method through a real-life example related to serving notifications at Linkedin. The solution significantly outperformed both heuristic solutions and the global treatment selection baseline leading to a sizable win on top-line metrics like member visits.

==> Definitions.tex <==
\RequirePackage{latexsym}
%\RequirePackage{amsmath}
% \RequirePackage{amsthm}
%\RequirePackage{amssymb}
\RequirePackage{bm}

%%%%%%%% Stock standard definitions %%%%%%%%%%%%%%%

\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\abtil}{\tilde{\ab}}
\newcommand{\bbtil}{\tilde{\bb}}
\newcommand{\cbtil}{\tilde{\cbb}}
\newcommand{\dbtil}{\tilde{\db}}
\newcommand{\ebtil}{\tilde{\eb}}
\newcommand{\fbtil}{\tilde{\fb}}
\newcommand{\gbtil}{\tilde{\gb}}
\newcommand{\hbtil}{\tilde{\hb}}
\newcommand{\ibtil}{\tilde{\ib}}
\newcommand{\jbtil}{\tilde{\jb}}
\newcommand{\kbtil}{\tilde{\kb}}
\newcommand{\lbtil}{\tilde{\lb}}
\newcommand{\mbtil}{\tilde{\mb}}
\newcommand{\nbtil}{\tilde{\nbb}}
\newcommand{\obtil}{\tilde{\ob}}
\newcommand{\pbtil}{\tilde{\pb}}
\newcommand{\qbtil}{\tilde{\qb}}
\newcommand{\rbtil}{\tilde{\rb}}
\newcommand{\sbtil}{\tilde{\sbb}}
\newcommand{\tbtil}{\tilde{\tb}}
\newcommand{\ubtil}{\tilde{\ub}}
\newcommand{\vbtil}{\tilde{\vb}}
\newcommand{\wbtil}{\tilde{\wb}}
\newcommand{\xbtil}{\tilde{\xb}}
\newcommand{\ybtil}{\tilde{\yb}}
\newcommand{\zbtil}{\tilde{\zb}}

\newcommand{\atil}{\tilde{a}}
\newcommand{\btil}{\tilde{b}}
\newcommand{\ctil}{\tilde{c}}
\newcommand{\dtil}{\tilde{d}}
\newcommand{\etil}{\tilde{e}}
\newcommand{\ftil}{\tilde{f}}
\newcommand{\gtil}{\tilde{g}}
\newcommand{\htil}{\tilde{h}}
\newcommand{\itil}{\tilde{i}}
\newcommand{\jtil}{\tilde{j}}
\newcommand{\ktil}{\tilde{k}}
\newcommand{\ltil}{\tilde{l}}
\newcommand{\mtil}{\tilde{m}}
\newcommand{\ntil}{\tilde{n}}
\newcommand{\otil}{\tilde{o}}
\newcommand{\ptil}{\tilde{p}}
\newcommand{\qtil}{\tilde{q}}
\newcommand{\rtil}{\tilde{r}}
\newcommand{\stil}{\tilde{s}}
\newcommand{\ttil}{\tilde{t}}
\newcommand{\util}{\tilde{u}}
\newcommand{\vtil}{\tilde{v}}
\newcommand{\wtil}{\tilde{w}}
\newcommand{\xtil}{\tilde{x}}
\newcommand{\ytil}{\tilde{y}}
\newcommand{\ztil}{\tilde{z}}

\newcommand{\ahat}{\hat{a}}
\newcommand{\bhat}{\hat{b}}
\newcommand{\chat}{\hat{c}}
\newcommand{\dhat}{\hat{d}}
\newcommand{\ehat}{\hat{e}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\ihat}{\hat{i}}
\newcommand{\jhat}{\hat{j}}
\newcommand{\khat}{\hat{k}}
\newcommand{\lhat}{\hat{l}}
\newcommand{\mhat}{\hat{m}}
\newcommand{\nhat}{\hat{n}}
\newcommand{\ohat}{\hat{o}}
\newcommand{\phat}{\hat{p}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\rhat}{\hat{r}}
\newcommand{\shat}{\hat{s}}
\newcommand{\that}{\hat{t}}
\newcommand{\uhat}{\hat{u}}
\newcommand{\vhat}{\hat{v}}
\newcommand{\what}{\hat{w}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\yhat}{\hat{y}}
\newcommand{\zhat}{\hat{z}}

\newcommand{\abhat}{\hat{\ab}}
\newcommand{\bbhat}{\hat{\bb}}
\newcommand{\cbhat}{\hat{\cb}}
\newcommand{\dbhat}{\hat{\db}}
\newcommand{\ebhat}{\hat{\eb}}
\newcommand{\fbhat}{\hat{\fb}}
\newcommand{\gbhat}{\hat{\gb}}
\newcommand{\hbhat}{\hat{\hb}}
\newcommand{\ibhat}{\hat{\ib}}
\newcommand{\jbhat}{\hat{\jb}}
\newcommand{\kbhat}{\hat{\kb}}
\newcommand{\lbhat}{\hat{\lb}}
\newcommand{\mbhat}{\hat{\mb}}
\newcommand{\nbhat}{\hat{\nb}}
\newcommand{\obhat}{\hat{\ob}}
\newcommand{\pbhat}{\hat{\pb}}
\newcommand{\qbhat}{\hat{\qb}}
\newcommand{\rbhat}{\hat{\rb}}
\newcommand{\sbhat}{\hat{\sb}}
\newcommand{\tbhat}{\hat{\tb}}
\newcommand{\ubhat}{\hat{\ub}}
\newcommand{\vbhat}{\hat{\vb}}
\newcommand{\wbhat}{\hat{\wb}}
\newcommand{\xbhat}{\hat{\xb}}
\newcommand{\ybhat}{\hat{\yb}}
\newcommand{\zbhat}{\hat{\zb}}

\newcommand{\Atil}{\tilde{A}}
\newcommand{\Btil}{\tilde{B}}
\newcommand{\Ctil}{\tilde{C}}
\newcommand{\Dtil}{\tilde{D}}
\newcommand{\Etil}{\tilde{E}}
\newcommand{\Ftil}{\tilde{F}}
\newcommand{\Gtil}{\tilde{G}}
\newcommand{\Htil}{\tilde{H}}
\newcommand{\Itil}{\tilde{I}}
\newcommand{\Jtil}{\tilde{J}}
\newcommand{\Ktil}{\tilde{K}}
\newcommand{\Ltil}{\tilde{L}}
\newcommand{\Mtil}{\tilde{M}}
\newcommand{\Ntil}{\tilde{N}}
\newcommand{\Otil}{\tilde{O}}
\newcommand{\Ptil}{\tilde{P}}
\newcommand{\Qtil}{\tilde{Q}}
\newcommand{\Rtil}{\tilde{R}}
\newcommand{\Stil}{\tilde{S}}
\newcommand{\Ttil}{\tilde{T}}
\newcommand{\Util}{\tilde{U}}
\newcommand{\Vtil}{\tilde{V}}
\newcommand{\Wtil}{\tilde{W}}
\newcommand{\Xtil}{\tilde{X}}
\newcommand{\Ytil}{\tilde{Y}}
\newcommand{\Ztil}{\tilde{Z}}

\newcommand{\abar}{\bar{a}}
\newcommand{\bbar}{\bar{b}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\dbar}{\bar{d}}
\newcommand{\ebar}{\bar{e}}
\newcommand{\fbar}{\bar{f}}
\newcommand{\gbar}{\bar{g}}
\newcommand{\hbr}{\bar{h}}
\newcommand{\ibar}{\bar{i}}
\newcommand{\jbar}{\bar{j}}
\newcommand{\kbar}{\bar{k}}
\newcommand{\lbar}{\bar{l}}
\newcommand{\mbar}{\bar{m}}
\newcommand{\nbar}{\bar{n}}
\newcommand{\obar}{\bar{o}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\qbar}{\bar{q}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\tbar}{\bar{t}}
\newcommand{\ubar}{\bar{u}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\wbar}{\bar{w}}
\newcommand{\xbar}{\bar{x}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\zbar}{\bar{z}}

\newcommand{\abbar}{\bar{\ab}}
\newcommand{\bbbar}{\bar{\bb}}
\newcommand{\cbbar}{\bar{\cb}}
\newcommand{\dbbar}{\bar{\db}}
\newcommand{\ebbar}{\bar{\eb}}
\newcommand{\fbbar}{\bar{\fb}}
\newcommand{\gbbar}{\bar{\gb}}
\newcommand{\hbbar}{\bar{\hb}}
\newcommand{\ibbar}{\bar{\ib}}
\newcommand{\jbbar}{\bar{\jb}}
\newcommand{\kbbar}{\bar{\kb}}
\newcommand{\lbbar}{\bar{\lb}}
\newcommand{\mbbar}{\bar{\mb}}
\newcommand{\nbbar}{\bar{\nbb}}
\newcommand{\obbar}{\bar{\ob}}
\newcommand{\pbbar}{\bar{\pb}}
\newcommand{\qbbar}{\bar{\qb}}
\newcommand{\rbbar}{\bar{\rb}}
\newcommand{\sbbar}{\bar{\sbb}}
\newcommand{\tbbar}{\bar{\tb}}
\newcommand{\ubbar}{\bar{\ub}}
\newcommand{\vbbar}{\bar{\vb}}
\newcommand{\wbbar}{\bar{\wb}}
\newcommand{\xbbar}{\bar{\xb}}
\newcommand{\ybbar}{\bar{\yb}}
\newcommand{\zbbar}{\bar{\zb}}

\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sbb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

\newcommand{\Abtil}{\tilde{\Ab}}
\newcommand{\Bbtil}{\tilde{\Bb}}
\newcommand{\Cbtil}{\tilde{\Cb}}
\newcommand{\Dbtil}{\tilde{\Db}}
\newcommand{\Ebtil}{\tilde{\Eb}}
\newcommand{\Fbtil}{\tilde{\Fb}}
\newcommand{\Gbtil}{\tilde{\Gb}}
\newcommand{\Hbtil}{\tilde{\Hb}}
\newcommand{\Ibtil}{\tilde{\Ib}}
\newcommand{\Jbtil}{\tilde{\Jb}}
\newcommand{\Kbtil}{\tilde{\Kb}}
\newcommand{\Lbtil}{\tilde{\Lb}}
\newcommand{\Mbtil}{\tilde{\Mb}}
\newcommand{\Nbtil}{\tilde{\Nb}}
\newcommand{\Obtil}{\tilde{\Ob}}
\newcommand{\Pbtil}{\tilde{\Pb}}
\newcommand{\Qbtil}{\tilde{\Qb}}
\newcommand{\Rbtil}{\tilde{\Rb}}
\newcommand{\Sbtil}{\tilde{\Sbb}}
\newcommand{\Tbtil}{\tilde{\Tb}}
\newcommand{\Ubtil}{\tilde{\Ub}}
\newcommand{\Vbtil}{\tilde{\Vb}}
\newcommand{\Wbtil}{\tilde{\Wb}}
\newcommand{\Xbtil}{\tilde{\Xb}}
\newcommand{\Ybtil}{\tilde{\Yb}}
\newcommand{\Zbtil}{\tilde{\Zb}}

\newcommand{\Abar}{\bar{A}}
\newcommand{\Bbar}{\bar{B}}
\newcommand{\Cbar}{\bar{C}}
\newcommand{\Dbar}{\bar{D}}
\newcommand{\Ebar}{\bar{E}}
\newcommand{\Fbar}{\bar{F}}
\newcommand{\Gbar}{\bar{G}}
\newcommand{\Hbar}{\bar{H}}
\newcommand{\Ibar}{\bar{I}}
\newcommand{\Jbar}{\bar{J}}
\newcommand{\Kbar}{\bar{K}}
\newcommand{\Lbar}{\bar{L}}
\newcommand{\Mbar}{\bar{M}}
\newcommand{\Nbar}{\bar{N}}
\newcommand{\Obar}{\bar{O}}
\newcommand{\Pbar}{\bar{P}}
\newcommand{\Qbar}{\bar{Q}}
\newcommand{\Rbar}{\bar{R}}
\newcommand{\Sbar}{\bar{S}}
\newcommand{\Tbar}{\bar{T}}
\newcommand{\Ubar}{\bar{U}}
\newcommand{\Vbar}{\bar{V}}
\newcommand{\Wbar}{\bar{W}}
\newcommand{\Xbar}{\bar{X}}
\newcommand{\Ybar}{\bar{Y}}

\newcommand{\Abbar}{\bar{\Ab}}
\newcommand{\Bbbar}{\bar{\Bb}}
\newcommand{\Cbbar}{\bar{\Cb}}
\newcommand{\Dbbar}{\bar{\Db}}
\newcommand{\Ebbar}{\bar{\Eb}}
\newcommand{\Fbbar}{\bar{\Fb}}
\newcommand{\Gbbar}{\bar{\Gb}}
\newcommand{\Hbbar}{\bar{\Hb}}
\newcommand{\Ibbar}{\bar{\Ib}}
\newcommand{\Jbbar}{\bar{\Jb}}
\newcommand{\Kbbar}{\bar{\Kb}}
\newcommand{\Lbbar}{\bar{\Lb}}
\newcommand{\Mbbar}{\bar{\Mb}}
\newcommand{\Nbbar}{\bar{\Nb}}
\newcommand{\Obbar}{\bar{\Ob}}
\newcommand{\Pbbar}{\bar{\Pb}}
\newcommand{\Qbbar}{\bar{\Qb}}
\newcommand{\Rbbar}{\bar{\Rb}}
\newcommand{\Sbbar}{\bar{\Sb}}
\newcommand{\Tbbar}{\bar{\Tb}}
\newcommand{\Ubbar}{\bar{\Ub}}
\newcommand{\Vbbar}{\bar{\Vb}}
\newcommand{\Wbbar}{\bar{\Wb}}
\newcommand{\Xbbar}{\bar{\Xb}}
\newcommand{\Ybbar}{\bar{\Yb}}
\newcommand{\Zbbar}{\bar{\Zb}}

\newcommand{\Ahat}{\hat{A}}
\newcommand{\Bhat}{\hat{B}}
\newcommand{\Chat}{\hat{C}}
\newcommand{\Dhat}{\hat{D}}
\newcommand{\Ehat}{\hat{E}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\Ghat}{\hat{G}}
\newcommand{\Hhat}{\hat{H}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\Khat}{\hat{K}}
\newcommand{\Lhat}{\hat{L}}
\newcommand{\Mhat}{\hat{M}}
\newcommand{\Nhat}{\hat{N}}
\newcommand{\Ohat}{\hat{O}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Shat}{\hat{S}}
\newcommand{\That}{\hat{T}}
\newcommand{\Uhat}{\hat{U}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\What}{\hat{W}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\Yhat}{\hat{Y}}
\newcommand{\Zhat}{\hat{Z}}

\newcommand{\Abhat}{\hat{\Ab}}
\newcommand{\Bbhat}{\hat{\Bb}}
\newcommand{\Cbhat}{\hat{\Cb}}
\newcommand{\Dbhat}{\hat{\Db}}
\newcommand{\Ebhat}{\hat{\Eb}}
\newcommand{\Fbhat}{\hat{\Fb}}
\newcommand{\Gbhat}{\hat{\Gb}}
\newcommand{\Hbhat}{\hat{\Hb}}
\newcommand{\Ibhat}{\hat{\Ib}}
\newcommand{\Jbhat}{\hat{\Jb}}
\newcommand{\Kbhat}{\hat{\Kb}}
\newcommand{\Lbhat}{\hat{\Lb}}
\newcommand{\Mbhat}{\hat{\Mb}}
\newcommand{\Nbhat}{\hat{\Nb}}
\newcommand{\Obhat}{\hat{\Ob}}
\newcommand{\Pbhat}{\hat{\Pb}}
\newcommand{\Qbhat}{\hat{\Qb}}
\newcommand{\Rbhat}{\hat{\Rb}}
\newcommand{\Sbhat}{\hat{\Sb}}
\newcommand{\Tbhat}{\hat{\Tb}}
\newcommand{\Ubhat}{\hat{\Ub}}
\newcommand{\Vbhat}{\hat{\Vb}}
\newcommand{\Wbhat}{\hat{\Wb}}
\newcommand{\Xbhat}{\hat{\Xb}}
\newcommand{\Ybhat}{\hat{\Yb}}
\newcommand{\Zbhat}{\hat{\Zb}}

\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{{\mathcal{S}}}
\newcommand{\Tcal}{{\mathcal{T}}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

\newcommand{\Atilde}{\widetilde{A}}
\newcommand{\Btilde}{\widetilde{B}}
\newcommand{\Ctilde}{\widetilde{C}}
\newcommand{\Dtilde}{\widetilde{D}}
\newcommand{\Etilde}{\widetilde{E}}
\newcommand{\Ftilde}{\widetilde{F}}
\newcommand{\Gtilde}{\widetilde{G}}
\newcommand{\Htilde}{\widetilde{H}}
\newcommand{\Itilde}{\widetilde{I}}
\newcommand{\Jtilde}{\widetilde{J}}
\newcommand{\Ktilde}{\widetilde{K}}
\newcommand{\Ltilde}{\widetilde{L}}
\newcommand{\Mtilde}{\widetilde{M}}
\newcommand{\Ntilde}{\widetilde{N}}
\newcommand{\Otilde}{\widetilde{O}}
\newcommand{\Ptilde}{\widetilde{P}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Rtilde}{\widetilde{R}}
\newcommand{\Stilde}{\widetilde{S}}
\newcommand{\Ttilde}{\widetilde{T}}
\newcommand{\Utilde}{\widetilde{U}}
\newcommand{\Vtilde}{\widetilde{V}}
\newcommand{\Wtilde}{\widetilde{W}}
\newcommand{\Xtilde}{\widetilde{X}}
\newcommand{\Ytilde}{\widetilde{Y}}
\newcommand{\Ztilde}{\widetilde{Z}}

\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}

\newcommand{\avec}{\vec{a}}
\newcommand{\bvec}{\vec{b}}
\newcommand{\cvec}{\vec{c}}
\newcommand{\dvec}{\vec{d}}
\newcommand{\evec}{\vec{e}}
\newcommand{\fvec}{\vec{f}}
\newcommand{\gvec}{\vec{g}}
\newcommand{\hvec}{\vec{h}}
\newcommand{\ivec}{\vec{i}}
\newcommand{\jvec}{\vec{j}}
\newcommand{\kvec}{\vec{k}}
\newcommand{\mvec}{\vec{m}}
\newcommand{\nvec}{\vec{n}}
\newcommand{\ovec}{\vec{o}}
\newcommand{\pvec}{\vec{p}}
\newcommand{\qvec}{\vec{q}}
\newcommand{\rvec}{\vec{r}}
\newcommand{\svec}{\vec{s}}
\newcommand{\tvec}{\vec{t}}
\newcommand{\uvec}{\vec{u}}
\newcommand{\vvec}{\vec{v}}
\newcommand{\wvec}{\vec{w}}
\newcommand{\xvec}{\vec{x}}
\newcommand{\yvec}{\vec{y}}
\newcommand{\zvec}{\vec{z}}

\newcommand{\va}{\vec{a}}
\newcommand{\vecb}{\vec{b}}
\newcommand{\vc}{\vec{c}}
\newcommand{\vd}{\vec{d}}
\newcommand{\veee}{\vec{e}}
\newcommand{\vf}{\vec{f}}
\newcommand{\vg}{\vec{g}}
\newcommand{\vh}{\vec{h}}
\newcommand{\vi}{\vec{i}}
\newcommand{\vo}{\vec{o}}
\newcommand{\vp}{\vec{p}}
\newcommand{\vq}{\vec{q}}
\newcommand{\vr}{\vec{r}}
\newcommand{\vs}{\vec{s}}
\newcommand{\vt}{\vec{t}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vw}{\vec{w}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vz}{\vec{z}}

\newcommand{\Avec}{\vec{A}}
\newcommand{\Bvec}{\vec{B}}
\newcommand{\Cvec}{\vec{C}}
\newcommand{\Dvec}{\vec{D}}
\newcommand{\Evec}{\vec{E}}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\Gvec}{\vec{G}}
\newcommand{\Hvec}{\vec{H}}
\newcommand{\Ivec}{\vec{I}}
\newcommand{\Jvec}{\vec{J}}
\newcommand{\Kvec}{\vec{K}}
\newcommand{\Lvec}{\vec{L}}
\newcommand{\Mvec}{\vec{M}}
\newcommand{\Nvec}{\vec{N}}
\newcommand{\Ovec}{\vec{O}}
\newcommand{\Pvec}{\vec{P}}
\newcommand{\Qvec}{\vec{Q}}
\newcommand{\Rvec}{\vec{R}}
\newcommand{\Svec}{\vec{S}}
\newcommand{\Tvec}{\vec{T}}
\newcommand{\Uvec}{\vec{U}}
\newcommand{\Vvec}{\vec{V}}
\newcommand{\Wvec}{\vec{W}}
\newcommand{\Xvec}{\vec{X}}
\newcommand{\Yvec}{\vec{Y}}
\newcommand{\Zvec}{\vec{Z}}

\newcommand{\Amat}{\Ab}
\newcommand{\Bmat}{\Bb}
\newcommand{\Cmat}{\Cb}
\newcommand{\Dmat}{\Db}
\newcommand{\Emat}{\Eb}
\newcommand{\Fmat}{\Fb}
\newcommand{\Gmat}{\Gb}
\newcommand{\Hmat}{\Hb}
\newcommand{\Imat}{\Ib}

\newcommand{\Vmat}{\Vb}
\newcommand{\Wmat}{\Wb}
\newcommand{\Xmat}{\Xb}
\newcommand{\Ymat}{\Yb}
\newcommand{\Zmat}{\Zb}


\newcommand{\yvecbar}{\bar{\vec{y}}}
\newcommand{\wvecbar}{\bar{\vec{w}}}
\newcommand{\xvecbar}{\bar{\vec{x}}}
\newcommand{\yvectil}{\tilde{\vec{y}}}
\newcommand{\yvechat}{\hat{\vec{y}}}


%%%%%%%% Theorems and Friends %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\QED\undefined
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\ifx\proof\undefined
\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
\fi

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\fi

\ifx\example\undefined
\newtheorem{example}{Example}
\fi

\ifx\property\undefined
\newtheorem{property}{Property}
\fi

\ifx\proposition\undefined
\newtheorem{proposition}{Proposition}
\fi

\ifx\remark\undefined
\newtheorem{remark}{Remark}
\fi

\ifx\corollary\undefined
\newtheorem{corollary}{Corollary}
\fi

\ifx\definition\undefined
\newtheorem{definition}{Definition}
\fi

\ifx\conjecture\undefined
\newtheorem{conjecture}{Conjecture}
\fi

\ifx\axiom\undefined
\newtheorem{axiom}{Axiom}
\fi

\ifx\claim\undefined
\newtheorem{claim}{Claim}
\fi

\ifx\assumption\undefined
\newtheorem{assumption}{Assumption}
\fi

% \renewcommand{\qedsymbol}{$\blacksquare$}


%%%%%%%% Widely accepted Sets and Symbols %%%%%%%%%%%%%%%

\newcommand{\CC}{\mathbb{C}} % Complex numbers
\newcommand{\EE}{\mathbb{E}} % Expectation
\newcommand{\FF}{\mathbb{F}} % Fexpectation
\newcommand{\HH}{\mathbb{H}} % Arbitrary field
\newcommand{\II}{\mathbb{I}} % Delta Indicator
\newcommand{\KK}{\mathbb{K}} % Arbitrary field
\newcommand{\MM}{\mathbb{M}} % Median
\newcommand{\NN}{\mathbb{N}} % Natural numbers
\newcommand{\PP}{\mathbb{P}} % Probability
\newcommand{\QQ}{\mathbb{Q}} % Rationals
\newcommand{\RR}{\mathbb{R}} % Real numbers
\newcommand{\RRbar}{\overline{\RR}} % Real numbers
\newcommand{\VV}{\mathbb{V}} % Variance
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}} % Integers

%%%%%%%% Mathematical Operations %%%%%%%%%%%%%%%

\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand*{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand*{\arginf}{\mathop{\mathrm{arginf}}}
\newcommand*{\argsup}{\mathop{\mathrm{argsup}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\vect}{\mathop{\mathrm{vec}}}
\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\dom}{\mathop{\mathrm{dom}}}
\newcommand{\ri}{\mathop{\mathrm{ri}}}
\newcommand{\cl}{\mathop{\mathrm{cl}}}
\newcommand{\intr}{\mathop{\mathrm{int}}}
\newcommand{\bd}{\mathop{\mathrm{bd}}}
\newcommand{\emp}{\mathop{\mathrm{emp}}}
\newcommand{\core}{\mathop{\mathrm{core}}}
\newcommand{\co}{\mathop{\mathrm{co}}}
\newcommand{\nnz}{\mathop{\mathrm{nnz}}}
\newcommand{\eproof}{$\null\hfill\blacksquare$}

%\newcommand{\ln}{\mathop{\mathrm{ln}}}
%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\myspan}[1]{\mathrm{span}\cbr{#1}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{(\partial #1)^2}}
\newcommand{\aleq}{\preccurlyeq}
\newcommand{\ageq}{\succcurlyeq}
%%%%%%%% Short Forms %%%%%%%%%%%%%%%

\newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\iid}{\emph{iid}}
\newcommand{\cf}{\emph{cf.}\ }
\newcommand{\wrt}{\emph{w.r.t.}\ }

%%%%%%%% Brackets %%%%%%%%%%%%%%%

\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\ccc}[1]{|\!|\!|#1|\!|\!|}
\newcommand{\cccc}[1]{\left|\!\left|\!\left|#1\right|\!\right|\!\right|}
\newcommand{\sembrack}[1]{[\![#1]\!]}

%%%%%%%%%%%%%%%  Mathematical Constants  %%%%%%%%%%%%%%%

\newcommand{\one}{\mathbf{1}}  % Identity
\newcommand{\zero}{\mathbf{0}} % Zero
\newcommand{\ind}{\boldsymbol{\mathsf{I}}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\sqrttwo}{\sqrt{2}}
\newcommand{\invsqrttwo}{\frac{1}{\sqrt{2}}}
\newcommand{\rmd}{\ensuremath{\mathrm{d}}}

%%%%%%%% Greek Symbols %%%%%%%%%%%%%%%

\newcommand{\sigmab}{\bm{\sigma}}
\newcommand{\Sigmab}{\mathbf{\Sigma}}

\newcommand{\val}{\vec{\alpha}}
\newcommand{\vbeta}{\vec{\beta}}
\newcommand{\vde}{\vec{\delta}}
\newcommand{\vga}{\vec{\gamma}}
\newcommand{\vsig}{\vec{\sigma}}
\newcommand{\vth}{\vec{\theta}}
\newcommand{\veta}{\vec{\eta}}
\newcommand{\vnu}{\vec{\nu}}
\newcommand{\vpsi}{\vec{\psi}}
\newcommand{\vpi}{\vec{\pi}}
\newcommand{\vphi}{\vec{\phi}}
\newcommand{\vxi}{\vec{\xi}}
\newcommand{\vze}{\vec{\zeta}}

\newcommand{\valbar}{\bar{\val}}
\newcommand{\valhat}{\hat{\val}}
\newcommand{\valtil}{\tilde{\val}}
\newcommand{\vthtil}{\tilde{\vth}}
\newcommand{\vthhat}{\hat{\vth}}
\newcommand{\vthbar}{\bar{\vth}}
\newcommand{\vbetatil}{\tilde{\vbeta}}
\newcommand{\vbetahat}{\hat{\vbeta}}

\newcommand{\alphavec}{\val}
\newcommand{\alphavecbar}{\bar{\val}}
\newcommand{\alphavechat}{\hat{\val}}
\newcommand{\alphavectil}{\tilde{\val}}
\newcommand{\betavec}{\vec{\beta}}
\newcommand{\gammavec}{\vec{\gamma}}
\newcommand{\deltavec}{\vec{\delta}}
\newcommand{\etavec}{\vec{\eta}}
\newcommand{\phivec}{\vec{\phi}}
\newcommand{\psivec}{\vec{\psi}}
\newcommand{\thetavec}{\vec{\theta}}
\newcommand{\muvec}{\vec{\mu}}
\newcommand{\xivec}{\vec{\xi}}
\newcommand{\chivec}{\vec{\chi}}
\newcommand{\lambdavec}{\vec{\lambda}}

\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\mub}{\boldsymbol{\mu}}
\newcommand{\nub}{\boldsymbol{\nu}}
\newcommand{\xib}{\boldsymbol{\xi}}
\newcommand{\Deltab}{\boldsymbol{\Delta}}
\newcommand{\Pib}{\boldsymbol{\Pi}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\taub}{\boldsymbol{\tau}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\pitil}{\tilde{\pi}}
\newcommand{\elltil}{\tilde{\ell}}
\newcommand{\rhob}{\boldsymbol{\rho}}

\newcommand{\delhat}{\hat{\delta}}
\newcommand{\phihat}{\hat{\phi}}
\newcommand{\delbar}{\bar{\delta}}
\newcommand{\alphahat}{\hat{\alpha}}
\newcommand{\alphatil}{\tilde{\alpha}}
\newcommand{\mubar}{\bar{\mu}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\bar{\theta}}
\newcommand{\betahat}{\hat{\beta}}

\newcommand{\xibar}{\bar{\xi}}
\newcommand{\lambdavectil}{\tilde{\vec{\lambda}}}
\newcommand{\thetatil}{\tilde{\theta}}
\newcommand{\betatil}{\tilde{\beta}}

%%%%%%%% Various Optimizers %%%%%%%%%%%%%%%

\newcommand{\BMRM}{{\sf BMRM}}
\newcommand{\bmrm}{{\sf BMRM}}
\newcommand{\cpm}{{\sf CPM}}
\newcommand{\liblinear}{{\sf liblinear}}
\newcommand{\lsbmrm}{{\sf ls-bmrm}}
\newcommand{\qpbmrm}{{\sf qp-bmrm}}
\newcommand{\pegasos}{{\sf pegasos}}
\newcommand{\pegan}{{\sf pegasos-$n$}}
\newcommand{\pegaone}{{\sf pegasos-1}}
\newcommand{\svmstruct}{{\sf SVM-Struct}}
\newcommand{\svmperf}{{\sf SVM-Perf}}
\newcommand{\nest}{{\sf pragam}}
\newcommand{\nestb}{{\sf pragam-b}}
\newcommand{\mcn}{{\sf M$^3$N}}
\newcommand{\expgrad}{{\sf ExpGrad}}
\newcommand{\smo}{{\sf SMO}}
\newcommand{\lasvm}{{\sf LaSVM}}
\newcommand{\sms}{{\sf SMS}}
\newcommand{\agm}{{\sf AGM}}


\newcommand{\prbep}{{\sf PRBEP}}
\newcommand{\rocarea}{{\sf ROCArea}}

\newcommand{\arow}[2]{#1_{#2\cdot}}
\newcommand{\acol}[2]{#1_{\cdot#2}}
\newcommand{\expunder}[1]{\mathop{\EE}\limits_{#1}}
\newcommand{\mean}[1]{\mathop{\EE}\sbr{{#1}}}
\newcommand{\vars}[2]{\var_{{#1}}\sbr{{#2}}}
\newcommand{\expec}[2]{\mathop{\EE}_{{#1}}\sbr{{#2}}}

\newcommand{\twoco}[1]{\multicolumn{2}{c|}{#1}}
\def\ci{\perp\!\!\!\perp}

\newcommand{\ve}{\varepsilon}

\newcommand{\gstar}{g^{\star}}
\newcommand{\fstar}{f^{\star}}
\newcommand{\hstar}{h^{\star}}
\newcommand{\Astar}{A^{\star}}
\newcommand{\Kstar}{K^{\star}}

\newcommand{\var}{\mathrm{Var}}
\newcommand{\grad}{{\nabla}}
\newcommand{\gradtil}{{\tilde{\grad}}}
\newcommand{\MED}{{\text{MED}}}
\newcommand{\where}{{\quad \text{where} \quad}}
\newcommand{\lcg}{{\textit{l.c.g}}}
%\newcommand{\cp}{\mathrm{cp}}
\newcommand{\err}{{\sf err}}
\newcommand{\wvechat}{\hat{\vec{w}}}

\newcommand{\ydiff}[2]{\delta(#1, #2)}
\newcommand{\ykdiff}[2]{\delta(#1, #2)^{\kappa}}
\newcommand{\myfdiff}[2]{\Delta f(#1, #2)}


\newcommand{\Aone}{\textbf{A1}}
\newcommand{\Atwo}{\textbf{A2}}


==> ads-formulation.tex <==
LinkedIn Feed contains various types of updates. At a high level, they can be split into two categories: sponsored (ads) and organic updates. Organic updates are the main driver for engagement, while sponsored updates are the source of revenue. Both engagement and revenue are important yet conflicting because slots on the newsfeed are shared. How to rank both organic and sponsored updates to balance engagement and revenue is a critical problem \cite{Agarwal:2018:OPS:3219819.3219847, Agarwal:2015:PLF:2783258.2788614, Agarwal:2014:ARL:2623330.2623362}.

One solution is slotting sponsored updates at fixed positions for all members. A simplistic solution is to control the ads density using a parameter \textit{minGap}, that controls the number of organic updates between two consecutive ads. \footnote{The actual solution we use at LinkedIn considers the quality of organic and sponsored updates in a session to make the final decision, but the \textit{minGap} plays an important role nonetheless in determining the ads density.} Figure ~\ref{fig:ads-exp} shows an example of how minGap controls the position of ads. This solution is suboptimal because it cannot capture the variability in members' preference of ads density using a single global parameter.
%\vspace{-1cm}
%\begin{figure}[th]
%  \centering
%  \includegraphics[width=\linewidth]{ads-rank-exp.png}
%  \caption{Example of minGap of Ads in Feed}
%  \label{fig:ads-exp}
%\end{figure}

Instead, we formulate it as an optimization problem to select the best gap for each cohort of members. The objective is to maximize revenue with constraints on organic and ads engagement utility. Mathematically, the problem can be formulated as:
\begin{equation}\label{eq-ads}
\begin{aligned}
& \underset{x_{ij}}{\text{Maximize}}  && \sum_{i = 1}^n  \sum_{j = 1}^J x_{ij}  r_{ij}\\
& \text{such that} & &  \sum_{i = 1}^n  \sum_{j = 1}^J x_{ij}  c_{ij}  \geq w_c c_{control} \\
&&&  \sum_{i = 1}^n  \sum_{j = 1}^J x_{ij} o_{ij} \geq w_o   o_{control}  &\\ 
&& &  \sum_{j} x_{ij} = 1, \forall i, \qquad 0 \leq x_{ij} \leq 1.
\end{aligned}
\end{equation}
where $r_{ij}$ is the estimated causal effect on revenue (the primary metric), and $c_{ij}$ and $o_{ij}$ are the estimated causal effect on ads engagement and organic engagement respectively (the guardrail metrics) for cohort $C_i$ and treatment $j$. $w_c$ and $w_o$ denote the weights for the tradeoff when comparing with the control for both the utilities. Note that this optimization problem is also an explicit example of the generic problem stated in \eqref{eq:example_main}.



%Table \ref{table:ads} describes the meaning of each symbol in the formulation. 
%\begin{table}[h!]
%\centering
% \begin{tabular}{|c | p{6.5cm}|} 
% \hline
% Symbol & Meaning \\  
% \hline 
%$mg$ & minGap \\ 
% \hline 
%$S_k$ & $k$-th cohort \\
% \hline 
%$x(mg|S_k)$ & Probability of selecting minGap $mg$ for cohort $S_k$ \\
% \hline 
%$r(S_k, mg)$ & Revenue utility for $k$-th cohort with minGap $mg$  \\
% \hline 
%$c(S_k, mg)$ & Ads engagement utility for $k$-th cohort with minGap $mg$  \\
% \hline 
%$o(S_k, mg)$ & Organic engagement utility for $k$-th cohort with minGap $mg$ \\
% \hline 
%$w(o)$ & Constant weight for organic engagement utility tradeoff\\
% \hline 
%$w(c)$ & Constant weight for ads engagement utility tradeoff\\
% \hline
% \end{tabular}
%\caption{The meaning of each symbol in problem formulation.}
%\label{table:ads}
%\end{table}


==> notifications-formulation.tex <==

%\begin{figure}[!h]
%  \centering
%  \includegraphics[scale = 0.5]{notif.pdf}
%  \caption{Example of LinkedIn Activity Based Notification}
%  \label{fig:exnoti}
%\end{figure}

\subsection{Personalized Capping Problem} 
Notifications are an important driver for member visits and engagement to LinkedIn. Sending more notifications can increase visits, but it also has negative consequences in terms of members engaging less with notifications (reduction in click-through rate) and increase in notifications disables. The system initially had a fixed cap which was the same for all LinkedIn members. This cap determined the maximum number of notifications a user could receive in a 24-hour window. Our goal with introducing personalized volume caps is to maximize visits to LinkedIn with constraints on click-through rate and Notification disables metrics (detailed descriptions in Table \ref{tab:notmetrics}). 

 %The cap was set irrespective of the notification liquidity or a user's ability to consume the notifications.
%Our goal was to replace the global cap with a personalized volume cap per member, such that certain business metrics would be optimized with constraints on others. The primary metric is member visits to the LinkedIn site/app (referred to as Sessions), while the constraint metrics are Notification Sends, Click Through Rate and Notification Disables (detailed descriptions in Table \ref{tab:notmetrics}). 

%This problem falls exactly in the framework as described in this paper. 

 %reshape user coverage in finer granularity. 
%We exposed members to different level of cap parameter under randomized experiments. We leveraged a heuristic cohort definition which groups users into four segments according to their activeness: daily, weekly, monthly, and dormant users. Then, we fine-tune the cap parameter to customize at the pre-defined cohort level. However, the choice of the cohorts was ad-hoc and not necessarily the optimal for having the strongest heterogeneous effects across the metrics at hand. Hence, we apply the proposed method in Notification system to further personalize the cap parameter.
%cap where cap were shared across group of notification categories rather than on each individual category. 
% For instance `Shared By Network` and `Work Anniversary` both have an individual fixed cap of one. 
%For the purpose of this experiment, we choose a sub-set of 5 different notifications based on the volume.
%Thus, the main problems that we solve in this paper are:
%\begin{itemize}
%\item Automatically identifying cohorts which show the strongest heterogenous effects across the treatments (e.g., cap). Estimate the causal effects on the metrics of interests per each cohort.
%\item Solving an optimization problem to assign optimal treatment (optimal value of cap) to each of these cohorts.
%\end{itemize}


%Once we have the cohort level estimations of causal effects, the optimization problem in this example can be written out exactly as \eqref{eq:example_main} where the primary metric is sessions, while the constraint metrics are contributions, send volume, click through rate, notification disabled users and total notification disables. 
%The caps are modeled independently using the problem formulation we have explained in the paper and showed that our approach is able to deliver session gains in both the cases.


==> offline-analysis.tex <==
Figure \ref{fig:pepperCohorts1} visualizes the cohorts generated using an optimized value of $\alpha$ which balances the objective in the Causal Tree algorithm \cite{Athey7353}. Our experiments show that a lower value of $\alpha$ leads to smaller number of cohorts and lower variance (hence higher confidence) on the cohort-level effect estimations; and vice-versa. We select the cohorts with lower $\alpha$ to gain more confidence on the effect estimations. 

With a finalized cohorts set and the cohort-level effect estimations, we ran stochastic optimization analyses using both SGD and Adagrad options \footnote{SGD and Adagrad are different choices of the proximal projection operator in Algorithm \ref{algo:mcsa}. For further details, please see Section \ref{sec:reproducibility}}. We observe that the SGD method converges faster than Adagrad in the Notification use case. Figure \ref{fig:prophetsp} shows the convergence of metric and constraint for the SGD use case over 100,000 iterations. Offline analysis suggested that by optimally choosing the caps based on a member's network and notifications quality features, we can lift the sessions metric while satisfying the other constraint metrics (e.g., Notification CTR, Total Disables). 

\begin{figure}[ht]
    \centering
    \begin{subfigure}[t]{0.48\textwidth}
    \centering
        \begin{subfigure}[t]{0.5\textwidth}
                 \renewcommand\thesubfigure{\alph{subfigure}}
        		\includegraphics[width=\linewidth]{newCohortsViz.pdf}
  		\caption{Heterogeneous Cohorts}
  		\label{fig:pepperCohorts1}
    	\end{subfigure}%
	~ 
    	\begin{subfigure}[t]{0.5\textwidth}
        	\centering
	        \renewcommand\thesubfigure{\alph{subfigure}}
       		\includegraphics[width=\linewidth]{sgdObjConstraint.pdf}
  		\caption{Expectated Sessions Lift}
  		\label{fig:prophetsp}
   	\end{subfigure}
   \end{subfigure}

    \caption{ Heterogeneous cohorts in Notifications, where each color in (a) corresponds to one cohort. Figure (b) show the expected lift in sessions and expected decrease in disables as function along iterations of the Algorithm \ref{algo:mcsa}. } 
\end{figure}

==> online-experiments.tex <==
\subsection{Online Experiments}
\label{sec:online-experiments}

Online A/B tests have become the gold standard in evaluating new product developments in web-facing companies. We ran A/B tests to further validate our method, and report results comparing three variants against the existing baseline of a fixed global cap in Table \ref{tab:online_capnotification}. 
The first variant is the personalized cap treatment learnt using the proposed approach. Due to the high cost of implementing the pipeline and launching online A/B tests, we implemented only the cohort-level solution $CT.ST$ among the earlier proposed methods. 
The second and third variant exposes members to different caps based on a heuristic cohort definition. We grouped members into four segments according to their visit frequency on LinkedIn: members who visit daily, weekly, monthly, and dormant. We then manually selected the suitable cap parameter for each cohort to balance between the impacts on success and constraints metrics. Heuristic Cap A applies slightly larger caps compared to Heuristic Cap B which leads to higher impacts on Sessions but largely violating the constraints on Notification Sends and Notification Total Disables.

All reported metric lifts in Table \ref{tab:online_capnotification}) have a $p$-value of less than 0.05, otherwise we report the lift as neutral since it is not statistically significant. As can be seen from the results, our personalized cap treatment showed significant positive impact on Sessions, while the impact on the constraint metrics remained within acceptable bounds. Our method also outperforms the both heuristic solutions in terms of achieving the best gains on Sessions metric and balancing the negative impacts on the constraint metrics.

\begin{table}[ht]
\centering
\begin{tabular}{p{2.6cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}} 
\hline\hline 
Metrics & ATE \% & ATE \% & ATE \%\\ 
& Personalized Cap &  Heuristic Cap A & Heuristic Cap B\\
[0.5ex]
\hline 
Sessions &  $\boldsymbol{+1.39\%}$  & $+1.31\%$ & $+0.54\%$ \\
Notification Sends & $ \boldsymbol{+1.64\%}$ & $+6.62\%$ & $+3.07\%$ \\
Notification CTR & $-1.24\%$ & $-1.73\%$ & -1.18\% \\
Total Disables & Neutral & $+9.23\%$ & Neutral\\
\hline 
\end{tabular}
\caption{Notification Cap Experiment Results} 
\label{tab:online_capnotification}
\end{table}


==> simulation_causal_graph_files/rs=AA2YrTvZgm6-L4kY1fcsPTeLK-qRHnwbvQ <==
this.gbar_=this.gbar_||{};(function(_){var window=this;
try{
var De=function(a){var c=arguments.length;if(1==c&&_.Ba(arguments[0]))return De.apply(null,arguments[0]);for(var d={},e=0;e<c;e++)d[arguments[e]]=!0;return d},Ee;
De("A AREA BUTTON HEAD INPUT LINK MENU META OPTGROUP OPTION PROGRESS STYLE SELECT SOURCE TEXTAREA TITLE TRACK".split(" "));_.Fe=function(a,c){c?a.setAttribute("role",c):a.removeAttribute("role")};
_.Ge=function(a,c,d){_.Ba(d)&&(d=d.join(" "));var e="aria-"+c;""===d||void 0==d?(Ee||(Ee={atomic:!1,autocomplete:"none",dropeffect:"none",haspopup:!1,live:"off",multiline:!1,multiselectable:!1,orientation:"vertical",readonly:!1,relevant:"additions text",required:!1,sort:"none",busy:!1,disabled:!1,hidden:!1,invalid:"false"}),d=Ee,c in d?a.setAttribute(e,d[c]):a.removeAttribute(e)):a.setAttribute(e,d)};

}catch(e){_._DumpException(e)}
try{
/*

 Copyright The Closure Library Authors.
 SPDX-License-Identifier: Apache-2.0
*/

}catch(e){_._DumpException(e)}
try{
/*

 Copyright The Closure Library Authors.
 SPDX-License-Identifier: Apache-2.0
*/
_.He=function(a){a=a.split(".");for(var c=_.q,d=0;d<a.length;d++)if(c=c[a[d]],null==c)return null;return c};

}catch(e){_._DumpException(e)}
try{
var Je;_.Ie=function(a,c){c=(0,_.La)(a,c);var d;(d=0<=c)&&Array.prototype.splice.call(a,c,1);return d};Je=function(a,c){for(var d in a)if(c.call(void 0,a[d],d,a))return!0;return!1};_.Ke=function(a,c){try{return _.Lb(a[c]),!0}catch(d){}return!1};
_.Le=function(a,c){this.type=a;this.b=this.target=c;this.defaultPrevented=this.f=!1};_.Le.prototype.stopPropagation=function(){this.f=!0};_.Le.prototype.preventDefault=function(){this.defaultPrevented=!0};
_.Me=function(a,c){_.Le.call(this,a?a.type:"");this.relatedTarget=this.b=this.target=null;this.button=this.screenY=this.screenX=this.clientY=this.clientX=0;this.key="";this.j=this.keyCode=0;this.metaKey=this.shiftKey=this.altKey=this.ctrlKey=!1;this.state=null;this.pointerId=0;this.pointerType="";this.ab=null;a&&this.init(a,c)};_.w(_.Me,_.Le);var Ne={2:"touch",3:"pen",4:"mouse"};
_.Me.prototype.init=function(a,c){var d=this.type=a.type,e=a.changedTouches&&a.changedTouches.length?a.changedTouches[0]:null;this.target=a.target||a.srcElement;this.b=c;(c=a.relatedTarget)?_.Rb&&(_.Ke(c,"nodeName")||(c=null)):"mouseover"==d?c=a.fromElement:"mouseout"==d&&(c=a.toElement);this.relatedTarget=c;e?(this.clientX=void 0!==e.clientX?e.clientX:e.pageX,this.clientY=void 0!==e.clientY?e.clientY:e.pageY,this.screenX=e.screenX||0,this.screenY=e.screenY||0):(this.clientX=void 0!==a.clientX?a.clientX:
a.pageX,this.clientY=void 0!==a.clientY?a.clientY:a.pageY,this.screenX=a.screenX||0,this.screenY=a.screenY||0);this.button=a.button;this.keyCode=a.keyCode||0;this.key=a.key||"";this.j=a.charCode||("keypress"==d?a.keyCode:0);this.ctrlKey=a.ctrlKey;this.altKey=a.altKey;this.shiftKey=a.shiftKey;this.metaKey=a.metaKey;this.pointerId=a.pointerId||0;this.pointerType="string"===typeof a.pointerType?a.pointerType:Ne[a.pointerType]||"";this.state=a.state;this.ab=a;a.defaultPrevented&&this.preventDefault()};
_.Me.prototype.stopPropagation=function(){_.Me.L.stopPropagation.call(this);this.ab.stopPropagation?this.ab.stopPropagation():this.ab.cancelBubble=!0};_.Me.prototype.preventDefault=function(){_.Me.L.preventDefault.call(this);var a=this.ab;if(a.preventDefault)a.preventDefault();else if(a.returnValue=!1,_.Md)try{if(a.ctrlKey||112<=a.keyCode&&123>=a.keyCode)a.keyCode=-1}catch(c){}};
var Qe;_.Oe="closure_listenable_"+(1E6*Math.random()|0);_.Pe=function(a){return!(!a||!a[_.Oe])};Qe=0;
var Re;Re=function(a,c,d,e,f){this.listener=a;this.b=null;this.src=c;this.type=d;this.capture=!!e;this.Zd=f;this.key=++Qe;this.Yc=this.Ld=!1};_.Se=function(a){a.Yc=!0;a.listener=null;a.b=null;a.src=null;a.Zd=null};
_.Te=function(a){this.src=a;this.b={};this.f=0};_.Te.prototype.add=function(a,c,d,e,f){var g=a.toString();a=this.b[g];a||(a=this.b[g]=[],this.f++);var h=Ue(a,c,e,f);-1<h?(c=a[h],d||(c.Ld=!1)):(c=new Re(c,this.src,g,!!e,f),c.Ld=d,a.push(c));return c};_.Te.prototype.remove=function(a,c,d,e){a=a.toString();if(!(a in this.b))return!1;var f=this.b[a];c=Ue(f,c,d,e);return-1<c?(_.Se(f[c]),Array.prototype.splice.call(f,c,1),0==f.length&&(delete this.b[a],this.f--),!0):!1};
_.Ve=function(a,c){var d=c.type;if(!(d in a.b))return!1;var e=_.Ie(a.b[d],c);e&&(_.Se(c),0==a.b[d].length&&(delete a.b[d],a.f--));return e};_.Te.prototype.Rc=function(a,c){a=this.b[a.toString()];var d=[];if(a)for(var e=0;e<a.length;++e){var f=a[e];f.capture==c&&d.push(f)}return d};_.Te.prototype.Dc=function(a,c,d,e){a=this.b[a.toString()];var f=-1;a&&(f=Ue(a,c,d,e));return-1<f?a[f]:null};
_.Te.prototype.hasListener=function(a,c){var d=void 0!==a,e=d?a.toString():"",f=void 0!==c;return Je(this.b,function(g){for(var h=0;h<g.length;++h)if(!(d&&g[h].type!=e||f&&g[h].capture!=c))return!0;return!1})};var Ue=function(a,c,d,e){for(var f=0;f<a.length;++f){var g=a[f];if(!g.Yc&&g.listener==c&&g.capture==!!d&&g.Zd==e)return f}return-1};
var We,Xe,Ye,af,cf,df,jf,hf,ef,kf;We="closure_lm_"+(1E6*Math.random()|0);Xe={};Ye=0;_.O=function(a,c,d,e,f){if(e&&e.once)return _.Ze(a,c,d,e,f);if(_.Ba(c)){for(var g=0;g<c.length;g++)_.O(a,c[g],d,e,f);return null}d=_.$e(d);return _.Pe(a)?a.H(c,d,_.Da(e)?!!e.capture:!!e,f):af(a,c,d,!1,e,f)};
af=function(a,c,d,e,f,g){if(!c)throw Error("n");var h=_.Da(f)?!!f.capture:!!f,l=_.bf(a);l||(a[We]=l=new _.Te(a));d=l.add(c,d,e,h,g);if(d.b)return d;e=cf();d.b=e;e.src=a;e.listener=d;if(a.addEventListener)_.Nd||(f=h),void 0===f&&(f=!1),a.addEventListener(c.toString(),e,f);else if(a.attachEvent)a.attachEvent(df(c.toString()),e);else if(a.addListener&&a.removeListener)a.addListener(e);else throw Error("o");Ye++;return d};
cf=function(){var a=ef,c=_.Ld?function(d){return a.call(c.src,c.listener,d)}:function(d){d=a.call(c.src,c.listener,d);if(!d)return d};return c};_.Ze=function(a,c,d,e,f){if(_.Ba(c)){for(var g=0;g<c.length;g++)_.Ze(a,c[g],d,e,f);return null}d=_.$e(d);return _.Pe(a)?a.nb(c,d,_.Da(e)?!!e.capture:!!e,f):af(a,c,d,!0,e,f)};_.ff=function(a,c,d,e,f){if(_.Ba(c))for(var g=0;g<c.length;g++)_.ff(a,c[g],d,e,f);else e=_.Da(e)?!!e.capture:!!e,d=_.$e(d),_.Pe(a)?a.Ba(c,d,e,f):a&&(a=_.bf(a))&&(c=a.Dc(c,d,e,f))&&_.gf(c)};
_.gf=function(a){if("number"===typeof a||!a||a.Yc)return!1;var c=a.src;if(_.Pe(c))return c.ye(a);var d=a.type,e=a.b;c.removeEventListener?c.removeEventListener(d,e,a.capture):c.detachEvent?c.detachEvent(df(d),e):c.addListener&&c.removeListener&&c.removeListener(e);Ye--;(d=_.bf(c))?(_.Ve(d,a),0==d.f&&(d.src=null,c[We]=null)):_.Se(a);return!0};df=function(a){return a in Xe?Xe[a]:Xe[a]="on"+a};
jf=function(a,c,d,e){var f=!0;if(a=_.bf(a))if(c=a.b[c.toString()])for(c=c.concat(),a=0;a<c.length;a++){var g=c[a];g&&g.capture==d&&!g.Yc&&(g=hf(g,e),f=f&&!1!==g)}return f};hf=function(a,c){var d=a.listener,e=a.Zd||a.src;a.Ld&&_.gf(a);return d.call(e,c)};
ef=function(a,c){if(a.Yc)return!0;if(!_.Ld){var d=c||_.He("window.event");c=new _.Me(d,this);var e=!0;if(!(0>d.keyCode||void 0!=d.returnValue)){a:{var f=!1;if(0==d.keyCode)try{d.keyCode=-1;break a}catch(h){f=!0}if(f||void 0==d.returnValue)d.returnValue=!0}d=[];for(f=c.b;f;f=f.parentNode)d.push(f);a=a.type;for(f=d.length-1;!c.f&&0<=f;f--){c.b=d[f];var g=jf(d[f],a,!0,c);e=e&&g}for(f=0;!c.f&&f<d.length;f++)c.b=d[f],g=jf(d[f],a,!1,c),e=e&&g}return e}return hf(a,new _.Me(c,this))};
_.bf=function(a){a=a[We];return a instanceof _.Te?a:null};kf="__closure_events_fn_"+(1E9*Math.random()>>>0);_.$e=function(a){if(_.Ca(a))return a;a[kf]||(a[kf]=function(c){return a.handleEvent(c)});return a[kf]};

}catch(e){_._DumpException(e)}
try{
_.lf=function(a){return a};_.mf=function(a){return a instanceof _.hb&&a.constructor===_.hb&&a.f===_.gb?a.b:"type_error:Const"};_.nf=function(a){return _.qb(_.mf(a))};_.of=function(a,c){a.src=_.Ud(c)};
_.pf=function(a){a.prototype.$goog_Thenable=!0};_.qf=function(a){if(!a)return!1;try{return!!a.$goog_Thenable}catch(c){return!1}};
/*

 Copyright The Closure Library Authors.
 SPDX-License-Identifier: Apache-2.0
*/
var rf=function(a,c){this.j=a;this.o=c;this.f=0;this.b=null};rf.prototype.get=function(){if(0<this.f){this.f--;var a=this.b;this.b=a.next;a.next=null}else a=this.j();return a};var sf=function(a,c){a.o(c);100>a.f&&(a.f++,c.next=a.b,a.b=c)};
var tf=function(a){_.q.setTimeout(function(){throw a;},0)},uf,vf=function(){var a=_.q.MessageChannel;"undefined"===typeof a&&"undefined"!==typeof window&&window.postMessage&&window.addEventListener&&!_.x("Presto")&&(a=function(){var f=_.ze("IFRAME");f.style.display="none";_.of(f,_.nf(_.jb));document.documentElement.appendChild(f);var g=f.contentWindow;f=g.document;f.open();f.write(_.Eb(_.Gb));f.close();var h="callImmediate"+Math.random(),l="file:"==g.location.protocol?"*":g.location.protocol+"//"+
g.location.host;f=(0,_.t)(function(m){if(("*"==l||m.origin==l)&&m.data==h)this.port1.onmessage()},this);g.addEventListener("message",f,!1);this.port1={};this.port2={postMessage:function(){g.postMessage(h,l)}}});if("undefined"!==typeof a&&!_.$a()){var c=new a,d={},e=d;c.port1.onmessage=function(){if(void 0!==d.next){d=d.next;var f=d.Cf;d.Cf=null;f()}};return function(f){e.next={Cf:f};e=e.next;c.port2.postMessage(0)}}return"undefined"!==typeof document&&"onreadystatechange"in _.ze("SCRIPT")?function(f){var g=
_.ze("SCRIPT");g.onreadystatechange=function(){g.onreadystatechange=null;g.parentNode.removeChild(g);g=null;f();f=null};document.documentElement.appendChild(g)}:function(f){_.q.setTimeout(f,0)}};
var wf=function(){this.f=this.b=null},yf=new rf(function(){return new xf},function(a){a.reset()});wf.prototype.add=function(a,c){var d=yf.get();d.set(a,c);this.f?this.f.next=d:this.b=d;this.f=d};wf.prototype.remove=function(){var a=null;this.b&&(a=this.b,this.b=this.b.next,this.b||(this.f=null),a.next=null);return a};var xf=function(){this.next=this.scope=this.Yb=null};xf.prototype.set=function(a,c){this.Yb=a;this.scope=c;this.next=null};
xf.prototype.reset=function(){this.next=this.scope=this.Yb=null};
var zf,Af,Bf,Cf,Ef;_.Df=function(a,c){zf||Af();Bf||(zf(),Bf=!0);Cf.add(a,c)};Af=function(){if(_.q.Promise&&_.q.Promise.resolve){var a=_.q.Promise.resolve(void 0);zf=function(){a.then(Ef)}}else zf=function(){var c=Ef;!_.Ca(_.q.setImmediate)||_.q.Window&&_.q.Window.prototype&&!_.x("Edge")&&_.q.Window.prototype.setImmediate==_.q.setImmediate?(uf||(uf=vf()),uf(c)):_.q.setImmediate(c)}};Bf=!1;Cf=new wf;Ef=function(){for(var a;a=Cf.remove();){try{a.Yb.call(a.scope)}catch(c){tf(c)}sf(yf,a)}Bf=!1};
var Hf,Uf,Qf,Of,Pf,Vf,Tf,Wf;_.Gf=function(a,c){this.b=0;this.B=void 0;this.o=this.f=this.j=null;this.w=this.A=!1;if(a!=_.xa)try{var d=this;a.call(c,function(e){_.Ff(d,2,e)},function(e){_.Ff(d,3,e)})}catch(e){_.Ff(this,3,e)}};Hf=function(){this.next=this.context=this.f=this.j=this.b=null;this.o=!1};Hf.prototype.reset=function(){this.context=this.f=this.j=this.b=null;this.o=!1};
var If=new rf(function(){return new Hf},function(a){a.reset()}),Jf=function(a,c,d){var e=If.get();e.j=a;e.f=c;e.context=d;return e};_.Gf.prototype.then=function(a,c,d){return Kf(this,_.Ca(a)?a:null,_.Ca(c)?c:null,d)};_.pf(_.Gf);_.Lf=function(a,c){return Kf(a,null,c,void 0)};_.Gf.prototype.cancel=function(a){if(0==this.b){var c=new _.Mf(a);_.Df(function(){Nf(this,c)},this)}};
var Nf=function(a,c){if(0==a.b)if(a.j){var d=a.j;if(d.f){for(var e=0,f=null,g=null,h=d.f;h&&(h.o||(e++,h.b==a&&(f=h),!(f&&1<e)));h=h.next)f||(g=h);f&&(0==d.b&&1==e?Nf(d,c):(g?(e=g,e.next==d.o&&(d.o=e),e.next=e.next.next):Of(d),Pf(d,f,3,c)))}a.j=null}else _.Ff(a,3,c)},Rf=function(a,c){a.f||2!=a.b&&3!=a.b||Qf(a);a.o?a.o.next=c:a.f=c;a.o=c},Kf=function(a,c,d,e){var f=Jf(null,null,null);f.b=new _.Gf(function(g,h){f.j=c?function(l){try{var m=c.call(e,l);g(m)}catch(n){h(n)}}:g;f.f=d?function(l){try{var m=
d.call(e,l);void 0===m&&l instanceof _.Mf?h(l):g(m)}catch(n){h(n)}}:h});f.b.j=a;Rf(a,f);return f.b};_.Gf.prototype.G=function(a){this.b=0;_.Ff(this,2,a)};_.Gf.prototype.F=function(a){this.b=0;_.Ff(this,3,a)};_.Ff=function(a,c,d){0==a.b&&(a===d&&(c=3,d=new TypeError("p")),a.b=1,_.Sf(d,a.G,a.F,a)||(a.B=d,a.b=c,a.j=null,Qf(a),3!=c||d instanceof _.Mf||Tf(a,d)))};
_.Sf=function(a,c,d,e){if(a instanceof _.Gf)return Rf(a,Jf(c||_.xa,d||null,e)),!0;if(_.qf(a))return a.then(c,d,e),!0;if(_.Da(a))try{var f=a.then;if(_.Ca(f))return Uf(a,f,c,d,e),!0}catch(g){return d.call(e,g),!0}return!1};Uf=function(a,c,d,e,f){var g=!1,h=function(m){g||(g=!0,d.call(f,m))},l=function(m){g||(g=!0,e.call(f,m))};try{c.call(a,h,l)}catch(m){l(m)}};Qf=function(a){a.A||(a.A=!0,_.Df(a.D,a))};Of=function(a){var c=null;a.f&&(c=a.f,a.f=c.next,c.next=null);a.f||(a.o=null);return c};
_.Gf.prototype.D=function(){for(var a;a=Of(this);)Pf(this,a,this.b,this.B);this.A=!1};Pf=function(a,c,d,e){if(3==d&&c.f&&!c.o)for(;a&&a.w;a=a.j)a.w=!1;if(c.b)c.b.j=null,Vf(c,d,e);else try{c.o?c.j.call(c.context):Vf(c,d,e)}catch(f){Wf.call(null,f)}sf(If,c)};Vf=function(a,c,d){2==c?a.j.call(a.context,d):a.f&&a.f.call(a.context,d)};Tf=function(a,c){a.w=!0;_.Df(function(){a.w&&Wf.call(null,c)})};Wf=tf;_.Mf=function(a){_.Ka.call(this,a)};_.w(_.Mf,_.Ka);_.Mf.prototype.name="cancel";

}catch(e){_._DumpException(e)}
try{
var $f,kg,lg;_.Xf=function(a){a&&"function"==typeof a.sa&&a.sa()};_.Yf=function(a,c){c=_.Sd(_.Xf,c);a.Sa?c():(a.Lb||(a.Lb=[]),a.Lb.push(c))};_.Zf=function(a){var c=[],d=0,e;for(e in a)c[d++]=a[e];return c};_.ag=function(a,c){if((0,_.Ib)())for(;a.lastChild;)a.removeChild(a.lastChild);a.innerHTML=_.Eb(c)};_.bg=function(a,c){return"string"===typeof c?a.getElementById(c):c};_.cg=function(a){return"CSS1Compat"==a.compatMode};
_.dg=function(a){a=(a||window).document;a=_.cg(a)?a.documentElement:a.body;return new _.pe(a.clientWidth,a.clientHeight)};_.eg=function(a){return a?a.parentWindow||a.defaultView:window};_.fg=function(a){for(var c;c=a.firstChild;)a.removeChild(c)};_.gg=function(a){return _.me&&void 0!=a.children?a.children:(0,_.Na)(a.childNodes,function(c){return 1==c.nodeType})};
_.hg=function(a,c){if(!a||!c)return!1;if(a.contains&&1==c.nodeType)return a==c||a.contains(c);if("undefined"!=typeof a.compareDocumentPosition)return a==c||!!(a.compareDocumentPosition(c)&16);for(;c&&a!=c;)c=c.parentNode;return c==a};_.ig=function(a,c){if("textContent"in a)a.textContent=c;else if(3==a.nodeType)a.data=String(c);else if(a.firstChild&&3==a.firstChild.nodeType){for(;a.lastChild!=a.firstChild;)a.removeChild(a.lastChild);a.firstChild.data=String(c)}else _.fg(a),a.appendChild(_.Ce(a).createTextNode(String(c)))};
kg={SCRIPT:1,STYLE:1,HEAD:1,IFRAME:1,OBJECT:1};lg={IMG:" ",BR:"\n"};_.mg=function(a,c,d){if(!(a.nodeName in kg))if(3==a.nodeType)d?c.push(String(a.nodeValue).replace(/(\r\n|\r|\n)/g,"")):c.push(a.nodeValue);else if(a.nodeName in lg)c.push(lg[a.nodeName]);else for(a=a.firstChild;a;)_.mg(a,c,d),a=a.nextSibling};_.ng=function(a){try{var c=a&&a.activeElement;return c&&c.nodeName?c:null}catch(d){return null}};_.og=function(a){this.b=a||_.q.document||document};_.k=_.og.prototype;
_.k.C=function(a){return _.bg(this.b,a)};_.k.wa=function(a,c,d){return _.ue(this.b,arguments)};_.k.createElement=function(a){return _.we(this.b,a)};_.k.Rd=function(a,c){a.appendChild(c)};_.k.Xf=_.fg;_.k.Sd=_.Ae;_.k.Ph=_.gg;_.k.Wf=_.hg;_.pg=function(a){return a?new _.og(_.Ce(a)):$f||($f=new _.og)};_.Q=function(){_.J.call(this);this.Mb=new _.Te(this);this.Sg=this;this.kf=null};_.w(_.Q,_.J);_.Q.prototype[_.Oe]=!0;_.k=_.Q.prototype;_.k.vd=function(){return this.kf};_.k.Kc=function(a){this.kf=a};
_.k.addEventListener=function(a,c,d,e){_.O(this,a,c,d,e)};_.k.removeEventListener=function(a,c,d,e){_.ff(this,a,c,d,e)};
_.k.dispatchEvent=function(a){var c,d=this.vd();if(d)for(c=[];d;d=d.vd())c.push(d);d=this.Sg;var e=a.type||a;if("string"===typeof a)a=new _.Le(a,d);else if(a instanceof _.Le)a.target=a.target||d;else{var f=a;a=new _.Le(e,d);_.Za(a,f)}f=!0;if(c)for(var g=c.length-1;!a.f&&0<=g;g--){var h=a.b=c[g];f=h.Pc(e,!0,a)&&f}a.f||(h=a.b=d,f=h.Pc(e,!0,a)&&f,a.f||(f=h.Pc(e,!1,a)&&f));if(c)for(g=0;!a.f&&g<c.length;g++)h=a.b=c[g],f=h.Pc(e,!1,a)&&f;return f};_.k.P=function(){_.Q.L.P.call(this);this.re();this.kf=null};
_.k.H=function(a,c,d,e){return this.Mb.add(String(a),c,!1,d,e)};_.k.nb=function(a,c,d,e){return this.Mb.add(String(a),c,!0,d,e)};_.k.Ba=function(a,c,d,e){return this.Mb.remove(String(a),c,d,e)};_.k.ye=function(a){return _.Ve(this.Mb,a)};_.k.re=function(a){if(this.Mb){var c=this.Mb;a=a&&a.toString();var d=0,e;for(e in c.b)if(!a||e==a){for(var f=c.b[e],g=0;g<f.length;g++)++d,_.Se(f[g]);delete c.b[e];c.f--}c=d}else c=0;return c};
_.k.Pc=function(a,c,d){a=this.Mb.b[String(a)];if(!a)return!0;a=a.concat();for(var e=!0,f=0;f<a.length;++f){var g=a[f];if(g&&!g.Yc&&g.capture==c){var h=g.listener,l=g.Zd||g.src;g.Ld&&this.ye(g);e=!1!==h.call(l,d)&&e}}return e&&!d.defaultPrevented};_.k.Rc=function(a,c){return this.Mb.Rc(String(a),c)};_.k.Dc=function(a,c,d,e){return this.Mb.Dc(String(a),c,d,e)};_.k.hasListener=function(a,c){return this.Mb.hasListener(void 0!==a?String(a):void 0,c)};
/*

 Copyright The Closure Library Authors.
 SPDX-License-Identifier: Apache-2.0
*/
_.qg=function(a,c){_.Q.call(this);this.f=a||1;this.b=c||_.q;this.j=(0,_.t)(this.qk,this);this.o=(0,_.Ha)()};_.w(_.qg,_.Q);_.k=_.qg.prototype;_.k.sc=!1;_.k.Gb=null;_.k.qk=function(){if(this.sc){var a=(0,_.Ha)()-this.o;0<a&&a<.8*this.f?this.Gb=this.b.setTimeout(this.j,this.f-a):(this.Gb&&(this.b.clearTimeout(this.Gb),this.Gb=null),this.dispatchEvent("tick"),this.sc&&(this.stop(),this.start()))}};_.k.start=function(){this.sc=!0;this.Gb||(this.Gb=this.b.setTimeout(this.j,this.f),this.o=(0,_.Ha)())};
_.k.stop=function(){this.sc=!1;this.Gb&&(this.b.clearTimeout(this.Gb),this.Gb=null)};_.k.P=function(){_.qg.L.P.call(this);this.stop();delete this.b};_.rg=function(a,c,d){if(_.Ca(a))d&&(a=(0,_.t)(a,d));else if(a&&"function"==typeof a.handleEvent)a=(0,_.t)(a.handleEvent,a);else throw Error("q");return 2147483647<Number(c)?-1:_.q.setTimeout(a,c||0)};_.sg=function(a){_.q.clearTimeout(a)};

}catch(e){_._DumpException(e)}
try{
var tg;tg=[1,4,2];_.ug=function(a){return(_.Kd?0==a.ab.button:"click"==a.type?!0:!!(a.ab.button&tg[0]))&&!(_.Sb&&_.Tb&&a.ctrlKey)};_.vg=function(a){_.J.call(this);this.T=a;this.O={}};_.w(_.vg,_.J);var wg=[];_.vg.prototype.H=function(a,c,d,e){return xg(this,a,c,d,e)};_.vg.prototype.o=function(a,c,d,e,f){return xg(this,a,c,d,e,f)};
var xg=function(a,c,d,e,f,g){_.Ba(d)||(d&&(wg[0]=d.toString()),d=wg);for(var h=0;h<d.length;h++){var l=_.O(c,d[h],e||a.handleEvent,f||!1,g||a.T||a);if(!l)break;a.O[l.key]=l}return a};_.vg.prototype.nb=function(a,c,d,e){return yg(this,a,c,d,e)};var yg=function(a,c,d,e,f,g){if(_.Ba(d))for(var h=0;h<d.length;h++)yg(a,c,d[h],e,f,g);else{c=_.Ze(c,d,e||a.handleEvent,f,g||a.T||a);if(!c)return a;a.O[c.key]=c}return a};
_.vg.prototype.Ba=function(a,c,d,e,f){if(_.Ba(c))for(var g=0;g<c.length;g++)this.Ba(a,c[g],d,e,f);else d=d||this.handleEvent,e=_.Da(e)?!!e.capture:!!e,f=f||this.T||this,d=_.$e(d),e=!!e,c=_.Pe(a)?a.Dc(c,d,e,f):a?(a=_.bf(a))?a.Dc(c,d,e,f):null:null,c&&(_.gf(c),delete this.O[c.key]);return this};_.zg=function(a){_.Xa(a.O,function(c,d){this.O.hasOwnProperty(d)&&_.gf(c)},a);a.O={}};_.vg.prototype.P=function(){_.vg.L.P.call(this);_.zg(this)};_.vg.prototype.handleEvent=function(){throw Error("s");};

}catch(e){_._DumpException(e)}
try{
var Bg,Gg;_.Ag=function(a){return new _.pe(a.width,a.height)};Bg=0;_.Cg=function(a){return Object.prototype.hasOwnProperty.call(a,_.Ea)&&a[_.Ea]||(a[_.Ea]=++Bg)};_.Dg=function(a,c,d){return 2>=arguments.length?Array.prototype.slice.call(a,c):Array.prototype.slice.call(a,c,d)};_.Eg=function(a,c,d,e){Array.prototype.splice.apply(a,_.Dg(arguments,1))};_.Fg=function(a){return String(a).replace(/\-([a-z])/g,function(c,d){return d.toUpperCase()})};
Gg=function(a){return a.replace(/(^|[\s]+)([a-z])/g,function(c,d,e){return d+e.toUpperCase()})};_.Hg=function(a,c){return a==c?!0:a&&c?a.width==c.width&&a.height==c.height:!1};
var Kg;_.Jg=function(a,c,d){if("string"===typeof c)(c=_.Ig(a,c))&&(a.style[c]=d);else for(var e in c){d=a;var f=c[e],g=_.Ig(d,e);g&&(d.style[g]=f)}};Kg={};_.Ig=function(a,c){var d=Kg[c];if(!d){var e=_.Fg(c);d=e;void 0===a.style[e]&&(e=(_.Sb?"Webkit":_.Rb?"Moz":_.y?"ms":_.Ob?"O":null)+Gg(e),void 0!==a.style[e]&&(d=e));Kg[c]=d}return d};_.Lg=function(a,c){var d=_.Ce(a);return d.defaultView&&d.defaultView.getComputedStyle&&(a=d.defaultView.getComputedStyle(a,null))?a[c]||a.getPropertyValue(c)||"":""};
_.Mg=function(a,c){return _.Lg(a,c)||(a.currentStyle?a.currentStyle[c]:null)||a.style&&a.style[c]};_.Ng=function(a){try{var c=a.getBoundingClientRect()}catch(d){return{left:0,top:0,right:0,bottom:0}}_.y&&a.ownerDocument.body&&(a=a.ownerDocument,c.left-=a.documentElement.clientLeft+a.body.clientLeft,c.top-=a.documentElement.clientTop+a.body.clientTop);return c};_.Og=function(a,c){"number"==typeof a&&(a=(c?Math.round(a):a)+"px");return a};
_.Qg=function(a){var c=_.Pg;if("none"!=_.Mg(a,"display"))return c(a);var d=a.style,e=d.display,f=d.visibility,g=d.position;d.visibility="hidden";d.position="absolute";d.display="inline";a=c(a);d.display=e;d.position=g;d.visibility=f;return a};_.Pg=function(a){var c=a.offsetWidth,d=a.offsetHeight,e=_.Sb&&!c&&!d;return(void 0===c||e)&&a.getBoundingClientRect?(a=_.Ng(a),new _.pe(a.right-a.left,a.bottom-a.top)):new _.pe(c,d)};_.Rg=_.Rb?"MozUserSelect":_.Sb||_.Pb?"WebkitUserSelect":null;

}catch(e){_._DumpException(e)}
try{
/*

 Copyright The Closure Library Authors.
 SPDX-License-Identifier: Apache-2.0
*/
var Sg,Vg;Sg=function(a,c){return null!==a&&c in a?a[c]:void 0};_.Tg=function(a){return null==a?"":String(a)};_.Ug=function(a){if(48<=a&&57>=a||96<=a&&106>=a||65<=a&&90>=a||(_.Sb||_.Pb)&&0==a)return!0;switch(a){case 32:case 43:case 63:case 64:case 107:case 109:case 110:case 111:case 186:case 59:case 189:case 187:case 61:case 188:case 190:case 191:case 192:case 222:case 219:case 220:case 221:case 163:case 58:return!0;case 173:return _.Rb;default:return!1}};
Vg=function(a){switch(a){case 61:return 187;case 59:return 186;case 173:return 189;case 224:return 91;case 0:return 224;default:return a}};_.Wg=function(a){if(_.Rb)a=Vg(a);else if(_.Tb&&_.Sb)switch(a){case 93:a=91}return a};
_.Xg=function(a,c,d,e,f,g){if(_.Sb&&!_.gc("525"))return!0;if(_.Tb&&f)return _.Ug(a);if(f&&!e)return!1;if(!_.Rb){"number"===typeof c&&(c=_.Wg(c));var h=17==c||18==c||_.Tb&&91==c;if((!d||_.Tb)&&h||_.Tb&&16==c&&(e||g))return!1}if((_.Sb||_.Pb)&&e&&d)switch(a){case 220:case 219:case 221:case 192:case 186:case 189:case 187:case 188:case 190:case 191:case 192:case 222:return!1}if(_.y&&e&&c==a)return!1;switch(a){case 13:return _.Rb?g||f?!1:!(d&&e):!0;case 27:return!(_.Sb||_.Pb||_.Rb)}return _.Rb&&(e||f||
g)?!1:_.Ug(a)};
_.Yg=function(){};_.ya(_.Yg);_.Yg.prototype.b=0;_.Zg=function(a){return":"+(a.b++).toString(36)};
var $g,dh;_.ah=function(a){_.Q.call(this);this.b=a||_.pg();this.ma=$g;this.W=null;this.Da=!1;this.f=null;this.M=void 0;this.G=this.w=this.j=this.A=null;this.Ja=!1};_.w(_.ah,_.Q);_.ah.prototype.tb=_.Yg.ta();$g=null;_.bh=function(a){return a.W||(a.W=_.Zg(a.tb))};_.ah.prototype.C=function(){return this.f};_.ch=function(a){a.M||(a.M=new _.vg(a));return a.M};
dh=function(a,c){if(a==c)throw Error("u");var d;if(d=c&&a.j&&a.W){d=a.j;var e=a.W;d=d.G&&e?Sg(d.G,e)||null:null}if(d&&a.j!=c)throw Error("u");a.j=c;_.ah.L.Kc.call(a,c)};_.ah.prototype.Kc=function(a){if(this.j&&this.j!=a)throw Error("v");_.ah.L.Kc.call(this,a)};_.ah.prototype.Hb=function(){this.f=this.b.createElement("DIV")};_.ah.prototype.Ha=function(a){eh(this,a)};var eh=function(a,c,d){if(a.Da)throw Error("w");a.f||a.Hb();c?c.insertBefore(a.f,d||null):a.b.b.body.appendChild(a.f);a.j&&!a.j.Da||a.Ea()};
_.k=_.ah.prototype;_.k.Bf=function(){return!0};_.k.Wb=function(a){this.f=a};_.k.Ea=function(){this.Da=!0;_.fh(this,function(a){!a.Da&&a.C()&&a.Ea()})};_.k.hb=function(){_.fh(this,function(a){a.Da&&a.hb()});this.M&&_.zg(this.M);this.Da=!1};_.k.P=function(){this.Da&&this.hb();this.M&&(this.M.sa(),delete this.M);_.fh(this,function(a){a.sa()});!this.Ja&&this.f&&_.Ae(this.f);this.j=this.A=this.f=this.G=this.w=null;_.ah.L.P.call(this)};
_.k.Bc=function(a,c,d){if(a.Da&&(d||!this.Da))throw Error("w");if(0>c||c>_.gh(this))throw Error("y");this.G&&this.w||(this.G={},this.w=[]);if(a.j==this){var e=_.bh(a);this.G[e]=a;_.Ie(this.w,a)}else{e=this.G;var f=_.bh(a);if(null!==e&&f in e)throw Error("g`"+f);e[f]=a}dh(a,this);_.Eg(this.w,c,0,a);a.Da&&this.Da&&a.j==this?(d=this.Uc(),c=d.childNodes[c]||null,c!=a.C()&&d.insertBefore(a.C(),c)):d?(this.f||this.Hb(),c=_.hh(this,c+1),eh(a,this.Uc(),c?c.f:null)):this.Da&&!a.Da&&a.f&&a.f.parentNode&&1==
a.f.parentNode.nodeType&&a.Ea()};_.k.Uc=function(){return this.f};_.gh=function(a){return a.w?a.w.length:0};_.hh=function(a,c){return a.w?a.w[c]||null:null};_.fh=function(a,c,d){a.w&&(0,_.Ma)(a.w,c,d)};_.ah.prototype.removeChild=function(a,c){if(a){var d="string"===typeof a?a:_.bh(a);a=this.G&&d?Sg(this.G,d)||null:null;if(d&&a){var e=this.G;d in e&&delete e[d];_.Ie(this.w,a);c&&(a.hb(),a.f&&_.Ae(a.f));dh(a,null)}}if(!a)throw Error("z");return a};

}catch(e){_._DumpException(e)}
try{
var jh,kh,lh;_.ih=function(a,c){var d=a.length-c.length;return 0<=d&&a.indexOf(c,d)==d};jh=function(a){return"string"==typeof a.className?a.className:a.getAttribute&&a.getAttribute("class")||""};kh=function(a){return a.classList?a.classList:jh(a).match(/\S+/g)||[]};lh=function(a,c){"string"==typeof a.className?a.className=c:a.setAttribute&&a.setAttribute("class",c)};_.R=function(a,c){return a.classList?a.classList.contains(c):_.Qa(kh(a),c)};
_.S=function(a,c){if(a.classList)a.classList.add(c);else if(!_.R(a,c)){var d=jh(a);lh(a,d+(0<d.length?" "+c:c))}};_.mh=function(a,c){if(a.classList)(0,_.Ma)(c,function(f){_.S(a,f)});else{var d={};(0,_.Ma)(kh(a),function(f){d[f]=!0});(0,_.Ma)(c,function(f){d[f]=!0});c="";for(var e in d)c+=0<c.length?" "+e:e;lh(a,c)}};_.T=function(a,c){a.classList?a.classList.remove(c):_.R(a,c)&&lh(a,(0,_.Na)(kh(a),function(d){return d!=c}).join(" "))};
_.nh=function(a,c){a.classList?(0,_.Ma)(c,function(d){_.T(a,d)}):lh(a,(0,_.Na)(kh(a),function(d){return!_.Qa(c,d)}).join(" "))};

}catch(e){_._DumpException(e)}
try{
_.ph=function(a,c,d){_.oh.H(c,d,void 0,a.T||a,a);return a};_.qh=function(a,c){c=c instanceof _.tb?c:_.xb(c);a.href=_.ub(c)};_.rh=function(a,c){var d=c||document;return d.querySelectorAll&&d.querySelector?d.querySelectorAll("."+a):_.re(document,"*",a,c)};_.sh=function(a,c){c.parentNode&&c.parentNode.insertBefore(a,c.nextSibling)};_.th=function(a,c,d){for(var e=0;a&&(null==d||e<=d);){if(c(a))return a;a=a.parentNode;e++}return null};
_.uh=function(a,c){return c?_.th(a,function(d){return!c||"string"===typeof d.className&&_.Qa(d.className.split(/\s+/),c)},void 0):null};
var vh,wh;vh=function(){};_.oh=new vh;wh=["click","keydown","keyup"];vh.prototype.H=function(a,c,d,e,f){var g=function(h){var l=_.$e(c),m=_.Be(h.target)?h.target.getAttribute("role")||null:null;"click"==h.type&&_.ug(h)?l.call(e,h):13!=h.keyCode&&3!=h.keyCode||"keyup"==h.type?32!=h.keyCode||"keyup"!=h.type||"button"!=m&&"tab"!=m||(l.call(e,h),h.preventDefault()):(h.type="keypress",l.call(e,h))};g.wb=c;g.Zj=e;f?f.H(a,wh,g,d):_.O(a,wh,g,d)};
vh.prototype.Ba=function(a,c,d,e,f){for(var g,h=0;g=wh[h];h++){var l=a;var m=g;var n=!!d;m=_.Pe(l)?l.Rc(m,n):l?(l=_.bf(l))?l.Rc(m,n):[]:[];for(l=0;n=m[l];l++){var r=n.listener;if(r.wb==c&&r.Zj==e){f?f.Ba(a,g,n.listener,d,e):_.ff(a,g,n.listener,d,e);break}}}};

}catch(e){_._DumpException(e)}
try{
_.xh=!_.y&&!_.cb();

}catch(e){_._DumpException(e)}
try{
/*

 Copyright The Closure Library Authors.
 SPDX-License-Identifier: Apache-2.0
*/
_.yh=function(a){return/^[\s\xa0]*$/.test(a)};

}catch(e){_._DumpException(e)}
try{
var zh;zh=function(a,c,d){if(a.f)return null;if(d instanceof Array){var e=null,f;for(f in d){var g=zh(a,c,d[f]);g&&(e=g)}return e}e=null;a.b&&a.b.type==d&&a.j==c&&(e=a.b,a.b=null);if(f=c.getAttribute("data-eqid"))c.removeAttribute("data-eqid"),(f=a.o[f])?c.removeEventListener?c.removeEventListener(d,f,!1):c.detachEvent&&c.detachEvent("on"+d,f):a.w.log(Error("l`"+c));return e};_.Ah=function(a,c,d){return function(){try{return c.apply(d,arguments)}catch(e){a.log(e)}}};
_.Ch=function(a,c,d,e,f,g){e=_.Ah(a,e,g);a=_.O(c,d,e,f,g);_.Bh(c,d);return a};_.Bh=function(a,c){if(a instanceof Element&&(c=zh(_.Xc("eq"),a,c||[])))if(_.y&&c instanceof MouseEvent&&a.dispatchEvent){var d=document.createEvent("MouseEvent");d.initMouseEvent(c.type,!0,!0,c.view,c.detail,c.screenX,c.screenY,c.clientX,c.clientY,c.ctrlKey,c.altKey,c.shiftKey,c.metaKey,c.button,c.relatedTarget);a.dispatchEvent(d)}else a.dispatchEvent&&a.dispatchEvent(c)};

}catch(e){_._DumpException(e)}
try{
_.Dh=function(a,c){_.vg.call(this,c);this.w=a;this.Ga=c||this};_.w(_.Dh,_.vg);_.Dh.prototype.H=function(a,c,d,e){if(d){if("function"!=typeof d)throw new TypeError("A");d=_.Ah(this.w,d,this.Ga);d=_.Dh.L.H.call(this,a,c,d,e);_.Bh(a,Eh(c));return d}return _.Dh.L.H.call(this,a,c,d,e)};_.Dh.prototype.o=function(a,c,d,e,f){if(d){if("function"!=typeof d)throw new TypeError("A");d=_.Ah(this.w,d,f||this.Ga);d=_.Dh.L.o.call(this,a,c,d,e,f);_.Bh(a,Eh(c));return d}return _.Dh.L.o.call(this,a,c,d,e,f)};
_.Dh.prototype.nb=function(a,c,d,e){if(d){if("function"!=typeof d)throw new TypeError("A");d=_.Ah(this.w,d,this.Ga);d=_.Dh.L.nb.call(this,a,c,d,e);_.Bh(a,Eh(c));return d}return _.Dh.L.nb.call(this,a,c,d,e)};var Eh=function(a){return _.Ba(a)?(0,_.Oa)(a,Eh):"string"===typeof a?a:a?a.toString():a};
_.Fh=function(a,c){_.Dh.call(this,c);this.f=a};_.w(_.Fh,_.Dh);_.Fh.prototype.C=function(){return this.f};_.Fh.prototype.P=function(){this.f=null;_.Fh.L.P.call(this)};

}catch(e){_._DumpException(e)}
try{
_.Gh=function(a,c,d){_.Fh.call(this,a,c);this.j=d;(a=_.M("gb_nc",this.f))&&_.ph(this,a,this.b)};_.w(_.Gh,_.Fh);_.Gh.prototype.b=function(a){var c;(a=a.b)&&(a=a.getAttributeNode("data-ved"))&&a.value&&(c={ved:a.value});this.j.log(39,c)};

}catch(e){_._DumpException(e)}
try{
var Lh,Mh,Ph,Qh,Sh,Uh,Vh,Wh,Xh,Yh,Zh,ai,ei,gi;_.Kh=function(a,c){c&&_.qh(a,a.href.replace(/([?&](continue|followup)=)[^&]*/g,"$1"+encodeURIComponent(c)))};Lh=function(a,c){if(void 0!==a.b||void 0!==a.f)throw Error("m");a.f=c;_.qd(a)};Mh=function(a){_.A(this,a,0,-1,null,null)};_.w(Mh,_.z);_.Nh=function(a,c){c.parentNode&&c.parentNode.insertBefore(a,c)};_.Oh=function(a,c,d){_.J.call(this);this.wb=a;this.f=c||0;this.b=d;this.Oa=(0,_.t)(this.Oh,this)};_.w(_.Oh,_.J);_.k=_.Oh.prototype;_.k.Sc=0;
_.k.P=function(){_.Oh.L.P.call(this);this.stop();delete this.wb;delete this.b};_.k.start=function(a){this.stop();this.Sc=_.rg(this.Oa,void 0!==a?a:this.f)};_.k.stop=function(){0!=this.Sc&&_.sg(this.Sc);this.Sc=0};_.k.Oh=function(){this.Sc=0;this.wb&&this.wb.call(this.b)};_.U=function(a,c,d){d?_.S(a,c):_.T(a,c)};Ph=function(a){a=a.getAttribute("src");return null!=a&&""!=a};
Qh=function(a,c,d){a=_.M("gb_ua",a.C());if(""!=c||""!=d)if(_.R(a,"gb_ra")){var e=a.style[_.Fg("background-image")];""!=("undefined"!==typeof e?e:a.style[_.Ig(a,"background-image")]||"")&&(c=""!=d?d:c,_.Jg(a,"background-image","url('"+c+"')"),a=_.M("gb_qc",a),null!=a&&Ph(a)&&a.setAttribute("src",c))}else"IMG"==a.tagName&&(e=""!=c?c:d,null!=a&&Ph(a)&&a.setAttribute("src",e),c!=d&&(d=""!=d?d+" 2x ":"",""!=c&&(d=d+(""==d?"":",")+(c+" 1x")),a.setAttribute("srcset",d)))};
_.Rh=function(a,c){c&&_.Ih(a)&&c!=_.Ih(a)&&_.Ih(a).me(!1);a.j=c};Sh=function(a){return String(a).replace(/([A-Z])/g,"-$1").toLowerCase()};_.Th=function(a,c){return _.M(a,c)};Uh=function(a,c){var d=c.parentNode;d&&d.replaceChild(a,c)};Vh=function(a,c,d,e){if(null!=a)for(a=a.firstChild;a;){if(c(a)&&(d.push(a),e)||Vh(a,c,d,e))return!0;a=a.nextSibling}return!1};Wh=function(a,c){var d=[];return Vh(a,c,d,!0)?d[0]:void 0};Xh=function(a,c){var d=[];Vh(a,c,d,!1);return d};
Yh=function(a){return _.y&&!_.gc("9")?(a=a.getAttributeNode("tabindex"),null!=a&&a.specified):a.hasAttribute("tabindex")};Zh=function(a){a=a.tabIndex;return"number"===typeof a&&0<=a&&32768>a};_.$h=function(a,c){c?a.tabIndex=0:(a.tabIndex=-1,a.removeAttribute("tabIndex"))};
ai=function(a){var c;if((c="A"==a.tagName&&a.hasAttribute("href")||"INPUT"==a.tagName||"TEXTAREA"==a.tagName||"SELECT"==a.tagName||"BUTTON"==a.tagName?!a.disabled&&(!Yh(a)||Zh(a)):Yh(a)&&Zh(a))&&_.y){var d;!_.Ca(a.getBoundingClientRect)||_.y&&null==a.parentElement?d={height:a.offsetHeight,width:a.offsetWidth}:d=a.getBoundingClientRect();a=null!=d&&0<d.height&&0<d.width}else a=c;return a};
_.bi=function(a){if(_.ne&&null!==a&&"innerText"in a)a=a.innerText.replace(/(\r\n|\r|\n)/g,"\n");else{var c=[];_.mg(a,c,!0);a=c.join("")}a=a.replace(/ \xAD /g," ").replace(/\xAD/g,"");a=a.replace(/\u200B/g,"");_.ne||(a=a.replace(/ +/g," "));" "!=a&&(a=a.replace(/^\s*/,""));return a};_.ci=function(a,c){a=a.getAttribute("aria-"+c);return null==a||void 0==a?"":String(a)};_.di=function(a,c,d){if(_.xh&&a.dataset)a.dataset[c]=d;else{if(/-[a-z]/.test(c))throw Error("j");a.setAttribute("data-"+Sh(c),d)}};
ei=function(a){if(/-[a-z]/.test("item"))return null;if(_.xh&&a.dataset){if(_.db()&&!("item"in a.dataset))return null;a=a.dataset.item;return void 0===a?null:a}return a.getAttribute("data-"+Sh("item"))};gi=function(a,c){return/-[a-z]/.test(c)?!1:_.xh&&a.dataset?c in a.dataset:a.hasAttribute?a.hasAttribute("data-"+Sh(c)):!!a.getAttribute("data-"+Sh(c))};_.ii=function(a,c){_.Q.call(this);this.b=a;this.j=hi(this.b);this.B=c||100;this.o=_.O(a,"resize",this.w,!1,this)};_.w(_.ii,_.Q);
_.ii.prototype.P=function(){_.gf(this.o);_.ii.L.P.call(this)};_.ii.prototype.w=function(){this.f||(this.f=new _.Oh(this.A,this.B,this),_.Yf(this,this.f));this.f.start()};_.ii.prototype.A=function(){if(!this.b.Sa){var a=this.j,c=hi(this.b);this.j=c;if(a){var d=!1;a.width!=c.width&&(this.dispatchEvent("b"),d=!0);a.height!=c.height&&(this.dispatchEvent("a"),d=!0);d&&this.dispatchEvent("resize")}else this.dispatchEvent("a"),this.dispatchEvent("b"),this.dispatchEvent("resize")}};
var ji=function(a){_.Q.call(this);this.f=a||window;this.j=_.O(this.f,"resize",this.o,!1,this);this.b=_.dg(this.f)},ki,hi;_.w(ji,_.Q);_.li=function(){var a=window,c=_.Cg(a);return ki[c]=ki[c]||new ji(a)};ki={};hi=function(a){return a.b?_.Ag(a.b):null};ji.prototype.P=function(){ji.L.P.call(this);this.j&&(_.gf(this.j),this.j=null);this.b=this.f=null};ji.prototype.o=function(){var a=_.dg(this.f);_.Hg(a,this.b)||(this.b=a,this.dispatchEvent("resize"))};
var mi;mi=function(a){return null!=_.th(a,function(c){return 1==c.nodeType&&"true"==_.ci(c,"hidden")})};_.ni=function(a){return a?Xh(a,function(c){return 1==c.nodeType&&ai(c)&&!mi(c)}):[]};
_.oi=function(a){this.f=a;this.b=null};_.pi=function(a){a.b||(a.b=_.O(a.f,"keydown",a.j,!1,a))};_.ri=function(a){qi(a);_.U(a.f,"gb_u",!1)};_.oi.prototype.j=function(a){9!=a.keyCode||_.R(this.f,"gb_u")||(_.U(this.f,"gb_u",!0),qi(this))};var qi=function(a){a.b&&(_.gf(a.b),a.b=null)};
_.si=function(a,c){_.Q.call(this);this.A=a;c&&(this.A.id=c)};_.w(_.si,_.Q);_.si.prototype.C=function(){return this.A};_.si.prototype.Ga=function(){return this.A.id};_.si.prototype.Y=function(){var a=this.A.id;a||(a="gb$"+_.Zg(_.Yg.ta()),this.A.id=a);return a};_.si.prototype.P=function(){_.Ae(this.A);_.si.L.P.call(this)};
_.ti=function(a){_.si.call(this,a);_.oh.H(a,this.b,!1,this)};_.w(_.ti,_.si);_.ti.prototype.b=function(a){this.dispatchEvent("click")||a.preventDefault()};
_.ui=function(a){return Wh(a,function(c){return _.Be(c)&&ai(c)})};_.vi=function(a){(a=_.ui(a))&&a.focus()};
var wi=function(){};
var xi=function(a,c,d){this.f=a;this.j=c;this.b=d||_.q};
var yi=function(){this.b=[]};yi.prototype.f=function(a,c,d){this.w(a,c,d);this.b.push(new xi(a,c,d))};yi.prototype.w=function(a,c,d){d=d||_.q;for(var e=0,f=this.b.length;e<f;e++){var g=this.b[e];if(g.f==a&&g.j==c&&g.b==d){this.b.splice(e,1);break}}};yi.prototype.j=function(a){for(var c=0,d=this.b.length;c<d;c++){var e=this.b[c];"catc"==e.f&&e.j.call(e.b,a)}};
var Ai=function(a,c){this.o=new yi;this.D=a;this.A=c;this.b=zi(a.offsetWidth,this.A);this.G=new _.ii(_.li(),10);_.O(this.G,"b",function(){window.requestAnimationFrame?window.requestAnimationFrame((0,_.t)(this.B,this)):this.B()},!1,this)},zi=function(a,c){for(var d=0,e=c.length-1,f=c[0];d<e;){if(a<=f.max)return f.id;f=c[++d]}return c[e].id};Ai.prototype.B=function(){var a=zi(this.D.offsetWidth,this.A);a!=this.b&&(this.b=a,this.j(new wi))};Ai.prototype.f=function(a,c,d){this.o.f(a,c,d)};
Ai.prototype.w=function(a,c){this.o.w(a,c)};Ai.prototype.j=function(a){this.o.j(a)};
var Bi={Uk:"gb_ta",ll:"gb_Vd",Dk:"gb_Dc"};
var Ci={id:"unlimitedProductControl",ke:Number.MAX_SAFE_INTEGER};
var Di=function(a,c){c||(c=this.createElement(),a.Dd().appendChild(c));_.si.call(this,c);this.w=new _.vg(this);_.ph(this.w,this.C(),this.Yh)};_.w(Di,_.si);_.k=Di.prototype;_.k.createElement=function(){var a=_.ze("LI");_.S(a,"gb_Lc");_.Fe(a,"menuitem");return a};_.k.uj=function(a){a?_.di(this.C(),"item",a):(a=this.C(),!/-[a-z]/.test("item")&&(_.xh&&a.dataset?gi(a,"item")&&delete a.dataset.item:a.removeAttribute("data-"+Sh("item"))));return this};_.k.Cd=function(){return ei(this.C())};
_.k.Zc=function(a){_.U(this.C(),"gb_Nc",a);return this};_.k.focus=function(){_.vi(this.C())};_.k.Yh=function(){this.dispatchEvent("click")};
var Ei=function(a,c){Di.call(this,a,c);this.j=_.Th("gb_Oc",this.C());this.o=_.M("gb_Qc",this.j);this.b=null;this.f=_.M("gb_Pc",this.j)};_.p(Ei,Di);_.k=Ei.prototype;_.k.createElement=function(){var a=Di.prototype.createElement.call(this);_.S(a,"gb_Rc");var c=_.ve("A","gb_Oc");_.$h(c,!0);a.appendChild(c);var d=_.ve("SPAN","gb_Pc");c.appendChild(d);return a};_.k.Cd=function(){return Di.prototype.Cd.call(this)||this.wg()};_.k.wg=function(){return _.bi(this.f)};_.k.wj=function(a){_.ig(this.f,a);return this};
_.k.vj=function(a){this.o||(this.o=_.ve("IMG","gb_Qc"),this.o.setAttribute("alt",""),this.b?(Uh(this.o,this.b),this.b=null):_.Nh(this.o,this.f));this.o.setAttribute("src",a);return this};_.k.fk=function(a){if(!(a instanceof Element&&"svg"==a.tagName.toLowerCase()))return this;this.o?(Uh(a,this.o),this.o=null):this.b?Uh(a,this.b):_.Nh(a,this.f);var c=a.getAttribute("class");c?a.setAttribute("class",c+" gb_Qc"):a.setAttribute("class","gb_Qc");this.b=a;return this};_.k.focus=function(){this.j.focus()};
_.Fi=function(a){_.si.call(this,a);this.f=[];this.F={}};_.w(_.Fi,_.si);_.si.prototype.Dd=function(){return this.C()};_.Fi.prototype.Aa=function(a){var c=this.F[a];if(c)return c;var d=document.getElementById(a);if(d)for(var e=0,f=this.f.length;e<f;++e)if(c=this.f[e],c.C()==d)return this.F[a]=c;return null};_.Fi.prototype.Db=function(a){a.Kc(this);this.f.push(a);var c=a.A.id;c&&(this.F[c]=a)};_.Fi.prototype.V=function(){for(var a=0,c=this.f.length;a<c;a++)this.f[a].sa();this.F={};this.f=[]};
var Gi=function(a,c){_.Fi.call(this,c||this.createElement());this.j=a;a=this.C().getElementsByClassName("gb_Lc");for(c=0;c<a.length;c++){var d=a[c];_.R(d,"gb_Rc")?this.Db(new Ei(this,d)):this.Db(new Di(this,d))}this.b=_.M("gb_Mc",this.C())};_.w(Gi,_.Fi);_.k=Gi.prototype;_.k.createElement=function(){var a=_.ze("UL");_.S(a,"gb_Ic");var c=_.ve("SPAN","gb_Mc");a.appendChild(c);return a};_.k.Db=function(a){Gi.L.Db.call(this,a);var c=this.j,d=a.C();d=d.id||(d.id="gbm"+_.Zg(_.Yg.ta()));c.O[d]=a};
_.k.sj=function(){return null!=this.b?_.bi(this.b):null};_.k.tj=function(a){return null!=this.b?(_.ig(this.b,a),this):null};_.k.Xg=function(){var a=new Di(this);this.Db(a);return a};_.k.Yg=function(){var a=new Ei(this);this.Db(a);return a};
var V=function(a,c,d,e,f,g,h){_.Fi.call(this,a);this.b=c;this.B=a;this.w=d;this.M=e;this.J=f;this.o=_.M("gb_Ec",this.b);this.K=new _.oi(this.o);this.D=_.M("gb_Fc",this.o);this.G=_.M("gb_Hc",this.o);this.O={};this.N=[];this.R=g||!1;this.U=h||!1;this.j=new _.vg(this);Hi(this);a=this.o.getElementsByClassName("gb_Ic");for(c=0;c<a.length;c++)this.Db(new Gi(this,a[c]))};_.p(V,_.Fi);_.k=V.prototype;_.k.P=function(){_.Fi.prototype.P.call(this);Ii(this)};_.k.Dd=function(){return this.o};
_.k.xj=function(){return _.M("gb_le",this.b)};_.k.Wg=function(){Ji(this);return Ki(this,this.D)};_.k.Vg=function(){Ji(this);return Ki(this,this.G)};var Ki=function(a,c){var d=new Gi(a),e=d.C();c.appendChild(e);a.Db(d);return d},Ji=function(a){a.D||(a.D=_.ze("DIV"),_.S(a.D,"gb_Fc"),a.o.appendChild(a.D),a.G=_.ze("DIV"),_.S(a.G,"gb_Hc"),a.o.appendChild(a.G))};V.prototype.va=function(a){_.U(this.b,"gb_Cc",1==a);this.dispatchEvent("msc")};V.prototype.$=function(){return Li(this)?0:1};
var Mi=function(a,c){switch(c){case "menu":_.T(a.C(),"gb_Fa");break;case "back":_.T(a.w,"gb_Fa");break;case "close":_.T(a.M,"gb_Fa")}},Ni=function(a){_.S(a.C(),"gb_Fa");_.S(a.w,"gb_Fa");_.S(a.M,"gb_Fa")},Oi=function(a){return!_.R(a,"gb_Fa")};_.k=V.prototype;_.k.isVisible=function(a){switch(a){case "menu":return Oi(this.C());case "back":return Oi(this.w);case "close":return Oi(this.M)}return!1};
_.k.ef=function(a){this.J||(a&&_.Jg(this.b,"transition","none"),this.dispatchEvent("beforeshow"),_.S(this.b,"gb_na"),_.Ge(this.C(),"expanded",!0),_.vi(this.o),_.pi(this.K),this.dispatchEvent("open"),this.j.o(document.body,Pi,this.T,!0,this),this.j.H(document.body,"focusin",this.S),a&&_.rg(function(){_.Jg(this.b,"transition","")},0,this))};_.k.ak=function(a){this.J&&_.Ge(this.C(),"expanded",a)};
_.k.close=function(a){this.J||(a&&_.Jg(this.b,"transition","none"),_.T(this.b,"gb_na"),_.Ge(this.C(),"expanded",!1),document.activeElement==this.C()&&this.C().blur(),_.ri(this.K),this.dispatchEvent("close"),Ii(this),a&&_.rg(function(){_.Jg(this.b,"transition","")},0,this))};_.k.nk=function(a){Oi(this.B)&&_.S(this.B,"gb_wc");_.T(this.w,"gb_Fa");a&&_.Ze(this.w,"click",a)};_.k.Ri=function(){_.S(this.w,"gb_Fa");_.R(this.B,"gb_wc")&&_.T(this.B,"gb_wc")};_.k.Sb=function(){return _.R(this.b,"gb_na")};
var Hi=function(a){_.ph(a.j,a.C(),a.ka);a.C().addEventListener("keydown",function(c){32==c.keyCode&&c.preventDefault()});_.ph(a.j,a.o,a.Z);a.j.H(a.b,"keydown",a.ua);a.j.H(a.b,"keyup",a.ma);_.ph(a.j,a.w,function(){this.dispatchEvent("bbc")});_.ph(a.j,a.M,function(){this.dispatchEvent("cbc")});if(_.R(a.b,"gb_ta")||_.R(a.b,"gb_Vd"))a.j.H(window,"resize",a.W),a.W();_.R(a.b,"gb_yc")||a.j.nb(window,"touchstart",function(){_.Jg(a.b,"overflow-y","auto")})};
V.prototype.W=function(){var a=window.visualViewport?window.visualViewport.height:window.innerHeight;a&&_.Jg(this.b,"height","calc("+a+"px - 100%)")};V.prototype.ka=function(){this.dispatchEvent("mbc");if(!this.J){if(this.Sb()){this.close();var a=!0}else this.ef(),a=!1;a&&this.C().focus()}};var Li=function(a){return!_.R(a.b,"gb_Cc")||_.R(a.b,"gb_ta")||_.R(a.b,"gb_Vd")};V.prototype.ma=function(a){9===a.keyCode&&this.Sb()&&(a=this.K,_.U(a.f,"gb_u",!0),qi(a))};
V.prototype.ua=function(a){a:{if(36==a.keyCode||35==a.keyCode){var c=_.ni(this.b);if(0<c.length){var d=c[c.length-1];36==a.keyCode&&(d=!Li(this)&&1<c.length?c[1]:c[0]);d.focus();a.preventDefault();break a}}27!=a.keyCode||this.R&&!Li(this)||(this.close(),null!=this.B&&this.B.focus())}9===a.keyCode&&this.Sb()&&Li(this)&&(c=a.target,d=_.ni(this.b),0<d.length&&(c==d[0]&&a.shiftKey?(d[d.length-1].focus(),a.preventDefault()):c!=d[d.length-1]||a.shiftKey||(d[0].focus(),a.preventDefault())))};
V.prototype.Z=function(a){if(a.target instanceof Node){a:{a=a.target;for(var c=this.o;a&&a!==c;){var d=a.id;if(d in this.O){a=this.O[d];break a}a=a.parentNode}a=null}if(a){a=a.Cd();c=0;for(d=this.N.length;c<d;++c){var e=this.N[c];e.Oa.call(e.b,a)}this.R&&!Li(this)||this.close()}}};var Qi=function(a){return a instanceof HTMLElement&&gi(a,"ogobm")};
V.prototype.T=function(a){this.Sb()&&a.target instanceof Node&&!(!Li(this)||this.U&&_.th(a.target,Qi))&&("keydown"==a.type?27==a.keyCode&&(a.preventDefault(),a.stopPropagation(),this.close(),this.C().focus()):_.uh(a.target,"gb_F")||_.uh(a.target,"gb_rc")||_.hg(this.b,a.target)||("touchstart"==a.type&&(a.preventDefault(),a.stopPropagation()),this.close()))};
V.prototype.S=function(){this.Sb()&&(!Li(this)||"IFRAME"!=document.activeElement.tagName&&(this.U&&_.th(document.activeElement,Qi)||_.uh(document.activeElement,"gb_xc")||_.uh(document.activeElement,"gb_F")||_.vi(this.o)))};var Ii=function(a){a.j.Ba(document.body,Pi,a.T,!1,a);a.j.Ba(document.body,"focusin",a.S)};V.prototype.X=function(a,c){this.N.push(new Ri(a,c))};var Pi="click mousedown scroll touchstart wheel keydown".split(" "),Ri=function(a,c){this.Oa=a;this.b=c};
_.Si=function(a){_.si.call(this,a);_.O(a,"click",this.b,!1,this)};_.w(_.Si,_.si);_.Si.prototype.f=function(){var a=this.C().getAttribute("aria-pressed");return(null==a?a:"boolean"===typeof a?a:"true"==a)||!1};_.Si.prototype.b=function(a){a=a.b;var c=_.ci(a,"pressed");_.yh(_.Tg(c))||"true"==c||"false"==c?_.Ge(a,"pressed","true"==c?"false":"true"):a.removeAttribute("aria-pressed");this.dispatchEvent("click")};
_.Ti=function(){_.u("gbar.I",_.si);_.si.prototype.ia=_.si.prototype.Ga;_.si.prototype.ib=_.si.prototype.C;_.si.prototype.ic=_.si.prototype.Y;_.u("gbar.J",_.Fi);_.Fi.prototype.ja=_.Fi.prototype.Aa;_.Fi.prototype.jb=_.Fi.prototype.V;_.u("gbar.K",_.ti);_.u("gbar.L",_.Si);_.Si.prototype.la=_.Si.prototype.f};
var W=function(a,c,d,e){_.Q.call(this);this.j=a;_.T(this.j,"gb_Nd");this.f=c;this.M=d;this.tb="";this.Vb=e;this.D=this.b=null;this.Ma=this.O=this.X=!1;this.ua=_.K(_.C(this.f,16),!1);this.V=new _.vg(this);this.Ga=_.M("gb_Xc",this.j);this.S=_.K(_.C(c,6),!1);this.nd=_.M("gb_2c",this.Ga);this.w=_.M("gb_Od",this.j);this.K=_.M("gb_Zd",this.j);(this.$=_.K(_.C(this.f,21),!1))&&this.w&&(this.va=_.M("gb_ze",this.j),this.R=_.M("gb_De",this.j),this.N=_.M("gb_Ae",this.j));this.F=_.M("gb_Tc",this.j);this.U=_.M("gb_Kc",
this.j);this.Ae=_.M("gb_Uc",this.j);this.B=_.M("gb_0c",this.j);this.A=_.M("gb_1d",this.j);this.Y=Array.prototype.slice.call(_.rh("gb_6d",this.j));this.T=!1;this.Ac=_.K(_.C(this.f,19),!1);this.yc=_.K(_.C(this.f,20),!1);a=Ui(this,!0);c=Ui(this,!1);this.kd=Math.max(a,c);this.W=_.C(this.f,15);d=_.Mc(_.B(this.f,30),0);0!=d&&Vi(this,d);a=Wi(this,a,c);this.G=new Ai(this.j,Xi);this.hc=_.L(_.B(this.f,37));this.bc=_.L(_.B(this.f,38));this.zc=_.R(this.j,"gb_3d");this.rd=_.K(_.C(this.f,39));this.$&&this.w&&(this.$a=
new Ai(this.j,Yi),this.$a.f("catc",this.ka,this),this.ka(),_.ph(this.V,this.va,function(){var f=this.R,g=!_.R(f,"gb_Fa");_.U(f,"gb_Fa",g)}));this.jd=_.K(_.C(this.f,1),!1);this.hd=_.K(_.C(this.f,40),!1);this.jc=_.K(_.C(this.f,42),!1);Zi(this);$i(this,this.G.b);this.G.f("catc",this.lc,this);_.C(this.f,8)&&document.addEventListener("scroll",(0,_.t)(function(){_.U(this.j,"gb_Qd",0<window.scrollY)},this));null!=this.A&&_.C(this.f,7)&&(this.ma=new Ai(this.A,a),this.ma.f("catc",this.Re,this),this.Re())};
_.w(W,_.Q);var aj="click mousedown scroll touchstart wheel keydown".split(" "),Xi=[{id:"gb_ta",max:599},{id:"gb_Vd",max:1023},{id:"gb_Dc"}],Yi=[{id:{id:"oneProductControl",ke:1},max:320},{id:{id:"twoProductControl",ke:2},max:360},{id:{id:"threeProductControl",ke:3},max:410},{id:Ci}];_.k=W.prototype;_.k.C=function(){return this.j};_.k.hk=function(a){this.D=a;bj(this,this.X);a=cj(this);0!=a&&dj(this,a)};_.k.ik=function(a,c){this.D&&Qh(this.D,a,c)};
_.k.dk=function(a){this.Ub(a||this.rd?1:0);this.Fb(a?this.hc:this.bc);var c=_.M("gb_4");null!=c&&_.U(c,"gb_ja",a);this.b&&this.hd&&_.U(this.b.b,"gb_Bc",a);_.sd.ta().b.then(function(d){this.jc&&d.sk(a);d.qj(a)},void 0,this)};_.k.jk=function(a){this.Ga&&(_.ig(this.nd,a||""),_.U(this.Ga,"gb_Fa",!a),this.S=!!a,$i(this,this.G.b))};_.k.yj=function(){return _.M("gb_le",this.w)};_.k.Re=function(){if(null!=this.ma){var a=this.ma.b;3==a?ej(this,!1):1==a?ej(this,!0):ej(this,"gb_Dc"==this.G.b)}};
var ej=function(a,c){if(_.C(a.f,7)&&(!a.T||c)){if(a.W){var d=_.M("gb_re",a.j);if(d){var e=_.M("gb_se",a.j),f="gb_Dc"!=a.G.b||c?"":a.kd+"px";_.Jg(d,"min-width",f);_.Jg(e,"min-width",f)}}_.R(a.A,"gb_Fe")!=c&&(_.U(a.A,"gb_Fe",c),c?a.dispatchEvent("sfi"):a.dispatchEvent("sfu"),_.U(_.M("gb_Te",a.A),"gb_Fe",c),c&&a.ka())}},Zi=function(a){var c=_.sd.ta();a.w||Lh(c.f,Error("F"));_.K(_.C(a.f,11))||Lh(c.D,Error("G"));_.K(_.C(a.f,7))||Lh(c.B,Error("H"));_.K(_.C(a.f,12))||Lh(c.w,Error("I"));_.K(_.C(a.f,13))||
Lh(c.A,Error("J"));_.K(_.C(a.f,41))||Lh(c.j,Error("K"))},$i=function(a,c){if(!a.b&&a.w){var d=_.M("gb_rc",a.j);if(d){var e=_.M("gb_xc");if(e){var f=_.M("gb_uc");if(f){var g=_.M("gb_vc");if(g){a.b=new V(d,e,f,g,_.K(_.C(a.f,16),!1),_.K(_.C(a.f,9),!1),_.K(_.C(a.f,33),!1));a.b.H("open",a.nc,!1,a);a.b.H("close",a.mc,!1,a);a.b.H("msc",a.qc,!1,a);switch(_.B(a.f,32)){case 1:a.J("back");break;case 2:a.J("close");break;case 3:a.J("none");break;default:a.J("default")}_.Ti();_.u("gbar.C",V);V.prototype.ca=V.prototype.Dd;
V.prototype.cb=V.prototype.Wg;V.prototype.cc=V.prototype.X;V.prototype.cd=V.prototype.va;V.prototype.ce=V.prototype.Vg;V.prototype.cf=V.prototype.ef;V.prototype.cg=V.prototype.close;V.prototype.ch=V.prototype.$;V.prototype.ci=V.prototype.nk;V.prototype.cj=V.prototype.Ri;V.prototype.ck=V.prototype.Sb;V.prototype.cl=V.prototype.ak;V.prototype.cm=V.prototype.xj;_.u("gbar.D",Gi);Gi.prototype.da=Gi.prototype.Xg;Gi.prototype.db=Gi.prototype.Yg;Gi.prototype.dc=Gi.prototype.sj;Gi.prototype.dd=Gi.prototype.tj;
_.u("gbar.E",Di);Di.prototype.ea=Di.prototype.C;Di.prototype.eb=Di.prototype.Zc;Di.prototype.ec=Di.prototype.uj;Di.prototype.ed=Di.prototype.Cd;_.u("gbar.F",Ei);Ei.prototype.fa=Ei.prototype.wj;Ei.prototype.fb=Ei.prototype.vj;Ei.prototype.fc=Ei.prototype.fk;Ei.prototype.fd=Ei.prototype.wg;Ei.prototype.ed=Ei.prototype.Cd;_.rd(_.sd.ta().f,a.b)}else a.M.log(Error("B"))}else a.M.log(Error("C"))}else a.M.log(Error("D"))}else a.M.log(Error("E"))}a.b&&!a.O&&a.J("default");a.b&&a.yc&&a.J("none");fj(a);a.Ac||
a.ua?a.X=!0:(d="gb_ta"==c,e=_.K(_.C(a.f,5),!1),f=_.K(_.C(a.f,7),!1),a.X=!(a.S||d&&(e||f)));d=gj(a,c);a.b&&d?_.hj(a)||null==a.U||(d=_.M("gb_Jc"),a.U.parentNode!=d&&d.insertBefore(a.U,d.childNodes[0]||null),_.S(a.F,"gb_2d"),a.Z(),a.dispatchEvent("upi")):_.hj(a)&&a.w&&null!=a.U&&(d=a.Ae,d.insertBefore(a.U,d.childNodes[0]||null),_.T(a.F,"gb_2d"),a.Z(),a.dispatchEvent("upo"));d="gb_ta"==c;a.D&&!a.ua&&(e=a.D.C(),f=!a.S,_.U(e,"gb_Fa",!f),f&&bj(a,a.X));a.b&&(a.b.isVisible("menu")||a.b.isVisible("back"))&&
!Li(a.b)&&(a.Ma=a.b.Sb());e=_.Zf(Bi);_.nh(a.j,e);_.S(a.j,c);_.C(a.f,7);a.W&&null!=a.B&&("gb_Dc"!=c?(_.Jg(a.B,"min-width",""),_.Jg(a.F,"min-width","")):(f=_.Qg(a.B).width,g=_.Qg(a.F).width,f=Math.max(f,g),_.Jg(a.B,"min-width",f+"px"),_.Jg(a.F,"min-width",f+"px")));d?a.T||(a.T=!0,ej(a,a.T)):(a.T=!1,a.Re());null!=a.A&&(f="gb_Vd"==c,_.U(a.A,"gb_Me",!d&&!f),_.U(a.A,"gb_Le",d||f));a.b&&(d=a.b.b,_.nh(d,e),_.S(d,c),Li(a.b)?_.M("gb_ae",void 0).appendChild(d):a.j.appendChild(d),a.b.isVisible("menu")||a.b.isVisible("back"))&&
(c=!Li(a.b),d=a.b.Sb(),c&&!d&&a.Ma?a.b.ef():!c&&d&&a.b.close());_.ij(a)},bj=function(a,c){var d=_.M("gb_ua",a.D.C());_.U(d,"gb_Fa",!c);a=_.M("gb_8d",a.D.C());null!=a&&_.U(a,"gb_ke",!c)},Wi=function(a,c,d){var e=320,f=_.Mc(_.B(a.f,29),0);0<f&&(e=f);f=e+2*Math.max(c,d);c=e+c+d;return f!=c&&a.W?[{id:1,max:c},{id:2,max:f},{id:3}]:[{id:1,max:c},{id:3}]},Ui=function(a,c){if(a=_.M(c?"gb_re":"gb_se",a.j)){var d=a.offsetWidth;(0,_.Ma)(a.children,function(e){_.R(e,"gb_Fa")&&(d-=e.offsetWidth)});return d}return 0},
jj=function(a){return function(){a.click()}},kj=function(a){var c=_.M("gb_re",a.j),d=_.M("gb_se",a.j),e=[];c&&(0,_.Ma)(c.children,function(f){e.push(f)});_.K(_.C(a.f,7),!1)&&(a=_.M("gb_Fe",a.A))&&(a=_.M("gb_nf",a),a.b=!0,e.push(a));d&&(0,_.Ma)(d.children,function(f){e.push(f)});return e};
W.prototype.ka=function(){if(this.$&&this.w){var a=kj(this),c=!1;a=(0,_.Na)(a,function(g){c=c||_.R(g,"gb_ue");return _.R(g,"gb_Wc")||_.R(g,"gb_Ff")||_.R(g,"gb_nf")});var d=this.$a.b.ke,e=!1;if(a.length>d||c)e=!0,d--;var f=a.length-d;if(e!=!_.R(this.va,"gb_Fa")||f!=this.N.children){_.U(this.va,"gb_Fa",!e);if(e)for(;this.N.firstChild;)this.N.removeChild(this.N.firstChild);lj(this,a,d);e?this.V.o(document.body,aj,this.Ja,!0,this):this.V.Ba(document.body,aj,this.Ja,!1,this)}}};
var lj=function(a,c,d){c=(0,_.Na)(c,function(g){return _.R(g,"gb_ue")?(mj(this,g),!1):!0},a);for(var e=0;e<c.length;e++){var f=c[e];e>=d?mj(a,f):_.T(f,"gb_Fa")}},mj=function(a,c){_.S(c,"gb_Fa");var d=_.ze("LI");_.mh(d,["gb_Be","gb_Lc","gb_Rc"]);_.$h(d,!0);_.ph(a.V,d,jj(c));var e=_.ve("A","gb_Oc");d.appendChild(e);var f=_.ve("SPAN","gb_Pc");e.appendChild(f);e=c.b?c.getAttribute("aria-label"):c.title;_.ig(f,e);e=!1;_.R(c,"gb_Ff")&&(e=!0);var g,h=c.children[0];e?g=h.children[0].children[0].src:c.b?g=
"https://www.gstatic.com/images/icons/material/system/1x/search_black_24dp.png":g=h.src;a.o=_.ve("IMG");_.mh(a.o,["gb_Qc","gb_Ce"]);a.o.setAttribute("src",g);_.Nh(a.o,f);a.N.appendChild(d)};W.prototype.Ja=function(a){!_.R(this.R,"gb_Fa")&&a.target instanceof Node&&("keydown"==a.type?27==a.keyCode&&(a.preventDefault(),a.stopPropagation(),_.S(this.R,"gb_Fa"),this.C().focus()):_.hg(this.R,a.target)||("touchstart"==a.type&&(a.preventDefault(),a.stopPropagation()),_.S(this.R,"gb_Fa")))};
W.prototype.lc=function(){$i(this,this.G.b);this.b&&_.nj(this,this.b.Sb(),!1);this.dispatchEvent("ffc")};_.nj=function(a,c,d){a.b&&(Li(a.b)&&(d=c=!1),a=document.body,_.U(a,"gb_pe",c),_.U(a,"gb_oe",d))};W.prototype.nc=function(){_.nj(this,!0,!0)};W.prototype.mc=function(){_.nj(this,!1,!0)};W.prototype.qc=function(){var a=Li(this.b),c=this.b.b;a?_.M("gb_ae",void 0).appendChild(c):this.j.appendChild(c)};_.hj=function(a){return!!a.b&&_.R(a.F,"gb_2d")};
W.prototype.J=function(a){var c=!1;switch(a){case "back":this.O=!0;Ni(this.b);Mi(this.b,"back");c=!0;break;case "close":this.O=!0;Ni(this.b);Mi(this.b,"close");c=!0;break;case "default":this.O=!1;gj(this,this.G.b)||this.jd?(this.b&&!this.b.isVisible("menu")&&(Ni(this.b),Mi(this.b,"menu")),c=!0):(this.b&&this.b.isVisible("back")&&Ni(this.b),this.b&&this.b.isVisible("menu")?(a=this.b,a.close(),_.S(a.C(),"gb_Fa"),Oi(a.w)&&_.T(a.C(),"gb_wc")):(a=_.M("gb_rc",this.j))&&_.S(a,"gb_Fa"),c=!1);break;case "none":this.O=
!0,Ni(this.b),c=!1}null!=this.B&&_.U(this.B,"gb_1c",c)};var gj=function(a,c){var d="gb_ta"==c;c="gb_Vd"==c;var e=_.K(_.C(a.f,5),!1),f=_.K(_.C(a.f,2),!1);return!(_.K(_.C(a.f,10),!1)||a.ua)&&f&&(d||c&&(e||a.S))};W.prototype.getHeight=function(){var a=this.j.offsetHeight;if(this.zc){var c=_.M("gb_Id");c&&(a+=c.offsetHeight)}return a};_.ij=function(a){var c=a.getHeight()+"px";a.tb!=c&&(a.tb=c,a.Vb&&(a.Vb.style.height=c),a.dispatchEvent("resize"))};W.prototype.md=function(){this.K&&_.ij(this)};
W.prototype.Aa=function(){if(!this.K){var a=_.ze("DIV");_.mh(a,["gb_Zd","gb_6d"]);oj(a,cj(this));a.style.backgroundColor=this.j.style.backgroundColor;this.Y.push(a);_.sh(a,this.w);this.K=a}return this.K};W.prototype.od=function(){_.Ae(this.K);this.K=null;_.ij(this)};W.prototype.Ub=function(a){2==a&&(a=0);for(var c=0;c<this.Y.length;c++)oj(this.Y[c],a);dj(this,a)};
var dj=function(a,c){if(a.D){if(2==c){c=_.L(_.B(a.f,24),"");var d=_.L(_.B(a.f,27),"")}else 1==c?(c=_.L(_.B(a.f,23),""),d=_.L(_.B(a.f,26),"")):(c=_.L(_.B(a.f,22),""),d=_.L(_.B(a.f,25),""));""==c&&""==d||Qh(a.D,c,d)}},cj=function(a){a=a.Y[0];return a.classList.contains("gb_sc")?1:a.classList.contains("gb_7d")?2:0},oj=function(a,c){_.nh(a,["gb_7d","gb_sc"]);1==c?_.S(a,"gb_sc"):2==c&&_.S(a,"gb_7d")};W.prototype.Fb=function(a){this.j.style.backgroundColor=a};W.prototype.kc=function(){return this.j.style.backgroundColor};
W.prototype.Z=function(){var a=_.Xc("dd");_.Ih(a)&&_.Ih(a).me(!1);_.Rh(a,null)};W.prototype.Id=function(a){Vi(this,a-8-10);fj(this)};var Vi=function(a,c){null==a.A?a.M.log(Error("M")):a.W?a.M.log(Error("N")):a.Kb=0>c?0:c},fj=function(a){null!=a.B&&("gb_ta"==a.G.b?_.Jg(a.B,"min-width",""):null!=a.Kb&&_.Jg(a.B,"min-width",a.Kb+"px"))};W.prototype.ze=function(a){_.U(_.M("gb_lc",this.w),"gb_Fa",!a)};W.prototype.qd=function(a){if(a){var c=_.M("gb_4");null!=c&&_.Kh(c,a);_.sd.ta().b.then(function(d){d.Fg(a)})}};
var pj=function(a,c){c.xa=c.type;c.xb=c.target;return a.call(this,c)};
var qj;_.Q.prototype.za=_.Sd(function(a,c,d,e,f){return a.call(this,c,_.Sd(pj,d),e,f)},_.Q.prototype.H);_.Q.prototype.zb=_.Q.prototype.vd;var rj=_.M("gb_sa");
if(null==rj)qj=null;else{var sj=_.H(_.ud,Mh,6)||new Mh,tj=new W(rj,sj,_.yd,_.M("gb_Rd"));_.u("gbar.P",W);W.prototype.pa=W.prototype.getHeight;W.prototype.pb=W.prototype.jk;W.prototype.pc=W.prototype.Ub;W.prototype.pd=W.prototype.Fb;W.prototype.pe=W.prototype.Aa;W.prototype.pf=W.prototype.md;W.prototype.pg=W.prototype.od;W.prototype.ph=W.prototype.yj;W.prototype.pi=W.prototype.Z;W.prototype.pj=W.prototype.Id;W.prototype.pk=W.prototype.ze;W.prototype.pl=W.prototype.qd;W.prototype.pm=W.prototype.J;W.prototype.pn=
W.prototype.kc;W.prototype.po=W.prototype.ik;W.prototype.pp=W.prototype.dk;_.rd(_.sd.ta().o,tj);qj=tj}_.uj=qj;

}catch(e){_._DumpException(e)}
try{
/*

 Copyright The Closure Library Authors.
 SPDX-License-Identifier: Apache-2.0
*/
_.yl=function(a){(0,_.xl)();return _.qb(a)};_.xl=_.xa;

}catch(e){_._DumpException(e)}
try{
/*
 gapi.loader.OBJECT_CREATE_TEST_OVERRIDE &&*/
var zl=window,Al=document,Bl=zl.location,Cl=function(){},Dl=/\[native code\]/,El=function(a,c,d){return a[c]=a[c]||d},Fl=function(a){a=a.sort();for(var c=[],d=void 0,e=0;e<a.length;e++){var f=a[e];f!=d&&c.push(f);d=f}return c},Gl=function(){var a;if((a=Object.create)&&Dl.test(a))a=a(null);else{a={};for(var c in a)a[c]=void 0}return a},Hl=El(zl,"gapi",{});
var Il;Il=El(zl,"___jsl",Gl());El(Il,"I",0);El(Il,"hel",10);var Jl=function(){var a=Bl.href;if(Il.dpo)var c=Il.h;else{c=Il.h;var d=/([#].*&|[#])jsh=([^&#]*)/g,e=/([?#].*&|[?#])jsh=([^&#]*)/g;if(a=a&&(d.exec(a)||e.exec(a)))try{c=decodeURIComponent(a[2])}catch(f){}}return c},Kl=function(a){var c=El(Il,"PQ",[]);Il.PQ=[];var d=c.length;if(0===d)a();else for(var e=0,f=function(){++e===d&&a()},g=0;g<d;g++)c[g](f)},Ll=function(a){return El(El(Il,"H",Gl()),a,Gl())};
var Ml=El(Il,"perf",Gl());El(Ml,"g",Gl());var Nl=El(Ml,"i",Gl());El(Ml,"r",[]);Gl();Gl();var Pl=function(a,c,d){c&&0<c.length&&(c=Ol(c),d&&0<d.length&&(c+="___"+Ol(d)),28<c.length&&(c=c.substr(0,28)+(c.length-28)),d=c,c=El(Nl,"_p",Gl()),El(c,d,Gl())[a]=(new Date).getTime(),c=Ml.r,"function"===typeof c?c(a,"_p",d):c.push([a,"_p",d]))},Ol=function(a){return a.join("__").replace(/\./g,"_").replace(/\-/g,"_").replace(/,/g,"_")};
var Ql=Gl(),Rl=[],Sl=function(a){throw Error("Y`"+(a?": "+a:""));};Rl.push(["jsl",function(a){for(var c in a)if(Object.prototype.hasOwnProperty.call(a,c)){var d=a[c];"object"==typeof d?Il[c]=El(Il,c,[]).concat(d):El(Il,c,d)}if(c=a.u)a=El(Il,"us",[]),a.push(c),(c=/^https:(.*)$/.exec(c))&&a.push("http:"+c[1])}]);
var Tl=/^(\/[a-zA-Z0-9_\-]+)+$/,Ul=[/\/amp\//,/\/amp$/,/^\/amp$/],Vl=/^[a-zA-Z0-9\-_\.,!]+$/,Wl=/^gapi\.loaded_[0-9]+$/,Xl=/^[a-zA-Z0-9,._-]+$/,am=function(a,c,d,e){var f=a.split(";"),g=f.shift(),h=Ql[g],l=null;h?l=h(f,c,d,e):Sl("no hint processor for: "+g);l||Sl("failed to generate load url");c=l;d=c.match(Yl);(e=c.match(Zl))&&1===e.length&&$l.test(c)&&d&&1===d.length||Sl("failed sanity: "+a);return l},dm=function(a,c,d,e){a=bm(a);Wl.test(d)||Sl("invalid_callback");c=cm(c);e=e&&e.length?cm(e):null;
var f=function(g){return encodeURIComponent(g).replace(/%2C/g,",")};return[encodeURIComponent(a.pathPrefix).replace(/%2C/g,",").replace(/%2F/g,"/"),"/k=",f(a.version),"/m=",f(c),e?"/exm="+f(e):"","/rt=j/sv=1/d=1/ed=1",a.vf?"/am="+f(a.vf):"",a.Hg?"/rs="+f(a.Hg):"",a.Kg?"/t="+f(a.Kg):"","/cb=",f(d)].join("")},bm=function(a){"/"!==a.charAt(0)&&Sl("relative path");for(var c=a.substring(1).split("/"),d=[];c.length;){a=c.shift();if(!a.length||0==a.indexOf("."))Sl("empty/relative directory");else if(0<a.indexOf("=")){c.unshift(a);
break}d.push(a)}a={};for(var e=0,f=c.length;e<f;++e){var g=c[e].split("="),h=decodeURIComponent(g[0]),l=decodeURIComponent(g[1]);2==g.length&&h&&l&&(a[h]=a[h]||l)}c="/"+d.join("/");Tl.test(c)||Sl("invalid_prefix");d=0;for(e=Ul.length;d<e;++d)Ul[d].test(c)&&Sl("invalid_prefix");d=em(a,"k",!0);e=em(a,"am");f=em(a,"rs");a=em(a,"t");return{pathPrefix:c,version:d,vf:e,Hg:f,Kg:a}},cm=function(a){for(var c=[],d=0,e=a.length;d<e;++d){var f=a[d].replace(/\./g,"_").replace(/-/g,"_");Xl.test(f)&&c.push(f)}return c.join(",")},
em=function(a,c,d){a=a[c];!a&&d&&Sl("missing: "+c);if(a){if(Vl.test(a))return a;Sl("invalid: "+c)}return null},$l=/^https?:\/\/[a-z0-9_.-]+\.google(rs)?\.com(:\d+)?\/[a-zA-Z0-9_.,!=\-\/]+$/,Zl=/\/cb=/g,Yl=/\/\//g,fm=function(){var a=Jl();if(!a)throw Error("Z");return a};Ql.m=function(a,c,d,e){(a=a[0])||Sl("missing_hint");return"https://apis.google.com"+dm(a,c,d,e)};
var gm=decodeURI("%73cript"),hm=/^[-+_0-9\/A-Za-z]+={0,2}$/,im=function(a,c){for(var d=[],e=0;e<a.length;++e){var f=a[e],g;if(g=f){a:{for(g=0;g<c.length;g++)if(c[g]===f)break a;g=-1}g=0>g}g&&d.push(f)}return d},jm=function(){var a=Il.nonce;return void 0!==a?a&&a===String(a)&&a.match(hm)?a:Il.nonce=null:Al.querySelector?(a=Al.querySelector("script[nonce]"))?(a=a.nonce||a.getAttribute("nonce")||"",a&&a===String(a)&&a.match(hm)?Il.nonce=a:Il.nonce=null):null:null},mm=function(a){if("loading"!=Al.readyState)km(a);
else{var c=jm(),d="";null!==c&&(d=' nonce="'+c+'"');a="<"+gm+' src="'+encodeURI(a)+'"'+d+"></"+gm+">";Al.write(lm?lm.createHTML(a):a)}},km=function(a){var c=Al.createElement(gm);c.setAttribute("src",lm?lm.createScriptURL(a):a);a=jm();null!==a&&c.setAttribute("nonce",a);c.async="true";(a=Al.getElementsByTagName(gm)[0])?a.parentNode.insertBefore(c,a):(Al.head||Al.body||Al.documentElement).appendChild(c)},nm=function(a,c){var d=c&&c._c;if(d)for(var e=0;e<Rl.length;e++){var f=Rl[e][0],g=Rl[e][1];g&&Object.prototype.hasOwnProperty.call(d,
f)&&g(d[f],a,c)}},pm=function(a,c,d){om(function(){var e=c===Jl()?El(Hl,"_",Gl()):Gl();e=El(Ll(c),"_",e);a(e)},d)},rm=function(a,c){var d=c||{};"function"==typeof c&&(d={},d.callback=c);nm(a,d);c=a?a.split(":"):[];var e=d.h||fm(),f=El(Il,"ah",Gl());if(f["::"]&&c.length){a=[];for(var g=null;g=c.shift();){var h=g.split(".");h=f[g]||f[h[1]&&"ns:"+h[0]||""]||e;var l=a.length&&a[a.length-1]||null,m=l;l&&l.hint==h||(m={hint:h,Nd:[]},a.push(m));m.Nd.push(g)}var n=a.length;if(1<n){var r=d.callback;r&&(d.callback=
function(){0==--n&&r()})}for(;c=a.shift();)qm(c.Nd,d,c.hint)}else qm(c||[],d,e)},qm=function(a,c,d){a=Fl(a)||[];var e=c.callback,f=c.config,g=c.timeout,h=c.ontimeout,l=c.onerror,m=void 0;"function"==typeof l&&(m=l);var n=null,r=!1;if(g&&!h||!g&&h)throw"Timeout requires both the timeout parameter and ontimeout parameter to be set";l=El(Ll(d),"r",[]).sort();var v=El(Ll(d),"L",[]).sort(),N=l.concat(),D=function(za,Ic){if(r)return 0;zl.clearTimeout(n);v.push.apply(v,P);var jg=((Hl||{}).config||{}).update;
jg?jg(f):f&&El(Il,"cu",[]).push(f);if(Ic){Pl("me0",za,N);try{pm(Ic,d,m)}finally{Pl("me1",za,N)}}return 1};0<g&&(n=zl.setTimeout(function(){r=!0;h()},g));var P=im(a,v);if(P.length){P=im(a,l);var G=El(Il,"CP",[]),fa=G.length;G[fa]=function(za){if(!za)return 0;Pl("ml1",P,N);var Ic=function(fi){G[fa]=null;D(P,za)&&Kl(function(){e&&e();fi()})},jg=function(){var fi=G[fa+1];fi&&fi()};0<fa&&G[fa-1]?G[fa]=function(){Ic(jg)}:Ic(jg)};if(P.length){var Hc="loaded_"+Il.I++;Hl[Hc]=function(za){G[fa](za);Hl[Hc]=
null};a=am(d,P,"gapi."+Hc,l);l.push.apply(l,P);Pl("ml0",P,N);c.sync||zl.___gapisync?mm(a):km(a)}else G[fa](Cl)}else D(P)&&e&&e()},lm=_.Ja("ogb-qtm#gapi"),om=function(a,c){if(Il.hee&&0<Il.hel)try{return a()}catch(d){c&&c(d),Il.hel--,rm("debug_error",function(){try{window.___jsl.hefn(d)}catch(e){throw d;}})}else try{return a()}catch(d){throw c&&c(d),d;}};Hl.load=function(a,c){return om(function(){return rm(a,c)})};

}catch(e){_._DumpException(e)}
try{
var Rj;_.Qj=function(a){this.b=a||{cookie:""}};_.k=_.Qj.prototype;
_.k.set=function(a,c,d){var e=!1;if("object"===typeof d){var f=d.Il;e=d.$j||!1;var g=d.domain||void 0;var h=d.path||void 0;var l=d.je}if(/[;=\s]/.test(a))throw Error("R`"+a);if(/[;\r\n]/.test(c))throw Error("S`"+c);void 0===l&&(l=-1);d=g?";domain="+g:"";h=h?";path="+h:"";e=e?";secure":"";l=0>l?"":0==l?";expires="+(new Date(1970,1,1)).toUTCString():";expires="+(new Date((0,_.Ha)()+1E3*l)).toUTCString();this.b.cookie=a+"="+c+d+h+l+e+(null!=f?";samesite="+f:"")};
_.k.get=function(a,c){for(var d=a+"=",e=(this.b.cookie||"").split(";"),f=0,g;f<e.length;f++){g=(0,_.Ra)(e[f]);if(0==g.lastIndexOf(d,0))return g.substr(d.length);if(g==a)return""}return c};_.k.remove=function(a,c,d){var e=void 0!==this.get(a);this.set(a,"",{je:0,path:c,domain:d});return e};_.k.kb=function(){return Rj(this).keys};_.k.Pa=function(){return Rj(this).values};_.k.vc=function(){return!this.b.cookie};_.k.clear=function(){for(var a=Rj(this).keys,c=a.length-1;0<=c;c--)this.remove(a[c])};
Rj=function(a){a=(a.b.cookie||"").split(";");for(var c=[],d=[],e,f,g=0;g<a.length;g++)f=(0,_.Ra)(a[g]),e=f.indexOf("="),-1==e?(c.push(""),d.push(f)):(c.push(f.substring(0,e)),d.push(f.substring(e+1)));return{keys:c,values:d}};_.Sj=new _.Qj("undefined"==typeof document?null:document);

}catch(e){_._DumpException(e)}
try{
_.Tj=function(a){switch(a){case 200:case 201:case 202:case 204:case 206:case 304:case 1223:return!0;default:return!1}};
_.Uj=function(){};_.Uj.prototype.f=null;
var Wj;Wj=function(){};_.w(Wj,_.Uj);Wj.prototype.b=function(){var a=Xj(this);return a?new ActiveXObject(a):new XMLHttpRequest};Wj.prototype.o=function(){var a={};Xj(this)&&(a[0]=!0,a[1]=!0);return a};var Xj=function(a){if(!a.j&&"undefined"==typeof XMLHttpRequest&&"undefined"!=typeof ActiveXObject){for(var c=["MSXML2.XMLHTTP.6.0","MSXML2.XMLHTTP.3.0","MSXML2.XMLHTTP","Microsoft.XMLHTTP"],d=0;d<c.length;d++){var e=c[d];try{return new ActiveXObject(e),a.j=e}catch(f){}}throw Error("T");}return a.j};
_.Vj=new Wj;

}catch(e){_._DumpException(e)}
try{
/*

 Copyright The Closure Library Authors.
 SPDX-License-Identifier: Apache-2.0
*/
_.Yj=function(a,c,d){a.b||(a.b={});if(!a.b[d]){for(var e=_.B(a,d),f=[],g=0;g<e.length;g++)f[g]=new c(e[g]);a.b[d]=f}};_.Zj=function(a,c,d){_.Yj(a,c,d);c=a.b[d];c==_.uc&&(c=a.b[d]=[]);return c};_.ak=function(a){return a.contentDocument||a.contentWindow.document};
_.bk=function(a,c){this.f={};this.b=[];this.j=0;var d=arguments.length;if(1<d){if(d%2)throw Error("h");for(var e=0;e<d;e+=2)this.set(arguments[e],arguments[e+1])}else if(a)if(a instanceof _.bk)for(d=a.kb(),e=0;e<d.length;e++)this.set(d[e],a.get(d[e]));else for(e in a)this.set(e,a[e])};_.bk.prototype.Pa=function(){ck(this);for(var a=[],c=0;c<this.b.length;c++)a.push(this.f[this.b[c]]);return a};_.bk.prototype.kb=function(){ck(this);return this.b.concat()};_.ek=function(a,c){return dk(a.f,c)};
_.bk.prototype.vc=function(){return 0==this.j};_.bk.prototype.clear=function(){this.f={};this.j=this.b.length=0};_.bk.prototype.remove=function(a){return dk(this.f,a)?(delete this.f[a],this.j--,this.b.length>2*this.j&&ck(this),!0):!1};var ck=function(a){if(a.j!=a.b.length){for(var c=0,d=0;c<a.b.length;){var e=a.b[c];dk(a.f,e)&&(a.b[d++]=e);c++}a.b.length=d}if(a.j!=a.b.length){var f={};for(d=c=0;c<a.b.length;)e=a.b[c],dk(f,e)||(a.b[d++]=e,f[e]=1),c++;a.b.length=d}};
_.bk.prototype.get=function(a,c){return dk(this.f,a)?this.f[a]:c};_.bk.prototype.set=function(a,c){dk(this.f,a)||(this.j++,this.b.push(a));this.f[a]=c};_.bk.prototype.forEach=function(a,c){for(var d=this.kb(),e=0;e<d.length;e++){var f=d[e],g=this.get(f);a.call(c,g,f,this)}};var dk=function(a,c){return Object.prototype.hasOwnProperty.call(a,c)};

}catch(e){_._DumpException(e)}
try{
/*

 Copyright The Closure Library Authors.
 SPDX-License-Identifier: Apache-2.0
*/
var mk,nk;_.fk=function(a){return encodeURIComponent(String(a))};_.gk=function(a,c,d,e,f,g){var h="";a&&(h+=a+":");d&&(h+="//",c&&(h+=c+"@"),h+=d,e&&(h+=":"+e));f&&(h+=f);g&&(h+="?"+g);return h};_.hk=/^(?:([^:/?#.]+):)?(?:\/\/(?:([^/?#]*)@)?([^/#?]*?)(?::([0-9]+))?(?=[/\\#?]|$))?([^?#]+)?(?:\?([^#]*))?(?:#([\s\S]*))?$/;_.ik=function(a){a=a.match(_.hk)[1]||null;!a&&_.q.self&&_.q.self.location&&(a=_.q.self.location.protocol,a=a.substr(0,a.length-1));return a?a.toLowerCase():""};
_.jk=function(a){var c=a.indexOf("#");0>c&&(c=a.length);var d=a.indexOf("?");if(0>d||d>c){d=c;var e=""}else e=a.substring(d+1,c);return[a.substr(0,d),e,a.substr(c)]};_.kk=function(a,c){return c?a?a+"&"+c:c:a};_.lk=function(a,c){if(!c)return a;a=_.jk(a);a[1]=_.kk(a[1],c);return a[0]+(a[1]?"?"+a[1]:"")+a[2]};mk=function(a,c,d){if(_.Ba(c))for(var e=0;e<c.length;e++)mk(a,String(c[e]),d);else null!=c&&d.push(a+(""===c?"":"="+_.fk(c)))};
nk=function(a,c){var d=[];for(c=c||0;c<a.length;c+=2)mk(a[c],a[c+1],d);return d.join("&")};_.ok=function(a){var c=[],d;for(d in a)mk(d,a[d],c);return c.join("&")};_.pk=function(a,c){var d=2==arguments.length?nk(arguments[1],0):nk(arguments,1);return _.lk(a,d)};

}catch(e){_._DumpException(e)}
try{
var qk,sk,uk,vk,xk,yk,Ak,Bk,Gk;qk=function(a){if(_.Ba(a)){for(var c=Array(a.length),d=0;d<a.length;d++){var e=a[d];null!=e&&(c[d]="object"==typeof e?qk(e):e)}return c}if(_.tc&&a instanceof Uint8Array)return new Uint8Array(a);c={};for(d in a)e=a[d],null!=e&&(c[d]="object"==typeof e?qk(e):e);return c};_.rk=function(a){return new a.constructor(qk(a.sb()))};sk=function(a,c){a.f=c;a.Gb&&a.sc?(a.stop(),a.start()):a.Gb&&a.stop()};
_.tk=function(a,c,d){a.b||(a.b={});d=d||[];for(var e=[],f=0;f<d.length;f++)e[f]=d[f].sb();a.b[c]=d;return _.F(a,c,e)};uk=function(a){return a.f||(a.f=a.o())};vk=function(a){if(a.Pa&&"function"==typeof a.Pa)return a.Pa();if("string"===typeof a)return a.split("");if(_.Yd(a)){for(var c=[],d=a.length,e=0;e<d;e++)c.push(a[e]);return c}return _.Zf(a)};
xk=function(a){a:{var c=wk;for(var d=a.length,e="string"===typeof a?a.split(""):a,f=0;f<d;f++)if(f in e&&c.call(void 0,e[f],f,a)){c=f;break a}c=-1}return 0>c?null:"string"===typeof a?a.charAt(c):a[c]};yk=function(a){var c=c||0;return function(){return a.apply(this,Array.prototype.slice.call(arguments,0,c))}};Ak=function(){this.b=zk};Ak.prototype.f=function(){return!!this.b};Bk=function(a,c){return a+Math.random()*(c-a)};
_.Ck=function(a,c){if(a.forEach&&"function"==typeof a.forEach)a.forEach(c,void 0);else if(_.Yd(a)||"string"===typeof a)(0,_.Ma)(a,c,void 0);else{if(a.kb&&"function"==typeof a.kb)var d=a.kb();else if(a.Pa&&"function"==typeof a.Pa)d=void 0;else if(_.Yd(a)||"string"===typeof a){d=[];for(var e=a.length,f=0;f<e;f++)d.push(f)}else for(f in d=[],e=0,a)d[e++]=f;e=vk(a);f=e.length;for(var g=0;g<f;g++)c.call(void 0,e[g],d&&d[g],a)}};_.Dk=function(a,c,d){d=null!=d?"="+_.fk(d):"";return _.lk(a,c+d)};
_.Ek=function(a,c,d,e){for(var f=d.length;0<=(c=a.indexOf(d,c))&&c<e;){var g=a.charCodeAt(c-1);if(38==g||63==g)if(g=a.charCodeAt(c+f),!g||61==g||38==g||35==g)return c;c+=f+1}return-1};_.Fk=/#|$/;Gk=/[?&]($|#)/;_.Hk=function(a,c){for(var d=a.search(_.Fk),e=0,f,g=[];0<=(f=_.Ek(a,e,c,d));)g.push(a.substring(e,f)),e=Math.min(a.indexOf("&",f)+1||d,d);g.push(a.substr(e));return g.join("").replace(Gk,"$1")};
var Ik=function(a){if(!a)return"";a=a.split("#")[0].split("?")[0];a=a.toLowerCase();0==a.indexOf("//")&&(a=window.location.protocol+a);/^[\w\-]*:\/\//.test(a)||(a=window.location.href);var c=a.substring(a.indexOf("://")+3),d=c.indexOf("/");-1!=d&&(c=c.substring(0,d));a=a.substring(0,a.indexOf("://"));if("http"!==a&&"https"!==a&&"chrome-extension"!==a&&"file"!==a&&"android-app"!==a&&"chrome-search"!==a&&"app"!==a)throw Error("U`"+a);d="";var e=c.indexOf(":");if(-1!=e){var f=c.substring(e+1);c=c.substring(0,
e);if("http"===a&&"80"!==f||"https"===a&&"443"!==f)d=":"+f}return a+"://"+c+d};
var Jk=function(){function a(){f[0]=1732584193;f[1]=4023233417;f[2]=2562383102;f[3]=271733878;f[4]=3285377520;r=n=0}function c(v){for(var N=h,D=0;64>D;D+=4)N[D/4]=v[D]<<24|v[D+1]<<16|v[D+2]<<8|v[D+3];for(D=16;80>D;D++)v=N[D-3]^N[D-8]^N[D-14]^N[D-16],N[D]=(v<<1|v>>>31)&4294967295;v=f[0];var P=f[1],G=f[2],fa=f[3],Hc=f[4];for(D=0;80>D;D++){if(40>D)if(20>D){var za=fa^P&(G^fa);var Ic=1518500249}else za=P^G^fa,Ic=1859775393;else 60>D?(za=P&G|fa&(P|G),Ic=2400959708):(za=P^G^fa,Ic=3395469782);za=((v<<5|v>>>
27)&4294967295)+za+Hc+Ic+N[D]&4294967295;Hc=fa;fa=G;G=(P<<30|P>>>2)&4294967295;P=v;v=za}f[0]=f[0]+v&4294967295;f[1]=f[1]+P&4294967295;f[2]=f[2]+G&4294967295;f[3]=f[3]+fa&4294967295;f[4]=f[4]+Hc&4294967295}function d(v,N){if("string"===typeof v){v=unescape(encodeURIComponent(v));for(var D=[],P=0,G=v.length;P<G;++P)D.push(v.charCodeAt(P));v=D}N||(N=v.length);D=0;if(0==n)for(;D+64<N;)c(v.slice(D,D+64)),D+=64,r+=64;for(;D<N;)if(g[n++]=v[D++],r++,64==n)for(n=0,c(g);D+64<N;)c(v.slice(D,D+64)),D+=64,r+=
64}function e(){var v=[],N=8*r;56>n?d(l,56-n):d(l,64-(n-56));for(var D=63;56<=D;D--)g[D]=N&255,N>>>=8;c(g);for(D=N=0;5>D;D++)for(var P=24;0<=P;P-=8)v[N++]=f[D]>>P&255;return v}for(var f=[],g=[],h=[],l=[128],m=1;64>m;++m)l[m]=0;var n,r;a();return{reset:a,update:d,digest:e,qh:function(){for(var v=e(),N="",D=0;D<v.length;D++)N+="0123456789ABCDEF".charAt(Math.floor(v[D]/16))+"0123456789ABCDEF".charAt(v[D]%16);return N}}};
var Lk=function(a,c,d){var e=[],f=[];if(1==(_.Ba(d)?2:1))return f=[c,a],(0,_.Ma)(e,function(l){f.push(l)}),Kk(f.join(" "));var g=[],h=[];(0,_.Ma)(d,function(l){h.push(l.key);g.push(l.value)});d=Math.floor((new Date).getTime()/1E3);f=0==g.length?[d,c,a]:[g.join(":"),d,c,a];(0,_.Ma)(e,function(l){f.push(l)});a=Kk(f.join(" "));a=[d,a];0==h.length||a.push(h.join(""));return a.join("_")},Kk=function(a){var c=Jk();c.update(a);return c.qh().toLowerCase()};
var Mk=function(a){var c=Ik(String(_.q.location.href)),d;(d=_.q.__SAPISID||_.q.__APISID||_.q.__OVERRIDE_SID)?d=!0:(d=new _.Qj(document),d=d.get("SAPISID")||d.get("APISID")||d.get("__Secure-3PAPISID")||d.get("SID"),d=!!d);if(d&&(d=(c=0==c.indexOf("https:")||0==c.indexOf("chrome-extension:"))?_.q.__SAPISID:_.q.__APISID,d||(d=new _.Qj(document),d=d.get(c?"SAPISID":"APISID")||d.get("__Secure-3PAPISID")),d)){c=c?"SAPISIDHASH":"APISIDHASH";var e=String(_.q.location.href);return e&&d&&c?[c,Lk(Ik(e),d,a||
null)].join(" "):null}return null};
var Nk=function(a){this.b=this.f=this.j=a};Nk.prototype.reset=function(){this.b=this.f=this.j};Nk.prototype.ya=function(){return this.f};
/*

 Copyright The Closure Library Authors.
 SPDX-License-Identifier: Apache-2.0
*/
_.Ok=function(a){a=String(a);if(/^\s*$/.test(a)?0:/^[\],:{}\s\u2028\u2029]*$/.test(a.replace(/\\["\\\/bfnrtu]/g,"@").replace(/(?:"[^"\\\n\r\u2028\u2029\x00-\x08\x0a-\x1f]*"|true|false|null|-?\d+(?:\.\d*)?(?:[eE][+\-]?\d+)?)[\s\u2028\u2029]*(?=:|,|]|}|$)/g,"]").replace(/(?:^|:|,)(?:[\s\u2028\u2029]*\[)+/g,"")))try{return eval("("+a+")")}catch(c){}throw Error("V`"+a);};_.Pk=/\uffff/.test("\uffff")?/[\\"\x00-\x1f\x7f-\uffff]/g:/[\\"\x00-\x1f\x7f-\xff]/g;
var Qk=function(a){_.Q.call(this);this.headers=new _.bk;this.D=a||null;this.f=!1;this.B=this.b=null;this.F="";this.j=this.J=this.w=this.G=!1;this.A=0;this.o=null;this.N="";this.K=this.M=!1},Rk,Sk,Tk;_.w(Qk,_.Q);Rk=/^https?$/i;Sk=["POST","PUT"];Tk=[];_.Uk=function(a,c,d,e,f,g,h){var l=new Qk;Tk.push(l);c&&l.H("complete",c);l.nb("ready",l.R);g&&(l.A=Math.max(0,g));h&&(l.M=h);l.send(a,d,e,f)};Qk.prototype.R=function(){this.sa();_.Ie(Tk,this)};
Qk.prototype.send=function(a,c,d,e){if(this.b)throw Error("X`"+this.F+"`"+a);c=c?c.toUpperCase():"GET";this.F=a;this.G=!1;this.f=!0;this.b=this.D?this.D.b():_.Vj.b();this.B=this.D?uk(this.D):uk(_.Vj);this.b.onreadystatechange=(0,_.t)(this.O,this);try{this.J=!0,this.b.open(c,String(a),!0),this.J=!1}catch(g){Vk(this);return}a=d||"";var f=new _.bk(this.headers);e&&_.Ck(e,function(g,h){f.set(h,g)});e=xk(f.kb());d=_.q.FormData&&a instanceof _.q.FormData;!_.Qa(Sk,c)||e||d||f.set("Content-Type","application/x-www-form-urlencoded;charset=utf-8");
f.forEach(function(g,h){this.b.setRequestHeader(h,g)},this);this.N&&(this.b.responseType=this.N);"withCredentials"in this.b&&this.b.withCredentials!==this.M&&(this.b.withCredentials=this.M);try{Wk(this),0<this.A&&((this.K=Xk(this.b))?(this.b.timeout=this.A,this.b.ontimeout=(0,_.t)(this.Fd,this)):this.o=_.rg(this.Fd,this.A,this)),this.w=!0,this.b.send(a),this.w=!1}catch(g){Vk(this)}};
var Xk=function(a){return _.y&&_.gc(9)&&"number"===typeof a.timeout&&void 0!==a.ontimeout},wk=function(a){return"content-type"==a.toLowerCase()};Qk.prototype.Fd=function(){"undefined"!=typeof _.wa&&this.b&&(this.dispatchEvent("timeout"),this.abort(8))};var Vk=function(a){a.f=!1;a.b&&(a.j=!0,a.b.abort(),a.j=!1);Yk(a);Zk(a)},Yk=function(a){a.G||(a.G=!0,a.dispatchEvent("complete"),a.dispatchEvent("error"))};
Qk.prototype.abort=function(){this.b&&this.f&&(this.f=!1,this.j=!0,this.b.abort(),this.j=!1,this.dispatchEvent("complete"),this.dispatchEvent("abort"),Zk(this))};Qk.prototype.P=function(){this.b&&(this.f&&(this.f=!1,this.j=!0,this.b.abort(),this.j=!1),Zk(this,!0));Qk.L.P.call(this)};Qk.prototype.O=function(){this.Sa||(this.J||this.w||this.j?$k(this):this.T())};Qk.prototype.T=function(){$k(this)};
var $k=function(a){if(a.f&&"undefined"!=typeof _.wa&&(!a.B[1]||4!=(a.b?a.b.readyState:0)||2!=a.Nb()))if(a.w&&4==(a.b?a.b.readyState:0))_.rg(a.O,0,a);else if(a.dispatchEvent("readystatechange"),4==(a.b?a.b.readyState:0)){a.f=!1;try{a.ee()?(a.dispatchEvent("complete"),a.dispatchEvent("success")):(a.Nb(),Yk(a))}finally{Zk(a)}}},Zk=function(a,c){if(a.b){Wk(a);var d=a.b,e=a.B[0]?_.xa:null;a.b=null;a.B=null;c||a.dispatchEvent("ready");try{d.onreadystatechange=e}catch(f){}}},Wk=function(a){a.b&&a.K&&(a.b.ontimeout=
null);a.o&&(_.sg(a.o),a.o=null)};Qk.prototype.ee=function(){var a=this.Nb(),c;if(!(c=_.Tj(a))){if(a=0===a)a=_.ik(String(this.F)),a=!Rk.test(a);c=a}return c};Qk.prototype.Nb=function(){try{return 2<(this.b?this.b.readyState:0)?this.b.status:-1}catch(a){return-1}};Qk.prototype.Vf=function(){try{return this.b?this.b.responseText:""}catch(a){return""}};Qk.prototype.Uf=function(){if(this.b){a:{var a=this.b.responseText;if(_.q.JSON)try{var c=_.q.JSON.parse(a);break a}catch(d){}c=_.Ok(a)}return c}};
var al=function(a,c,d){_.Uk(a.url,function(e){e=e.target;e.ee()?c(e.Vf()):d(e.Nb())},a.Yj,a.body,a.Xj,a.rk,a.withCredentials)};
var bl=function(a){_.A(this,a,0,-1,null,null)};_.w(bl,_.z);
var cl=function(a){_.A(this,a,0,-1,null,null)};_.w(cl,_.z);
var dl;_.el=function(a){_.A(this,a,0,30,dl,null)};_.w(_.el,_.z);dl=[3,20,27];_.fl=function(a){var c=(0,_.Ha)().toString();_.F(a,1,c)};_.gl=function(a,c){return _.F(a,8,c)};
var il=function(a){_.A(this,a,0,17,hl,null)};_.w(il,_.z);var hl=[3,5],jl=function(a){var c=(0,_.Ha)().toString();return _.F(a,4,c)},kl=function(a,c){return _.tk(a,3,c)},ll=function(a,c){return _.F(a,14,c)};
var nl=function(a){_.A(this,a,0,6,ml,null)};_.w(nl,_.z);var ml=[5];
var zk=function(a){_.A(this,a,0,-1,null,null)};_.w(zk,_.z);
var ol=new Ak;
var ql=function(a,c,d,e,f,g,h,l,m,n,r){_.Q.call(this);this.V=a;this.N=c||_.xa;this.w=new il;this.X=e;this.T=r;this.b=[];this.R="";this.Z=_.Sd(Bk,0,1);this.G=f||null;this.B=d||null;this.F=h||!1;this.J=m||null;this.S=!1;this.U=this.K=-1;this.O=!1;this.j=null;this.Y=!l;this.M=0;this.ma=1;this.W=g||!1;a=new cl;a=_.F(a,1,1);g||(g=new bl,c=document.documentElement.getAttribute("lang"),g=_.F(g,5,c),_.I(a,11,g));_.I(this.w,1,a);_.F(this.w,2,this.V);this.o=new Nk(1E4);this.f=new _.qg(this.o.ya());_.Yf(this,
this.f);_.O(this.f,"tick",yk(pl(this,n)),!1,this);this.D=new _.qg(6E5);_.Yf(this,this.D);_.O(this.D,"tick",yk(pl(this,n)),!1,this);this.F||this.D.start();this.W||(_.O(_.eg(),"beforeunload",this.A,!1,this),_.O(_.eg(),"unload",this.A,!1,this),_.O(document,"pagehide",this.A,!1,this))};_.w(ql,_.Q);var pl=function(a,c){return c?function(){c().then(a.flush.bind(a))}:a.flush};ql.prototype.P=function(){this.A();ql.L.P.call(this)};
var rl=function(a){a.G||(a.G=.01>a.Z()?"https://www.google.com/log?format=json&hasfast=true":"https://play.google.com/log?format=json&hasfast=true");return a.G};ql.prototype.Cc=function(a){a instanceof _.el?this.log(a):(a=_.gl(new _.el,a.f()),this.log(a))};_.sl=function(a,c){a.o=new Nk(1>c?1:c);sk(a.f,a.o.ya())};
ql.prototype.log=function(a){a=_.rk(a);var c=this.ma++;_.F(a,21,c);_.B(a,1)||_.fl(a);this.j&&(c=_.rk(this.j),_.I(a,16,c));for(;1E3<=this.b.length;)this.b.shift(),++this.M;this.b.push(a);this.dispatchEvent(new tl(a));this.F||this.f.sc||this.f.start()};
ql.prototype.flush=function(a,c){if(0==this.b.length)a&&a();else{var d=(0,_.Ha)();if(this.U>d&&this.K<d)c&&c("throttled");else{var e=ll(kl(jl(_.rk(this.w)),this.b),this.M);d={};var f=this.N();f&&(d.Authorization=f);var g=rl(this);this.B&&(d["X-Goog-AuthUser"]=this.B,g=_.Dk(g,"authuser",this.B));this.J&&(d["X-Goog-PageId"]=this.J,g=_.Dk(g,"pageId",this.J));if(f&&this.R==f)c&&c("stale-auth-token");else{this.b=[];this.f.sc&&this.f.stop();this.M=0;var h=e.f();d={url:g,body:h,sl:1,Xj:d,Yj:"POST",withCredentials:this.Y,
rk:0};g=(0,_.t)(function(l){this.o.reset();sk(this.f,this.o.ya());if(l){try{var m=JSON.parse(l.replace(")]}'\n",""));var n=new nl(m)}catch(r){}n&&(l=_.E(n,1,"-1"),l=Number(l),0<l&&(this.K=(0,_.Ha)(),this.U=this.K+l),n.o?(n.b||(n.b={}),ol.f()?(!n.b[175237375]&&n.o[175237375]&&(n.b[175237375]=new ol.b(n.o[175237375])),n=n.b[175237375]):n=n.o[175237375]):n=void 0,n&&(n=_.E(n,1,-1),-1!=n&&(this.O||_.sl(this,n))))}a&&a()},this);h=(0,_.t)(function(l){var m=_.Zj(e,_.el,3),n=this.o;n.b=Math.min(3E5,2*n.b);
n.f=Math.min(3E5,n.b+Math.round(.2*(Math.random()-.5)*n.b));sk(this.f,this.o.ya());401==l&&f&&(this.R=f);if(500<=l&&600>l||401==l||0==l)this.b=m.concat(this.b),this.F||this.f.sc||this.f.start();c&&c("net-send-failed",l)},this);this.T?this.T.send(d,g,h):this.X(d,g,h)}}}};ql.prototype.A=function(){this.S&&ul(this);this.flush()};
var ul=function(a){vl(a,function(c,d){c=_.Dk(c,"format","json");return _.eg().navigator.sendBeacon(c,d.f())})},vl=function(a,c){if(0!=a.b.length){var d=_.Hk(rl(a),"format");d=_.pk(d,"auth",a.N(),"authuser",a.B||"0");for(var e=0;10>e&&a.b.length;++e){var f=a.b.slice(0,32),g=kl(jl(_.rk(a.w)),f);if(!c(d,g))break;a.b=a.b.slice(f.length)}}},tl=function(){this.type="event-logged"};_.w(tl,_.Le);
_.wl=function(a,c,d,e,f,g,h){ql.call(this,a,Mk,c,al,d,e,f,void 0,g,h)};_.w(_.wl,ql);

}catch(e){_._DumpException(e)}
try{
_.sm=function(a,c){c=c instanceof _.tb?c:_.xb(c);a.href=_.ub(c)};

}catch(e){_._DumpException(e)}
try{
/*

 Copyright The Closure Library Authors.
 SPDX-License-Identifier: Apache-2.0
*/
var tm,vm,Em,Gm,Qm,Hm,Jm,Im,Mm,Km,Fm,Rm,Sm,Lm;tm=function(a){return Array.prototype.concat.apply([],arguments)};_.um=function(){return Math.floor(2147483648*Math.random()).toString(36)+Math.abs(Math.floor(2147483648*Math.random())^(0,_.Ha)()).toString(36)};vm=function(a,c){if(a){a=a.split("&");for(var d=0;d<a.length;d++){var e=a[d].indexOf("="),f=null;if(0<=e){var g=a[d].substring(0,e);f=a[d].substring(e+1)}else g=a[d];c(g,f?decodeURIComponent(f.replace(/\+/g," ")):"")}}};
_.wm=function(a,c){this.f=this.D=this.j="";this.B=null;this.w=this.o="";this.A=!1;var d;a instanceof _.wm?(this.A=void 0!==c?c:a.A,_.xm(this,a.j),this.D=a.D,_.ym(this,a.f),_.zm(this,a.B),_.Am(this,a.o),_.Bm(this,_.Cm(a.b)),_.Dm(this,a.w)):a&&(d=String(a).match(_.hk))?(this.A=!!c,_.xm(this,d[1]||"",!0),this.D=Em(d[2]||""),_.ym(this,d[3]||"",!0),_.zm(this,d[4]),_.Am(this,d[5]||"",!0),_.Bm(this,d[6]||"",!0),_.Dm(this,d[7]||"",!0)):(this.A=!!c,this.b=new Fm(null,this.A))};
_.wm.prototype.toString=function(){var a=[],c=this.j;c&&a.push(Gm(c,Hm,!0),":");var d=this.f;if(d||"file"==c)a.push("//"),(c=this.D)&&a.push(Gm(c,Hm,!0),"@"),a.push(_.fk(d).replace(/%25([0-9a-fA-F]{2})/g,"%$1")),d=this.B,null!=d&&a.push(":",String(d));if(d=this.o)this.f&&"/"!=d.charAt(0)&&a.push("/"),a.push(Gm(d,"/"==d.charAt(0)?Im:Jm,!0));(d=this.b.toString())&&a.push("?",d);(d=this.w)&&a.push("#",Gm(d,Km));return a.join("")};
_.xm=function(a,c,d){a.j=d?Em(c,!0):c;a.j&&(a.j=a.j.replace(/:$/,""));return a};_.ym=function(a,c,d){a.f=d?Em(c,!0):c;return a};_.zm=function(a,c){if(c){c=Number(c);if(isNaN(c)||0>c)throw Error("$`"+c);a.B=c}else a.B=null;return a};_.Am=function(a,c,d){a.o=d?Em(c,!0):c;return a};_.Bm=function(a,c,d){c instanceof Fm?(a.b=c,Lm(a.b,a.A)):(d||(c=Gm(c,Mm)),a.b=new Fm(c,a.A));return a};_.Nm=function(a,c,d){a.b.set(c,d);return a};_.Om=function(a,c){return a.b.get(c)};_.Dm=function(a,c,d){a.w=d?Em(c):c;return a};
_.Pm=function(a){return a instanceof _.wm?new _.wm(a):new _.wm(a,void 0)};Em=function(a,c){return a?c?decodeURI(a.replace(/%25/g,"%2525")):decodeURIComponent(a):""};Gm=function(a,c,d){return"string"===typeof a?(a=encodeURI(a).replace(c,Qm),d&&(a=a.replace(/%25([0-9a-fA-F]{2})/g,"%$1")),a):null};Qm=function(a){a=a.charCodeAt(0);return"%"+(a>>4&15).toString(16)+(a&15).toString(16)};Hm=/[#\/\?@]/g;Jm=/[#\?:]/g;Im=/[#\?]/g;Mm=/[#\?@]/g;Km=/#/g;
Fm=function(a,c){this.f=this.b=null;this.j=a||null;this.o=!!c};Rm=function(a){a.b||(a.b=new _.bk,a.f=0,a.j&&vm(a.j,function(c,d){a.add(decodeURIComponent(c.replace(/\+/g," ")),d)}))};Fm.prototype.add=function(a,c){Rm(this);this.j=null;a=Sm(this,a);var d=this.b.get(a);d||this.b.set(a,d=[]);d.push(c);this.f+=1;return this};Fm.prototype.remove=function(a){Rm(this);a=Sm(this,a);return _.ek(this.b,a)?(this.j=null,this.f-=this.b.get(a).length,this.b.remove(a)):!1};
Fm.prototype.clear=function(){this.b=this.j=null;this.f=0};Fm.prototype.vc=function(){Rm(this);return 0==this.f};_.Tm=function(a,c){Rm(a);c=Sm(a,c);return _.ek(a.b,c)};_.k=Fm.prototype;_.k.forEach=function(a,c){Rm(this);this.b.forEach(function(d,e){(0,_.Ma)(d,function(f){a.call(c,f,e,this)},this)},this)};_.k.kb=function(){Rm(this);for(var a=this.b.Pa(),c=this.b.kb(),d=[],e=0;e<c.length;e++)for(var f=a[e],g=0;g<f.length;g++)d.push(c[e]);return d};
_.k.Pa=function(a){Rm(this);var c=[];if("string"===typeof a)_.Tm(this,a)&&(c=tm(c,this.b.get(Sm(this,a))));else{a=this.b.Pa();for(var d=0;d<a.length;d++)c=tm(c,a[d])}return c};_.k.set=function(a,c){Rm(this);this.j=null;a=Sm(this,a);_.Tm(this,a)&&(this.f-=this.b.get(a).length);this.b.set(a,[c]);this.f+=1;return this};_.k.get=function(a,c){if(!a)return c;a=this.Pa(a);return 0<a.length?String(a[0]):c};_.Um=function(a,c,d){a.remove(c);0<d.length&&(a.j=null,a.b.set(Sm(a,c),_.Zd(d)),a.f+=d.length)};
Fm.prototype.toString=function(){if(this.j)return this.j;if(!this.b)return"";for(var a=[],c=this.b.kb(),d=0;d<c.length;d++){var e=c[d],f=_.fk(e);e=this.Pa(e);for(var g=0;g<e.length;g++){var h=f;""!==e[g]&&(h+="="+_.fk(e[g]));a.push(h)}}return this.j=a.join("&")};_.Cm=function(a){var c=new Fm;c.j=a.j;a.b&&(c.b=new _.bk(a.b),c.f=a.f);return c};Sm=function(a,c){c=String(c);a.o&&(c=c.toLowerCase());return c};
Lm=function(a,c){c&&!a.o&&(Rm(a),a.j=null,a.b.forEach(function(d,e){var f=e.toLowerCase();e!=f&&(this.remove(e),_.Um(this,f,d))},a));a.o=c};

}catch(e){_._DumpException(e)}
try{
/*

Math.uuid.js (v1.4)
http://www.broofa.com
mailto:robert@broofa.com
Copyright (c) 2010 Robert Kieffer
Dual licensed under the MIT and GPL licenses.
*/
var Vm=function(a){_.A(this,a,0,-1,null,null)},$m,an,bn,cn,dn,en;_.w(Vm,_.z);var Wm=[2],Xm=function(a){_.A(this,a,0,-1,Wm,null)};_.w(Xm,_.z);_.Ym=function(a){var c=Number(a);return 0==c&&_.yh(a)?NaN:c};_.Zm=function(a,c,d){_.B(a,c).push(d);return a};$m=/^(?:(.*?)\.)?([a-zA-Z_$][\w$]*(?:\/.?<)?)?(\(.*\))?@(?::0|((?:http|https|file):\/\/[^\s)]+|javascript:.*))$/;an=/^\s{3,4}at(?: (?:(.*?)\.)?((?:new )?(?:[a-zA-Z_$][\w$]*|<anonymous>))(?: \[as ([a-zA-Z_$][\w$]*)\])?)? (?:\(unknown source\)|\(native\)|\((?:eval at )?((?:http|https|file):\/\/[^\s)]+|javascript:.*)\)|((?:http|https|file):\/\/[^\s)]+|javascript:.*))$/;
bn=function(a,c,d,e,f){this.f=a;this.name=c;this.b=d;this.o=e;this.j=f};cn=function(a){this.b=[];if(a.stack){a=a.stack.replace(/\s*$/,"").split("\n");for(var c=0;c<a.length;c++){var d,e=$m;if(d=a[c].match(an))d=new bn(d[1]||"",d[2]||"",d[3]||"","",d[4]||d[5]||""),this.b.push(d);else if(d=a[c].match(e))d=new bn(d[1]||"",d[2]||"","",d[3]||"",d[4]||""),this.b.push(d)}}};
dn=function(a){return(0,_.Oa)(a.b,function(c){var d=[c.f?c.f+".":"",c.name?c.name:"anonymous",c.o,c.b?" [as "+c.b+"]":""];if(c.j){d.push(" at ");c=c.j;var e="",f=c.match(/(.*?)(:\d+(:\d+)?)$/);f&&(c=f[1],e=f[2]);d.push(c.replace(window.location.href.replace(/#.*/,""),"[page]").replace(/http.*?extern_js.*?\.js/,"[xjs]"));d.push(e)}return d.join("")})};en=function(a,c,d,e,f){_.Pc.call(this,a,c,d,e,f);this.j=new cn(d)};_.w(en,_.Pc);
en.prototype.b=function(){en.L.b.call(this);window.console&&window.console.log&&window.console.log("Stack: ",this.j)};en.prototype.f=function(a){var c=en.L.f.call(this,a)+"&jsst=";var d=this.j;a-=c.length;if(4>a)a="";else if(0==d.b.length)a="none";else{d=dn(d);var e;var f=d.length-2;for(e=_.fk(d.join("\n"));0<f&&e.length>a;f--,e=_.fk(d.join("\n")))f==d.length-2?d[f]="[...]":d.splice(f,1);a=e.substr(0,a)}return c+a};var fn=function(a,c,d){_.J.call(this);this.f=a;this.j=c;this.o=d};_.p(fn,_.J);
fn.prototype.b=function(a,c){return new en(this.f,this.j,a,this.o,c)};var gn=[1,2,3,4],hn=function(a){_.A(this,a,0,-1,gn,null)};_.w(hn,_.z);var jn=function(){return"xxxxxxxx-xxxx-4xxx-yxxx-xxxxxxxxxxxx".replace(/[xy]/g,function(a){var c=16*Math.random()|0;return("x"==a?c:c&3|8).toString(16)})};
var kn=function(a,c){_.J.call(this);this.B=c;this.W=0;this.w=_.Mc(_.yc(a,2,1E-4),.001);this.o=_.Mc(_.yc(a,10,0),0);this.T=_.L(_.B(a,21),"");this.S=_.Mc(_.B(a,4),0);this.R=_.Mc(_.B(a,5),-1);this.N=_.L(_.B(a,7),"");this.K=_.L(_.B(a,6),"");this.J=_.L(_.B(a,8),"");this.F=_.B(a,9);this.U=!!_.C(a,11);this.O=!!_.C(a,12);this.G=!!_.C(a,15);this.D=!!_.C(a,16);this.f=null!=_.B(a,17)?_.B(a,17).split(","):[];var d=Math.random();this.A=_.K(_.C(a,1))&&d<this.w;this.j=_.K(_.C(a,1))&&d<this.o;this.M="og-"+jn();if(this.A||
this.j){a=_.C(a,3)?"https://play.googleapis.com/staging/log":void 0;c=this.b=new _.wl(373,_.L(_.B(c,5)),a);c.O=!0;_.sl(c,1E3);this.b.S=!!_.eg().navigator.sendBeacon&&(_.oc||_.kc&&_.gc(45));if(0!=this.f.length){c=new hn;for(a=0;a<this.f.length;a++)d=Number(this.f[a]),isNaN(d)||0==d||_.Zm(c,3,d);a=this.b;c?(a.j||(a.j=new Xm),c=c.f(),_.F(a.j,4,c)):a.j&&_.F(a.j,4,void 0)}_.Yf(this,this.b)}};_.w(kn,_.J);var ln=[1];
kn.prototype.log=function(a,c){var d=!_.Qa(ln,a);if(d?this.A:this.j)c=(void 0===c?null:c)||new _.Cc,_.F(c,1,a),a=++this.W,_.F(c,38,a),_.F(c,2,this.S),_.F(c,4,d?this.w:this.o),_.F(c,6,this.T),_.F(c,3,this.R),_.F(c,11,this.K),_.F(c,10,this.N),_.F(c,5,this.J),window.performance&&window.performance.timing&&_.F(c,14,(new Date).getTime()-window.performance.timing.navigationStart),_.F(c,13,this.F),_.F(c,16,this.U),_.F(c,17,this.O),_.F(c,19,this.M),d=0,_.C(this.B,1)&&(d|=1),_.C(this.B,3)&&(d|=4),_.F(c,12,
d),_.F(c,25,this.G),_.F(c,26,this.D),d=new _.el,_.gl(d,c.f()),this.b.log(d)};
var mn,nn,pn,qn,rn;mn=_.H(_.ud,Vm,16)||new Vm;nn=_.wd()||new _.Fc;_.on=new kn(mn,nn);pn=_.vd()||new _.Ec;rn=_.H(_.ud,_.Kc,14)||new _.Kc;qn=_.B(rn,9);var sn=_.yc(_.H(_.ud,_.Uc,3)||new _.Uc,2,.001);_.yd.f=new fn(pn,qn,sn);_.yd.b=_.on;

}catch(e){_._DumpException(e)}
try{
var un;_.tn=function(a,c){return _.F(a,27,c)};un=function(a,c){c=c instanceof _.tb?c:_.xb(c);a.action=_.ub(c)};_.vn=function(){};_.w(_.vn,_.Uj);_.vn.prototype.b=function(){var a=new XMLHttpRequest;if("withCredentials"in a)return a;if("undefined"!=typeof XDomainRequest)return new wn;throw Error("ba");};_.vn.prototype.o=function(){return{}};
var wn=function(){this.b=new XDomainRequest;this.readyState=0;this.onreadystatechange=null;this.responseType=this.responseText="";this.status=-1;this.statusText="";this.b.onload=(0,_.t)(this.Qh,this);this.b.onerror=(0,_.t)(this.Yf,this);this.b.onprogress=(0,_.t)(this.Ei,this);this.b.ontimeout=(0,_.t)(this.Li,this)};_.k=wn.prototype;_.k.open=function(a,c,d){if(null!=d&&!d)throw Error("ca");this.b.open(a,c)};_.k.send=function(a){if(a)if("string"==typeof a)this.b.send(a);else throw Error("da");else this.b.send()};
_.k.abort=function(){this.b.abort()};_.k.setRequestHeader=function(){};_.k.getResponseHeader=function(a){return"content-type"==a.toLowerCase()?this.b.contentType:""};_.k.Qh=function(){this.status=200;this.responseText=this.b.responseText;xn(this,4)};_.k.Yf=function(){this.status=500;this.responseText="";xn(this,4)};_.k.Li=function(){this.Yf()};_.k.Ei=function(){this.status=200;xn(this,1)};var xn=function(a,c){a.readyState=c;if(a.onreadystatechange)a.onreadystatechange()};
wn.prototype.getAllResponseHeaders=function(){return"content-type: "+this.b.contentType};
/*

 Copyright The Closure Library Authors.
 SPDX-License-Identifier: Apache-2.0
*/
var An=function(){_.Q.call(this);this.f="closure_frame"+yn++;this.j=[];zn[this.f]=this},Bn;_.w(An,_.Q);var zn={},yn=0,Cn=function(a,c){var d=_.pg(a);_.Ck(c,function(e,f){_.Ba(e)||(e=[e]);(0,_.Ma)(e,function(g){g=d.wa("INPUT",{type:"hidden",name:f,value:g});a.appendChild(g)})})};_.k=An.prototype;_.k.Fa=null;_.k.Ka=null;_.k.Ic=null;_.k.lj=0;_.k.tc=!1;_.k.ue=!1;_.k.ie=null;_.k.Hc=null;
_.k.send=function(a,c,d,e){if(this.tc)throw Error("ea");a=new _.wm(a);c=c?c.toUpperCase():"GET";d&&_.Nm(a,"zx",_.um());Bn||(Bn=_.ve("FORM"),Bn.acceptCharset="utf-8",d=Bn.style,d.position="absolute",d.visibility="hidden",d.top=d.left="-10px",d.width=d.height="10px",d.overflow="hidden",document.body.appendChild(Bn));this.Fa=Bn;"GET"==c&&Cn(this.Fa,a.b);e&&Cn(this.Fa,e);e=this.Fa;a=a.toString();(0,_.xl)();un(e,new _.tb(_.rb,a));this.Fa.method=c;this.tc=!0;this.Ic=this.f+"_"+(this.lj++).toString(36);
this.Ka=_.pg(this.Fa).wa("IFRAME",{name:this.Ic,id:this.Ic});_.y&&7>Number(_.fc)&&un(this.Ka,new _.tb(_.rb,_.mf(_.ib('javascript:""'))));e=this.Ka.style;e.visibility="hidden";e.width=e.height="10px";e.display="none";_.Sb?e.marginTop=e.marginLeft="-10px":(e.position="absolute",e.top=e.left="-10px");if(_.y&&!_.gc("11")){this.Fa.target=this.Ic||"";_.pg(this.Fa).b.body.appendChild(this.Ka);_.O(this.Ka,"readystatechange",this.jf,!1,this);try{this.b=!1,this.Fa.submit()}catch(v){_.ff(this.Ka,"readystatechange",
this.jf,!1,this),Dn(this)}}else{_.pg(this.Fa).b.body.appendChild(this.Ka);e=this.Ic+"_inner";a=_.ak(this.Ka);document.baseURI?(c=_.ke(e),c=_.Fb('<head><base href="'+_.ke(document.baseURI)+'"></head><body><iframe id="'+c+'" name="'+c+'"></iframe>',null)):(c=_.ke(e),c=_.Fb('<body><iframe id="'+c+'" name="'+c+'"></iframe>',null));_.Ob&&!_.Sb?_.ag(a.documentElement,c):a.write(_.Eb(c));_.O(a.getElementById(e),"load",this.ne,!1,this);var f=_.qe("TEXTAREA",this.Fa);c=0;for(d=f.length;c<d;c++){var g=f[c].value,
h=[];_.mg(f[c],h,!1);h.join("")!=g&&(_.ig(f[c],g),f[c].value=g)}f=a.importNode(this.Fa,!0);f.target=e;f.action=this.Fa.action;a.body.appendChild(f);g=_.qe("SELECT",this.Fa);h=_.qe("SELECT",f);c=0;for(d=g.length;c<d;c++)for(var l=_.qe("OPTION",g[c]),m=_.qe("OPTION",h[c]),n=0,r=l.length;n<r;n++)m[n].selected=l[n].selected;g=_.qe("INPUT",this.Fa);h=_.qe("INPUT",f);c=0;for(d=g.length;c<d;c++)if("file"==g[c].type&&g[c].value!=h[c].value){this.Fa.target=e;f=this.Fa;break}try{this.b=!1,f.submit(),a.close(),
_.Rb&&_.rg(this.A,250,this)}catch(v){_.ff(a.getElementById(e),"load",this.ne,!1,this),a.close(),Dn(this)}}En(this)};_.k.abort=function(){if(this.tc){var a=Fn(this);if(a)if(_.Pe(a))a.re(void 0);else if(a=_.bf(a)){var c=0,d;for(d in a.b)for(var e=a.b[d].concat(),f=0;f<e.length;++f)_.gf(e[f])&&++c}this.ue=this.tc=!1;this.dispatchEvent("abort");Gn(this)}};_.k.P=function(){this.tc&&this.abort();An.L.P.call(this);this.Ka&&Hn(this);En(this);delete this.w;this.ie=this.Fa=null;delete zn[this.f]};_.k.ee=function(){return this.ue};
_.k.Vf=function(){return this.ie};_.k.Uf=function(){return _.Ok(this.ie)};_.k.jf=function(){if("complete"==this.Ka.readyState){_.ff(this.Ka,"readystatechange",this.jf,!1,this);try{var a=_.ak(this.Ka);if(_.y&&"about:blank"==a.location&&!navigator.onLine){Dn(this);return}}catch(c){Dn(this);return}In(this,a)}};_.k.ne=function(){if(!_.Ob||_.Sb||"about:blank"!=(this.Ka?_.ak(Fn(this)):null).location){_.ff(Fn(this),"load",this.ne,!1,this);try{In(this,this.Ka?_.ak(Fn(this)):null)}catch(a){Dn(this)}}};
var In=function(a,c){a.tc=!1;try{var d=c.body;a.ie=d.textContent||d.innerText}catch(f){var e=1}e||"function"!=typeof a.w||(c=a.w(c))&&(e=4);e?Dn(a):(a.ue=!0,a.dispatchEvent("complete"),a.dispatchEvent("success"),Gn(a))},Dn=function(a){a.b||(a.ue=!1,a.tc=!1,a.dispatchEvent("complete"),a.dispatchEvent("error"),Gn(a),a.b=!0)},Gn=function(a){Hn(a);En(a);a.Fa=null;a.dispatchEvent("ready")},Hn=function(a){var c=a.Ka;c&&(c.onreadystatechange=null,c.onload=null,c.onerror=null,a.j.push(c));a.Hc&&(_.sg(a.Hc),
a.Hc=null);_.Rb||_.Ob&&!_.Sb?a.Hc=_.rg(a.o,2E3,a):a.o();a.Ka=null;a.Ic=null};An.prototype.o=function(){this.Hc&&(_.sg(this.Hc),this.Hc=null);for(;0!=this.j.length;){var a=this.j.pop();_.Ae(a)}};var En=function(a){a.Fa&&a.Fa==Bn&&_.fg(a.Fa)},Fn=function(a){return a.Ka?_.y&&!_.gc("11")?a.Ka:_.ak(a.Ka).getElementById(a.Ic+"_inner"):null};An.prototype.A=function(){if(this.tc){var a=this.Ka?_.ak(Fn(this)):null;a&&!_.Ke(a,"documentUri")?(_.ff(Fn(this),"load",this.ne,!1,this),Dn(this)):_.rg(this.A,250,this)}};
var Jn=function(a,c,d){this.groupId=a;this.A="dp_"+a;this.B="count_"+a;this.o=c;this.b=!!d},Kn=/google(?:.[a-z]{2,3}){1,2}$/i,Ln=function(){var a=_.q.location.hostname.match(Kn);return a&&a[0]?a[0]:null};Jn.prototype.te=function(){return!!navigator.cookieEnabled};Jn.prototype.La=function(a){this.te()&&this.Oc(!1,a)};Jn.prototype.accept=function(a){this.te()&&this.Oc(!0,a)};Jn.prototype.Oc=function(){throw Error("fa");};_.Mn=function(a){0<a.o&&a.te()&&a.Ad(void 0,void 0)};
Jn.prototype.Ad=function(){throw Error("fa");};Jn.prototype.Zb=function(){return 0};Jn.prototype.Xe=function(){return!1};
_.Nn=function(a,c,d,e,f){Jn.call(this,c,d);this.f=f;this.j=!e||-2==e||31536E3<e?31536E3:e;this.w=new RegExp("\\b"+this.groupId+"-([0-9]+):")};_.w(_.Nn,Jn);_.k=_.Nn.prototype;_.k.te=function(){navigator.cookieEnabled||(this.j=-1);return!0};_.k.Oc=function(a,c){var d=_.Sj.get("OGP",""),e="-"+this.groupId+":";(new RegExp(e)).test(d)||(d+=e);(e=Ln())&&_.Sj.set("OGP",d,{je:this.j,path:"/",domain:e});this.f&&this.f.Oc(a,c)};
_.k.Ad=function(a){var c=_.Sj.get("OGPC",""),d=this.Zb(c),e=!0;-1==d&&(e=!1,d=0);a=this.groupId+"-"+(d+(a||1))+":";c=e?c.replace(this.w,a):(c?c:"")+a;(e=Ln())&&_.Sj.set("OGPC",c,{je:this.j,path:"/",domain:e});this.f&&this.f.Ad()};_.k.Zb=function(a){var c=a||_.Sj.get("OGPC","");a=-1;c&&(c=c.match(this.w))&&1<c.length&&(a=parseInt(c[1],10)||0);return a};_.k.Xe=function(){return-1!=_.Sj.get("OGP","").indexOf("-"+this.groupId+":")};
var On;On=window.location.protocol+"//www.google.com/_/og/promos/";_.Pn=function(a,c,d,e,f,g,h){var l={};l.p=d;l.g=c;l.a=e;l.at=f;l.eid=g;l.pid=1;if(h)l.t=h;else return a.log(Error("ga")),null;return l};_.Qn=function(a,c,d){if(a){var e=[On,d?"g":"z"];d&&c&&e.push(["?authuser=",c].join(""));c=e.join("");try{_.Vj=new _.vn;d=[];for(var f in a)a.hasOwnProperty(f)&&d.push(f+"="+a[f]);_.Uk(c,null,"POST",d.join("&"),null,void 0,!0)}catch(g){f=new An,_.O(f,"ready",f.sa,!1,f),f.send(c,"POST",!1,a)}}};
var Rn=function(a,c,d,e,f,g,h,l){Jn.call(this,c,d);this.f=a;h||l?(this.j=e,this.D=f,this.w=h||l||"",this.G=!!l,this.F=g):a.log(Error("ha"))};_.w(Rn,Jn);Rn.prototype.Oc=function(a,c){a?(a=this.D,(c=_.Pn(this.f,this.groupId,this.j,"a",3,c||"",this.w))&&(c.u=a)):(a=this.D,(c=_.Pn(this.f,this.groupId,this.j,"d",2,c||"",this.w))&&(c.u=a));_.Qn(c,this.F,this.G)};Rn.prototype.Ad=function(a,c){a=a||1;(c=_.Pn(this.f,this.groupId,this.j,"i",1,c||"",this.w))&&(c.c=a);_.Qn(c,this.F,this.G)};
var Sn=function(a,c,d,e,f){Jn.call(this,c,d,f);this.j=a;this.f=e};_.w(Sn,Jn);Sn.prototype.Oc=function(){this.j.qf(this.f,this.A,"1",this.b)};Sn.prototype.Ad=function(a){a=this.Zb()+(a||1);this.j.qf(this.f,this.B,a.toString(),this.b)};Sn.prototype.Xe=function(){return!!this.j.Ke(this.f,this.A,this.b)};Sn.prototype.Zb=function(){var a=this.j.Ke(this.f,this.B,this.b);return parseInt(a||0,10)};
_.Tn=function(a,c,d,e,f,g,h,l,m,n,r){if(n||r)try{var v=new Rn(a,f,g,h,l,d,n,r)}catch(N){v=null}else v=null;switch(e){case 2:case 6:return v;case 1:return new Sn(c,f,g,m,void 0);default:return new _.Nn(a,f,g,l)}};
var Un;Un=function(a){switch(a){case "i":return 36;case "x":return 37;case "n":return 37;case "a":return 38;case "d":return 37;case "er_em":return 72;case "rl":return 77;case "lc":return 111;case "hc":return 112;default:return 0}};
_.Vn=function(a,c,d,e,f,g,h,l){var m=Un(c);if(0!==m){var n=new _.Cc;switch(c){case "x":_.F(n,28,1);break;case "n":_.F(n,28,2);break;case "a":_.F(n,29,1);break;case "er_em":_.F(n,30,1)}_.F(n,34,g);_.F(n,48,h);_.F(n,31,d);_.F(n,39,e);try{var r=f.getBoundingClientRect()}catch(v){}null!=r&&(_.F(n,43,r.top),_.F(n,44,r.bottom),_.F(n,45,r.left),_.F(n,46,r.right));null!=l&&_.tn(n,l);a.log(m,n)}};
_.Wn=function(){this.wb=null;this.b=!1};_.ya(_.Wn);

}catch(e){_._DumpException(e)}
try{
var Zn,co;_.Xn=function(a,c,d,e,f,g){d.H(c,e,f,g||a.T||a,a)};_.Yn=function(a,c){c=a.f[c]||c;return _.Ih(a)==c};Zn=function(a,c,d){d=d.Bd();if(a.b[c]&&a.b[c][d])for(var e=0;e<a.b[c][d].length;e++)try{a.b[c][d][e]()}catch(f){a.A.log(f)}};_.$n=function(a,c){a.w?a.w.appendChild(c):a.F?a.F.appendChild(c):a.M.log(Error("L"))};_.ao=function(a){_.A(this,a,0,-1,null,null)};_.w(_.ao,_.z);
_.bo=function(a,c,d){if(c instanceof _.pe)d=c.height,c=c.width;else if(void 0==d)throw Error("t");a.style.width=_.Og(c,!0);a.style.height=_.Og(d,!0)};co=function(){_.J.call(this);this.b=new _.vg};_.p(co,_.J);co.prototype.H=function(a,c,d,e,f){(f||this.b).o(a,eo,c,d,e)};co.prototype.Ba=function(a,c,d,e,f){(f||this.b).Ba(a,eo,c,d,e)};co.prototype.P=function(){this.b.sa();_.J.prototype.P.call(this)};var fo=new co,eo=["click","keydown","mousedown","touchstart"];
var go=function(){this.b=0};go.prototype.ya=function(){return++this.b};go.prototype.reset=function(){this.b=0};
var lo;_.io=function(a,c,d,e,f,g,h){g=void 0===g?!1:g;_.Fh.call(this,a,d);this.$=new go;this.G=f;this.B=e;this.Z=this.J=null;this.Pg=c;this.W=null;(this.j=h||_.M("gb_D",this.f))&&this.j.setAttribute("aria-expanded","false");this.M=_.Xc("dd");this.M.o(this);(a=_.M("gb_F",this.f))&&_.ho(this,a,!1);g||this.Wc()};_.w(_.io,_.Fh);_.k=_.io.prototype;
_.k.Wc=function(){_.Xn(this,document,fo,this.fg,!0,this);this.o(document,_.Xg(27)?"keypress":"keyup",this.jd,!1,this);this.o(this.f,"mouseover",this.bc,!1,this);this.o(this.f,"mouseout",this.Vb,!1,this);this.o(this.f,["keyup","keydown"],this.Ji,!1,this);this.o(document.body,"focusin",this.Aj,!1,this)};_.k.Ji=function(a){var c=a.target;c instanceof Element&&jo(this,c)&&32==a.keyCode&&(a.preventDefault(),a.stopPropagation())};_.k.Aj=function(){this.Rb()&&(jo(this,document.activeElement)||this.Ie())};
_.k.Te=function(){_.Xn(this,this.b,_.oh,this.zc,!1,this);_.hg(this.f,this.b)||(this.o(this.b,"mouseover",this.bc,!1,this),this.o(this.b,"mouseout",this.Vb,!1,this));this.H(this.b,"keydown",this.hd,!0)};_.k.Bd=function(){return this.Pg};_.ko=function(a,c){a.W&&a.W.sa();a.W=c};_.io.prototype.Yd=function(a){if(null==this.f.getAttribute("data-ogsr-fb")){var c="click"!=a.type;this.Rb()?this.close(void 0,!0,1):this.wc(c);a.preventDefault();a.stopPropagation()}};
_.io.prototype.zc=function(a){for(a=a.target;a&&a!=this.b;){if("A"==a.tagName&&!_.R(a,"gb_bg")){this.close(!0,!0,3);break}a=a.parentNode}};var jo=function(a,c){if(!c)return!1;var d=!!a.b&&_.hg(a.b,c);return _.hg(a.f,c)||d};_.io.prototype.fg=function(a){var c=a.target;if(lo(this)){a:{var d=a.ab;if(null!=d&&(d=_.Ca(d.composedPath)?d.composedPath():void 0,null!=d&&0<d.length&&(d=d[0],!(d instanceof Window))))break a;d=null}null!=d&&(c=d)}jo(this,c)||27==a.keyCode||this.close(void 0,!0,2)};
_.io.prototype.hd=function(a){if(9===a.keyCode&&this.Rb()){var c=a.target,d=_.ni(this.b);0<d.length&&(c==d[0]&&a.shiftKey?(d[d.length-1].focus(),a.preventDefault()):c!=d[d.length-1]||a.shiftKey||(d[0].focus(),a.preventDefault()))}};_.io.prototype.bc=function(a){mo(this,(0,_.t)(this.Oe,this),a)};_.io.prototype.Vb=function(a){mo(this,(0,_.t)(this.Ac,this),a)};
var mo=function(a,c,d){var e=d.relatedTarget&&(_.hg(a.f,d.relatedTarget)||_.hg(a.b,d.relatedTarget)),f=d.relatedTarget&&no(a,d.relatedTarget);a=no(a,d.target);e||c(0,d);e&&!f||a||c(1,d);!f&&a&&c(2,d)};_.io.prototype.jd=function(a){if(27==a.keyCode){a=_.ng(document);var c=jo(this,a),d=this.Rb();this.close(void 0,!1,1);d&&c?this.j.focus():a&&a.focus()}};_.io.prototype.Oe=_.xa;_.io.prototype.Ac=_.xa;var no=function(a,c){return c&&a.b?_.R(c,"gb_1a")||_.R(c,"gb_2a")||!!a.b&&_.hg(a.b,c):!1};
_.io.prototype.P=function(){_.io.L.P.call(this);this.b=null};_.oo=function(a){if(a.j&&(a=a.j.getAttribute("data-ved")))return{ved:a}};_.k=_.io.prototype;_.k.me=function(a){a?this.wc():this.close()};_.k.ng=function(){return!1};
_.k.wc=function(a){if(!this.Rb()){this.$.reset();Zn(this.M,0,this);_.Rh(this.M,this);_.S(this.f,"gb_na");_.S(this.b,"gb_na");this.b.setAttribute("aria-hidden","false");this.j&&this.j.setAttribute("aria-expanded","true");if(_.y&&this.b){var c=_.M("gb_Lf");if(!c){c=_.ve("IFRAME",{"class":"gb_Lf",src:'javascript:""',frameBorder:0});var d=_.M("gb_Uc");d&&d.appendChild(c)}_.T(c,"gb_Fa");this.le()}this.J&&this.B.log(this.J,_.oo(this));this.Aa&&_.po(this,this.Aa,void 0,!1);Zn(this.M,1,this);this.W&&this.W.ha(!1);
a&&this.Ie()}};_.k.Ie=function(){var a=_.ni(this.b);a[0]?a[0].focus():this.b.focus()};_.k.le=function(){if(_.y&&this.b){var a=_.M("gb_Lf");a&&_.bo(a,_.Qg(this.b))}};
_.k.close=function(a,c,d){a=void 0===a?!1:a;c=void 0===c?!1:c;d=void 0===d?0:d;return this.Rb()&&!this.M.B[this.Bd()]?(_.Yn(this.M,this)&&_.Rh(this.M,null),_.T(this.f,"gb_na"),_.T(this.b,"gb_na"),this.b.setAttribute("aria-hidden","true"),this.j&&(this.j.setAttribute("aria-expanded","false"),!c&&jo(this,document.activeElement)&&setTimeout((0,_.t)(this.j.focus,this.j),0)),_.y&&(c=_.M("gb_Lf"))&&_.S(c,"gb_Fa"),!a&&this.Z&&this.B.log(this.Z,_.oo(this)),!a&&this.ma&&_.po(this,this.ma,void 0,!0,d),Zn(this.M,
2,this),!0):!1};_.k.Rb=function(){return _.R(this.f,"gb_na")};_.ho=function(a,c,d){a.b||(a.b=c,d&&(c=a.b,d=a.f,c&&d&&c.parentNode!=d&&d.appendChild(c)),a.b.setAttribute("aria-hidden","true"),a.j&&_.Xn(a,a.j,_.oh,a.Yd,!1,a),a.Te())};lo=function(a){a=[a.f,a.b].filter(function(e){return null!=e});for(var c,d=0;d<a.length;d++){c=a[d];if(!_.Ca(c.getRootNode))break;if(11===c.getRootNode().nodeType)return!0}return!1};
_.po=function(a,c,d,e,f){d=void 0===d?new _.Cc:d;e=void 0===e?!1:e;var g=new _.ao,h=a.$.ya();_.F(g,1,h);e&&_.F(g,2,e);void 0!=f&&_.F(g,3,f);_.I(d,37,g);a.G.log(c,d)};

}catch(e){_._DumpException(e)}
try{
/*
 Portions of this code are from MochiKit, received by
 The Closure Authors under the MIT license. All other code is Copyright
 2005-2009 The Closure Authors. All Rights Reserved.
*/
_.qo=function(a,c){this.w=[];this.M=a;this.Sa=c||null;this.o=this.b=!1;this.j=void 0;this.G=this.J=this.B=!1;this.A=0;this.f=null;this.D=0};_.qo.prototype.cancel=function(a){if(this.b)this.j instanceof _.qo&&this.j.cancel();else{if(this.f){var c=this.f;delete this.f;a?c.cancel(a):(c.D--,0>=c.D&&c.cancel())}this.M?this.M.call(this.Sa,this):this.G=!0;this.b||(a=new ro(this),_.so(this),_.to(this,!1,a))}};_.qo.prototype.F=function(a,c){this.B=!1;_.to(this,a,c)};
_.to=function(a,c,d){a.b=!0;a.j=d;a.o=!c;uo(a)};_.so=function(a){if(a.b){if(!a.G)throw new vo(a);a.G=!1}};_.qo.prototype.Mc=function(a){_.so(this);_.to(this,!0,a)};_.wo=function(a,c,d,e){a.w.push([c,d,e]);a.b&&uo(a)};_.qo.prototype.then=function(a,c,d){var e,f,g=new _.Gf(function(h,l){e=h;f=l});_.wo(this,e,function(h){h instanceof ro?g.cancel():f(h)});return g.then(a,c,d)};_.pf(_.qo);_.qo.prototype.isError=function(a){return a instanceof Error};
var xo=function(a){return(0,_.Pa)(a.w,function(c){return _.Ca(c[1])})},uo=function(a){if(a.A&&a.b&&xo(a)){var c=a.A,d=yo[c];d&&(_.q.clearTimeout(d.b),delete yo[c]);a.A=0}a.f&&(a.f.D--,delete a.f);c=a.j;for(var e=d=!1;a.w.length&&!a.B;){var f=a.w.shift(),g=f[0],h=f[1];f=f[2];if(g=a.o?h:g)try{var l=g.call(f||a.Sa,c);void 0!==l&&(a.o=a.o&&(l==c||a.isError(l)),a.j=c=l);if(_.qf(c)||"function"===typeof _.q.Promise&&c instanceof _.q.Promise)e=!0,a.B=!0}catch(m){c=m,a.o=!0,xo(a)||(d=!0)}}a.j=c;e&&(l=(0,_.t)(a.F,
a,!0),e=(0,_.t)(a.F,a,!1),c instanceof _.qo?(_.wo(c,l,e),c.J=!0):c.then(l,e));d&&(c=new zo(c),yo[c.b]=c,a.A=c.b)},vo=function(){_.Ka.call(this)};_.w(vo,_.Ka);vo.prototype.message="Deferred has already fired";vo.prototype.name="AlreadyCalledError";var ro=function(){_.Ka.call(this)};_.w(ro,_.Ka);ro.prototype.message="Deferred was canceled";ro.prototype.name="CanceledError";var zo=function(a){this.b=_.q.setTimeout((0,_.t)(this.j,this),0);this.f=a};
zo.prototype.j=function(){delete yo[this.b];throw this.f;};var yo={};
var Ao=function(a,c){_.J.call(this);this.j=a;this.w=c;this.b=new _.qo};_.p(Ao,_.J);Ao.prototype.o=function(a){try{var c=_.He("gadgets.config.update");c({"googleapis.config":{gcv:_.L(_.B(a,2)),sessionIndex:_.L(_.B(a,4)),elog:this.j.log,ilog:_.Sd(this.w.log,16)}});c({gwidget:{lang:_.L(_.B(a,5))}});this.b.Mc()}catch(d){this.j.log(d)}};Ao.prototype.f=function(a){a&&_.wo(this.b,a,null,void 0)};
Ao.prototype.init=function(a,c){try{if(_.B(a,1)){var d=(0,_.t)(this.o,this,a);_.wo(c.f,d,null,void 0)}else this.b.Mc();_.u("gbar.lGC",(0,_.t)(this.f,this));_.u("gbar.lPWF",(0,_.t)(this.f,this));_.Wc(_.Vc.ta(),"api").Cc()}catch(e){this.j.log(e)}return this};
var Bo=function(){_.Ka.call(this)};_.p(Bo,_.Ka);var Co=function(a,c){_.J.call(this);this.j=a;this.b=c;this.f=new _.qo};_.p(Co,_.J);
Co.prototype.init=function(a){try{if(!this.b)throw new Bo("gapi-lm");var c={isPlusUser:_.L(_.B(a,4)),"googleapis.config":{signedIn:_.L(_.B(a,5))},lang:_.L(_.B(a,10))},d=_.L(_.B(a,6));d&&(c.iframes={":socialhost:":d});this.b("",{config:c});try{var e=_.Xc("gs");if(!e)throw new Bo("gapi-ss");this.b(e.b.join(":"),(0,_.t)(this.f.Mc,this.f));var f=_.Zd(e.f);for(a=0;a<f.length;a++)this.b(f[a].Nd,f[a].options)}catch(g){this.j.log(g)}}catch(g){this.j.log(g)}return this};
_.Do=function(){var a=_.H(_.ud,_.Kc,14)||new _.Kc,c=new Co(_.yd,_.He("gapi.load"));c.init(a);a=_.H(_.ud,_.Lc,9)||new _.Lc;var d=new Ao(_.yd,_.zd);d.init(a,c);d.f(function(){_.rd(_.sd.ta().G,!0)});return d}();

}catch(e){_._DumpException(e)}
try{
var Eo=function(a){_.A(this,a,0,-1,null,null)};_.w(Eo,_.z);var Fo=function(a){_.A(this,a,0,-1,null,null)};_.w(Fo,_.z);Fo.prototype.B=function(){return _.B(this,7)};Fo.prototype.D=function(){return _.B(this,8)};var Go=function(a){_.A(this,a,0,-1,null,null)};_.w(Go,_.z);var Ho=function(a){_.A(this,a,0,-1,null,null)};_.w(Ho,_.z);var Io=function(a){_.A(this,a,0,-1,null,null)};_.w(Io,_.z);
var Jo=function(a){var c;(c=a.Xe())||(c=0<a.o&&a.Zb()>=a.o);return c},Ko=function(a,c){_.oh.H(a,c,void 0,void 0)},Lo=function(a,c,d,e,f,g,h,l){this.data={};_.Za(this.data,{ogsr:Math.round(1/a),ei:c,ct:e,cad:f,id:d,loc:window.google?window.google.sn:"",prid:g,ogd:h,ogprm:"up"});if(l)for(a=l.split("&"),c=0;c<a.length;c++)d=a[c].split("="),2==d.length&&(this.data[d[0]]=d[1])};_.w(Lo,_.Nc);
var Mo=function(a,c,d,e,f,g,h){_.J.call(this);this.b=a;this.A=c;this.j=d;this.B=e;this.w=f;this.o=g;this.f=h;_.u("gbar.up.sl",(0,_.t)(this.log,this))};_.p(Mo,_.J);Mo.prototype.log=function(a,c,d,e,f){try{var g=this.A;if(void 0!=f&&null!=f)if(0<=f&&1>=f)g=f;else{this.b.log(Error("ia`"+c+"`"+d+"`"+f));return}if(Math.random()<=g){var h=new Lo(g,this.j,a,c,d,this.w,this.B,e);this.f?h.b():_.Rc(h)}}catch(l){this.b.log(Error("ia`"+c+"`"+d+"`"+f))}};
var No=function(a){_.J.call(this);this.b=a;_.u("gbar.up.spd",(0,_.t)(this.qf,this));_.u("gbar.up.gpd",(0,_.t)(this.Ke,this));_.u("gbar.up.dpc",(0,_.t)(this.Zi,this));_.u("gbar.up.iic",(0,_.t)(this.Ui,this));_.u("gbar.up.gcc",(0,_.t)(this.Fh,this))};_.p(No,_.J);var Oo=function(){try{return!!_.q.localStorage&&"object"==typeof _.q.localStorage}catch(a){return!1}},Po=function(a){return a&&a.style&&a.style.behavior&&"undefined"!=typeof a.load};_.k=No.prototype;
_.k.qf=function(a,c,d,e){try{navigator.cookieEnabled&&(e||(c="og-up-"+c),Oo()?_.q.localStorage.setItem(c,d):Po(a)&&(a.setAttribute(c,d),a.save(a.id)))}catch(f){f.code!=DOMException.QUOTA_EXCEEDED_ERR&&this.b.log(f)}};_.k.Ke=function(a,c,d){try{if(!navigator.cookieEnabled)return"";d||(c="og-up-"+c);if(Oo())return _.q.localStorage.getItem(c);if(Po(a))return a.load(a.id),a.getAttribute(c)}catch(e){e.code!=DOMException.QUOTA_EXCEEDED_ERR&&this.b.log(e)}return""};
_.k.Zi=function(a,c){(new _.Nn(this.b,a,1,c)).La()};_.k.Ui=function(a,c){_.Mn(new _.Nn(this.b,a,1,c))};_.k.Fh=function(a,c){return(new _.Nn(this.b,a,1)).Zb(c)};
var Qo=function(a){_.A(this,a,0,-1,null,null)};_.w(Qo,_.z);
_.pg();
var So=function(a,c,d,e,f,g){_.Fh.call(this,a,e);this.f=a;this.D=_.L(_.B(c,1));this.ma=_.L(_.B(c,2));this.X=_.L(_.B(c,3));_.E(c,4,25);this.U=_.Mc(_.B(c,5));this.Z=_.Mc(_.E(c,6,-1));this.N=_.K(_.C(c,9));this.B={wl:"i",accept:"a",La:"d",Gd:"x"};this.b=Ro;this.W=!1;this.R=f;this.Aa=g;this.F=_.M(this.b.Mg,this.f);this.Gd=_.M(this.b.Og,this.f);this.M=_.M(this.b.Ng,this.f);this.Y="";this.V=!1;var h,l;c.D&&(h=_.L(c.D()));c.B&&(l=_.L(c.B()));if(l||h)this.Y=l||h||"",this.V=!!l;this.j=_.Tn(e,this.Aa,d,this.U,
this.ma,_.Mc(_.E(c,4,25)),this.D,this.Z,this.f,h,l)};_.w(So,_.Fh);So.prototype.P=function(){So.L.P.call(this);this.M=this.Gd=this.F=null};var Ro={Mg:"gb_nd",Og:"gb_Jd",Ng:"gb_kd",Hd:"gb_na"};So.prototype.S=function(){_.R(this.f,this.b.Hd)||(_.S(this.f,this.b.Hd),this.f.removeAttribute("aria-hidden"))};So.prototype.close=function(){_.R(this.f,this.b.Hd)&&(_.T(this.f,this.b.Hd),this.f.setAttribute("aria-hidden","true"))};var To=function(a,c,d){var e=_.oh;c&&_.Xn(a,c,e,d,!1,a)};So.prototype.J=function(){return""};
var Uo=function(a){var c="";a&&(a=a.getAttributeNode("data-ved"))&&a.value&&(c=["&ved=",a.value].join(""));return c},Vo=function(a){var c=a.J();a.N&&(c+="&vis=0");a.R.log(a.D,a.X,"i",c,1)},Wo=function(a,c,d,e,f,g){var h=c==a.B.accept;a.W||(h&&!g||a.R.log(a.D,a.X,c,a.J()+Uo(d),1),f||0==a.U?2==a.U&&(c=a.R,d=a.V,e=_.Pn(c.b,a.ma,a.D,"l",3,e,a.Y),_.Qn(e,c.o,d)):(h?a.j.accept(e):a.j.La(e),a.W=!0));a.close()};So.prototype.K=function(a,c,d){Wo(this,this.B.accept,a.target,"2",c,d)};
So.prototype.ka=function(a,c){Wo(this,this.B.Gd,a.target,"1",c);a.preventDefault();a.stopPropagation()};So.prototype.$=function(a,c){Wo(this,this.B.La,a.target,"3",c);a.preventDefault();a.stopPropagation()};
var Xo=function(a,c,d,e,f){this.w=new _.Dh(f,this);this.b=f;this.o=d;this.B=e;this.j=a;this.f=c;a=_.li();this.w.o(a,"resize",this.A,!1,this)};Xo.prototype.A=function(){try{var a=276,c=document.getElementById("hplogo");c&&(a=Math.max(a,c.offsetWidth));2*(this.j+this.f)+a>document.body.clientWidth?this.o():this.B()}catch(d){this.b&&this.b.log(d)}};
var Yo=function(a,c){this.f=c;this.b={};this.b.mouseout=_.L(_.B(a,1));this.b.mouseover=_.L(_.B(a,2));this.b.mousedown=_.L(_.B(a,3))},Zo=function(a,c){if(c)for(var d in a.b){var e=a.b[d];e&&_.Ch(a.f,c,d,(0,_.t)(function(f){c.style.color=f},a,e))}},$o=function(a,c){for(var d=0;d<c.length;d++)Zo(a,c[d])};
var dp=function(a,c,d,e,f,g){_.io.call(this,a,"pc",e,f,g,!0);f=_.H(c,Fo,1)||new Fo;this.ze=d;this.N=_.L(_.B(f,1));this.K=/[^0-9]/.test(this.N)?0:_.Ym(this.N);this.lc=_.L(_.B(f,3));this.nc=_.L(_.B(f,2));this.Qi=_.L(f.B());this.yc=_.Mc(_.B(c,6));this.rd=_.Mc(_.E(f,4,25),25);this.od=_.K(_.C(c,21))||_.K(_.C(c,22));this.jc=_.K(_.C(c,16));a=this.od&&this.jc;this.mc=!_.K(_.C(f,9))&&!a;this.hc=!1;this.R=_.M("gb_nd",this.f);this.nd=_.K(_.C(c,10));this.md=_.K(_.C(c,14));this.D=_.K(_.C(c,19));this.va=this.nd||
this.md;this.Ja=_.M("gb_0f");this.dj=_.M("gb_1f");this.Wi=_.M("gb_Xf");this.Xi=_.M("gb_Zf");this.Ub=_.L(_.B(c,12));this.A=_.M("gb_Wf");this.X=_.M("gb_Dd");this.V=document.getElementById("gb");g=_.Vc.ta();this.kc=_.Wc(g,"p_log");this.Ae=_.Wc(g,"p_st");this.qd=_.Mc(_.B(f,5));this.Id=_.K(_.C(c,20));this.tb=_.K(_.C(c,18));this.U=_.Tn(e,this.Ae,d,this.qd,this.nc,this.rd,this.N,this.yc,this.f,_.L(f.D()),_.L(f.B()));this.F=this.U.Zb();this.V&&(this.Y=_.M("gb_Ua",this.V));this.S=!1;if(this.Y&&!Jo(this.U)&&
!this.S){d=_.L(_.B(c,2));if("n"!=d&&(this.qc=(f=ap[d])?_.M(f,this.Y):null,!this.qc)){this.w.log(Error("ja"),{target:d});return}1==_.B(c,3)&&_.S(this.R,"gb_xd");bp(this);c=_.H(c,Go,4)||new Go;$o(new Yo(c,this.w),[this.R]);this.kc.log(this.N,this.lc,"i","&vis="+(this.mc?"1":"0")+(this.tb?"&ap=0":""),1);a?cp(this):_.Vn(this.G,"i",this.K,this.F,this.C(),!1,this.D);this.Fb=0;this.mc?(this.wc(),new Xo(this.Fb,parseInt(this.b.style.right,10)||0,(0,_.t)(this.Si,this),(0,_.t)(this.tk,this),e)):this.J&&this.B.log(this.J,
_.oo(this));_.Mn(this.U)}this.Wc()};_.w(dp,_.io);var ap={p:"gb_Pa",s:"shareboxWidget",i:"gb_lg",v:"gb_C"};dp.prototype.P=function(){dp.L.P.call(this);this.V=this.Y=this.qc=this.button=this.Ma=null};dp.prototype.Ie=function(){};var ep=function(a){var c=_.M("gb_wd",a.f);if(c)return c;c=_.ze("IFRAME");c.frameBorder="0";c.tabIndex=-1;_.S(c,"gb_wd");var d=_.nf(_.ib("about:blank"));_.of(c,d);a.V.appendChild(c);return c};_.k=dp.prototype;
_.k.wc=function(){dp.L.wc.call(this);var a=ep(this);if(a){var c=_.M("gb_F",this.f);c.appendChild(a);a=a.style;a.width=c.offsetWidth+"px";a.height=c.offsetHeight+"px";a.visibility="visible";a.top="-1px";a.left="-1px"}this.Fb=this.b.offsetWidth};_.k.Si=function(){this.close();cp(this)};_.k.tk=function(){Jo(this.U)||this.S||this.wc()};_.k.close=function(){if(dp.L.close.call(this)){var a=ep(this);a&&(a=a.style,a.width="",a.height="",a.visibility="",a.top="",a.left="");return!0}return!1};_.k.fg=function(){};
_.k.Yd=function(){};var bp=function(a){a.Ma=_.M("gb_gd",a.f);a.Ma&&_.Xn(a,a.Ma,_.oh,a.Pi,!0,a);a.Kb=_.M("gb_kd",a.f);a.Kb&&_.Xn(a,a.Kb,_.oh,a.ii,!0,a);a.R&&_.Xn(a,a.R,_.oh,a.Xh,!0,a);a.$a=_.M("gb_vd",a.f);a.$a&&_.Xn(a,a.$a,_.oh,a.ui,!0,a);for(var c=_.rh("gb_D",a.Y),d=0;d<c.length;d++)_.Xn(a,c[d],_.oh,a.Mi,!0,a);a.A&&(a.o(a.A,"focus",a.Rg,!1,a),a.o(a.A,"blur",a.Lg,!1,a),a.o(a.A,"keyup",function(e){13==e.keyCode&&(e.preventDefault(),this.R.click())},!1,a),a.A.pattern="^\\+?1?[-()\\s]*([\\d][-()\\s]*){0,10}")};
dp.prototype.Rg=function(){this.X&&_.S(this.X,"gb_Ed")};dp.prototype.Lg=function(){this.X&&_.T(this.X,"gb_Ed")};var fp=function(a,c){a.S||(a.U.La(),("a"!=c||a.va)&&a.kc.log(a.N,a.lc,c,a.tb?"&ap=0":void 0,1),a.close(),a.S=!0)};_.k=dp.prototype;_.k.Mi=function(){this.va?(this.S=!0,this.close()):fp(this,"a")};_.k.Pi=function(a){fp(this,"x");_.Vn(this.G,"x",this.K,this.F,this.C(),!1,this.D);a.preventDefault();a.stopPropagation()};
_.k.ii=function(a){fp(this,"n");_.Vn(this.G,"n",this.K,this.F,this.C(),!1,this.D);a.preventDefault();a.stopPropagation()};_.k.ui=function(){_.Vn(this.G,"lc",this.K,this.F,this.C(),!1,this.D)};
_.k.Xh=function(a){_.Vn(this.G,"a",this.K,this.F,this.C(),!1,this.D);if(this.A&&11!=gp(this.A.value).length)this.A.pattern&&(this.A.pattern="^\\+?1?[-()\\s]*([0,2-9][-()\\s]*)([\\d][-()\\s]*){9}$",this.A.dispatchEvent(new Event("input"))),a.preventDefault(),a.stopPropagation();else if(this.jc){var c=_.He("window.launchConsentDialog");c?c():this.w.log(Error("ka"));this.close();a.preventDefault();a.stopPropagation()}else this.Id?this.close():fp(this,"a"),this.va&&(a.preventDefault(),a.stopPropagation(),
hp(this))};var hp=function(a){if(a.A&&11!=gp(a.A.value).length)a.ka();else{ip(a,a.Ja);var c=(0,_.t)(a.kd,a),d=(0,_.t)(a.ka,a);_.Vj=new _.vn;_.Uk("//www.google.com/_/og/promos/g?authuser="+a.ze,function(){this.ee()?c(this.Uf()):d()},"POST",jp(a),null,void 0,!0)}},jp=function(a){var c="d2m=igs&g="+a.nc+"&p="+a.N+"&t="+a.Qi;a.A&&(c+="&pn="+gp(a.A.value));a.Ub&&(c+="&s="+a.Ub);return c},ip=function(a,c,d){_.T(c,"gb_Fa");d&&0<d&&setTimeout((0,_.t)(a.ua,a,c),d)};
dp.prototype.ua=function(a){_.U(a,"gb_Fa",!0)};dp.prototype.kd=function(a){var c=new Qo(a.PromoAsyncResponse);a=_.C(c,1);c=_.B(c,2);a&&c&&0!=c.length?(_.ig(this.Xi," "+c+" "),this.ua(this.Ja),ip(this,this.dj,15E3)):this.ka()};dp.prototype.ka=function(){this.ua(this.Ja);ip(this,this.Wi,15E3)};var cp=function(a){a.hc||(_.Vn(a.G,"hc",a.K,a.F,a.C(),!1,a.D),a.hc=!0)},gp=function(a){a=a.replace(/[^0-9]/g,"");a.startsWith("1")||(a="1"+a);return a};
var lp=function(a,c,d,e,f,g,h){So.call(this,a,c,e,f,g,h);this.A=[];d&&$o(new Yo(d,f),[this.F,this.Gd,this.M]);kp(this)};_.w(lp,So);var kp=function(a){_.Ch(a.w,a.f,"mouseover",function(c){c.stopPropagation()})};lp.prototype.J=function(){return"ic="+this.j.Zb()};lp.prototype.S=function(){lp.L.S.call(this);for(var a=0;a<this.A.length;a++)this.A[a]("o")};lp.prototype.close=function(){lp.L.close.call(this);for(var a=0;a<this.A.length;a++)this.A[a]("c")};
var mp={consent:function(){return window.launchConsentDialog}},np=function(a){return _.$d(a,"js:")?null!=mp[a.slice(3)]:!1};
var op=function(a,c,d,e,f,g){lp.call(this,a,_.H(c,Fo,1),_.H(c,Go,3),d,e,f,g);this.ua=_.K(_.xc(c,5,!1));this.G=_.L(_.B(c,2));this.va=_.K(_.xc(c,4,!1))};_.w(op,lp);
op.prototype.K=function(a){op.L.K.call(this,a,this.ua,"string"===typeof this.G?np(this.G):!1);a=this.w;var c=this.G,d=this.va;c&&("function"==typeof c?c.call():"string"==typeof c&&(_.$d(c,"js:")?(c=c.slice(3),d=mp[c],!d&&a?a.log(Error("la`"+c)):(d=d(),!d&&a?a.log(Error("ma`"+c)):d())):d?(a=_.wb(c),_.q.open(_.ub(a))):null!=_.q.location&&_.sm(_.q.location,c)))};
var pp=function(a,c,d,e,f,g){var h=_.M("gb_3c"),l=_.H(a,Io,5);l&&h&&(d.He("up","up",["2","9","6"]),d.register("up",function(m){m&&(m=_.Mc(_.B(a,8)),m=new op(h,l,m,c,f,e),m.A.push(g),m.N||Jo(m.j)?m.N&&!Jo(m.j)&&Vo(m):(To(m,m.F,m.K),To(m,m.Gd,m.ka),To(m,m.M,m.$),m.S(),_.Mn(m.j),Vo(m)))}))};
var qp=function(){_.J.call(this);this.Oa=null};_.p(qp,_.J);
var rp=function(){_.J.call(this)};_.p(rp,_.J);
var sp=function(a,c){_.J.call(this);this.o=c;this.f={};this.A={};this.b=null;this.j=1;this.w=!1;this.B=a;_.u("gbar.up.r",(0,_.t)(this.register,this));_.u("gbar.up.nap",(0,_.t)(this.He,this));_.u("gbar.up.aop",(0,_.t)(this.Tg,this));_.u("gbar.up.tp",(0,_.t)(this.sg,this));_.u("gbar.up.ssp",(0,_.t)(this.rf,this))};_.p(sp,_.J);var tp=function(a,c,d){return-1==(0,_.La)(c,a.j)?(a.o.log(Error("na`"+a.j+"`"+d)),!1):!0};_.k=sp.prototype;
_.k.register=function(a,c){tp(this,[1,2],"r")&&(this.f[a]=this.f[a]||[],this.f[a].push(c),2==this.j&&_.q.setTimeout((0,_.t)(function(){c(this.rf(a))},this),0))};_.k.He=function(a,c,d){if(tp(this,[1],"nap")&&d){for(var e=0;e<d.length;e++)this.A[d[e]]=!0;this.B.log(a,c,"nap","tpt="+d.join(","))}};_.k.Tg=function(a,c,d){if(tp(this,[1],"aop")&&d){if(this.b)for(var e in this.b)this.b[e]=this.b[e]&&-1!=(0,_.La)(d,e);else for(this.b={},e=0;e<d.length;e++)this.b[d[e]]=!0;this.B.log(a,c,"aop","tpt="+d.join(","))}};
_.k.sg=function(){try{if(this.j=2,!this.w){this.w=!0;for(var a in this.f)for(var c=this.f[a],d=0;d<c.length;d++)try{var e=c[d],f=this.rf(a);e.apply(null,[f])}catch(g){this.o.log(g)}}}catch(g){this.o.log(g)}};_.k.rf=function(a){if(tp(this,[2],"ssp")){var c=!this.A[a];this.b&&(c=c&&!!this.b[a]);return c}return!1};
(function(){_.on.log(1);var a=document.querySelector(".gb_5");a&&Ko(a,function(){_.on.log(62);_.He("silk.s.sis.ca")&&_.on.log(106)});a=document.querySelector(".gb_Oa");var c=document.querySelector("#gb.gb_Ac");a&&c&&Ko(a,function(){_.on.log(79)})})();
var up=_.M("gb_xc");if(up){var vp=_.M("gb_lc",up);vp&&new _.Gh(vp,_.yd,_.zd)}
;var Bp=function(){var a=wp,c=xp,d=yp,e=zp,f=Ap;this.o=_.uj;this.f=_.yd;this.j=f;this.b=a;this.F=c;this.G=d;this.D=_.zd;this.w=e},Cp,Dp=function(a){a&&(a=_.Wn.ta(),a.b=!0,a.wb&&a.wb.Y())};
Bp.prototype.A=function(){var a=_.H(this.j,Ho,4);if(a){if(_.C(a,15))this.b.register("7",Dp);else{var c=a&&_.C(a,13)?_.M("gb_6c"):_.M("gb_fd"),d=_.M("gb_Vf");if(!c||!d)return;var e=this.j,f=this.f,g=this.D,h=this.o;this.b.register("7",function(l){l&&(_.$n(h,d),l=_.Mc(_.B(e,8)),new dp(c,a,l,f,g,_.on))})}this.b.He("7","7",["5"])}};Bp.prototype.B=function(){var a=this.o;pp(this.j,this.f,this.b,this.F,this.G,function(){_.ij(a)})};
var Ap=_.H(_.ud,Eo,15);
if(Ap&&_.uj){var Ep=_.L(_.B(_.vd(),10)),Fp=_.Vc.ta(),Gp=_.Mc(_.B(Ap,8)),Hp;Hp=_.yc(Ap,1,1E-4);var Ip=_.Mc(Hp,1E-4),Jp;Jp=_.B(Ap,2);var Kp=_.L(Jp),Lp;Lp=_.B(Ap,3);var Mp=new Mo(_.yd,Ip,Ep,Kp,_.L(Lp),Gp,!1),Np=new No(_.yd);_.Zc("p_log",Mp);_.Zc("p_st",Np);_.Zc("p_tr",new sp(Mp,_.yd));_.Zc("p_mgmhp",new rp(_.yd,Np));_.Zc("p_dse",new qp(_.yd));var wp=_.Wc(Fp,"p_tr"),xp=_.Wc(Fp,"p_st"),yp=_.Wc(Fp,"p_log"),Op,zp=_.Xc("api");Cp||(Cp=new Bp);Op=Cp;var Pp={};Pp.up=Op.B;Pp["7"]=Op.A;for(var Qp in Pp)try{Pp[Qp].apply(Op)}catch(a){Op.f.log(Error(Qp))}Op.w.Cc();
Op.b.sg()}
;
}catch(e){_._DumpException(e)}
try{
var gq,qq,vq,zq,Aq,Cq,Dq;_.eq=function(a,c){return _.Fb(a,c)};_.fq=function(a){if(a instanceof _.Db)return a;var c="object"==typeof a,d=null;c&&a.Se&&(d=a.b());return _.eq(_.he(c&&a.Ob?a.Bb():String(a)),d)};gq=function(a){var c=_.fq(_.Gb),d=c.b(),e=[],f=function(g){_.Ba(g)?(0,_.Ma)(g,f):(g=_.fq(g),e.push(_.Eb(g).toString()),g=g.b(),0==d?d=g:0!=g&&d!=g&&(d=null))};(0,_.Ma)(a,f);return _.eq(e.join(_.Eb(c).toString()),d)};_.hq=function(a){return gq(Array.prototype.slice.call(arguments))};
_.iq=function(a,c){this.x=void 0!==a?a:0;this.b=void 0!==c?c:0};_.iq.prototype.ceil=function(){this.x=Math.ceil(this.x);this.b=Math.ceil(this.b);return this};_.iq.prototype.floor=function(){this.x=Math.floor(this.x);this.b=Math.floor(this.b);return this};_.iq.prototype.round=function(){this.x=Math.round(this.x);this.b=Math.round(this.b);return this};_.jq=function(a){return new _.iq(a.x,a.b)};_.kq=function(a){return a.scrollingElement?a.scrollingElement:!_.Sb&&_.cg(a)?a.documentElement:a.body||a.documentElement};
_.lq=function(a){var c=_.kq(a);a=a.parentWindow||a.defaultView;return _.y&&_.gc("10")&&a.pageYOffset!=c.scrollTop?new _.iq(c.scrollLeft,c.scrollTop):new _.iq(a.pageXOffset||c.scrollLeft,a.pageYOffset||c.scrollTop)};_.mq=function(a,c){var d=_.we(a,"DIV");_.y?(c=_.hq(_.Hb,c),_.ag(d,c),d.removeChild(d.firstChild)):_.ag(d,c);if(1==d.childNodes.length)d=d.removeChild(d.firstChild);else{for(a=a.createDocumentFragment();d.firstChild;)a.appendChild(d.firstChild);d=a}return d};
_.nq=function(a){a=a.b;return a.parentWindow||a.defaultView};_.oq=function(a){return"rtl"==_.Mg(a,"direction")};_.pq=function(a){for(var c in a)return!1;return!0};qq=function(a,c){return new _.iq(a.x-c.x,a.b-c.b)};_.rq=function(a,c,d,e){this.top=a;this.right=c;this.bottom=d;this.left=e};_.k=_.rq.prototype;_.k.getHeight=function(){return this.bottom-this.top};
_.k.expand=function(a,c,d,e){_.Da(a)?(this.top-=a.top,this.right+=a.right,this.bottom+=a.bottom,this.left-=a.left):(this.top-=a,this.right+=Number(c),this.bottom+=Number(d),this.left-=Number(e));return this};_.k.ceil=function(){this.top=Math.ceil(this.top);this.right=Math.ceil(this.right);this.bottom=Math.ceil(this.bottom);this.left=Math.ceil(this.left);return this};
_.k.floor=function(){this.top=Math.floor(this.top);this.right=Math.floor(this.right);this.bottom=Math.floor(this.bottom);this.left=Math.floor(this.left);return this};_.k.round=function(){this.top=Math.round(this.top);this.right=Math.round(this.right);this.bottom=Math.round(this.bottom);this.left=Math.round(this.left);return this};_.sq=function(a,c,d,e){this.left=a;this.top=c;this.width=d;this.height=e};
_.sq.prototype.ceil=function(){this.left=Math.ceil(this.left);this.top=Math.ceil(this.top);this.width=Math.ceil(this.width);this.height=Math.ceil(this.height);return this};_.sq.prototype.floor=function(){this.left=Math.floor(this.left);this.top=Math.floor(this.top);this.width=Math.floor(this.width);this.height=Math.floor(this.height);return this};
_.sq.prototype.round=function(){this.left=Math.round(this.left);this.top=Math.round(this.top);this.width=Math.round(this.width);this.height=Math.round(this.height);return this};_.tq=function(a,c,d){if(c instanceof _.iq){var e=c.x;c=c.b}else e=c,c=d;a.style.left=_.Og(e,!1);a.style.top=_.Og(c,!1)};_.uq=function(a){a=a?_.Ce(a):document;return!_.y||_.ic(9)||_.cg(_.pg(a).b)?a.documentElement:a.body};
vq=function(a){if(_.y&&!_.ic(8))return a.offsetParent;var c=_.Ce(a),d=_.Mg(a,"position"),e="fixed"==d||"absolute"==d;for(a=a.parentNode;a&&a!=c;a=a.parentNode)if(11==a.nodeType&&a.host&&(a=a.host),d=_.Mg(a,"position"),e=e&&"static"==d&&a!=c.documentElement&&a!=c.body,!e&&(a.scrollWidth>a.clientWidth||a.scrollHeight>a.clientHeight||"fixed"==d||"absolute"==d||"relative"==d))return a;return null};
_.wq=function(a){var c=_.Ce(a),d=new _.iq(0,0),e=_.uq(c);if(a==e)return d;a=_.Ng(a);c=_.lq(_.pg(c).b);d.x=a.left+c.x;d.b=a.top+c.b;return d};
_.xq=function(a){for(var c=new _.rq(0,Infinity,Infinity,0),d=_.pg(a),e=d.b.body,f=d.b.documentElement,g=_.kq(d.b);a=vq(a);)if(!(_.y&&0==a.clientWidth||_.Sb&&0==a.clientHeight&&a==e)&&a!=e&&a!=f&&"visible"!=_.Mg(a,"overflow")){var h=_.wq(a),l=new _.iq(a.clientLeft,a.clientTop);h.x+=l.x;h.b+=l.b;c.top=Math.max(c.top,h.b);c.right=Math.min(c.right,h.x+a.clientWidth);c.bottom=Math.min(c.bottom,h.b+a.clientHeight);c.left=Math.max(c.left,h.x)}e=g.scrollLeft;g=g.scrollTop;c.left=Math.max(c.left,e);c.top=
Math.max(c.top,g);d=_.dg(_.nq(d));c.right=Math.min(c.right,e+d.width);c.bottom=Math.min(c.bottom,g+d.height);return 0<=c.top&&0<=c.left&&c.bottom>c.top&&c.right>c.left?c:null};_.yq=function(a){a=_.Ng(a);return new _.iq(a.left,a.top)};_.X=function(a,c){a.style.display=c?"":"none"};zq=function(a,c){if(/^\d+px?$/.test(c))return parseInt(c,10);var d=a.style.left,e=a.runtimeStyle.left;a.runtimeStyle.left=a.currentStyle.left;a.style.left=c;c=a.style.pixelLeft;a.style.left=d;a.runtimeStyle.left=e;return+c};
Aq=function(a,c){return(c=a.currentStyle?a.currentStyle[c]:null)?zq(a,c):0};_.Bq=function(a,c){if(_.y){var d=Aq(a,c+"Left"),e=Aq(a,c+"Right"),f=Aq(a,c+"Top");a=Aq(a,c+"Bottom");return new _.rq(f,e,a,d)}d=_.Lg(a,c+"Left");e=_.Lg(a,c+"Right");f=_.Lg(a,c+"Top");a=_.Lg(a,c+"Bottom");return new _.rq(parseFloat(f),parseFloat(e),parseFloat(a),parseFloat(d))};Cq={thin:2,medium:4,thick:6};
Dq=function(a,c){if("none"==(a.currentStyle?a.currentStyle[c+"Style"]:null))return 0;c=a.currentStyle?a.currentStyle[c+"Width"]:null;return c in Cq?Cq[c]:zq(a,c)};_.Eq=function(a){if(_.y&&!_.ic(9)){var c=Dq(a,"borderLeft"),d=Dq(a,"borderRight"),e=Dq(a,"borderTop");a=Dq(a,"borderBottom");return new _.rq(e,d,a,c)}c=_.Lg(a,"borderLeftWidth");d=_.Lg(a,"borderRightWidth");e=_.Lg(a,"borderTopWidth");a=_.Lg(a,"borderBottomWidth");return new _.rq(parseFloat(e),parseFloat(d),parseFloat(a),parseFloat(c))};
_.Fq=function(a){_.Q.call(this);this.b=a;a=_.y?"focusout":"blur";this.f=_.O(this.b,_.y?"focusin":"focus",this,!_.y);this.j=_.O(this.b,a,this,!_.y)};_.w(_.Fq,_.Q);_.Fq.prototype.handleEvent=function(a){var c=new _.Me(a.ab);c.type="focusin"==a.type||"focus"==a.type?"focusin":"focusout";this.dispatchEvent(c)};_.Fq.prototype.P=function(){_.Fq.L.P.call(this);_.gf(this.f);_.gf(this.j);delete this.b};
var Gq=function(){if(_.Ub){var a=/Windows NT ([0-9.]+)/;return(a=a.exec(_.Ua))?a[1]:"0"}return _.Tb?(a=/10[_.][0-9_.]+/,(a=a.exec(_.Ua))?a[0].replace(/_/g,"."):"10"):_.Wb?(a=/Android\s+([^\);]+)(\)|;)/,(a=a.exec(_.Ua))?a[1]:""):_.Xb||_.Yb||_.Zb?(a=/(?:iPhone|CPU)\s+OS\s+(\S+)/,(a=a.exec(_.Ua))?a[1].replace(/_/g,"."):""):""}();
var Hq=function(a){return(a=a.exec(_.Ua))?a[1]:""},Iq=function(){if(_.kc)return Hq(/Firefox\/([0-9.]+)/);if(_.y||_.Pb||_.Ob)return _.fc;if(_.oc)return _.Kb()?Hq(/CriOS\/([0-9.]+)/):Hq(/Chrome\/([0-9.]+)/);if(_.pc&&!_.Kb())return Hq(/Version\/([0-9.]+)/);if(_.lc||_.mc){var a=/Version\/(\S+).*Mobile\/(\S+)/.exec(_.Ua);if(a)return a[1]+"."+a[2]}else if(_.nc)return(a=Hq(/Android\s+([0-9.]+)/))?a:Hq(/Version\/([0-9.]+)/);return""}();
/*

 Copyright The Closure Library Authors.
 SPDX-License-Identifier: Apache-2.0
*/
var Jq;
_.Lq=function(a,c,d,e,f,g,h,l,m){var n;if(n=d.offsetParent){var r="HTML"==n.tagName||"BODY"==n.tagName;if(!r||"static"!=_.Mg(n,"position")){var v=_.wq(n);if(!r){r=_.oq(n);var N;if(N=r){if(N=_.pc)N=0<=_.Ta(Iq,10);var D;if(D=_.$b)D=0<=_.Ta(Gq,10);N=_.Rb||N||D}r=N?-n.scrollLeft:!r||_.Qb&&_.gc("8")||"visible"==_.Mg(n,"overflowX")?n.scrollLeft:n.scrollWidth-n.clientWidth-n.scrollLeft;v=qq(v,new _.iq(r,n.scrollTop))}}}n=v||new _.iq;v=_.wq(a);r=_.Qg(a);v=new _.sq(v.x,v.b,r.width,r.height);if(r=_.xq(a)){var P=new _.sq(r.left,
r.top,r.right-r.left,r.bottom-r.top);r=Math.max(v.left,P.left);N=Math.min(v.left+v.width,P.left+P.width);r<=N&&(D=Math.max(v.top,P.top),P=Math.min(v.top+v.height,P.top+P.height),D<=P&&(v.left=r,v.top=D,v.width=N-r,v.height=P-D))}r=_.pg(a);D=_.pg(d);if(r.b!=D.b){N=r.b.body;D=_.nq(D);P=new _.iq(0,0);var G=_.eg(_.Ce(N));if(_.Ke(G,"parent")){var fa=N;do{var Hc=G==D?_.wq(fa):_.yq(fa);P.x+=Hc.x;P.b+=Hc.b}while(G&&G!=D&&G!=G.parent&&(fa=G.frameElement)&&(G=G.parent))}N=qq(P,_.wq(N));!_.y||_.ic(9)||_.cg(r.b)||
(N=qq(N,_.lq(r.b)));v.left+=N.x;v.top+=N.b}a=Jq(a,c);c=v.left;a&4?c+=v.width:a&2&&(c+=v.width/2);c=new _.iq(c,v.top+(a&1?v.height:0));c=qq(c,n);f&&(c.x+=(a&4?-1:1)*f.x,c.b+=(a&1?-1:1)*f.b);if(h)if(m)var za=m;else if(za=_.xq(d))za.top-=n.b,za.right-=n.x,za.bottom-=n.b,za.left-=n.x;return _.Kq(c,d,e,g,za,h,l)};
_.Kq=function(a,c,d,e,f,g,h){a=_.jq(a);var l=Jq(c,d);d=_.Qg(c);h=h?_.Ag(h):_.Ag(d);a=_.jq(a);h=_.Ag(h);var m=0;if(e||0!=l)l&4?a.x-=h.width+(e?e.right:0):l&2?a.x-=h.width/2:e&&(a.x+=e.left),l&1?a.b-=h.height+(e?e.bottom:0):e&&(a.b+=e.top);if(g){if(f){e=a;l=h;m=0;65==(g&65)&&(e.x<f.left||e.x>=f.right)&&(g&=-2);132==(g&132)&&(e.b<f.top||e.b>=f.bottom)&&(g&=-5);e.x<f.left&&g&1&&(e.x=f.left,m|=1);if(g&16){var n=e.x;e.x<f.left&&(e.x=f.left,m|=4);e.x+l.width>f.right&&(l.width=Math.min(f.right-e.x,n+l.width-
f.left),l.width=Math.max(l.width,0),m|=4)}e.x+l.width>f.right&&g&1&&(e.x=Math.max(f.right-l.width,f.left),m|=1);g&2&&(m|=(e.x<f.left?16:0)|(e.x+l.width>f.right?32:0));e.b<f.top&&g&4&&(e.b=f.top,m|=2);g&32&&(n=e.b,e.b<f.top&&(e.b=f.top,m|=8),e.b+l.height>f.bottom&&(l.height=Math.min(f.bottom-e.b,n+l.height-f.top),l.height=Math.max(l.height,0),m|=8));e.b+l.height>f.bottom&&g&4&&(e.b=Math.max(f.bottom-l.height,f.top),m|=2);g&8&&(m|=(e.b<f.top?64:0)|(e.b+l.height>f.bottom?128:0));f=m}else f=256;m=f}g=
new _.sq(0,0,0,0);g.left=a.x;g.top=a.b;g.width=h.width;g.height=h.height;f=m;if(f&496)return f;_.tq(c,new _.iq(g.left,g.top));h=new _.pe(g.width,g.height);_.Hg(d,h)||(d=h,h=_.cg(_.pg(_.Ce(c)).b),!_.y||_.gc("10")||h&&_.gc("8")?(c=c.style,_.Rb?c.MozBoxSizing="border-box":_.Sb?c.WebkitBoxSizing="border-box":c.boxSizing="border-box",c.width=Math.max(d.width,0)+"px",c.height=Math.max(d.height,0)+"px"):(a=c.style,h?(h=_.Bq(c,"padding"),c=_.Eq(c),a.pixelWidth=d.width-c.left-h.left-h.right-c.right,a.pixelHeight=
d.height-c.top-h.top-h.bottom-c.bottom):(a.pixelWidth=d.width,a.pixelHeight=d.height)));return f};Jq=function(a,c){return(c&8&&_.oq(a)?c^4:c)&-9};

}catch(e){_._DumpException(e)}
try{
_.Mq=function(a,c){_.Q.call(this);this.b=a;a=_.Be(this.b)?this.b:this.b?this.b.body:null;this.w=!!a&&_.oq(a);this.f=_.O(this.b,_.Rb?"DOMMouseScroll":"mousewheel",this,c)};_.w(_.Mq,_.Q);
_.Mq.prototype.handleEvent=function(a){var c=0,d=0,e=a.ab;"mousewheel"==e.type?(a=Nq(-e.wheelDelta),void 0!==e.wheelDeltaX?(c=Nq(-e.wheelDeltaX),d=Nq(-e.wheelDeltaY)):d=a):(a=e.detail,100<a?a=3:-100>a&&(a=-3),void 0!==e.axis&&e.axis===e.HORIZONTAL_AXIS?c=a:d=a);"number"===typeof this.j&&(c=Math.min(Math.max(c,-this.j),this.j));"number"===typeof this.o&&(d=Math.min(Math.max(d,-this.o),this.o));this.w&&(c=-c);c=new Oq(a,e,c,d);this.dispatchEvent(c)};
var Nq=function(a){return _.Sb&&(_.Tb||_.Vb)&&0!=a%40?a:a/40};_.Mq.prototype.P=function(){_.Mq.L.P.call(this);_.gf(this.f);this.f=null};var Oq=function(a,c,d,e){_.Me.call(this,c);this.type="mousewheel";this.detail=a;this.deltaX=d;this.deltaY=e};_.w(Oq,_.Me);
/*

 Copyright The Closure Library Authors.
 SPDX-License-Identifier: Apache-2.0
*/
_.Qq=function(a,c,d){_.Q.call(this);this.target=a;this.D=c||a;this.w=d||new _.sq(NaN,NaN,NaN,NaN);this.j=_.Ce(a);this.b=new _.vg(this);_.Yf(this,this.b);this.deltaY=this.deltaX=this.K=this.J=this.screenY=this.screenX=this.clientY=this.clientX=0;this.f=!1;_.O(this.D,["touchstart","mousedown"],this.B,!1,this);this.A=Pq};_.w(_.Qq,_.Q);var Pq=_.q.document&&_.q.document.documentElement&&!!_.q.document.documentElement.setCapture&&!!_.q.document.releaseCapture;
_.Qq.prototype.P=function(){_.Qq.L.P.call(this);_.ff(this.D,["touchstart","mousedown"],this.B,!1,this);_.zg(this.b);this.A&&this.j.releaseCapture();this.D=this.target=null};
_.Qq.prototype.B=function(a){var c="mousedown"==a.type;if(this.f||c&&!_.ug(a))this.dispatchEvent("earlycancel");else if(this.dispatchEvent(new Rq("start",this,a.clientX,a.clientY,a))){this.f=!0;c&&a.preventDefault();c=this.j;var d=c.documentElement,e=!this.A;this.b.H(c,["touchmove","mousemove"],this.O,{capture:e,passive:!1});this.b.H(c,["touchend","mouseup"],this.o,e);this.A?(d.setCapture(!1),this.b.H(d,"losecapture",this.o)):this.b.H(_.eg(c),"blur",this.o);this.F&&this.b.H(this.F,"scroll",this.M,
e);this.clientX=this.J=a.clientX;this.clientY=this.K=a.clientY;this.screenX=a.screenX;this.screenY=a.screenY;this.deltaX=this.target.offsetLeft;this.deltaY=this.target.offsetTop;this.G=_.lq(_.pg(this.j).b)}};_.Qq.prototype.o=function(a,c){_.zg(this.b);this.A&&this.j.releaseCapture();this.f?(this.f=!1,this.dispatchEvent(new Rq("end",this,a.clientX,a.clientY,a,Sq(this,this.deltaX),Tq(this,this.deltaY),c||"touchcancel"==a.type))):this.dispatchEvent("earlycancel")};
_.Qq.prototype.O=function(a){var c=a.clientX-this.clientX,d=a.clientY-this.clientY;this.clientX=a.clientX;this.clientY=a.clientY;this.screenX=a.screenX;this.screenY=a.screenY;if(!this.f){var e=this.J-this.clientX,f=this.K-this.clientY;if(0<e*e+f*f)if(this.dispatchEvent(new Rq("start",this,a.clientX,a.clientY,a)))this.f=!0;else{this.Sa||this.o(a);return}}d=Uq(this,c,d);c=d.x;d=d.b;this.f&&this.dispatchEvent(new Rq("beforedrag",this,a.clientX,a.clientY,a,c,d))&&(Vq(this,a,c,d),a.preventDefault())};
var Uq=function(a,c,d){var e=_.lq(_.pg(a.j).b);c+=e.x-a.G.x;d+=e.b-a.G.b;a.G=e;a.deltaX+=c;a.deltaY+=d;return new _.iq(Sq(a,a.deltaX),Tq(a,a.deltaY))};_.Qq.prototype.M=function(a){var c=Uq(this,0,0);a.clientX=this.clientX;a.clientY=this.clientY;Vq(this,a,c.x,c.b)};
var Vq=function(a,c,d,e){a.target.style.left=d+"px";a.target.style.top=e+"px";a.dispatchEvent(new Rq("drag",a,c.clientX,c.clientY,c,d,e))},Sq=function(a,c){var d=a.w;a=isNaN(d.left)?null:d.left;d=isNaN(d.width)?0:d.width;return Math.min(null!=a?a+d:Infinity,Math.max(null!=a?a:-Infinity,c))},Tq=function(a,c){var d=a.w;a=isNaN(d.top)?null:d.top;d=isNaN(d.height)?0:d.height;return Math.min(null!=a?a+d:Infinity,Math.max(null!=a?a:-Infinity,c))},Rq=function(a,c,d,e,f,g,h,l){_.Le.call(this,a);this.clientX=
d;this.clientY=e;this.o=f;this.left=void 0!==g?g:c.deltaX;this.top=void 0!==h?h:c.deltaY;this.j=!!l};_.w(Rq,_.Le);

}catch(e){_._DumpException(e)}
try{
var mr=function(a,c){_.Q.call(this);this.j=new _.vg(this);this.se(a||null);c&&(this.Vc=c)};_.w(mr,_.Q);_.k=mr.prototype;_.k.vb=null;_.k.zf=null;_.k.Xc=!1;_.k.$e=-1;_.k.Vc="toggle_display";_.k.C=function(){return this.vb};_.k.se=function(a){if(this.Xc)throw Error("pa");this.vb=a};_.k.isVisible=function(){return this.Xc};
_.k.ha=function(a){this.M&&this.M.stop();this.F&&this.F.stop();if(a){if(!this.Xc&&this.hf()){if(!this.vb)throw Error("qa");this.xd();a=_.Ce(this.vb);this.j.H(a,"mousedown",this.yg,!0);if(_.y){try{var c=a.activeElement}catch(e){}for(;c&&"IFRAME"==c.nodeName;){try{var d=_.ak(c)}catch(e){break}a=d;c=a.activeElement}this.j.H(a,"mousedown",this.yg,!0);this.j.H(a,"deactivate",this.xg)}else this.j.H(a,"blur",this.xg);"toggle_display"==this.Vc?(this.vb.style.visibility="visible",_.X(this.vb,!0)):"move_offscreen"==
this.Vc&&this.xd();this.Xc=!0;this.$e=(0,_.Ha)();this.M?(_.Ze(this.M,"end",this.ag,!1,this),this.M.play()):this.ag()}}else nr(this)};_.k.xd=_.xa;var nr=function(a,c){a.Xc&&a.dispatchEvent({type:"beforehide",target:c})&&(a.j&&_.zg(a.j),a.Xc=!1,(0,_.Ha)(),a.F?(_.Ze(a.F,"end",_.Sd(a.Df,c),!1,a),a.F.play()):a.Df(c))};_.k=mr.prototype;_.k.Df=function(a){"toggle_display"==this.Vc?this.Ti():"move_offscreen"==this.Vc&&(this.vb.style.top="-10000px");this.Me(a)};
_.k.Ti=function(){this.vb.style.visibility="hidden";_.X(this.vb,!1)};_.k.hf=function(){return this.dispatchEvent("beforeshow")};_.k.ag=function(){this.dispatchEvent("show")};_.k.Me=function(a){this.dispatchEvent({type:"hide",target:a})};_.k.yg=function(a){a=a.target;_.hg(this.vb,a)||or(this,a)||150>(0,_.Ha)()-this.$e||nr(this,a)};
_.k.xg=function(a){var c=_.Ce(this.vb);if("undefined"!=typeof document.activeElement){if(a=c.activeElement,!a||_.hg(this.vb,a)||"BODY"==a.tagName||or(this,a))return}else if(a.target!=c)return;150>(0,_.Ha)()-this.$e||nr(this)};var or=function(a,c){return(0,_.Pa)(a.zf||[],function(d){return c===d||_.hg(d,c)})};mr.prototype.P=function(){mr.L.P.call(this);this.j.sa();_.Xf(this.M);_.Xf(this.F);delete this.vb;delete this.j;delete this.zf};
/*

 Copyright The Closure Library Authors.
 SPDX-License-Identifier: Apache-2.0
*/
var pr=function(){};pr.prototype.b=function(){};
var qr=function(a,c){this.$=8;this.T=c||void 0;mr.call(this,a)};_.w(qr,mr);qr.prototype.xd=function(){if(this.T){var a=!this.isVisible()&&"move_offscreen"!=this.Vc,c=this.C();a&&(c.style.visibility="hidden",_.X(c,!0));this.T.b(c,this.$,this.ua);a&&_.X(c,!1)}};
var rr=function(a,c,d){this.f=a;this.j=c;this.o=d};_.w(rr,pr);rr.prototype.b=function(a,c,d){_.Lq(this.f,this.j,a,c,void 0,d,this.o)};
var sr=function(a,c){this.f=a instanceof _.iq?a:new _.iq(a,c)};_.w(sr,pr);sr.prototype.b=function(a,c,d){_.Lq(_.uq(a),0,a,c,this.f,d,null,void 0)};
var tr=function(){this.b=new _.bk},ur=function(a){var c=typeof a;return"object"==c&&a||"function"==c?"o"+_.Cg(a):c.charAt(0)+a};_.k=tr.prototype;_.k.add=function(a){this.b.set(ur(a),a)};_.k.remove=function(a){return this.b.remove(ur(a))};_.k.clear=function(){this.b.clear()};_.k.vc=function(){return this.b.vc()};_.k.Pa=function(){return this.b.Pa()};
var vr=function(a,c,d){this.D=d||(a?_.pg(_.bg(document,a)):_.pg());qr.call(this,this.D.wa("DIV",{style:"position:absolute;display:none;"}));this.N=new _.iq(1,1);this.A=new tr;this.w=null;a&&(a=_.bg(document,a),this.A.add(a),_.O(a,"mouseover",this.X,!1,this),_.O(a,"mouseout",this.J,!1,this),_.O(a,"mousemove",this.V,!1,this),_.O(a,"focus",this.S,!1,this),_.O(a,"blur",this.J,!1,this));null!=c&&_.ig(this.C(),c)};_.w(vr,qr);var wr=[];vr.prototype.f=null;vr.prototype.className="gb_Aa-gb_Re";
vr.prototype.se=function(a){var c=this.C();c&&_.Ae(c);vr.L.se.call(this,a);a?(c=this.D.b.body,c.insertBefore(a,c.lastChild),_.Xf(this.w),this.w=new _.Fq(this.C()),_.Yf(this,this.w),_.O(this.w,"focusin",this.B,void 0,this),_.O(this.w,"focusout",this.O,void 0,this)):(_.Xf(this.w),this.w=null)};var xr=function(a){return a.o?a.isVisible()?4:1:a.G?3:a.isVisible()?2:0};
vr.prototype.hf=function(){if(!mr.prototype.hf.call(this))return!1;if(this.b)for(var a,c=0;a=wr[c];c++)_.hg(a.C(),this.b)||a.ha(!1);_.Qa(wr,this)||wr.push(this);a=this.C();a.className=this.className;this.B();_.O(a,"mouseover",this.ma,!1,this);_.O(a,"mouseout",this.Y,!1,this);yr(this);return!0};
vr.prototype.Me=function(){_.Ie(wr,this);for(var a=this.C(),c,d=0;c=wr[d];d++)c.b&&_.hg(a,c.b)&&c.ha(!1);this.Z&&this.Z.O();_.ff(a,"mouseover",this.ma,!1,this);_.ff(a,"mouseout",this.Y,!1,this);this.b=void 0;0==xr(this)&&(this.K=!1);mr.prototype.Me.call(this)};vr.prototype.W=function(a,c){this.b==a&&_.ek(this.A.b,ur(this.b))&&(this.K||!this.va?(this.ha(!1),this.isVisible()||(this.b=a,this.T=c||this.R(0)||void 0,this.isVisible()&&this.xd(),this.ha(!0))):this.b=void 0);this.o=void 0};
vr.prototype.ka=function(a){this.G=void 0;if(a==this.b){a=this.D;var c;a=(c=_.ng(a.b))&&this.C()&&a.Wf(this.C(),c);null!=this.f&&(this.f==this.C()||_.ek(this.A.b,ur(this.f)))||a||this.U&&this.U.f||this.ha(!1)}};var zr=function(a,c){var d=_.lq(a.D.b);a.N.x=c.clientX+d.x;a.N.b=c.clientY+d.b};vr.prototype.X=function(a){var c=Ar(this,a.target);this.f=c;this.B();c!=this.b&&(this.b=c,this.o||(this.o=_.rg((0,_.t)(this.W,this,c,void 0),500)),Br(this),zr(this,a))};
var Ar=function(a,c){try{for(;c&&!_.ek(a.A.b,ur(c));)c=c.parentNode;return c}catch(d){return null}};vr.prototype.V=function(a){zr(this,a);this.K=!0};vr.prototype.S=function(a){this.f=a=Ar(this,a.target);this.K=!0;if(this.b!=a){this.b=a;var c=this.R(1);this.B();this.o||(this.o=_.rg((0,_.t)(this.W,this,a,c),500));Br(this)}};vr.prototype.R=function(a){return 0==a?new Cr(_.jq(this.N)):new Dr(this.f)};var Br=function(a){if(a.b)for(var c,d=0;c=wr[d];d++)_.hg(c.C(),a.b)&&(c.U=a,a.Z=c)};
vr.prototype.J=function(a){var c=Ar(this,a.target),d=Ar(this,a.relatedTarget);c!=d&&(c==this.f&&(this.f=null),yr(this),this.K=!1,!this.isVisible()||a.relatedTarget&&_.hg(this.C(),a.relatedTarget)?this.b=void 0:this.O())};vr.prototype.ma=function(){var a=this.C();this.f!=a&&(this.B(),this.f=a)};vr.prototype.Y=function(a){var c=this.C();this.f!=c||a.relatedTarget&&_.hg(c,a.relatedTarget)||(this.f=null,this.O())};var yr=function(a){a.o&&(_.sg(a.o),a.o=void 0)};
vr.prototype.O=function(){2==xr(this)&&(this.G=_.rg((0,_.t)(this.ka,this,this.b),0))};vr.prototype.B=function(){this.G&&(_.sg(this.G),this.G=void 0)};vr.prototype.P=function(){var a;this.ha(!1);yr(this);for(var c=this.A.Pa(),d=0;a=c[d];d++)_.ff(a,"mouseover",this.X,!1,this),_.ff(a,"mouseout",this.J,!1,this),_.ff(a,"mousemove",this.V,!1,this),_.ff(a,"focus",this.S,!1,this),_.ff(a,"blur",this.J,!1,this);this.A.clear();this.C()&&_.Ae(this.C());this.f=null;delete this.D;vr.L.P.call(this)};
var Cr=function(a,c){sr.call(this,a,c)};_.w(Cr,sr);Cr.prototype.b=function(a,c,d){c=_.uq(a);c=_.xq(c);d=d?new _.rq(d.top+10,d.right,d.bottom,d.left+10):new _.rq(10,0,0,10);_.Kq(this.f,a,8,d,c,9)&496&&_.Kq(this.f,a,8,d,c,5)};var Dr=function(a){rr.call(this,a,5)};_.w(Dr,rr);Dr.prototype.b=function(a,c,d){var e=new _.iq(10,0);_.Lq(this.f,this.j,a,c,e,d,9)&496&&_.Lq(this.f,4,a,1,e,d,5)};
_.Er=function(a,c){vr.call(this,a);this.className="gb_Re";this.se(c);this.$=2;this.isVisible()&&this.xd()};_.p(_.Er,vr);_.Er.prototype.R=function(){return new Fr(this.f)};_.Er.prototype.ha=function(a){a||yr(this);return vr.prototype.ha.call(this,a)};var Fr=function(a){rr.call(this,a,3)};_.p(Fr,rr);Fr.prototype.b=function(a,c,d){var e=new _.iq(0,0),f=_.dg();_.Lq(this.f,this.j,a,c,e,d,9,void 0,new _.rq(0,f.width-8,f.height,8))&496&&_.Lq(this.f,4,a,1,e,d,5)};

}catch(e){_._DumpException(e)}
try{
var Tt=/^([^?#]*)(\?[^#]*)?(#[\s\S]*)?/,Ut=function(a,c,d){if(null==d)return c;if("string"===typeof d)return d?a+encodeURIComponent(d):"";for(var e in d){var f=d[e];f=_.Ba(f)?f:[f];for(var g=0;g<f.length;g++){var h=f[g];null!=h&&(c||(c=a),c+=(c.length>a.length?"&":"")+encodeURIComponent(e)+"="+encodeURIComponent(String(h)))}}return c},Vt=function(a,c){a=_.Ud(a);a=Tt.exec(a);var d=a[3]||"";return _.qb(a[1]+Ut("?",a[2]||"",c)+Ut("#",d,void 0))},Wt=function(a){_.A(this,a,0,-1,null,null)};_.w(Wt,_.z);
var Xt=function(a,c){a=a.style;"opacity"in a?a.opacity=c:"MozOpacity"in a?a.MozOpacity=c:"filter"in a&&(a.filter=""===c?"":"alpha(opacity="+100*Number(c)+")")},Yt=function(a){for(var c="string"===typeof a?a.split(""):a,d=a.length-1;0<=d;d--)if(d in c&&_.lf.call(void 0,c[d],d,a))return d;return-1},Zt=function(a,c){var d={},e;for(e in a)c.call(void 0,a[e],e,a)&&(d[e]=a[e]);return d},$t=function(a){var c={},d;for(d in a)c[d]=a[d];return c},au=function(a,c){this.key=a;this.value=c;this.b=void 0},bu=function(a){this.f=
a;this.b={};this.j=!0;if(0<this.f.length){for(a=0;a<this.f.length;a++){var c=this.f[a],d=c[0];this.b[d.toString()]=new au(d,c[1])}this.j=!0}};_.k=bu.prototype;_.k.sb=function(){var a;if(!this.j){this.f.length=0;var c=cu(this);c.sort();for(var d=0;d<c.length;d++){var e=this.b[c[d]];(a=e.b)&&a.sb();this.f.push([e.key,e.value])}this.j=!0}return this.f};_.k.clear=function(){this.b={};this.j=!1};
_.k.entries=function(){var a=[],c=cu(this);c.sort();for(var d=0;d<c.length;d++){var e=this.b[c[d]];a.push([e.key,e.value])}return new _.sc(a)};_.k.keys=function(){var a=[],c=cu(this);c.sort();for(var d=0;d<c.length;d++)a.push(this.b[c[d]].key);return new _.sc(a)};_.k.values=function(){var a=[],c=cu(this);c.sort();for(var d=0;d<c.length;d++)a.push(this.b[c[d]].value);return new _.sc(a)};
_.k.forEach=function(a,c){var d=cu(this);d.sort();for(var e=0;e<d.length;e++){var f=this.b[d[e]];a.call(c,f.value,f.key,this)}};_.k.set=function(a,c){var d=new au(a);d.value=c;this.b[a.toString()]=d;this.j=!1;return this};_.k.get=function(a){if(a=this.b[a.toString()])return a.value};_.k.has=function(a){return a.toString()in this.b};
var cu=function(a){a=a.b;var c=[],d;for(d in a)Object.prototype.hasOwnProperty.call(a,d)&&c.push(d);return c},du=function(a,c,d,e){d!==e?_.F(a,c,d):a.j[c+a.w]=null;return a},Y=function(a,c,d){return du(a,c,d,0)},fu=function(a,c){var d=eu[0];a.b||(a.b={});var e=c?c.sb():c;a.b[3]=c;(c=_.wc(a,d))&&3!==c&&void 0!==e&&(a.b&&c in a.b&&(a.b[c]=void 0),_.F(a,c,void 0));return _.F(a,3,e)},gu=function(a,c,d,e,f){_.Yj(a,e,c);var g=a.b[c];g||(g=a.b[c]=[]);d=d?d:new e;a=_.B(a,c);void 0!=f?(g.splice(f,0,d),a.splice(f,
0,d.sb())):(g.push(d),a.push(d.sb()));return d},hu=function(a){_.A(this,a,0,-1,null,null)};_.w(hu,_.z);
var iu=function(a,c){return _.F(a,4,c)},ju=function(a,c){_.xe(_.Ce(a),a,arguments,1)},ku=function(a,c,d){this.b=a;this.j=c;this.f=d},lu=function(a,c,d){_.Sf(a,c,d,null)||_.Df(_.Sd(c,a))},mu=function(){var a,c,d=new _.Gf(function(e,f){a=e;c=f});return new ku(d,a,c)},nu=function(a){return new _.Gf(function(c,d){var e=a.length,f=[];if(e)for(var g=function(n){c(n)},h=function(n,r){e--;f[n]=r;0==e&&d(f)},l=0,m;l<a.length;l++)m=a[l],lu(m,g,_.Sd(h,l));else c(void 0)})},ou=function(){var a=Error("Ca");return new _.Gf(function(c,
d){d(a)})},pu=function(a){if(a instanceof _.Gf)return a;var c=new _.Gf(_.xa);_.Ff(c,2,a);return c},qu=function(){var a=null;return _.Lf(new _.Gf(function(c,d){a=_.rg(function(){c(void 0)},5E3);-1==a&&d(Error("r"))}),function(c){_.sg(a);throw c;})},ru={'"':'\\"',"\\":"\\\\","/":"\\/","\b":"\\b","\f":"\\f","\n":"\\n","\r":"\\r","\t":"\\t","\x0B":"\\u000b"},su=function(){},tu=function(a,c,d){if(null==c)d.push("null");else{if("object"==typeof c){if(_.Ba(c)){var e=c;c=e.length;d.push("[");for(var f="",
g=0;g<c;g++)d.push(f),tu(a,e[g],d),f=",";d.push("]");return}if(c instanceof String||c instanceof Number||c instanceof Boolean)c=c.valueOf();else{d.push("{");f="";for(e in c)Object.prototype.hasOwnProperty.call(c,e)&&(g=c[e],"function"!=typeof g&&(d.push(f),uu(e,d),d.push(":"),tu(a,g,d),f=","));d.push("}");return}}switch(typeof c){case "string":uu(c,d);break;case "number":d.push(isFinite(c)&&!isNaN(c)?String(c):"null");break;case "boolean":d.push(String(c));break;case "function":d.push("null");break;
default:throw Error("W`"+typeof c);}}},uu=function(a,c){c.push('"',a.replace(_.Pk,function(d){var e=ru[d];e||(e="\\u"+(d.charCodeAt(0)|65536).toString(16).substr(1),ru[d]=e);return e}),'"')},vu=function(a){var c=[];tu(new su,a,c);return c.join("")},wu=function(a){_.A(this,a,0,-1,null,null)};_.w(wu,_.z);
var xu=function(a){_.A(this,a,0,-1,null,null)};_.w(xu,_.z);
var yu=function(a){_.A(this,a,0,-1,null,null)};_.w(yu,_.z);yu.prototype.getOrigin=function(){return _.E(this,1,"")};
var zu=function(a){_.A(this,a,0,-1,null,null)};_.w(zu,_.z);
var Au=function(a){_.A(this,a,0,-1,null,null)};_.w(Au,_.z);
var Bu=function(a){_.A(this,a,0,-1,null,null)};_.w(Bu,_.z);Bu.prototype.getHeight=function(){return _.E(this,2,0)};
var Cu=function(a){_.A(this,a,0,-1,null,null)};_.w(Cu,_.z);
var Eu=function(a){_.A(this,a,0,-1,Du,null)};_.w(Eu,_.z);var Du=[1,2];
var Fu=function(a){_.A(this,a,0,-1,null,null)};_.w(Fu,_.z);
var Gu=function(a){_.A(this,a,0,-1,null,null)};_.w(Gu,_.z);
var Hu=function(a){_.A(this,a,0,-1,null,null)};_.w(Hu,_.z);var Ju=function(a){_.A(this,a,0,-1,Iu,null)};_.w(Ju,_.z);var Iu=[5,10,22],Ku=function(a){return _.H(a,Au,1)},Lu=function(a){return _.E(a,3,"")},Mu=function(a){return _.Zj(a,Bu,10)};
var Nu=function(a){_.A(this,a,0,-1,null,null)};_.w(Nu,_.z);Nu.prototype.getHeight=function(){return _.E(this,2,0)};
var Pu=function(a){_.A(this,a,0,-1,Ou,null)};_.w(Pu,_.z);var Ou=[1,2,3,4],Z=function(a,c){_.Zm(a,1,c)};
var Qu=function(a){_.A(this,a,0,-1,null,null)};_.w(Qu,_.z);
var Ru=function(a){_.A(this,a,0,-1,null,eu)};_.w(Ru,_.z);var eu=[[2,3,4]],Su=function(a){var c=new Ru;return Y(c,1,a)};
var Tu=function(a){_.A(this,a,0,-1,null,null)};_.w(Tu,_.z);
var Vu=function(a){_.A(this,a,0,-1,Uu,null)};_.w(Vu,_.z);var Uu=[18,28],Wu=function(){var a=new Vu;return Y(a,23,20)},Xu=function(a,c){return du(a,8,c,"")};Vu.prototype.setTitle=function(a){return du(this,9,a,"")};var Yu=function(a){var c=new yu;var d=window.location.origin;d||(d=_.ym(_.xm(new _.wm,window.location.protocol),window.location.host).toString());c=du(c,1,d,"");c=Y(c,3,2);return _.I(a,20,c)};
var $u=function(a){_.A(this,a,0,-1,Zu,null)};_.w($u,_.z);var Zu=[2];$u.prototype.Nb=function(){return _.E(this,1,0)};
var av=function(a){_.A(this,a,0,-1,null,null)};_.w(av,_.z);
var bv=function(a){_.A(this,a,0,-1,null,null)};_.w(bv,_.z);
var dv=function(a){_.A(this,a,0,-1,cv,null)};_.w(dv,_.z);var cv=[1,3];
var ev=function(a){_.A(this,a,0,-1,null,null)};_.w(ev,_.z);
var fv=function(a){_.A(this,a,0,-1,null,null)};_.w(fv,_.z);
var gv=function(a){_.A(this,a,0,-1,null,null)};_.w(gv,_.z);
var iv=function(a){_.A(this,a,0,-1,hv,null)};_.w(iv,_.z);var hv=[8];
var kv=function(a){_.A(this,a,0,-1,jv,null)};_.w(kv,_.z);var jv=[14],lv=function(a,c){return du(a,8,c,"")};
var nv=function(a){_.A(this,a,0,-1,mv,null)};_.w(nv,_.z);var mv=[1],ov=function(a,c){gu(a,1,c,kv,void 0)};
var qv=function(a){_.A(this,a,0,-1,pv,null)};_.w(qv,_.z);var pv=[3,7];qv.prototype.ha=function(a){return du(this,5,a,!1)};
var sv=function(a){_.A(this,a,0,-1,rv,null)};_.w(sv,_.z);var rv=[4];
var uv=function(a){_.A(this,a,"ireq",-1,tv,null)};_.w(uv,_.z);var tv=[2],vv=function(a){var c=new uv;return _.I(c,1,a)},wv=function(a,c){return _.tk(a,2,c)};
var xv=function(a){_.A(this,a,"gaia.l.a",-1,null,null)};_.w(xv,_.z);xv.prototype.Zc=function(a){return _.F(this,5,a)};
var zv=function(a){_.A(this,a,"gaia.l.a.r",-1,yv,null)};_.w(zv,_.z);var yv=[1];zv.prototype.B=function(a,c){return gu(this,1,a,xv,c)};
var Av=function(a){this.b=a};Av.prototype.value=function(){return this.b};Av.prototype.getHeight=function(){return this.b.height};
var Bv=function(){this.b={}};Bv.prototype.value=function(){return this.b};
var Cv=function(a){this.o=a;this.f={}};Cv.prototype.b=function(a,c){var d=this.f.data||{};d[a]=c;this.f.data=d;return this};Cv.prototype.sb=function(){var a=Zt(this.f,function(d){return null!==d});a=_.pq(a)?null:a;a=[this.o,this.j,a];var c=Yt(a);return a=a.slice(0,c+1)};Cv.prototype.toString=function(){var a=this.sb();return"("+(0,_.Oa)(a,function(c){return vu(c)}).join(",")+")"};
var Dv=function(){Cv.call(this,"image-search")};_.w(Dv,Cv);Dv.prototype.b=function(a,c){Dv.L.b.call(this,a,c);return this};
var Ev=function(){Cv.call(this,"maps")};_.w(Ev,Cv);Ev.prototype.b=function(a,c){Ev.L.b.call(this,a,c);return this};
var Fv=function(){Cv.call(this,"photos")};_.w(Fv,Cv);Fv.prototype.b=function(a,c){Fv.L.b.call(this,a,c);return this};
var Gv=function(){Cv.call(this,"url")};_.w(Gv,Cv);Gv.prototype.b=function(a,c){Gv.L.b.call(this,a,c);return this};
var Hv=function(){Cv.call(this,"video-search")};_.w(Hv,Cv);Hv.prototype.b=function(a,c){Hv.L.b.call(this,a,c);return this};
var Iv=function(){Cv.call(this,"web")};_.w(Iv,Cv);Iv.prototype.b=function(a,c){Iv.L.b.call(this,a,c);return this};
var Jv=function(){this.b=[]},Kv=function(a){switch(a){case "image-search":return new Dv;case "maps":return new Ev;case "photos":return new Fv;case "url":return new Gv;case "video-search":return new Hv;case "web":return new Iv}return new Cv(a)},Lv=function(a){return"("+(0,_.Oa)(a.b,function(c){return c.toString()}).join(",")+")"};Jv.prototype.toString=function(){return Lv(this)};var Mv=function(a,c){c=void 0===c?[]:c;a.b.forEach(function(d){d instanceof Jv?Mv(d,c):c.push(d)});return c};
var Nv=function(a){this.w=a||"https://docs.google.com/picker";this.f=new Jv};Nv.prototype.f=null;Nv.prototype.j=null;var Ov=function(a,c){a.f.b.push("string"===typeof c?Kv(c):c);return a};
var Pv=function(a){this.action=a;this.wfv=!1};
var Yv=function(a,c){switch(_.E(Ku(a[0]),2,0)){case 13:return Qv(a,c);case 3:return Rv(a,c);case 10:return Sv(a,c,"upload");case 12:return Tv(a,c);case 2:return Uv(a,c);case 5:return Vv(a,c);case 9:return Wv(a,c);case 1:return null!=_.H(a[0],Cu,26)?Xv(a,c):Sv(a,c,"webcam");default:return{}}},Uv=function(a,c){a=a.map(function(d){return{id:_.E(Ku(d),1,""),serviceId:"docs",mimeType:_.E(d,7,""),name:_.E(d,2,""),type:_.E(d,6,0),lastEditedUtc:_.H(d,xu,12),url:_.E(d,8,""),sizeBytes:_.E(d,23,0),description:Lu(d),
iconUrl:_.E(d,11,""),thumbnails:Zv(Mu(d)),isShared:_.xc(_.H(d,Hu,21),1,!1),downloadUrl:_.E(_.H(d,Hu,21),10,""),embedUrl:_.E(d,13,""),copyable:_.xc(_.H(d,Hu,21),9,!1)}});return{action:c,docs:a,viewToken:$v("all","",{}),view:"all"}},Vv=function(a,c){a=a.map(function(d){var e=_.H(_.H(d,Gu,15),Bu,1);gu(d,10,e,Bu,void 0);return{id:_.E(Ku(d),1,""),serviceId:"web",mimeType:_.E(d,7,""),name:_.E(d,2,""),type:_.E(d,6,0),url:_.E(d,8,""),description:Lu(d),iconUrl:"https://ssl.gstatic.com/docs/doclist/images/icon_10_generic_list.png",
thumbnails:Zv(Mu(d))}});return{action:c,docs:a,viewToken:$v("image-search","Search",{}),view:"image-search"}},Wv=function(a,c){a=a.map(function(d){return{serviceId:"url",name:_.E(Mu(d)[0],1,"").split("/").pop(),type:_.E(d,6,0),mimeType:_.E(d,7,""),url:_.E(d,8,""),description:Lu(d),iconUrl:"https://ssl.gstatic.com/docs/doclist/images/icon_10_generic_list.png",thumbnails:Zv(Mu(d))}});return{action:c,docs:a,viewToken:$v("url","By URL",{}),view:"url"}},Xv=function(a,c){a=a.map(function(d){return{id:_.E(Ku(d),
1,""),serviceId:"picasa",name:_.E(d,2,""),type:_.E(d,6,0),description:Lu(d),iconUrl:"https://ssl.gstatic.com/docs/doclist/images/icon_10_generic_list.png",thumbnails:Zv(Mu(d))}});return{action:c,docs:a,viewToken:$v("webcam","",{}),view:"webcam"}},Sv=function(a,c,d){var e=a.map(function(f){return{id:_.E(Ku(f),1,""),serviceId:"photo",mimeType:_.E(f,7,""),name:_.E(f,2,""),type:_.E(f,6,0),sizeBytes:_.E(f,23,0),description:Lu(f),iconUrl:"https://ssl.gstatic.com/docs/doclist/images/icon_10_generic_list.png",
thumbnails:Zv(Mu(f))}});a=new Set(a.map(function(f){return _.E(f,6,0)}));a={allowedItemTypes:Array.from(a)};return{action:c,docs:e,viewToken:$v(d,"",a),view:d}},Rv=function(a,c){var d=a.map(function(e){return{id:_.E(Ku(e),1,""),serviceId:"picasa",mimeType:_.E(e,7,""),name:_.E(Mu(e)[0],1,"").split("/").pop(),type:_.E(e,6,0),lastEditedUtc:_.H(e,xu,12),url:_.E(e,8,""),sizeBytes:_.E(e,23,0),description:Lu(e),iconUrl:"https://ssl.gstatic.com/docs/doclist/images/icon_10_generic_list.png",thumbnails:Zv(Mu(e))}});
a=new Set(a.map(function(e){return _.E(e,6,0)}));a={allowedItemTypes:Array.from(a)};return{action:c,docs:d,viewToken:$v("photos","",a),view:"photos"}},Qv=function(a,c){var d=a.map(function(f){return{id:_.E(Ku(f),1,""),serviceId:"et",name:_.E(Mu(f)[0],1,"").split("/").pop(),description:Lu(f),type:"et",iconUrl:"https://ssl.gstatic.com/docs/doclist/images/icon_10_generic_list.png",thumbnails:Zv(Mu(f),"etjpg")}}),e={category:_.E(_.H(a[0],Fu,28),1,0)};a=$v("et",_.E(_.H(a[0],Fu,28),2,""),e);return{action:c,
docs:d,viewToken:a,view:"et"}},Tv=function(a,c){a=a.map(function(d){var e=_.B(_.H(d,Eu,27),1)[0];return{id:_.E(Ku(d),1,""),serviceId:"contacts",mimeType:_.E(d,7,""),name:_.E(d,2,""),description:Lu(d),url:"mailto:"+e,thumbnail:[{url:_.E(d,11,"")}],email:e}});return{action:c,docs:a,view:"contacts"}},$v=function(a,c,d){return{0:a,1:c,2:d}},Zv=function(a,c){c=void 0===c?"":c;if(!a.length)return null;"etjpg"==c&&(a=a.filter(function(d){return _.E(d,1,"").includes("w1200-h300")}));return a.map(function(d){return{url:_.E(d,
1,""),height:d.getHeight(),width:_.E(d,3,0),type:c}})};
var fw=function(){var a=aw,c={},d=c.document||document,e=_.Ud(a),f=_.ze("SCRIPT"),g={Ig:f,Fd:void 0},h=new _.qo(bw,g),l=null,m=null!=c.timeout?c.timeout:5E3;0<m&&(l=window.setTimeout(function(){cw(f,!0);var n=new dw(1,"Timeout reached for loading script "+e);_.so(h);_.to(h,!1,n)},m),g.Fd=l);f.onload=f.onreadystatechange=function(){f.readyState&&"loaded"!=f.readyState&&"complete"!=f.readyState||(cw(f,c.tl||!1,l),h.Mc(null))};f.onerror=function(){cw(f,!0,l);var n=new dw(0,"Error while loading script "+
e);_.so(h);_.to(h,!1,n)};g=c.attributes||{};_.Za(g,{type:"text/javascript",charset:"UTF-8"});_.te(f,g);_.je(f,a);ew(d).appendChild(f);return h},ew=function(a){var c=_.qe("HEAD",a);return c&&0!=c.length?c[0]:a.documentElement},bw=function(){if(this&&this.Ig){var a=this.Ig;a&&"SCRIPT"==a.tagName&&cw(a,!0,this.Fd)}},cw=function(a,c,d){null!=d&&_.q.clearTimeout(d);a.onload=_.xa;a.onerror=_.xa;a.onreadystatechange=_.xa;c&&window.setTimeout(function(){_.Ae(a)},0)},dw=function(a,c){var d="Jsloader error (code #"+
a+")";c&&(d+=": "+c);_.Ka.call(this,d);this.code=a};_.w(dw,_.Ka);
var aw=_.nf(_.ib("https://apis.google.com/js/api.js")),jw=function(a){var c=!1,d=gw(a).then(function(f){c=!0;return f}),e=qu().then(function(){return c?gw(a):hw().then(function(f){return iw(f,a)})});return nu([d,e])},gw=function(a){return(window.gapi&&window.gapi.load?pu(window.gapi):hw()).then(function(c){return iw(c,a)})},iw=function(a,c){var d=_.$d(c,"gapi.")?c.slice(5):c;return a[d]?pu(a[d]):new _.Gf(function(e,f){var g=_.rg(function(){f(Error("Ba"))},3E4);a.load(c,{callback:function(){_.sg(g);
e(a[d])},onerror:function(h){_.sg(g);f(h)}})})},hw=function(){return fw().then(function(){return window.gapi})},kw=function(){};kw.prototype.load=function(a){return jw(a).then(null,function(c){throw c instanceof Error?c:Error(String(c));})};
var mw=function(){var a=this;this.o=new kw;this.j=null;this.f=lw(this);this.b=mu();this.f.then(null,function(c){return void a.b.f(c)});this.b.b.then(null,function(){})},lw=function(a){return a.o.load("gapi.iframes").then(function(c){a.w=Date.now();return c})},ow=function(a,c,d,e,f){var g=!0;g=void 0===g?!1:g;a.f.then(function(){var h=void 0,l=f,m=g;h=void 0===h?null:h;l=void 0===l?null:l;m=void 0===m?!1:m;var n={};n["host-message-handler"]=d;var r=_.Pm(e);r=_.Pm(r);r=_.zm(_.ym(_.xm(new _.wm,r.j),
r.f),r.B).toString();a.j=r;r=new Bv;r.b.url=e;r.b.where=c;r.b.allowPost=m;r.b.messageHandlers=n;m=nw(a);r.b.messageHandlersFilter=m;null!==h&&(r.b.queryParams=h);null!==l&&(r.b.id=l);r.b.attributes=r.b.attributes||{};h=new Av(r.b.attributes);h.b.style={display:"block","min-width":"100%",width:"1px"};h.b.height="100%";return(_.eg(c.ownerDocument).gapi||window.gapi).iframes.getContext().openChild(r.value())}).then(function(h){return void a.b.j(h)},function(h){return void a.b.f(h)});return a.b.b},pw=
function(a,c){return a.b.b.then(function(d){return d?d.send("picker-message-handler",c,void 0,nw(a)):ou()})},nw=function(a){return _.He("gapi.iframes.makeWhiteListIframesFilter")([a.j])};
var qw=function(){};qw.prototype.b=0;
var sw=function(){var a=new kv,c=new fv;du(c,1,"root","");var d=rw();_.I(c,3,d);Y(c,4,1);_.I(a,3,c);Y(a,1,2);lv(a,"My Drive");return a},tw=function(){var a=new kv,c=new fv;du(c,5,!0,!1);var d=rw();Y(d,1,7);_.I(c,3,d);Y(c,4,1);_.I(a,3,c);Y(a,1,2);lv(a,"Shared with me");return a},uw=function(){var a=new kv,c=new fv,d=new ev;Y(d,1,10);Y(d,2,2);_.I(c,3,d);Y(c,4,1);_.I(a,3,c);Y(a,1,2);lv(a,"Recent");return a},vw=function(){var a=new kv,c=new fv;du(c,7,!0,!1);var d=rw();_.I(c,3,d);Y(c,4,1);_.I(a,3,c);Y(a,
1,2);lv(a,"Starred");return a},ww=function(){var a=new kv,c=new fv;du(c,11,!0,!1);_.I(a,3,c);Y(a,1,2);lv(a,"Shared drives");return a},rw=function(){var a=new ev;Y(a,1,4);Y(a,2,1);return a};
var zw=function(){var a=new nv;ov(a,xw());ov(a,yw());return a},xw=function(){var a=new kv,c=new iv;Y(c,3,1);Y(c,2,1);du(c,5,!0,!1);du(c,6,!1,!1);_.I(a,6,c);Y(a,1,3);lv(a,"Photos");return a},yw=function(){var a=new kv,c=new iv;Y(c,3,2);du(c,5,!0,!1);du(c,6,!1,!1);_.I(a,6,c);Y(a,1,3);lv(a,"Albums");return a},Aw=function(){var a=new kv,c=new iv;Y(c,3,1);Y(c,2,1);du(c,5,!1,!1);du(c,6,!0,!1);_.I(a,6,c);Y(a,1,3);lv(a,"Videos");return a};
var Bw=new Map([["birthday",14],["children",1],["dinner",2],["featured",3],["holiday",4],["nightlife",5],["other",6],["party",7],["school",8],["seasonal",9],["sport",10],["stationery",11],["travel",12],["wedding",13]]),Cw=new Set("all docs-images docs-images-and-videos docs-videos documents drawings folders forms pdfs presentations scripts sites spreadsheets tables".split(" ")),Fw=function(a,c,d,e){var f=Yu(Xu(Wu(),a));a=[];try{for(var g=0;g<e.length;g++){var h=e[g],l=h[0],m=h[1];switch(l){case "cropphoto":for(var n=
Su(2),r=new Qu,v=_.ba(Object.entries(m||{})),N=v.next();!N.done;N=v.next()){var D=_.ba(N.value),P=D.next().value;D.next();switch(P){case "ctta":break;default:throw Error("Da`"+P+"`"+l);}}fu(n,r);gu(f,28,n,Ru,void 0);break;default:throw Error("Ea`"+l);}}d.forEach(function(G,fa){switch(fa){case "hostId".toString():du(f,24,G,"");break;case "origin".toString():du(f,27,G,"");break;case "title".toString():f.setTitle(G);break;case "hl".toString():du(f,10,G,"");break;case "multiselectEnabled".toString():"true"==
G&&(G=new Tu,Y(G,1,1),_.I(f,3,G));break;case "st".toString():du(f,12,G,"");break;case "authuser".toString():G=parseInt(G,10);if(isNaN(G))throw Error("Fa");fa=new zu;G=du(fa,1,G,0);_.I(f,6,G);break;case "maxItems".toString():du(f,5,parseInt(G,10),0);break;case "profilePhoto".toString():f.setTitle("Select Profile Photo");G=Su(2);fa=new Qu;fa=du(fa,2,!0,!1);G=fu(G,fa);gu(f,28,G,Ru,void 0);G=Su(1);gu(f,28,G,Ru,void 0);break;case "gmailDelegatorId".toString():fa=new wu;G=du(fa,1,G,"");_.I(f,29,G);break;
case "minSize".toString():G=Dw(G);_.I(f,32,G);break;case "maxSize".toString():G=Dw(G);_.I(f,33,G);break;case "pp".toString():case "dff".toString():case "relayUrl".toString():case "navHidden".toString():case "nav".toString():case "protocol".toString():case "actions".toString():case "thumbs".toString():case "tt".toString():case "odv".toString():case "newDriveView".toString():case "cropMode".toString():case "maxSizeBytes".toString():case "selectButtonLabel".toString():case "view".toString():break;default:throw Error("Ga`"+
fa);}});a=Ew(c,f)}catch(G){return null}return wv(vv(f),a)},Dw=function(a){var c=a.split("x");a=c[0];c=c[1];var d=new Nu;a=du(d,1,parseInt(a,10),0);return du(a,2,parseInt(c,10),0)},Gw=function(a){var c=_.E(_.H(a,Vu,1),8,"");_.ih(c,"/")||(c+="/");c=_.Pm(c);_.Am(c,c.o+"home");_.Nm(c,"req",a.f());return c.toString()},Hw=function(a){var c="";switch(a.Nb()){case 2:c="cancel";break;case 1:c="picked";break;case 3:c="error"}a=_.Zj(a,Ju,2);return 0===a.length?{action:c}:Yv(a,c)},Jw=function(a,c){switch(a.action){case "select-contacts":a=
Iw(a.contacts);break;case "visibility":a=a.visible;var d=new qv;a=Y(d,1,7).ha(a);d={};d["iframe-command"]=a.f();a=d;break;default:a=null}return a?pw(c,a):pu()},Iw=function(a){if(!a||0==a.length)return null;var c=new qv;Y(c,1,11);var d=new qw;a.forEach(function(e){if(e.email){var f=new Ju;f=du(f,2,e.name?e.name:e.email,"");var g=new Eu;e=_.Zm(g,1,e.email);e=_.I(f,27,e);f=new Au;g=":"+(d.b++).toString(36);f=du(f,1,g,"");f=Y(f,2,12);e=_.I(e,1,f)}else e=null;e&&gu(c,7,e,Ju,void 0)});a={};a["iframe-command"]=
c.f();return a},Ew=function(a,c){var d=new Map,e=new Pu;Mv(a).forEach(function(f){var g=new kv,h=$t(f.f),l=f.o;if(null!=l&&Cw.has(l)){switch(l){case "all":break;case "docs-images":Z(e,1);Z(e,6);break;case "docs-images-and-videos":Z(e,2);Z(e,1);Z(e,6);break;case "docs-videos":Z(e,2);Z(e,6);break;case "documents":Z(e,3);Z(e,6);break;case "drawings":Z(e,12);Z(e,6);break;case "folders":Z(e,6);break;case "forms":Z(e,7);Z(e,6);break;case "pdfs":Z(e,9);Z(e,6);break;case "presentations":Z(e,5);Z(e,6);break;
case "scripts":Z(e,10);Z(e,6);break;case "sites":Z(e,8);Z(e,6);break;case "spreadsheets":Z(e,4);Z(e,6);break;case "tables":Z(e,11);Z(e,6);break;default:throw Error("Ma`"+l);}if(Object.keys(h).length){if(h.hasOwnProperty("sortKey")&&15!=h.sortKey||(g=uw(),d.set(g.f(),g)),h.starred&&(g=vw(),d.set(g.f(),g)),h.ownedByMe?(g=sw(),d.set(g.f(),g)):(g=tw(),d.set(g.f(),g)),h.td||h.dr)g=ww(),d.set(g.f(),g)}else{var m=void 0===m?!1:m;g=new nv;ov(g,uw());if(m){h=new kv;var n=new fv;du(n,14,!0,!1);Y(n,4,1);_.I(h,
3,n);Y(h,1,2);lv(h,"Recent");ov(g,h)}ov(g,sw());ov(g,ww());ov(g,tw());ov(g,vw());h=new kv;n=new fv;du(n,12,!0,!1);_.I(h,3,n);Y(h,1,2);lv(h,"Computers");ov(g,h);d.set(g.f(),g)}}else switch(l){case "contacts":Y(g,1,12);if(0!=Object.keys(h||{}).length)throw Error("Ha");d.set(g.f(),g);break;case "photos":Kw(h,d,e);break;case "upload":"docs"==h.query?(n=void 0===n?[]:n,g=new kv,h=lv(Y(g,1,2),"Upload"),f=new fv,m=new dv,n=_.F(m,3,n||[]),n=_.I(f,15,n),_.I(h,3,n)):(Y(g,1,10),h=Lw(h,e),_.I(g,10,h));d.set(g.f(),
g);break;case "url":Y(g,1,9);f.j&&lv(g,f.j);Z(e,1);d.set(g.f(),g);break;case "webcam":Y(g,1,1);switch(h.query){case "forms":case "spreadsheets":case "presentation":n=g,f=new bv,f=Y(f,1,1),h=Lw(h,e),h=_.I(f,2,h),_.I(n,16,h)}Z(e,1);d.set(g.f(),g);break;case "image-search":Y(g,1,5);Z(e,1);d.set(g.f(),g);break;case "et":Y(g,1,13);f.j&&lv(g,f.j);h=new gv;n=_.ba(Object.entries($t(f.f)||{}));for(f=n.next();!f.done;f=n.next())switch(m=_.ba(f.value),f=m.next().value,m=m.next().value,f){case "category":if(Bw.has(m))f=
Bw.get(m),Y(h,2,f);else throw Error("Ia`"+m);break;default:throw Error("Ja`"+f);}Z(e,1);_.I(g,13,h);d.set(g.f(),g);break;case null:break;default:throw Error("Ka`"+f.o);}});_.I(c,2,e);return Array.from(d.values())},Lw=function(a,c){var d=new av;a=_.ba(Object.entries(a||{}));for(var e=a.next();!e.done;e=a.next()){var f=_.ba(e.value);e=f.next().value;f=f.next().value;switch(e){case "query":switch(f){case "profile":Y(d,4,2);Z(c,1);break;case "photo":Y(d,4,1);Z(c,1);break;case "forms":Y(d,4,6);Z(c,1);
break;case "spreadsheets":Y(d,4,7);Z(c,1);break;case "presentation":Y(d,4,8);Z(c,1);break;default:throw Error("La`"+f);}break;case "data":for(e=_.ba(Object.entries(f||{})),f=e.next();!f.done;f=e.next()){var g=_.ba(f.value);f=g.next().value;g=g.next().value;var h=d;h.b||(h.b={});if(2 in h.b)h=h.b[2];else{var l=_.B(h,2);l||(l=[],_.F(h,2,l));h=h.b[2]=new bu(l)}h.set(f,g)}}}return d},Kw=function(a,c,d){var e=new nv;if(Object.keys(a).length){if(a.allowedItemTypes.includes("photo")&&(ov(e,xw()),Z(d,1)),
a.allowedItemTypes.includes("album")&&(ov(e,yw()),Z(d,14)),"videos-uploaded"==a.type||"videos-camerasync"==a.type)ov(e,Aw()),Z(d,2)}else e=zw(),Z(d,1),Z(d,14);_.Zj(e,kv,1).forEach(function(f){c.set(f.f(),f)})};
var Mw=function(a,c){Pv.call(this,"set-drive-options");this.appId=a;this.appOrigin=c};_.w(Mw,Pv);
var Nw=function(a){Pv.call(this,"visibility");this.visible=a};_.w(Nw,Pv);
var Ow=function(a){this.Cb=new Map;var c=arguments.length;if(1<c){if(c%2)throw Error("h");for(var d=0;d<c;d+=2)this.set(arguments[d],arguments[d+1])}else if(a)if(a instanceof Ow)for(c=_.ba(a.Cb),d=c.next();!d.done;d=c.next()){var e=_.ba(d.value);d=e.next().value;e=e.next().value;this.Cb.set(d,e)}else if(a)for(c=_.ba(Object.entries(a)),d=c.next();!d.done;d=c.next())e=_.ba(d.value),d=e.next().value,e=e.next().value,this.Cb.set(d,e)};_.k=Ow.prototype;_.k.Pa=function(){return Array.from(this.Cb.values())};
_.k.kb=function(){return Array.from(this.Cb.keys())};_.k.vc=function(){return 0==this.Cb.size};_.k.clear=function(){this.Cb.clear()};_.k.remove=function(a){return this.Cb.delete(a)};_.k.get=function(a,c){return this.Cb.has(a)?this.Cb.get(a):c};_.k.set=function(a,c){this.Cb.set(a,c);return this};_.k.forEach=function(a,c){var d=this;c=void 0===c?this:c;this.Cb.forEach(function(e,f){return a.call(c,e,f,d)})};
(function(){for(var a=["ms","moz","webkit","o"],c,d=0;c=a[d]&&!_.q.requestAnimationFrame;++d)_.q.requestAnimationFrame=_.q[c+"RequestAnimationFrame"],_.q.cancelAnimationFrame=_.q[c+"CancelAnimationFrame"]||_.q[c+"CancelRequestAnimationFrame"];if(!_.q.requestAnimationFrame){var e=0;_.q.requestAnimationFrame=function(f){var g=(new Date).getTime(),h=Math.max(0,16-(g-e));e=g+h;return _.q.setTimeout(function(){f(g+h)},h)};_.q.cancelAnimationFrame||(_.q.cancelAnimationFrame=function(f){clearTimeout(f)})}})();
var Pw=[[],[]],Qw=0,Rw=!1,Sw=0,Uw=function(a,c){var d=Sw++,e={ej:{id:d,Yb:a.measure,context:c},kj:{id:d,Yb:a.jj,context:c},state:{},Ta:void 0,de:!1};return function(){0<arguments.length?(e.Ta||(e.Ta=[]),e.Ta.length=0,e.Ta.push.apply(e.Ta,arguments),e.Ta.push(e.state)):e.Ta&&0!=e.Ta.length?(e.Ta[0]=e.state,e.Ta.length=1):e.Ta=[e.state];e.de||(e.de=!0,Pw[Qw].push(e));Rw||(Rw=!0,window.requestAnimationFrame(Tw))}},Tw=function(){Rw=!1;var a=Pw[Qw],c=a.length;Qw=(Qw+1)%2;for(var d,e=0;e<c;++e){d=a[e];
var f=d.ej;d.de=!1;f.Yb&&f.Yb.apply(f.context,d.Ta)}for(e=0;e<c;++e)d=a[e],f=d.kj,d.de=!1,f.Yb&&f.Yb.apply(f.context,d.Ta),d.state={};a.length=0};
var Vw=_.y?_.nf(_.ib('javascript:""')):_.nf(_.ib("about:blank")),Ww=_.Ud(Vw),Xw=_.y?_.nf(_.ib('javascript:""')):_.nf(_.ib("javascript:undefined"));_.Ud(Xw);
var Yw=function(a,c){this.j=a;this.f=c};
var Zw=function(a,c){_.ah.call(this,c);this.Fb=!!a;this.J=null;this.Aa=Uw({jj:this.Wd},this)};_.w(Zw,_.ah);_.k=Zw.prototype;_.k.Le=null;_.k.Xd=!1;_.k.ub=null;_.k.Wa=null;_.k.Ib=null;_.k.Ee=!1;_.k.ud=function(){return"gb_Aa-modalpopup"};_.k.sd=function(){return this.ub};_.k.Hb=function(){Zw.L.Hb.call(this);var a=this.C();_.mh(a,(0,_.Ra)(this.ud()).split(" "));_.$h(a,!0);_.X(a,!1);$w(this);ax(this)};
var $w=function(a){if(a.Fb&&!a.Wa){var c=a.b.wa("IFRAME",{frameborder:0,style:"border:0;vertical-align:bottom;"});_.of(c,Vw);a.Wa=c;a.Wa.className=a.ud()+"-c";_.X(a.Wa,!1);Xt(a.Wa,0)}a.ub||(a.ub=a.b.wa("DIV",a.ud()+"-c"),_.X(a.ub,!1))},ax=function(a){a.Ib||(a.Ib=a.b.createElement("SPAN"),_.X(a.Ib,!1),_.$h(a.Ib,!0),a.Ib.style.position="absolute")};_.k=Zw.prototype;_.k.Gg=function(){this.Ee=!1};_.k.Bf=function(a){return!!a&&"DIV"==a.tagName};
_.k.Wb=function(a){Zw.L.Wb.call(this,a);a=(0,_.Ra)(this.ud()).split(" ");_.mh(this.C(),a);$w(this);ax(this);_.$h(this.C(),!0);_.X(this.C(),!1)};_.k.Ea=function(){this.Wa&&_.Nh(this.Wa,this.C());_.Nh(this.ub,this.C());Zw.L.Ea.call(this);_.sh(this.Ib,this.C());this.Le=new _.Fq(this.b.b);_.ch(this).H(this.Le,"focusin",this.Fj);bx(this,!1)};_.k.hb=function(){this.isVisible()&&this.ha(!1);_.Xf(this.Le);Zw.L.hb.call(this);_.Ae(this.Wa);_.Ae(this.ub);_.Ae(this.Ib)};
_.k.ha=function(a){if(a!=this.Xd)if(this.O&&this.O.stop(),this.R&&this.R.stop(),this.K&&this.K.stop(),this.N&&this.N.stop(),this.Da&&bx(this,a),a){if(this.dispatchEvent("beforeshow")){try{this.J=this.b.b.activeElement}catch(f){}this.Wd();this.Vd();_.ch(this).H(_.nq(this.b),"resize",this.Wd).H(_.nq(this.b),"orientationchange",this.Aa);cx(this,!0);this.focus();this.Xd=!0;this.O&&this.R?(_.Ze(this.O,"end",this.Ud,!1,this),this.R.play(),this.O.play()):this.Ud()}}else if(this.dispatchEvent("beforehide")){_.ch(this).Ba(_.nq(this.b),
"resize",this.Wd).Ba(_.nq(this.b),"orientationchange",this.Aa);this.Xd=!1;this.K&&this.N?(_.Ze(this.K,"end",this.Td,!1,this),this.N.play(),this.K.play()):this.Td();a:{try{var c=this.b,d=c.b.body,e=c.b.activeElement||d;if(!this.J||this.J==d){this.J=null;break a}(e==d||c.Wf(this.C(),e))&&this.J.focus()}catch(f){}this.J=null}}};
var bx=function(a,c){a.$||(a.$=new Yw(a.f,a.b));a=a.$;if(c){a.b||(a.b=[]);c=a.f.Ph(a.f.b.body);for(var d=0;d<c.length;d++){var e=c[d];e==a.j||_.ci(e,"hidden")||(_.Ge(e,"hidden",!0),a.b.push(e))}}else if(a.b){for(d=0;d<a.b.length;d++)a.b[d].removeAttribute("aria-hidden");a.b=null}},cx=function(a,c){a.Wa&&_.X(a.Wa,c);a.ub&&_.X(a.ub,c);_.X(a.C(),c);_.X(a.Ib,c)};_.k=Zw.prototype;_.k.Ud=function(){this.dispatchEvent("show")};_.k.Td=function(){cx(this,!1);this.dispatchEvent("hide")};_.k.isVisible=function(){return this.Xd};
_.k.focus=function(){this.Pf()};_.k.Wd=function(){this.Wa&&_.X(this.Wa,!1);this.ub&&_.X(this.ub,!1);var a=this.b.b,c=_.dg(_.eg(a)||window),d=Math.max(c.width,Math.max(a.body.scrollWidth,a.documentElement.scrollWidth));a=Math.max(c.height,Math.max(a.body.scrollHeight,a.documentElement.scrollHeight));this.Wa&&(_.X(this.Wa,!0),_.bo(this.Wa,d,a));this.ub&&(_.X(this.ub,!0),_.bo(this.ub,d,a))};
_.k.Vd=function(){var a=_.eg(this.b.b)||window;if("fixed"==_.Mg(this.C(),"position"))var c=0,d=0;else d=_.lq(this.b.b),c=d.x,d=d.b;var e=_.Qg(this.C());a=_.dg(a);c=Math.max(c+a.width/2-e.width/2,0);d=Math.max(d+a.height/2-e.height/2,0);_.tq(this.C(),c,d);_.tq(this.Ib,c,d)};_.k.Fj=function(a){this.Ee?this.Gg():a.target==this.Ib&&_.rg(this.Pf,0,this)};_.k.Pf=function(){try{_.y&&this.b.b.body.focus(),this.C().focus()}catch(a){}};
_.k.P=function(){_.Xf(this.O);this.O=null;_.Xf(this.K);this.K=null;_.Xf(this.R);this.R=null;_.Xf(this.N);this.N=null;Zw.L.P.call(this)};
var hx=function(a,c,d){Zw.call(this,c,d);this.B=a||"gb_b-b";this.o=dx(dx(new ex,fx,!0),gx,!1,!0)};_.w(hx,Zw);_.k=hx.prototype;_.k.Of=!0;_.k.zd=!0;_.k.tg=!0;_.k.Kd=.5;_.k.tf="";_.k.uc=null;_.k.Zf=!1;_.k.rb=null;_.k.Za=null;_.k.xe=null;_.k.Xa=null;_.k.Fc=null;_.k.Na=null;_.k.ud=function(){return this.B};_.k.setTitle=function(a){this.tf=a;this.Za&&_.ig(this.Za,a)};_.k.Uc=function(){this.C()||this.Ha();return this.Fc};var ix=function(a){a.C()||a.Ha();return a.C()};
hx.prototype.sd=function(){this.C()||this.Ha();return hx.L.sd.call(this)};var jx=function(a,c){a.Kd=c;a.C()&&(c=a.sd())&&Xt(c,a.Kd)},kx=function(a,c){var d=(0,_.Ra)(a.B+"-f-draggable").split(" ");a.C()&&(c?_.mh(a.rb,d):_.nh(a.rb,d));c&&!a.uc?(c=new _.Qq(a.C(),a.rb),a.uc=c,_.mh(a.rb,d),_.O(a.uc,"start",a.ek,!1,a)):!c&&a.uc&&(a.uc.sa(),a.uc=null)};_.k=hx.prototype;
_.k.Hb=function(){hx.L.Hb.call(this);var a=this.C(),c=this.b;this.rb=c.wa("DIV",this.B+"-f",this.Za=c.wa("SPAN",{className:this.B+"-f-g",id:_.bh(this)},this.tf),this.Xa=c.wa("SPAN",this.B+"-f-close"));ju(a,this.rb,this.Fc=c.wa("DIV",this.B+"-e"),this.Na=c.wa("DIV",this.B+"-h"));_.Fe(this.Za,"heading");_.Fe(this.Xa,"button");_.$h(this.Xa,!0);_.Ge(this.Xa,"label","Close");this.xe=this.Za.id;_.Fe(a,"dialog");_.Ge(a,"labelledby",this.xe||"");_.X(this.Xa,this.zd);this.o&&(a=this.o,a.b=this.Na,a.Ha());
_.X(this.Na,!!this.o);jx(this,this.Kd)};
_.k.Wb=function(a){hx.L.Wb.call(this,a);a=this.C();var c=this.B+"-e";this.Fc=_.re(document,null,c,a)[0];this.Fc||(this.Fc=this.b.wa("DIV",c),a.appendChild(this.Fc));c=this.B+"-f";var d=this.B+"-f-g",e=this.B+"-f-close";(this.rb=_.re(document,null,c,a)[0])?(this.Za=_.re(document,null,d,this.rb)[0],this.Xa=_.re(document,null,e,this.rb)[0]):(this.rb=this.b.wa("DIV",c),a.insertBefore(this.rb,this.Fc));this.Za?(this.tf=_.bi(this.Za),this.Za.id||(this.Za.id=_.bh(this))):(this.Za=_.ve("SPAN",{className:d,
id:_.bh(this)}),this.rb.appendChild(this.Za));this.xe=this.Za.id;_.Ge(a,"labelledby",this.xe||"");this.Xa||(this.Xa=this.b.wa("SPAN",e),this.rb.appendChild(this.Xa));_.X(this.Xa,this.zd);c=this.B+"-h";if(this.Na=_.re(document,null,c,a)[0]){if(a=this.o=new ex(this.b),(c=this.Na)&&1==c.nodeType){a.b=c;c=_.qe("BUTTON",a.b);d=0;for(var f,g;e=c[d];d++)if(f=e.name||e.id,g=_.bi(e)||e.value,f){var h=0==d;a.set(f,g,h,"cancel"==e.name);h&&_.S(e,"gb_Aa-buttonset-default")}}}else this.Na=this.b.wa("DIV",c),a.appendChild(this.Na),
this.o&&(a=this.o,a.b=this.Na,a.Ha()),_.X(this.Na,!!this.o);jx(this,this.Kd)};_.k.Ea=function(){hx.L.Ea.call(this);_.ch(this).H(this.C(),"keydown",this.Y).H(this.C(),"keypress",this.Y);_.ch(this).H(this.Na,"click",this.$a);kx(this,!0);_.ch(this).H(this.Xa,"click",this.Tj);var a=this.C();_.Fe(a,"dialog");""!==this.Za.id&&_.Ge(a,"labelledby",this.Za.id);if(!this.tg){this.tg=!1;if(this.Da){a=this.b;var c=this.sd();a.Sd(this.Wa);a.Sd(c)}this.isVisible()&&bx(this,!1)}};
_.k.hb=function(){this.isVisible()&&this.ha(!1);kx(this,!1);hx.L.hb.call(this)};_.k.ha=function(a){a!=this.isVisible()&&(this.Da||this.Ha(),hx.L.ha.call(this,a))};_.k.Ud=function(){hx.L.Ud.call(this);this.dispatchEvent("aftershow")};_.k.Td=function(){hx.L.Td.call(this);this.dispatchEvent("afterhide");this.Zf&&this.sa()};
_.k.ek=function(){var a=this.b.b,c=_.dg(_.eg(a)||window),d=Math.max(a.body.scrollWidth,c.width);a=Math.max(a.body.scrollHeight,c.height);var e=_.Qg(this.C());"fixed"==_.Mg(this.C(),"position")?this.uc.w=new _.sq(0,0,Math.max(0,c.width-e.width),Math.max(0,c.height-e.height)):this.uc.w=new _.sq(0,0,d-e.width,a-e.height)};_.k.Tj=function(){lx(this)};var lx=function(a){if(a.zd){var c=a.o,d=c&&c.f;d?(c=c.get(d),a.dispatchEvent(new mx(d,c))&&a.ha(!1)):a.ha(!1)}},nx=function(a){a.zd=!1;a.Xa&&_.X(a.Xa,a.zd)};
hx.prototype.P=function(){this.Na=this.Xa=null;hx.L.P.call(this)};hx.prototype.$a=function(a){a:{for(a=a.target;null!=a&&a!=this.Na;){if("BUTTON"==a.tagName)break a;a=a.parentNode}a=null}if(a&&!a.disabled){a=a.name;var c=this.o.get(a);this.dispatchEvent(new mx(a,c))&&this.ha(!1)}};
hx.prototype.Y=function(a){var c=!1,d=!1,e=this.o,f=a.target;if("keydown"==a.type)if(this.Of&&27==a.keyCode){var g=e&&e.f;f="SELECT"==f.tagName&&!f.disabled;g&&!f?(d=!0,c=e.get(g),c=this.dispatchEvent(new mx(g,c))):f||(c=!0)}else{if(9==a.keyCode&&a.shiftKey&&f==this.C()){this.Ee=!0;try{this.Ib.focus()}catch(r){}_.rg(this.Gg,0,this)}}else if(13==a.keyCode){if("BUTTON"==f.tagName&&!f.disabled)g=f.name;else if(f==this.Xa)lx(this);else if(e){var h=e.j,l;if(l=h)a:{l=_.qe("BUTTON",e.b);for(var m=0,n;n=
l[m];m++)if(n.name==h||n.id==h){l=n;break a}l=null}f=("TEXTAREA"==f.tagName||"SELECT"==f.tagName||"A"==f.tagName)&&!f.disabled;!l||l.disabled||f||(g=h)}g&&e&&(d=!0,c=this.dispatchEvent(new mx(g,String(e.get(g)))))}else f!=this.Xa||32!=a.keyCode&&" "!=a.key||lx(this);if(c||d)a.stopPropagation(),a.preventDefault();c&&this.ha(!1)};var mx=function(a,c){this.type="dialogselect";this.key=a;this.caption=c};_.w(mx,_.Le);var ex=function(a){Ow.call(this);a||_.pg();this.f=this.b=this.j=null};_.w(ex,Ow);
ex.prototype.clear=function(){Ow.prototype.clear.call(this);this.j=this.f=null};ex.prototype.set=function(a,c,d,e){Ow.prototype.set.call(this,a,c);d&&(this.j=a);e&&(this.f=a);return this};var dx=function(a,c,d,e){return a.set(c.key,c.caption,d,e)};ex.prototype.Ha=function(){if(this.b){_.ag(this.b,_.Gb);var a=_.pg(this.b);this.forEach(function(c,d){c=a.wa("BUTTON",{name:d},c);d==this.j&&(c.className="gb_Aa-buttonset-default");this.b.appendChild(c)},this)}};ex.prototype.C=function(){return this.b};
var fx={key:"ok",caption:"OK"},gx={key:"cancel",caption:"Cancel"},ox={key:"yes",caption:"Yes"},px={key:"no",caption:"No"},qx={key:"save",caption:"Save"},rx={key:"continue",caption:"Continue"};"undefined"!=typeof document&&(dx(new ex,fx,!0,!0),dx(dx(new ex,fx,!0),gx,!1,!0),dx(dx(new ex,ox,!0),px,!1,!0),dx(dx(dx(new ex,ox),px,!0),gx,!1,!0),dx(dx(dx(new ex,rx),qx),gx,!0,!0));
var sx=function(a,c,d){hx.call(this,a,c,d)};_.w(sx,hx);
var tx=function(a){Nv.call(this,a)};_.w(tx,Nv);
var ux=_.nf(_.ib("//www-onepick-opensocial.googleusercontent.com/gadgets/js/rpc.js?c=1&container=onepick")),vx=_.nf(_.ib("//apis.google.com/js/rpc.js")),wx=function(a){a=a&&_.nq(a)||window;return a.gadgets&&a.gadgets.rpc},xx=null,yx=function(a,c){var d=c&&_.nq(c)||window;if(wx(c))a();else if(xx)xx.push(a);else var e=xx=[a],f=d.setInterval(function(){if(wx(c)){d.clearInterval(f);for(var g=0;g<e.length;g++)e[g]();xx=null}},100)};
var zx=function(a,c){var d;a:{for(d=c.target;d;){if(1==d.nodeType){var e=_.Mg(d,"overflowY");if("auto"==e||"scroll"==e)break a}d=d.parentNode}d=null}(!d||!_.hg(a,d)||d.scrollHeight==d.clientHeight||0<c.deltaY&&1>=Math.abs(d.scrollTop-(d.scrollHeight-d.clientHeight))||0>c.deltaY&&0==d.scrollTop)&&c.stopPropagation()};
var Ax,Bx=function(a,c,d){if(c){c=Math.max(320,Math.min(1051,c));d||(d=_.dg(a),d=.85*d.height);var e=Math.max(320,Math.min(650,d))}else d=_.dg(a),c=.618*d.width,e=c<d.height?Math.round(Math.max(320,Math.min(650,.85*c))):Math.round(Math.max(320,Math.min(650,.85*d.height))),c=Math.round(e/.618);d=_.dg(a);c=Math.min(c,Math.max(d.width,320));e=Math.min(e,Math.max(d.height,320));return new _.pe(c,e)};
var Cx=function(a,c,d,e,f,g,h){hx.call(this,g?g+" gb_a gb_b-b":"gb_a gb_b-b",!0,d);d=a.search(_.Fk);g=_.Ek(a,0,"protocol",d);if(!(0>g)){var l=a.indexOf("&",g);if(0>l||l>d)l=d;g+=9;decodeURIComponent(a.substr(g,l-g).replace(/\+/g," "))}this.S=new mw;this.F=_.um();this.X=_.um();this.T=!1;d=_.Nm(new _.wm(a),"rpcService",this.F);(this.T=void 0!==_.Om(d,"v2"))?_.Nm(d,"v1RpcToken",this.X):_.Nm(d,"rpctoken",this.X);_.xm(d,"https");this.Tb=d.toString();this.Ab&&(this.Ab.src=this.Tb);this.Ga=e;this.va=f;void 0!==
e||void 0!==f?e=!0:(e=_.Om(_.Pm(a),"hostId"),Ax||(Ax=new Set("DocVerse fusiontables geo geowiki gm gmail-gadget gws hotpot jointly presentations pwa sites templates trix trix-copy-sheet webstore".split(" "))),e=!Ax.has(e));this.Ma=e;this.ka=h||this.b;c&&(_.Om(_.Pm(a),"hostId"),c="true"==_.Om(_.Pm(this.Tb),"grugl")?vx:ux,h=this.ka,wx(h)||(h=h||_.pg(document),e=h.createElement("SCRIPT"),_.je(e,c),e.type="text/javascript",h.b.body.appendChild(e)));c=null;h=a.indexOf("/picker?");-1<h?c=a.substring(0,
h+8-1):_.ih(a,"/picker")&&(c=a);c&&this.setRelayUrl(c+"/resources/rpc_relay.html");this.Of=!1;this.o=null;this.Na&&(this.o?(a=this.o,a.b=this.Na,a.Ha()):_.ag(this.Na,_.Gb),_.X(this.Na,!!this.o))};_.w(Cx,sx);_.k=Cx.prototype;_.k.Tb="";_.k.Ab=null;_.k.qe=!1;_.k.df=!1;_.k.Oa=_.xa;_.k.Ea=function(){Cx.L.Ea.call(this);var a=this.sd(),c=_.ch(this),d=new _.Mq(a);_.Yf(c,d);c.H(d,"mousewheel",(0,_.t)(zx,void 0,a)).H(a,"scroll",(0,_.t)(zx,void 0,a))};
_.k.Ha=function(a){var c=this;Cx.L.Ha.call(this,a);this.T?this.S.f.then(function(){return Dx(c)}).then(null,function(){c.Oa({action:"error"})}):(this.Ab=this.b.wa("IFRAME",{id:this.F,name:this.F,"class":"gb_a-a",onload:(0,_.t)(this.Z,this),frameBorder:"0",allow:"camera"}),_.of(this.Ab,Ex(this)),this.Uc().appendChild(this.Ab),_.S(this.C(),"picker-dialog"),this.Ab.src=this.Tb,Fx(this),Gx(this))};
var Dx=function(a){var c=a.b.wa("div",["picker-dialog-content","gb_a-a"]);_.X(c,!1);a.Uc().appendChild(c);return ow(a.S,c,function(d){d=d["iframe-command"];d=new sv(d?JSON.parse(d):null);switch(_.E(d,1,0)){case 1:a.Oa(Hw(_.H(d,$u,2)));a.ha(!1);break;case 4:nx(a),a.Oa({action:"loaded"})}},a.Tb,a.F).then(function(d){a.Ab=d.getIframeEl();a.Z();_.X(a.Ab.parentElement,!0);_.S(a.C(),"picker-dialog");Fx(a);Gx(a);return d})},Fx=function(a){Hx(a,(0,_.t)(function(c){c.setAuthToken(this.F,this.X)},a))},Gx=function(a){var c=
_.Om(_.Pm(a.Tb),"title");c&&a.setTitle(c)},Ex=function(a){return _.y&&_.gc("7")&&_.$d(a.Tb,"https")?_.nf(_.ib("https://about:blank")):_.y?_.nf(_.ib('javascript:""')):_.nf(_.ib("about:blank"))};Cx.prototype.Z=function(){this.Ab.src!=_.Ud(Ex(this))&&(this.qe=!0,_.$h(this.Ab,!0),this.isVisible()&&this.focus())};Cx.prototype.U=function(a){27==a.keyCode&&(this.ha(!1),this.Oa({action:"cancel"}),a.stopPropagation(),a.preventDefault())};
var Hx=function(a,c){var d=a.ka;yx(function(){c(_.nq(d).gadgets.rpc)},d)},Ix=function(a,c){a.Oa=c;Hx(a,(0,_.t)(function(d){d.register(this.F,(0,_.t)(this.Kb,this))},a))};Cx.prototype.Kb=function(a){var c=a.action;"loaded"==c&&(this.df=!0,Jx(this,new Nw(this.isVisible())),Kx(this),nx(this),_.ch(this).Ba(_.nq(this.b),"keydown",this.U),_.$h(this.Ab,!0));"picked"!=c&&"cancel"!=c||this.ha(!1);this.Oa(a)};var Kx=function(a){a.ua&&Jx(a,new Mw(a.ua,window.location.protocol+"//"+window.location.host))};
Cx.prototype.setRelayUrl=function(a){Hx(this,(0,_.t)(function(c){c.setRelayUrl(this.F,a)},this))};var Jx=function(a,c){a.T&&Jw(c,a.S).then(null,function(){a.Oa({action:"error"})});Hx(a,(0,_.t)(function(d){d.call(this.F,"picker",null,c)},a))};
Cx.prototype.V=function(){var a=_.eg(this.b.b)||window;if("true"==_.Om(_.Pm(this.Tb),"ignoreLimits"))var c=new _.pe(this.Ga,this.va);else if("true"==_.Om(_.Pm(this.Tb),"shadeDialog")){c=_.Bq(ix(this),"margin");var d=_.dg(a);a=d.width-80;d=d.height-40;c&&(a-=c.left?c.left:0,a-=c.right?c.right:0,d-=c.top?c.top:0,d-=c.bottom?c.bottom:0);c=new _.pe(0<a?a:0,0<d?d:0)}else c=Bx(a,this.Ga,this.va);_.bo(this.Uc(),c);this.Vd()};
Cx.prototype.Vd=function(){if("true"==_.Om(_.Pm(this.Tb),"shadeDialog")){var a=_.Qg(this.C());a=Math.floor(_.dg(_.nq(this.b)).width/2-a.width/2);var c=_.Bq(ix(this),"margin");if(c){var d=c.left?c.left:0;d+=c.right?c.right:0;a=Math.floor(a-d/2)}a=0<a?a:0;c=_.lq(this.b.b).b;_.tq(this.C(),a,c)}else Cx.L.Vd.call(this)};
Cx.prototype.ha=function(a){if(a!=this.isVisible()&&this.Ma){var c=_.nq(this.b);a?(this.V(),_.ch(this).H(c,"resize",this.V),this.qe||_.ch(this).H(c,"keydown",this.U)):(_.ch(this).Ba(c,"resize",this.V),this.qe||_.ch(this).Ba(c,"keydown",this.U))}Cx.L.ha.call(this,a);Jx(this,new Nw(a))};Cx.prototype.focus=function(){Cx.L.focus.call(this);if(this.Ab&&this.qe&&this.df)try{this.Ab.focus()}catch(a){}};
var Mx=function(a){Nv.call(this,a);this.b=new Map;Lx(this,"gadgets");(a=window.location.origin)||(a=window.location.protocol+"//"+window.location.host);a&&this.b.set("origin",a);this.o=[]};_.w(Mx,tx);var Nx=function(a){a.b.set("profilePhoto","true");return a};Mx.prototype.getHeight=function(){return this.A};Mx.prototype.getRelayUrl=function(){return this.b.get("relayUrl")};
var Ox=function(a){a.b.set("actions","loaded");return a},Px=function(a,c){a.b.set("authuser",c);return a},Qx=function(a){a.b.set("hostId","og");return a},Rx=function(a,c){a.b.set("hl",c);return a},Sx=function(a,c){a.b.set("st",c);return a},Lx=function(a,c){a.b.set("protocol",c);return a};Mx.prototype.setRelayUrl=function(a){this.b.set("relayUrl",a);return this};var Tx=function(a,c){a.b.set("thumbs",c);return a};Mx.prototype.setTitle=function(a){this.b.set("title",a);return this};
var Ux=function(a){a.o.length&&a.b.set("pp",vu(a.o));a.b.set("nav",Lv(a.f));var c=new _.wm(a.w);a.b.forEach(function(f,g){_.Nm(c,g,f)});var d=Fw(a.w,a.f,a.b,a.o);if(null!==d){_.Nm(c,"amc","true");var e=!1;switch(a.b.get("hostId")){case "gmail-to":case "og":case "hangouts-profile-picture":case "testing":case "youtube-video-importer":case "ritz":case "punch":case "freebird-themes":case "freebird":case "atariImage":case "homeroom-doc-select":case "homeroom-doc-attach":e=!0}e&&_.Nm(c,"v2",Gw(d))}return c};
var Vx=function(a){Cv.call(this,"upload");this.f.query=a};_.w(Vx,Cv);Vx.prototype.b=function(a,c){Vx.L.b.call(this,a,c);return this};
var Wx=function(a,c){Cv.call(this,"webcam");a&&(this.f.type=a);c&&(this.f.query=c)};_.w(Wx,Cv);Wx.prototype.b=function(a,c){Wx.L.b.call(this,a,c);return this};
var Xx=function(a,c){this.b=a||new _.og;this.j=(0,_.t)(this.o,this);this.f=(0,_.t)(this.A,this);this.w=!!c};_.w(Xx,_.J);_.k=Xx.prototype;_.k.we=!1;_.k.Ra=null;_.k.Qa=null;_.k.Jb=null;_.k.ve=null;
var Yx=function(a){a.Ha();return a.ve},Zx=function(a,c,d){a.addEventListener?a.addEventListener(c,d,!1):a.attachEvent("on"+c,d)},$x=function(a,c,d){a.removeEventListener?a.removeEventListener(c,d,!1):a.detachEvent("on"+c,d)},by=function(a){a.Qa&&($x(a.Qa,"scroll",a.f),$x(a.Qa,ay(a),a.f))},ay=function(a){return"undefined"!=typeof _.nq(a.b).f?"DOMMouseScroll":"mousewheel"};
Xx.prototype.Ha=function(){if(!this.Ra){var a=this.b;this.Jb=a.wa("IFRAME",{frameborder:0,style:"border:0;left:0;position:absolute;top:0;vertical-align:bottom;z-index:1101",src:Ww});_.X(this.Jb,!1);Xt(this.Jb,0);this.Qa=a.wa("DIV",{style:"background:#fff;display:none;left:0;position:absolute;top:0;z-index:1101"});_.X(this.Qa,!1);Xt(this.Qa,.5);a=this.b;var c=this.Ra=a.wa("DIV",{style:"background:#fff;border:1px solid #bebebe;box-shadow:rgba(0,0,0,.2) 0 4px 16px;height:auto;overflow:hidden;position:absolute;width:auto;z-index:1101;-moz-box-shadow:rgba(0,0,0,.2) 0 4px 16px;-webkit-box-shadow:rgba(0,0,0,.2) 0 4px 16px",
name:"dialog"},this.ve=a.wa("DIV"));c.setAttribute("role","dialog");c.j="dialog";this.Ra.style.visibility="hidden";_.tq(this.Ra,-1E4,-1E4);a=a.b.body;a.appendChild(this.Jb);a.appendChild(this.Qa);a.appendChild(this.Ra)}};
Xx.prototype.ha=function(a){a!=this.we&&(this.Ra||this.Ha(),a?(cy(this),Zx(_.nq(this.b),"resize",this.j),this.Qa&&(Zx(this.Qa,"scroll",this.f),Zx(this.Qa,ay(this),this.f))):($x(_.nq(this.b),"resize",this.j),by(this)),_.X(this.Jb,a),_.X(this.Qa,a),a?dy(this):(this.Ra.style.visibility="hidden",_.tq(this.Ra,-1E4,-1E4)),(this.we=a)&&"hidden"==this.Ra.style.visibility&&(this.Ra.style.visibility="visible"),a?this.focus():this.w&&this.sa())};Xx.prototype.isVisible=function(){return this.we};
Xx.prototype.focus=function(){try{this.Ra.focus()}catch(a){}};var cy=function(a){_.X(a.Jb,!1);_.X(a.Qa,!1);var c=a.b.b,d=_.dg(_.eg(c)||window),e=Math.max(c.body.scrollWidth,d.width);c=Math.max(c.body.scrollHeight,d.height);_.X(a.Jb,!0);_.bo(a.Jb,e,c);_.X(a.Qa,!0);_.bo(a.Qa,e,c)};Xx.prototype.o=function(){cy(this);dy(this)};Xx.prototype.A=function(a){a.preventDefault?a.preventDefault():a.returnValue=!1;a.stopPropagation?a.stopPropagation():a.cancelBubble=!0};
var dy=function(a){var c=a.Ra,d=_.Qg(c),e=a.b;a=_.lq(e.b);e=_.dg(_.nq(e));_.tq(c,Math.max(a.x+(e.width-d.width)/2,0),Math.max(a.b+(e.height-d.height)/2,0))};Xx.prototype.P=function(){this.we&&($x(_.nq(this.b),"resize",this.j),by(this));this.Ra&&(_.Ae(this.Ra),this.Ra=null);this.Qa&&(_.Ae(this.Qa),this.Qa=null);this.Jb&&(_.Ae(this.Jb),this.Jb=null)};
var ey=function(a){this.b=a},fy=function(a){a=a.getOpenParams().onepick_dialog;if(!a)throw Error("Oa");return a};
ey.prototype.j=function(a){var c=a.getOpenParams(),d=new Xx(this.b,c.disposeOnHide);c.onepick_dialog=d;d.Ha();c=Bx(_.nq(this.b),c.width,c.height);var e=c.width,f=c.height;"string"===typeof e&&"string"===typeof f?(c=_.dg(_.nq(d.b)),e=parseFloat(e)/100,f=parseFloat(f)/100,_.Jg(d.Ra,"padding","1px"),_.bo(d.Ra,c.width*e,c.height*f),_.bo(d.ve,"100%","100%")):_.bo(d.ve,e,f);dy(d);d.ha(!0);a.openInto(Yx(d),{allow:"camera",style:"border:0;height:100%;overflow:hidden",allowtransparency:"true"})};
ey.prototype.f=function(a){fy(a).ha(!1)};
var gy=!1,hy="",iy=function(a){a=a.match(/[\d]+/g);if(!a)return"";a.length=3;return a.join(".")};
(function(){if(navigator.plugins&&navigator.plugins.length){var a=navigator.plugins["Shockwave Flash"];if(a&&(gy=!0,a.description)){hy=iy(a.description);return}if(navigator.plugins["Shockwave Flash 2.0"]){gy=!0;hy="2.0.0.11";return}}if(navigator.mimeTypes&&navigator.mimeTypes.length&&(a=navigator.mimeTypes["application/x-shockwave-flash"],gy=!(!a||!a.enabledPlugin))){hy=iy(a.enabledPlugin.description);return}if("undefined"!=typeof ActiveXObject){try{var c=new ActiveXObject("ShockwaveFlash.ShockwaveFlash.7");
gy=!0;hy=iy(c.GetVariable("$version"));return}catch(d){}try{c=new ActiveXObject("ShockwaveFlash.ShockwaveFlash.6");gy=!0;hy="6.0.21";return}catch(d){}try{c=new ActiveXObject("ShockwaveFlash.ShockwaveFlash"),gy=!0,hy=iy(c.GetVariable("$version"))}catch(d){}}})();var jy=hy;
var ky=function(){_.J.call(this);this.f=new _.Q};_.w(ky,_.J);ky.prototype[_.Oe]=!0;_.k=ky.prototype;_.k.H=function(a,c,d,e){return this.f.H(a,c,d,e)};_.k.nb=function(a,c,d,e){return this.f.nb(a,c,d,e)};_.k.Ba=function(a,c,d,e){return this.f.Ba(a,c,d,e)};_.k.ye=function(a){return this.f.ye(a)};_.k.dispatchEvent=function(a){return this.f.dispatchEvent(a)};_.k.re=function(a){return this.f.re(a)};_.k.vd=function(){return this.f.vd()};_.k.Pc=function(a,c,d){return this.f.Pc(a,c,d)};
_.k.Rc=function(a,c){return this.f.Rc(a,c)};_.k.Dc=function(a,c,d,e){return this.f.Dc(a,c,d,e)};_.k.hasListener=function(a,c){return this.f.hasListener(a,c)};
var ny=function(a,c,d,e,f,g){var h=this;_.J.call(this);this.Ga=e;this.zc=f;this.j=g;this.ua=a;this.b=_.M("gb_ag",a);this.Y=_.rh("gb_pb");this.K=_.M("gb_9b",a);this.Ub=_.L(_.B(c,20));this.Ma=_.L(_.B(c,16));this.w=new _.Dh(e,this);_.ph(this.w,this.K,function(){return h.j(16)});_.B(c,1);_.B(c,4);this.Ja=_.L(_.B(c,2));this.$a=_.L(_.B(c,45));this.Kb=_.L(_.B(c,46));this.Vb=_.L(_.B(c,24));this.Fb=_.L(_.B(c,39));this.tb=_.L(_.B(c,43));this.Z=_.R(this.b,"gb_Nb");this.W=_.L(_.B(c,27));this.V=_.L(_.B(c,28));
this.jd=_.K(_.C(c,3));this.hd=_.K(_.C(c,22));this.O=!1;this.jc=_.K(_.C(c,5));this.o=_.K(_.C(c,32));if(this.F=_.K(_.C(c,33)))this.D=_.M("gb_dg");this.S=this.U=!1;this.ma=_.yl(_.L(_.B(c,13)));this.hc=_.L(_.B(d,6));this.Ac=_.L(_.B(d,7));this.Aa=_.L(_.B(c,8));this.qc=_.B(c,21)||this.Aa;this.qd=_.L(_.B(c,25));this.nd=_.yl(_.L(_.B(c,26)));this.B=[];this.f=[];this.T=!1;this.A=null;this.R={};ly(this);this.M=!1;this.J=null;this.$=_.K(_.C(c,14));this.bc=_.L(_.B(c,15));this.X=!1;this.va="";this.ka=2E4;this.yc=
c;this.G=this.N=null;my(this);this.rd=_.K(_.C(c,29))&&!1};_.w(ny,_.J);ny.prototype.P=function(){ny.L.P.call(this);delete this.b;delete this.K;this.B=null;this.f=[];this.w.sa()};
var oy=/.*?\/(\d{6,})\/(?:\1\/)*(.*\/?)/,sy=function(a,c,d){_.ag(a.b,_.Gb);a.B=[];py(a,c,d);qy(a);ry(a,!1);a.O=!1},py=function(a,c,d){if(a.o)if(d){if(0!=a.f.length)for(c=a.f,a.f=[],d=0;d<c.length;d++)ty(a,c[d])}else a.f=[],null!=c&&a.o&&a.M&&(c?uy(a):a.T=!0);else a.f=[]},By=function(a,c){var d=2==c.type,e=3==c.type,f=c.name||c.email;e&&(f=c.email);var g=c.email;e&&(g=a.tb);var h=d?c.email:g,l=c.Dg;e||c.We?l=vy(a):l?a.R[h]=l:l=a.R[h]?a.R[h]:vy(a);h=_.ve("IMG",{"class":"gb_1b gb_hb",src:l,alt:2==c.type?
a.Ma:a.Ub});h.setAttribute("aria-hidden","true");h.setAttribute("alt","");l=_.ve("DIV","gb_3b",f);f="gb_5b";c.Pb&&(f+=" gb_6b");g=_.ve("DIV",{"class":f,dir:"ltr"},g);f=[];f.push(l);d||f.push(g);c.Pb&&(null==a.N&&(a.N=_.M("gb_Bb",a.ua)),null!=a.N&&f.push(a.N.cloneNode(!0)));l=[];var m=g=null;if(c.Md){var n=wy(a.Fb);f.unshift(n)}else if(c.Pb){g=wy(a.Vb);f.unshift(g);n=_.ve("BUTTON",["gb_Ub","gb_Xb","gb_Vb"],a.W);n.setAttribute("aria-hidden","true");n.setAttribute("aria-label",a.W);n.setAttribute("role",
"button");var r=xy(a);g=r;m=_.ve("DIV","gb_8b");a.w.H(n,"click",(0,_.t)(a.md,a,c.email));m.appendChild(r);m.appendChild(n);yy(a,n);yy(a,r)}else d?f.unshift(wy(a.Ja)):c.We?f.unshift(wy(a.Kb)):c.Ve&&f.unshift(wy(a.$a));f=_.ve("DIV","gb_Rb",f);l.push(h);l.push(f);l.push(m);h=_.ve(c.Pb?"DIV":"A","gb_Ob",l);c.Pb?(a.w.H(h,"click",a.od),h.setAttribute("tabindex","0"),h.setAttribute("role","group"),h.setAttribute("aria-haspopup","true"),h.setAttribute("aria-expanded","false")):g=h;c.Pb?(a.w.H(h,"keydown",
a.mc),_.S(h,"gb_Mb")):zy(a,h,c.Md?3:1);if(f=c.rg)a.$&&2==c.type&&(m=c.id,l=f.match(oy))&&(m=m||l[1],n=l[2],r=window.location.href,f=(l=r.match(oy))?r.replace(new RegExp(l[1],"g"),m):f.replace(n,a.bc)),_.qh(g,f);if(f=(f=2==c.type?a.hd:a.jd)||a.$&&2==c.type)g.target="_blank",_.oc&&(g.rel="noreferrer");e&&_.S(h,"gb_4b");d&&_.S(h,"gb_2b");if(c.og&&((d=_.M("gb_Zb",a.b))&&Ay(d,!1),Ay(h,!0),c.name))for(d=0;d<a.Y.length;d++)e=_.fq(c.name),_.ag(a.Y[d],e);return h},vy=function(a){return a.Z?"https://ssl.gstatic.com/gb/images/gm_silhouette_dark_mode_32.png":
"https://ssl.gstatic.com/gb/images/gm_silhouette_32.png"},Ay=function(a,c){_.U(a,"gb_Zb",c);a.setAttribute("aria-hidden",c?"true":"false")},my=function(a){(0,_.Ma)(a.ua.getElementsByClassName("gb_Ob"),(0,_.t)(function(c){zy(this,c,1)},a))},zy=function(a,c,d){_.ph(a.w,c,function(){return a.j(4,d,2!=d)})},wy=function(a){return _.ve("DIV","gb_7b",a)},xy=function(a){var c=_.ve("A",["gb_Ub","gb_Wb","gb_Vb"],a.V);c.setAttribute("aria-hidden","true");c.setAttribute("aria-label",a.V);c.setAttribute("role",
"link");_.ph(a.w,c,function(){return a.j(6,2,!0)});return c},yy=function(a,c){a.w.H(c,_.Xg(27)?"keypress":"keyup",a.lc)},Cy=function(a,c,d,e){e&&a.o&&0!=a.f.length?a.b.insertBefore(c,_.M("gb_Mb",a.b)):a.b.appendChild(c);a.B.push(c);qy(a);2==d&&(a.O&&ry(a,!0),a.O=!0)},ry=function(a,c){_.U(a.K,"gb_Fa",!c);a.K.setAttribute("aria-hidden",!c+"")},ly=function(a){for(var c=_.rh("gb_Ob",a.b),d=0;d<c.length;d++){var e=_.M("gb_5b",c[d]),f=_.M("gb_1b",c[d]);e&&f&&(e=_.bi(e),a.R[e]=f.getAttribute("data-src")||
f.src)}},qy=function(a){var c=a.b.children.length;c=0==c||1==c&&_.R(a.b.firstChild,"gb_Zb");_.U(a.b,"gb_Fa",c);a.b.setAttribute("aria-hidden",c+"")},uy=function(a){!a.jc||a.M&&!a.o||(Dy(a,!0,!0),a.M||_.Ch(a.Ga,window,"message",(0,_.t)(a.kc,a)),Ey(a),a.J=Fy(a,a.ma),a.M=!0)},Gy=function(){return window.location.origin||window.location.protocol+"//"+window.location.host};
ny.prototype.kc=function(a){if(0==this.f.length||!this.o){a=a.ab;var c=_.Ud(this.ma),d=a.origin;c=c.match(_.hk);d=d.match(_.hk);if(c[3]==d[3]&&c[1]==d[1]&&c[4]==d[4])try{b:{var e=a.data;if(e){a=null;try{a=new zv(e?JSON.parse(e):null)}catch(h){var f=null;break b}f=_.Zj(a,xv,1)}else f=null}if(f&&0!=f.length){this.o||sy(this);for(e=0;e<f.length;++e)ty(this,f[e]);var g=!0}else g=!1;g&&(this.T=!1,Dy(this,!1,!0),this.X&&Hy(this,this.va,!0),Ey(this))}catch(h){this.Ga.log(Error("Pa`"+(h.name?h.name:"")))}}};
var ty=function(a,c){var d={valid:!1};if(c){d.type=_.B(c,1);d.email=_.L(_.B(c,3));d.Ve=_.K(_.C(c,6));d.Pb=_.K(_.C(c,14));d.We=!1;d.name=_.L(_.B(c,2));d.id=_.L(_.B(c,10));d.Dg=_.L(_.B(c,4));d.Md=!_.K(_.C(c,14))&&!_.K(_.C(c,9));var e=_.B(c,7);e=null!=e?e.toString():"";var f=2==d.type,g=f?d.id:"none";d.og=f?a.Ac==g:a.hc==d.email;e=(f?a.qc:a.Aa).replace("$authuser",e).replace("$session_index",e).replace("$pageId",g).replace("$email",d.email);var h=new _.wm(Gy());f=new _.wm(e);g=new _.wm(h);var l=!!f.j;
l?_.xm(g,f.j):l=!!f.D;l?g.D=f.D:l=!!f.f;l?_.ym(g,f.f):l=null!=f.B;var m=f.o;if(l)_.zm(g,f.B);else if(l=!!f.o)if("/"!=m.charAt(0)&&(h.f&&!h.o?m="/"+m:(h=g.o.lastIndexOf("/"),-1!=h&&(m=g.o.substr(0,h+1)+m))),h=m,".."==h||"."==h)m="";else if(-1!=h.indexOf("./")||-1!=h.indexOf("/.")){m=_.$d(h,"/");h=h.split("/");for(var n=[],r=0;r<h.length;){var v=h[r++];"."==v?m&&r==h.length&&n.push(""):".."==v?((1<n.length||1==n.length&&""!=n[0])&&n.pop(),m&&r==h.length&&n.push("")):(n.push(v),m=!0)}m=n.join("/")}else m=
h;l?_.Am(g,m):l=""!==f.b.toString();l?_.Bm(g,_.Cm(f.b)):l=!!f.w;l&&_.Dm(g,f.w);f=g.toString();d.rg=d.Md&&3==d.type?_.Nm(_.Nm(_.Nm(new _.wm("https://accounts.google.com/signin/collaboratoraccount"),"source","ogb"),"continue",f),"atu",_.B(c,10)).toString():d.Pb||d.Md?a.qd.replace("$continue",_.fk(f)).replace("$email",_.fk(d.email)):e;d.valid=!0}!d.valid||a.o&&!d.Pb||(e=By(a,d),d.Pb?a.f.push(c):d.Ve||a.G&&a.G(),Cy(a,e,d.type))};
ny.prototype.md=function(a,c){var d=_.uh(c.target,"gb_Ob");_.Ae(d);qy(this);a=Fy(this,Vt(this.nd,{Email:a}));_.rg((0,_.t)(this.kd,this,a),this.ka,this);this.j(7,2);c.preventDefault();c.stopPropagation()};var Fy=function(a,c){var d={origin:Gy()};a=_.B(a.yc,38);"number"===typeof a&&(d.ts=a);c=Vt(c,d);c=_.ve("IFRAME",{width:0,height:0,frameborder:0,"class":"gb_Fa",src:_.Ud(c)});document.body.appendChild(c);return c};
ny.prototype.mc=function(a){var c=a.target;if(32==a.keyCode||13==a.keyCode){if(_.R(c,"gb_Ub")){c.click();a.preventDefault();a.stopPropagation();return}Iy(this,a,c)}27==a.keyCode&&null!=c.getAttribute("selected")&&(this.j(5,2),Jy(this))};ny.prototype.lc=function(a){27==a.keyCode&&(this.A.focus(),this.j(5,2),Jy(this),a.preventDefault(),a.stopPropagation())};ny.prototype.od=function(a){if(!_.R(a.target,"gb_Ub")){var c=a.b;null!=c&&Iy(this,a,c)}};
var Iy=function(a,c,d){var e=null!=d.getAttribute("selected");Jy(a);e?a.j(5,2):(d.setAttribute("selected","true"),a.A=d,d.setAttribute("aria-expanded","true"),d.focus(),Ky(d,!1),a.j(4,2));c.preventDefault();c.stopPropagation()},Ky=function(a,c){(0,_.Ma)(_.gg(_.M("gb_8b",a)),function(d){var e=_.R(d,"gb_Ub");d.setAttribute("aria-hidden",e?c:!c)})},Jy=function(a){null!=a.A&&(a.A.removeAttribute("selected"),a.A.setAttribute("aria-expanded","false"),Ky(a.A,!0),a.A=null)},Ly=function(a,c){var d=_.Pm(a);
c=_.Pm(c);for(var e=["authuser","pageId","Email"],f=0;f<e.length;f++){var g=e[f],h=_.Om(d,g);h?_.Nm(c,g,h):"authuser"==g&&(g=/\/u\/(\d+)[/$]/.exec(a))&&1<g.length&&(c=_.Pm(c.toString().replace(/\/u\/(\d+)/,"/u/"+g[1])))}return c.toString()},Hy=function(a,c,d){d||(a.va=c,a.X=!0);a=_.rh("gb_Ob",a.b);for(d=0;d<a.length;d++){var e=a[d];var f=c;if(e.href){var g=e.getAttribute("href"),h=/.*signin\/collaboratoraccount.*/.test(g);/.*AccountChooser.*/.test(g)||h?(g=_.Pm(g),h=_.Pm(_.Om(g,"continue")),f=_.Pm(f),
f.f||(_.xm(f,h.j),_.ym(f,h.f)),f=Ly(h.toString(),f.toString()),f=_.Nm(g,"continue",f).toString()):f=Ly(g,f);_.qh(e,f)}}},Dy=function(a,c,d){d?a.S=c:a.U=c;a.F&&a.D&&(c=!a.S&&!a.U,!c&&_.R(a.D,"gb_Fa")&&_.rg(a.nc,2E4,a),a.F&&a.D&&_.U(a.D,"gb_Fa",!!c))};ny.prototype.nc=function(){this.F&&this.D&&_.U(this.D,"gb_Fa",!0);this.U=this.S=!1;Ey(this)};ny.prototype.kd=function(a){null!=a&&_.Ae(a)};var Ey=function(a){null!=a.J&&(_.Ae(a.J),a.J=null)};
var My=function(a,c,d,e){this.A=a;this.url=c;this.B=d;this.G=e||0;this.f=0;this.j=[]};My.prototype.Nb=function(){return this.f};var Ny=function(a,c){a.f=c;if(3==c||5==c){for(c=0;c<a.j.length;c++)try{a.j[c]()}catch(d){a.B.log(d)}a.j=[]}};My.prototype.wf=function(){};My.prototype.Rf=function(){return{}};My.prototype.Sf=function(){return{}};My.prototype.Pe=function(){};
var Oy=function(a,c){_.Le.call(this,a);this.Ta=c};_.p(Oy,_.Le);
/*

 Copyright The Closure Library Authors.
 SPDX-License-Identifier: Apache-2.0
*/
var Qy=function(a,c,d,e,f,g){var h=_.pg(window);this.M=a;this.F=c;this.D=d;this.K=e;this.J=g;this.b={};My.call(this,"onepick",Ux(Py(this,h)).toString(),f);a=new ey(h);c=this.b;c.onOpen=(0,_.t)(a.j,a);c.onClose=(0,_.t)(a.f,a)};_.w(Qy,My);
var Py=function(a,c){var d=a.K.join("-c,")+"-c",e=Ox(Lx(Ov(Ov(Qx(Nx(new Mx)),(new Vx("profile")).b("silo_id","48")),new Fv),"iframes"));e.j=c;c=Sx(Px(Rx(Tx(e,d),a.M),a.F),a.J);a.D&&c.b.set("groupId",a.D);0<=_.Ta(jy,"10.1")&&Ov(c,(new Wx("profile","profile")).b("silo_id","48"));return c};_.k=Qy.prototype;_.k.Sf=function(){return{message:(0,_.t)(this.Pe,this)}};_.k.Pe=function(a){this.Sa.dispatchEvent(new Oy("message",[a]))};
_.k.Rf=function(){return{onOpen:(0,_.t)(this.zi,this),onReady:(0,_.t)(this.Ai,this),onClose:(0,_.t)(this.yi,this)}};_.k.wf=function(a){this.Sa=a};_.k.zi=function(a){var c=document.activeElement;null!=c&&(this.w=c);this.o=a;this.b.onOpen&&this.b.onOpen(a)};_.k.Ai=function(){Ny(this,3)};_.k.yi=function(a){this.b.onClose&&this.b.onClose(a);null!=this.w&&this.w.focus()};
var Ry=function(a,c,d,e,f,g,h,l,m,n,r){_.J.call(this);this.f=a;this.G=d;this.K=c;this.R=e;this.B=g;this.N=h;this.b=l;this.o=m;this.O=n;this.M=r;this.A=new _.Dh(f,this);this.F=_.K(_.C(this.b,41));this.F||(this.w=_.Xc("op"),this.A.H(this.w,"message",this.J))};_.w(Ry,_.J);Ry.prototype.P=function(){Ry.L.P.call(this);this.f&&delete this.f;delete this.G;this.A.sa()};
Ry.prototype.T=function(a){var c=this.w.b.o;if(c){var d=fy(c);if(d&&(d.ha(a),a&&(this.B.log(34),(a=c.getIframeEl())&&a.contentWindow)))try{a.focus(),a.contentWindow.focus()}catch(e){}}};Ry.prototype.J=function(a){this.D(a.Ta[0])};
Ry.prototype.D=function(a){var c=a.action;if("picked"==c){a=a.docs[0].thumbnails;(c=Sy(a,this.K))&&this.f&&(this.f.style.backgroundImage="url("+c+")");if(a=Sy(a,this.R))this.G.style.backgroundImage="url("+a+")";this.j&&this.j.ha(!1);this.B.log(35);Ty(this,12)}else"cancel"==c&&Ty(this,13)};
var Sy=function(a,c){for(var d=0;d<a.length;d++)if(a[d].height==c)return a[d].url;return null},Ty=function(a,c){var d=new _.ao,e=a.M.ya();_.F(d,1,e);e=new hu;iu(e,c);c=new _.Cc;_.I(c,37,d);_.I(c,35,e);a.N.log(97,c)};
var Vy=function(a,c,d,e,f,g,h){this.A=c;this.K=d;this.va=e;this.D=null;var l;_.C(this.A,35)&&(l=a);_.io.call(this,a,"gbd4",f,g,h,!0,l);this.X=this.V=!1;this.Ma=_.K(_.C(this.A,48),!1);this.S=_.L(_.B(c,47));(this.N=_.K(_.C(this.A,30),!1))&&_.K(_.C(this.K,3))&&Uy(this,!1);this.J=5;this.Aa=79;this.ma=80;this.Wc()};_.w(Vy,_.io);
var Wy={method:"POST",path:"https://people-pa.googleapis.com/v2/people:batchGet",body:{personId:"me",requestMask:{includeField:{paths:"person.photo"},includeContainer:"PROFILE"},extensionSet:{extensionNames:"ABOUT_ME_ADDITIONAL_DATA"},mergedPersonSourceOptions:{includedProfileStates:"CORE_ID"}}};_.k=Vy.prototype;_.k.P=function(){Vy.L.P.call(this);this.F&&this.F.sa();this.R&&this.R.sa()};
_.k.hi=function(){null!=this.D&&(this.D.setAttribute("src","https://www.gstatic.com/images/icons/material/system/1x/broken_image_grey600_18dp.png"),this.D.setAttribute("srcset","https://www.gstatic.com/images/icons/material/system/1x/broken_image_grey600_18dp.png 1x, https://www.gstatic.com/images/icons/material/system/2x/broken_image_grey600_18dp.png 2x"),_.Jg(this.D,"width",""),_.S(this.D.parentElement,"gb_qa"),_.Jg(this.D.parentElement,"line-height","30px"))};
_.k.close=function(a,c,d){this.F&&Jy(this.F);return Vy.L.close.call(this,a,c,d)};
_.k.Te=function(){Vy.L.Te.call(this);var a=_.M("gb_7f",this.b);a&&_.ph(this,a,(0,_.t)(this.Di,this));(a=_.M("gb_3f",this.b))&&_.ph(this,a,(0,_.t)(this.Zh,this));(a=_.M("gb_8f",this.b))&&_.ph(this,a,(0,_.t)(this.Ii,this));(a=_.M("manageAccountsButton",this.b))&&_.ph(this,a,(0,_.t)(this.vi,this));(a=_.M("gb_Kb",this.b))&&_.ph(this,a,(0,_.t)(this.Ci,this));(a=_.M("gb_Jb",this.b))&&_.ph(this,a,(0,_.t)(this.Ki,this));(a=_.M("gb_ab"))&&_.ph(this,a,(0,_.t)(this.ti,this))};
_.k.Wc=function(){Vy.L.Wc.call(this);this.j&&this.o(this.j,"focus",this.Ni,!1,this);_.C(this.A,35)&&(this.D=_.M("gb_ra",this.j),this.o(this.D,"error",this.hi,!1,this))};_.k.Yd=function(a){try{Xy(this)}catch(c){}this.B.log(_.R(a.target,"gb_Ka")?42:43);Vy.L.Yd.call(this,a)};
var Xy=function(a){_.C(a.A,12)&&a.N&&(a.V||_.K(_.C(a.K,3))&&_.C(a.A,31)&&_.He("gapi.load")("client",(0,_.t)(function(){var c=_.He("gapi.config.update");c("googleapis.config/auth/useFirstPartyAuth",!0);c("googleapis.config/auth/useFirstPartyAuthV2",!0);c("client/cors",!0);_.He("gapi.client.request")(Wy).then(this.Bi,this.Nj,this);this.V=!0},a)))};_.k=Vy.prototype;
_.k.Bi=function(a){a=a.result.personResponse;0!=a.length&&(a=a[0],null!=a&&(a=a.person.extendedData.aboutMeExtendedData.profileEditability.lockedField,null!=a&&-1!=a.indexOf("person.photo")||Yy(this)))};_.k.Nj=function(){this.w.log(Error("Qa"))};_.k.Ni=function(){Zy(this)};_.k.Di=function(){this.B.log(10);$y(this,8)};_.k.Ci=function(){az(this,2)};_.k.Ki=function(){az(this,1)};_.k.ti=function(){az(this,3)};_.k.Zh=function(){this.B.log(48);$y(this,9)};
_.k.Ii=function(a){this.B.log(9,{l:"o"});var c=bz(this),d=!1;c&&(d=!_.R(c.b,"gb_Fa"));c=d;a=(a=a.target)?_.bi(a)==this.S?2:1:0;d=iu(new hu,10);c=_.F(d,6,c);c=_.F(c,5,a);cz(this,c,!0)};_.k.vi=function(){this.B.log(49)};_.k.Oe=function(a,c){Vy.L.Oe.call(this,a,c);1==a&&dz(this)};_.k.wc=function(a){_.He("silk.s.sis.ca")&&_.po(this,106,void 0,!1);dz(this);Vy.L.wc.call(this,a);this.X||(this.X=!0,a=_.M("gb_vb"),null!=a&&24<_.Qg(a).height&&_.S(_.M("gb_Qa",a),"gb_Ha"))};
var bz=function(a){if(!a.F){var c=_.M("gb_Ib",a.b);c&&(a.F=new ny(c,a.A,a.K,a.w,a.B,(0,_.t)(a.Y,a)),a.Ma||(c=(0,_.t)(a.Ja,a),a.F.G=c))}return a.F};Vy.prototype.Y=function(a,c,d){d=void 0===d?!1:d;a=iu(new hu,a);c&&_.F(a,2,c);cz(this,a,d)};Vy.prototype.Ja=function(){var a=_.M("gb_8f",this.b);a&&(_.ig(a,this.S),this.F.G=null)};
var dz=function(a){var c=bz(a);a.ka?null!=c&&c.o&&c.T&&uy(c):(a.ka=!0,null!=c&&uy(c),a.N&&_.K(_.C(a.K,3))||Yy(a),Zy(a))},Yy=function(a){if(_.C(a.A,12)){var c=_.M("gb_6f",a.b);if(c){try{if(window.location.host!=top.location.host)return}catch(h){return}var d=_.M("gb_Ia",a.f),e=_.Mc(_.E(a.A,6,30)),f=_.M("gb_Ja",a.b),g=_.Mc(_.E(a.A,7,96));a.R=new Ry(d,e,f,g,a.w,a.B,a.G,a.A,a.K,a.va,a.$);_.ph(a,c,a.ua);Uy(a,!0)}}},Uy=function(a,c){var d=_.M("gb_Wa",a.b);d||(d=_.M("gb_mb",a.b));_.U(d,"gb_Ha",!c)};
Vy.prototype.ua=function(a){var c=this.R;if(c.F){if(!c.j){var d=[_.E(c.b,6,30),_.E(c.b,7,96)].join("-c,")+"-c",e=_.L(_.B(c.O,5)),f=new Mx(_.L(_.B(c.b,42))),g=Ox(Lx(Ov(Ov(Qx(Nx(f)),(new Vx("profile")).b("silo_id","48")),new Fv),"gadgets")),h=_.pg(window);g.j=h;d=Sx(Px(Rx(Tx(g,d),e),_.L(_.B(c.o,5))),_.B(c.b,36)||"");e=(0,_.t)(c.D,c);d.Oa=e;_.B(c.o,7)&&(d=_.L(_.B(c.o,7)),f.b.set("groupId",d));0<=_.Ta(jy,"10.1")&&Ov(f,(new Wx("profile","profile")).b("silo_id","48"));f.getRelayUrl()||f.setRelayUrl(_.Am(_.Dm(_.Bm(_.Pm(window.location.href),
void 0),""),"/favicon.ico").toString());if(f.b.get("minimal"))throw Error("Na");d=new Cx(Ux(f).toString(),!0,f.j,f.B,f.A,"",void 0);d.Zf=!1;d.ua=f.D;d.df&&Kx(d);Ix(d,f.Oa);c.j=d}c=c.j;c.ha(!0)}else if(f=c.w,c=(0,_.t)(c.T,c,!0),4!=f.b.Nb())if(f.w(),f=f.b,3==f.f||5==f.f)try{c()}catch(l){f.B.log(l)}else f.j.push(c);$y(this,11,!1);a.preventDefault()};
var Zy=function(a){if(a.b&&!a.b.hasAttribute("img-loaded")){for(var c=a.b.getElementsByTagName("img"),d=0,e;e=c[d];d++)e.hasAttribute("data-src")&&(e.setAttribute("src",e.getAttribute("data-src")),e.removeAttribute("data-src"));a.b.setAttribute("img-loaded","1")}};_.k=Vy.prototype;
_.k.mj=function(a,c,d,e,f,g,h,l,m,n){var r=bz(this);r.zc.log(44,{n:"paa"});n=n?2:1;c=By(r,{email:f,id:"",og:a,Ve:c,We:d,Pb:!1,rg:g?h||"":"",name:e||"",Dg:m||"",type:n});l&&(l["class"]&&(_.mh(c,l["class"].split(" ")),delete l["class"]),delete l.href,"_blank"==c.target&&delete l.target,_.te(c,l));g||_.S(c,"gb_0b");a||r.G&&r.G();Cy(r,c,n,!0)};_.k.oj=function(a){sy(bz(this),this.Rb(),a)};
_.k.nj=function(a){for(var c=bz(this),d=this.Rb(),e=0;e<c.B.length;e++)_.Ae(c.B[e]);c.B=[];py(c,d,a);qy(c);ry(c,!1);c.O=!1};_.k.Fg=function(a){if(a){for(var c=[_.M("gb_3f"),_.M("gb_gg")],d=0;d<c.length;d++){var e=c[d];null!=e&&_.Kh(e,a)}(c=bz(this))&&Hy(c,a)}};_.k.rj=function(a){var c=bz(this);c&&Dy(c,a)};_.k.sk=function(a){_.C(this.A,35)&&(_.U(this.j,"gb_ja",a),_.U(_.M("gb_la",this.j),"gb_ja",a),_.U(_.M("gb_oa",this.j),"gb_ja",a),_.U(this.D,"gb_ja",a))};
_.k.qj=function(a){_.U(this.b,"gb_6a",a);var c=bz(this);if(c){var d=_.rh("gb_Ob",c.b);c.Z=a;for(c=0;c<d.length;c++){var e=_.M("gb_1b",d[c]),f=e.src;("https://ssl.gstatic.com/gb/images/gm_silhouette_32.png"===f||"https://ssl.gstatic.com/gb/images/gm_silhouette_dark_mode_32.png"===f)&&(a?e.setAttribute("src","https://ssl.gstatic.com/gb/images/gm_silhouette_dark_mode_32.png"):e.setAttribute("src","https://ssl.gstatic.com/gb/images/gm_silhouette_32.png"))}}void 0==this.U&&(this.U=_.M("gb_8a",this.b));
null!=this.U&&_.U(this.U,"gb_9a",a)};var $y=function(a,c,d){d=void 0===d?!0:d;c=iu(new hu,c);cz(a,c,d)},az=function(a,c){var d=iu(new hu,14);c=_.F(d,3,c);cz(a,c,!0)},cz=function(a,c,d){d=void 0===d?!1:d;var e=_.R(a.b,"gb_6a"),f=new _.Cc;c=_.I(f,35,c);e=_.F(c,36,e);_.po(a,97,e,void 0===d?!1:d)};
var ez=function(a){_.A(this,a,0,-1,null,null)};_.w(ez,_.z);
var fz=function(a,c,d){ky.call(this);this.b=a;this.j=d;this.B=!1;this.G=_.Mc(_.E(c,12,3E4));this.o=[];this.b.wf(this);0<this.b.G&&window.setTimeout((0,_.t)(this.w,this),1E3*this.b.G)};_.p(fz,ky);fz.prototype.w=function(){this.B?gz(this):0==this.b.Nb()&&Ny(this.b,1)};fz.prototype.A=function(a,c){window.clearTimeout(this.D);var d=_.Dg(arguments,1);this.dispatchEvent("ifs.onready");a&&a.apply(null,d)};
var gz=function(a){try{if(!a.b.o){Ny(a.b,2);var c=a.b.Rf();c.open=(0,_.t)(a.A,a,c.open);c.onready=(0,_.t)(a.A,a,c.onready);iframes.setHandler(a.b.A,c);var d=iframes.open(a.b.url,{style:a.b.A},a.b.Sf(),{},(0,_.t)(a.b.Pe,a.b));a.b.o=d;0<a.G&&(window.clearTimeout(a.D),a.D=window.setTimeout((0,_.t)(a.dispatchEvent,a,"ifs.ontimeout"),a.G))}}catch(e){a.j.log(new hz(a.b))}};
fz.prototype.F=function(){try{this.B=!0;1==this.b.Nb()&&gz(this);for(var a=0;a<this.o.length;a++)try{this.o[a]()}catch(c){this.j.log(c)}this.o=null}catch(c){this.j.log(c)}};fz.prototype.init=function(a){try{var c=(0,_.t)(this.F,this);_.wo(a.b,c,null,void 0)}catch(d){this.j.log(d)}return this};var hz=function(){_.Ka.call(this)};_.p(hz,_.Ka);
var jz;jz=_.M("gb_Pa");
if(null!=jz){var kz=_.H(_.ud,Wt,7)||new Wt;_.C(kz,35)&&(jz=_.M("gb_ia",void 0));var lz=_.wd()||new _.Fc,mz;mz=_.C(kz,34);if(!_.K(mz)){var nz=_.vd()||new _.Ec,oz=new Vy(jz,kz,lz,nz,_.yd,_.zd,_.on),pz=new Qy(_.L(_.B(nz,5)),_.L(_.B(lz,5)),_.L(_.B(lz,7)),[_.E(kz,6,30),_.E(kz,7,96)],_.yd,_.B(kz,36)||""),qz=new ez;_.F(qz,12,3E4);var rz=new fz(pz,qz,_.yd);rz.init(_.Do);_.Zc("op",rz);var sz=_.M("gb_3a"),tz=_.M("gb_ee");sz&&(_.ho(oz,sz,!_.uj),_.uj&&_.$n(_.uj,sz));var uz;if(uz=oz.j){var vz;tz&&(vz=new _.Er(uz,
tz),_.ko(oz,vz))}_.iz=oz;_.Ti();_.u("gbar.Q",Vy);Vy.prototype.qa=Vy.prototype.Fg;Vy.prototype.qb=Vy.prototype.rj;_.rd(_.sd.ta().b,oz)}}
;
}catch(e){_._DumpException(e)}
try{
var Sp=function(a){_.A(this,a,0,-1,null,null)},Up;_.w(Sp,_.z);_.Tp=function(a,c){this.f=a;this.b=c};_.Tp.prototype.log=function(a,c){c=void 0===c?new _.Cc:c;Up(this,a,c)};_.Vp=function(a,c,d){d=void 0===d?new _.Cc:d;var e=a.b?103:14;_.F(d,18,c);Up(a,e,d)};_.Wp=function(a,c,d){d=void 0===d?new _.Cc:d;var e=a.b?94:8,f=new Sp;_.F(f,1,c);_.I(d,47,f);Up(a,e,d)};Up=function(a,c,d){var e=_.H(d,Sp,47)||new Sp;_.I(d,47,e);a.f.log(c,d)};

}catch(e){_._DumpException(e)}
try{
var Nz=function(a,c){if(Iz.test(c))return c;c=0<=c.indexOf("left")?c.replace(Jz,"right"):c.replace(Kz,"left");_.Qa(Lz,a)&&(a=c.split(Mz),4<=a.length&&(c=[a[0],a[3],a[2],a[1]].join(" ")));return c},Oz=function(a){_.A(this,a,0,-1,null,null)},Pz;_.w(Oz,_.z);Pz=[1];_.Qz=function(a){_.A(this,a,0,-1,Pz,null)};_.w(_.Qz,_.z);var Rz=function(a){_.A(this,a,0,-1,null,null)};_.w(Rz,_.z);Rz.prototype.getHeight=function(){return _.B(this,5)};
var Sz=function(a,c){a.wb=c;a.b&&(a.b=!0,a.wb&&a.wb.Y())},Tz=function(a){return a[a.length-1]},Uz=function(a,c){a=_.jk(a);var d=a[1],e=[];d&&(0,_.Ma)(d.split("&"),function(f){var g=f.indexOf("=");c.hasOwnProperty(0<=g?f.substr(0,g):f)||e.push(f)});a[1]=_.kk(e.join("&"),_.ok(c));return a[0]+(a[1]?"?"+a[1]:"")+a[2]};
var Vz=function(){window.addEventListener("message",function(a){"verify-origin"===a.data&&a.source.parent===window&&a.source.postMessage("verify-origin-reply",a.origin)})};
var Wz=function(){};
var Xz=function(a){this.b=a||{}};_.w(Xz,Wz);var $z=function(){Yz||(Yz=new Xz,-1==_.Ua.toLowerCase().indexOf("webkit")||_.x("Edge")?_.ab()?Zz("-moz-"):_.$a()?Zz("-ms-"):_.x("Opera")&&Zz("-o-"):Zz("-webkit-"),Yz.b.is_rtl=!1);var a=Yz.b.is_rtl;return!(null==a||!a)},Zz=function(a){Yz.b.css3_prefix=a};
var Yz=null;
var Iz=/['"\(]/,Lz=["border-color","border-style","border-width","margin","padding"],Jz=/left/g,Kz=/right/g,Mz=/\s+/;
var fA=function(a){if(null==a)return"";if(!aA.test(a))return a;-1!=a.indexOf("&")&&(a=a.replace(bA,"&amp;"));-1!=a.indexOf("<")&&(a=a.replace(cA,"&lt;"));-1!=a.indexOf(">")&&(a=a.replace(dA,"&gt;"));-1!=a.indexOf('"')&&(a=a.replace(eA,"&quot;"));return a},bA=/&/g,cA=/</g,dA=/>/g,eA=/"/g,aA=/[&<>"]/;
var gA=function(a){var c=a.match(/\bhref="/g);if(!c||1>=c.length)return a;var d=new _.wm;a=a.replace(/\bhref="(.*?)"/g,function(e,f){e=_.Pm(f);d.j||_.xm(d,e.j);d.f||_.ym(d,e.f);d.o||_.Am(d,e.o);d.w||_.Dm(d,e.w);f=_.ba(e.b.kb());for(var g=f.next();!g.done;g=f.next())g=g.value,_.Tm(d.b,g)||_.Um(d.b,g,e.b.Pa(g));return""});a=a.replace(/\s\s+/g," ").replace(/\s+$/g,"");return a+' href="'+d.toString()+'"'},hA=function(a){return""===a?"":' class="'+(" "===a.charAt(a.length-1)?a.slice(0,-1):a)+'"'},iA=function(a){return""!==
a?' style="'+a+'"':""};
var jA=function(a){this.b=a=void 0===a?document:a;this.j=null;this.f=[]};jA.prototype.document=function(){return this.b};var kA=function(a){var c=a.b.createElement("STYLE");a.b.head?a.b.head.appendChild(c):a.b.body.appendChild(c);return c},lA=function(a){if(!a.b||0==a.f.length)return"";var c=a.f.join("");if(_.y){a.j||(a.j=kA(a));var d=a.j}else d=kA(a);d.styleSheet&&!d.sheet?d.styleSheet.cssText+=c:d.textContent+=c;a.f.length=0;return""};
var mA=function(){var a=void 0===a?document:a;var c=void 0===c?new jA(a):c;this.w=a;this.o=c;new function(){};this.j={};this.b=[$z()]};mA.prototype.document=function(){return this.w};
var nA=function(a,c,d,e,f,g,h,l,m,n){var r="",v="",N="";g=void 0===g?null:g;h=void 0===h?null:h;r=void 0===r?"":r;l=void 0===l?null:l;v=void 0===v?"":v;m=void 0===m?null:m;N=void 0===N?"":N;n=void 0===n?null:n;a=a.j;if("array"!=_.Aa(d)){var D=[],P;for(P in d)D[d[P]]=P;d=D}a[c]={Ta:d,xl:e,yl:f,El:g,Al:h,Fl:r,Bl:l,Gl:v,Cl:m,Hl:N,Dl:n,zl:!0}};
var oA=function(a,c,d,e){this.parent=a;this.o=c;this.f=d;this.j=e?e:0},pA=function(a,c){var d={origin:document.location.protocol+"//"+document.location.host};0!==a.f&&(d.pid=a.f);0!==a.j&&(d.spid=a.j);a=Uz(a.o,d);c&&(c=_.ok(c),a=_.lk(a,c));return a},qA=function(a,c,d){if(a.b)return a.b;a.b=_.He("gapi.iframes.getContext")().openChild({attributes:{role:"presentation",style:{height:"100%",visibility:"hidden"},onload:c},where:a.parent,url:pA(a,d),dontclear:!0,hintInFragment:!0});return a.b};
var rA=function(a,c){_.Le.call(this,a,c)};_.p(rA,_.Le);
var sA=function(a,c,d,e,f){f=void 0===f?{}:f;_.Q.call(this);this.j=!1;this.A=a;this.b=null;this.f=new oA(this.A,c,/^\d+$/.test(d)?parseInt(d,10):0,/^\d+$/.test(e)?parseInt(e,10):0);this.w=f};_.p(sA,_.Q);var tA=function(a){if(a.j)return 3;a.j=!0;if(!_.He("gapi.iframes.getContext")){var c=_.He("gapi.load");if(!c)return 2;c("gapi.iframes",(0,_.t)(a.o,a));return 1}a.o();return 0};sA.prototype.getIframeEl=function(){return this.b?this.b.getIframeEl():null};var uA=function(a){return pA(a.f,a.w)};
sA.prototype.focus=function(){this.b.getIframeEl().focus()};var vA=function(a,c){a.b&&_.Jg(a.b.getIframeEl(),{visibility:c?"":"hidden"})};sA.prototype.o=function(){var a=this;_.He("gapi.iframes.getContext")&&(this.b=qA(this.f,function(){a.dispatchEvent("loaded")},this.w),wA(this,this.b))};var wA=function(a,c){_.Xa(xA,function(d){c.register(d,function(e){var f=new rA(d,a);f.data=e;a.dispatchEvent(f)},_.He("gapi.iframes.CROSS_ORIGIN_IFRAMES_FILTER"))})};
sA.prototype.remove=function(){var a=this.getIframeEl();a&&a.parentNode.removeChild(a)};var xA={xk:"blur",yk:"caev",Bk:"close",Ek:"dismiss",Nk:"_ready",Ok:"alogc",Pk:"alogn",Qk:"alogma",Sk:"alogmm",Rk:"alogm",Tk:"plog",al:"_renderfailed",bl:"_renderstart",el:"restyle",il:"savec",jl:"savek",kl:"_startuploaded",ol:"unload"};
var yA=["a","er_em","lc"],zA=function(a,c,d){this.o=_.on;this.A=a;this.j=c;this.w=d;this.f=this.b=!1};zA.prototype.log=function(a,c,d,e,f){yA.includes(a)||this.A.log(this.j.toString(),"7",a,"&ap=1"+c,d);if("i"===a){if(this.f)return;this.b&&(a="rl",this.f=!0);this.b=!0}_.Vn(this.o,a,this.j,this.w,e,!0,!0,f)};
var AA=function(a){this.f=a;this.b=!1};AA.prototype.La=function(){this.f.La()};
var CA=function(a,c,d){_.Q.call(this);this.f=new _.vg(this);_.Yf(this,this.f);this.b=a;this.Ga=c;this.V=new _.Tp(c,!0);this.A=_.ze("DIV");this.j=null;this.B=this.ma=this.Z=this.U=this.X=this.ka=this.O=this.$=this.K=this.G=!1;this.Ja=_.B(a,33)||"_renderstart";this.o=this.M=null;this.W=this.N=this.R=!1;this.S=d;this.J=null;a=this.A;c={};_.Za(c,BA,{position:"absolute"});this.b.getHeight()?c.height=this.b.getHeight()+"px":c.bottom="0px";_.B(this.b,6)&&(c.width=_.B(this.b,6)+"px");(d=_.B(this.b,7))&&(c["margin-top"]=
d+"px");if(3!=_.B(this.b,17))if(d){var e=_.wq(this.S).b;c["max-height"]="calc("+-1*(e+d)+"px + 100vh)"}else c["max-height"]="100vh";(d=_.C(this.b,11))?c.left=0:c.right=0;_.B(this.b,8)&&(d?c["margin-left"]=_.B(this.b,8)+"px":c["margin-right"]=_.B(this.b,8)+"px");_.Jg(a,c);this.S.appendChild(this.A)};_.p(CA,_.Q);CA.prototype.C=function(){return this.A};
var HA=function(a,c){DA(a);(a.B=c)?a.G?(EA(a,!0),vA(a.j,!0),a.dispatchEvent("rav"),null!=_.B(a.b,18)&&a.ua&&(c=a.D?_.rk(a.D):new _.Cc,_.F(c,24,Date.now()-a.ua),null!=a.va&&_.F(c,41,a.va),FA(a,_.B(a.b,18),c))):a.N?GA(a):a.dispatchEvent("sorp"):(EA(a,!1),vA(a.j,!1),a.dispatchEvent("h"))};CA.prototype.isVisible=function(){var a="hidden"!=this.A.style.visibility;return"none"!=this.A.style.display&&a};
var EA=function(a,c){_.Jg(a.A,{visibility:c?"":"hidden"})},JA=function(a,c,d,e){a.j=c;_.Be(d)?a.o=d:a.M=d;IA(a,e);if((c=_.C(a.b,10)||_.E(a.b,27,0))||null!=a.M)d=_.E(a.b,27,0),null==a.w&&0<d?a.w=_.rg(a.T,d,a):a.T();!c&&_.C(a.b,24)&&(c=_.ze("LINK"),d=uA(a.j)+"&usegapi=1",c.crossOrigin="use-credentials",_.oc&&(c.addEventListener("load",function(){a.Z=!0}),c.addEventListener("error",function(){a.ma=!0})),_.ie(c,d,"prefetch"),document.head.appendChild(c))},KA=function(a){_.zg(a.f);a.o.removeAttribute("data-ogsr-fb")};
CA.prototype.Y=function(){null!=_.B(this.b,31)&&FA(this,_.B(this.b,31));HA(this,!0)};
var IA=function(a,c){a.f.H(a.j,"_ready",a.Jj);a.f.H(a.j,"_startuploaded",function(){a.ka=!0});a.f.H(a.j,"_renderfailed",a.Oj);a.f.H(a.j,"_renderstart",a.Pj);a.f.H(a.j,"loaded",function(){a.X=!0});a.f.H(a.j,a.Ja,a.lk);_.C(a.b,9)&&a.f.H(a.j,"blur",a.Ej);a.f.H(a.j,"restyle",a.Qj);a.f.H(a.j,"unload",a.Hj);a.f.H(a.j,"close",a.ug);c&&0<c.length&&(0,_.Ma)(c,function(d){return _.ph(a.f,d,a.ug)});null!=a.o?(a.f.H(a.o,["mouseover","focus"],a.Uj),_.ph(a.f,a.o,a.Cg),a.f.H(a.o,"keydown",function(d){27==d.keyCode&&
a.isVisible()&&(a.W=!0,a.Cg(d))}),1==_.B(a.b,17)&&(a.f.H(a.j,"alogn",a.Cj),a.f.H(a.j,"alogm",a.Lj),a.f.H(a.j,"alogmm",a.Mj),a.f.H(a.j,"alogma",a.Kj),a.f.H(a.j,"alogc",a.Bj)),a.f.H(window,["keyup","keydown"],a.Rj),_.y&&a.f.H(a.o,"focusin",function(){a.R=!0}),_.Bh(a.o,"click"),(c=a.o.querySelector("[data-eqid]"))&&_.Bh(c,"click")):null!=a.M&&(Sz(a.M,a),a.f.H(a.j,"plog",a.Ug));a.f.H(window,"beforeunload",a.Dj)};_.k=CA.prototype;
_.k.Pj=function(a){this.$=!0;null!=_.B(this.b,32)&&FA(this,_.B(this.b,32));a.data&&("null"!==a.data.ttf&&(this.va=Number(a.data.ttf)||null),(a.data.height||a.data.width)&&LA(this,a.data.height,a.data.width))};_.k.Jj=function(){this.K=!0};_.k.Ug=function(a){"i"===a.data.ld.apatk&&FA(this,110)};_.k.Dj=function(){this.U=!0;null!=this.w&&(_.sg(this.w),this.w=null);this.isVisible()||this.K||this.j.remove()};_.k.lk=function(){this.G=!0;null!=this.F&&_.sg(this.F);HA(this,this.B)};
var DA=function(a){null!=a.w&&(_.sg(a.w),a.w=null);var c=tA(a.j);null==a.J&&(a.J=c);if(3!=c){if(c=_.B(a.b,14))a.F=_.rg(a.Aa,c,a);null!=_.B(a.b,30)&&FA(a,_.B(a.b,30))}};CA.prototype.T=function(){var a=this;"complete"==document.readyState?DA(this):window.addEventListener("load",function(){return DA(a)})};CA.prototype.Aa=function(){this.G||this.O||(this.N=!0,this.B&&GA(this))};var GA=function(a){null!=_.B(a.b,16)&&FA(a,_.B(a.b,16));a.dispatchEvent("sort")};_.k=CA.prototype;
_.k.Oj=function(){this.O=!0;null!=this.F&&_.sg(this.F);null!=_.B(this.b,26)&&this.B&&FA(this,_.B(this.b,26))};_.k.Cg=function(a){this.ua=Date.now();var c=!_.ug(a);c=void 0===c?!1:c;var d=!this.isVisible();HA(this,d);var e=this.j,f={};f.keyboardAction=void 0===c?!1:c;e.b&&e.b.send(d?"open":"close",f,void 0,_.He("gapi.iframes.CROSS_ORIGIN_IFRAMES_FILTER"));if(d?null!=_.B(this.b,12):null!=_.B(this.b,13))c=d?_.B(this.b,12):_.B(this.b,13),FA(this,c);this.R=!1;a.preventDefault();a.stopPropagation()};
_.k.Rj=function(a){32==a.keyCode&&a.target instanceof Element&&_.hg(this.o,a.target)&&(a.stopPropagation(),a.preventDefault())};_.k.Uj=function(){DA(this)};_.k.Qj=function(a){a.data&&LA(this,a.data.height,a.data.width)};var LA=function(a,c,d){c=void 0===c?"":c;d=void 0===d?"":d;var e={};c&&(e.height=c);d&&(e.width=d);_.Jg(a.A,e)};_.k=CA.prototype;_.k.Ej=function(){document.activeElement==this.o||_.hg(this.o,document.activeElement)||this.R||HA(this,!1)};_.k.Hj=function(){this.G=!1;HA(this,!1)};
_.k.ug=function(){HA(this,!1)};_.k.Cj=function(a){var c=Number(a.data.pid)||-1,d=a=a.data.vis;if(4<a||0>=a)d=0;a=d;d=new _.Cc;c=_.F(d,15,c);c=_.tn(c,MA(this));_.Wp(this.V,a,c)};_.k.Lj=function(){FA(this,104)};_.k.Mj=function(){FA(this,105)};_.k.Kj=function(a){a=a.data.an;var c=_.tn(new _.Cc,MA(this));_.Vp(this.V,a,c)};_.k.Bj=function(a){FA(this,a.data.mouseSession?99:100)};
var MA=function(a){var c=a.j&&a.j.getIframeEl(),d=0;a.K&&(d|=1);a.ka&&(d|=128);a.$&&(d|=32);a.O&&(d|=64);a.isVisible()&&(d|=2);a.N&&(d|=4);c&&(d|=8);a.X&&(d|=16);_.He("gapi.iframes")&&(d|=256);a.Z&&(d|=512);a.ma&&(d|=1024);a.W&&(d|=2048);switch(a.J){case 2:d|=4096;break;case 1:d|=8192}a.U&&(d|=16384);a.B&&(d|=32768);return d},FA=function(a,c,d){d=d||(a.D?_.rk(a.D):new _.Cc);_.tn(d,MA(a));if(null!=_.B(a.b,19)){var e=_.H(a.b,Oz,19);e=_.B(e,1);_.F(d,31,e);_.F(d,34,!0)}a.Ga.log(c,d)},BA={overflow:"hidden",
top:"0",visibility:"hidden",width:"350px","z-index":991};
var NA=function(a,c,d,e){_.Q.call(this);this.j=a;this.f=c;this.w=e;this.b=new _.vg(this);_.Yf(this,this.b);this.o=d;this.b.H(this.j,"plog",this.B);this.b.H(this.j,"savec",this.A);this.b.H(this.j,"savek",this.A);this.b.H(this.j,"caev",this.A);this.b.nb(this.f,"rav",this.D);this.b.nb(this.j,"dismiss",this.G)};_.p(NA,_.Q);NA.prototype.D=function(){var a=this.w;a.b||(_.Mn(a.f),a.b=!0);this.o.log("i","&vis=1",1,this.f.C(),MA(this.f))};
NA.prototype.G=function(a){a=a.data&&a.data.type?a.data.type:"d";this.w.La();this.o.log(a,"",1,this.f.C(),MA(this.f))};NA.prototype.A=function(a){switch(a.data.apatk){case "c":(a=_.He("window.launchConsentDialog"))&&a();break;case "d":this.w.La()}};NA.prototype.B=function(a){var c=a.data.ld;a=c.apatk;if("i"!=a){var d=c.sp;c=c.ad;var e=this.f.C(),f=MA(this.f);this.o.log(a,c,d,e,f)}};
var OA=function(a){this.b=a};OA.prototype.Ha=function(){var a=this.b,c=this.j,d=this.f;PA(a);c="<div"+hA("")+iA(QA(a,c,d)+"")+gA(RA(a,c,d)+"")+">";d=SA(d);var e=lA(a.o);""!==e&&(c+=" <style>"+e+"</style>");c+=d+"</div>";a.f&&a.f.Cc();return _.mq(document,_.Fb(c,null))};OA.prototype.fill=function(a,c){this.j=a;this.f=c};
var RA=function(){return' dir="'+fA("ltr")+'"'},TA=function(){return""},QA=function(a,c,d){return"padding:"+fA(Tz(a.b)?Nz("padding",c?"12px":"3px"):c?"12px":"3px")+";"+(d?"":"display:"+fA(Tz(a.b)?Nz("display","inline-block"):"inline-block")+";")+"vertical-align:"+fA(Tz(a.b)?Nz("vertical-align","middle"):"middle")+";"+(d&&!Tz(a.b)?"margin-left:"+fA("calc(50% - 24px)")+";":"")+(d&&Tz(a.b)?"margin-right:"+fA("calc(50% - 24px)")+";":"")+(d?"margin-top:"+fA(Tz(a.b)?Nz("margin-top","98px"):"98px")+";":
"")},UA=function(){return!0},VA=function(){return!1},WA=function(a,c){PA(a);return SA(c.qg)},XA=function(a,c){PA(a);var d=c.Vi;c=c.qg;a="<div"+hA("")+iA(QA(a,d,c)+"")+gA(RA(a,d,c)+"")+">";d=SA(c);return _.Fb(a+(d+"</div>"),null)},SA=function(a){return" <div"+hA((a?"mspin-medium ":"")+(a?"":"mspin-small "))+iA("")+gA("")+"> <div> <div></div> </div> </div> "},PA=function(a){YA in a.j||nA(a,YA,{Vi:0,qg:1},WA,XA,UA,VA,RA,TA,QA)},YA="t-s91B_Xq1PdE",ZA=function(a){this.b=a};
ZA.prototype.Ha=function(){var a=this.b;$A(a);var c="<div"+hA("")+iA(aB(a)+"")+gA("")+">";var d=lA(a.o);""!==d&&(c+=" <style>"+d+"</style>");c+="</div>";a.f&&a.f.Cc();return _.mq(document,_.Fb(c,null))};ZA.prototype.fill=function(){};
var bB=function(){return""},cB=function(){return""},aB=function(a){return"background:#FFF;box-shadow:0 -1px 2px 0 rgba(60,64,67,0.30),0 -2px 6px 2px rgba(60,64,67,0.15);height:calc(100% - 16px);"+(Tz(a.b)?"":"left:0;")+(Tz(a.b)?"right:0;":"")+"margin:8px;position:absolute;top:0;width:calc(100% - 16px);"},dB=function(){return!0},eB=function(){return!1},fB=function(a){$A(a);return""},gB=function(a){$A(a);a="<div"+hA("")+iA(aB(a)+"")+gA("")+">";return _.Fb(a+"</div>",null)},$A=function(a){hB in a.j||
nA(a,hB,{},fB,gB,dB,eB,bB,cB,aB)},hB="t-LSLm3aJIFAU",iB=function(a){this.b=a};iB.prototype.Ha=function(){var a=this.b,c=this.j,d=this.o,e=this.f;jB(a);var f="<div"+hA("")+iA(kB(a,c,d,e)+"")+gA("")+">";c=lB(c,d,e);d=lA(a.o);""!==d&&(f+=" <style>"+d+"</style>");f+=c+"</div>";a.f&&a.f.Cc();return _.mq(document,_.Fb(f,null))};iB.prototype.fill=function(a,c,d){this.j=a;this.o=c;this.f=d};
var mB=function(){return""},nB=function(){return""},kB=function(){return"font:14px/22px Roboto,RobotoDraft,Arial,sans-serif;color:#5F6368;letter-spacing:0.03px;padding:134px 50px;text-align:center;white-space:normal;"},oB=function(){return!0},pB=function(){return!1},qB=function(a,c){jB(a);return lB(c.Af,c.lg,c.xf)},rB=function(a,c){jB(a);var d=c.Af,e=c.lg;c=c.xf;a="<div"+hA("")+iA(kB(a,d,e,c)+"")+gA("")+">";d=lB(d,e,c);return _.Fb(a+(d+"</div>"),null)},lB=function(a,c,d){return' <svg height="28px" viewbox="0 0 24 24" width="28px" xmlns="http://www.w3.org/2000/svg"> <path d="M12 2C6.48 2 2 6.48 2 12s4.48 10 10 10 10-4.48 10-10S17.52 2 12 2zm1 15h-2v-2h2v2zm0-4h-2V7h2v6z" fill="#80868B"></path> </svg> <p'+
hA("")+iA("margin-top:4px;")+gA("")+"> "+fA(a)+" <a"+hA("")+iA("color:#4285F4;font:14px/22px Roboto,RobotoDraft,Arial,sans-serif;font-weight:bold;letter-spacing:0.03px;text-decoration:none;")+gA(' target="_blank"')+">"+fA(c)+"</a> "+fA(d)+" </p> "},jB=function(a){sB in a.j||nA(a,sB,{Af:0,lg:1,xf:2},qB,rB,oB,pB,mB,nB,kB)},sB="t-PFKuGYhRe5s";
var tB=function(a,c,d,e){_.Q.call(this);this.b=a;this.G=c;this.M=d;this.B=e;this.K=0;this.w=null;this.o=0;this.O=!0;this.D=null;this.N=!1;this.F=new mA;this.J=this.f=this.A=null;this.R=!1;this.j=new _.vg(this);_.Yf(this,this.j);_.Jg(this.b.C(),{transition:"height .3s ease-in-out"});this.j.H(this.b,"sorp",this.yf);this.j.H(this.b,"sort",this.$i);this.j.H(this.b,"rav",this.hj);this.j.H(this.b,"h",this.Gj);this.j.H(this.G,"close",this.fj)};_.p(tB,_.Q);_.k=tB.prototype;
_.k.hj=function(){uB(this);this.A&&this.A.ha(!1);this.G.focus();this.B.setAttribute("aria-expanded",!0)};_.k.Gj=function(){this.B.setAttribute("aria-expanded",!1)};_.k.fj=function(){this.B.focus()};
_.k.$i=function(){var a=this;switch(this.K){case 2:uB(this);KA(this.b);EA(this.b,!1);this.B.click();break;case 1:this.w&&_.sm(top.location,_.wb(this.w));case 3:vB(this)}if(this.N){var c=_.ze("IFRAME"),d=_.O(window,"message",function(e){if("afbp"===e.ab.data){e=a.b;switch(_.B(e.b,17)){case 1:FA(e,73)}a.b.C().removeChild(c);_.gf(d)}});_.of(c,wB);c.style.display="none";this.b.C().appendChild(c)}};
_.k.yf=function(){this.f&&uB(this);if(!this.J){if(!this.R){var a=1==this.o?xB:yB;var c=_.ze("LINK");_.ie(c,a,"stylesheet");document.head.appendChild(c);this.R=!0}a=new OA(this.F);a.fill(this.O,1==this.o);this.J=a.Ha()}a=this.J;switch(this.o){case 1:this.f=(new ZA(this.F)).Ha();this.f.appendChild(a);this.b.C().appendChild(this.f);vA(this.G,!1);EA(this.b,!0);break;default:this.f=a,_.X(this.M,!1),_.sh(this.f,this.M)}};
var vB=function(a){a.yf();if(1==a.o&&a.w&&a.D){_.fg(a.f);var c=new iB(a.F);zB(c,a.D);c=c.Ha();var d=c.querySelectorAll("a")[0];_.qh(d,a.w);a.j.H(d,"click",function(){var e=a.b;null!=_.B(e.b,21)&&FA(e,_.B(e.b,21))});a.f.appendChild(c)}},uB=function(a){a.f&&(_.Ae(a.f),1!=a.o&&_.X(a.M,!0),a.f=null)},zB=function(a,c){c=/(.*)%1\$s(.*)%2\$s(.*)/.exec(c);a.fill(c[1],c[2],c[3])},wB=_.nf(_.ib("https://www.gstatic.com/gb/html/afbp.html")),yB=_.nf(_.ib("https://www.gstatic.com/images/icons/material/anim/mspin/mspin_googcolor_small.css")),
xB=_.nf(_.ib("https://www.gstatic.com/images/icons/material/anim/mspin/mspin_googcolor_medium.css"));
var AB=function(a,c){this.f=a;this.b=c};_.k=AB.prototype;_.k.Bd=function(){return this.f};_.k.me=function(a){HA(this.b,a)};_.k.ng=function(){return!0};_.k.Rb=function(){return this.b.isVisible()};_.k.le=function(){};
_.BB=function(a){if(a){var c=document.querySelector("#gb [data-ogsr-up]");if(c){var d=0!==_.E(a,7,0),e=_.Zj(a,Rz,1);if(d||e&&e.length){Vz();d=_.Vc.ta().b.dd||null;for(var f=0;f<e.length;f++){var g=e[f];if(_.B(g,3)){var h=new CA(g,_.on,c),l=h.C(),m=a,n={};switch(_.B(g,17)){case 3:var r=_.H(g,Oz,19);r&&(n.prid=_.B(r,1).toString(),n.pgid=_.B(r,2).toString(),n.puid=_.B(r,10));break;case 1:n.gm=""}l=new sA(l,_.B(g,3),_.B(m,4),_.B(m,5),n);if(3===_.B(g,17)){m=_.H(g,Oz,19);n=g=0;m&&(g=_.B(m,1),n=_.B(m,2));
r=new _.Cc;_.F(r,31,g);h.D=r;var v=_.M("gb_Uc");r=Array.from(_.rh("gb_D",v));(v=_.M("gb_ia",v))&&_.Eg(r,void 0,0,v);JA(h,l,_.Wn.ta(),r);n=_.Tn(_.yd,_.Vc.ta().b.p_st||null,_.B(m,8)||0,_.E(m,5,0),n.toString(),_.E(m,4,25),g.toString(),_.B(m,9)||0,null,_.B(m,6)||void 0,_.B(m,7)||void 0);m=new AA(n);n=n.Zb();r=_.Wc(_.Vc.ta(),"p_log");new NA(l,h,new zA(r,g,n),m)}else if(m=null,1===_.B(g,17)?(m=document.querySelector("#gb [data-ogsr-alt]"),d.o(new AB("app",h))):2===_.B(g,17)&&(m=(m=_.M("gb_Pa"))?_.M("gb_D",
m):null,d.o(new AB("account",h))),null!=m&&(JA(h,l,m),h=new tB(h,l,m,m.getElementsByClassName("gb_D")[0]||m),r=_.B(g,15),l=_.C(a,6),n=_.B(g,22),v=_.E(g,23,0),h.K=v,h.w=r,r=h,v=_.B(g,20),r.o=v,r.O=l,r.D=n,n=r,r=!!_.C(g,25),n.N=r,l&&1===_.B(g,17)&&(g=_.M("gb_Md"))))g=new _.Er(m,g),h.A&&h.A.sa(),h.A=g}else _.yd.log(Error("Sa"))}}else _.yd.log(Error("Ta"))}else _.yd.log(Error("Ua"))}else _.yd.log(Error("Va"))};

}catch(e){_._DumpException(e)}
try{
_.BB(_.H(_.ud,_.Qz,21));

}catch(e){_._DumpException(e)}
try{
var tE=function(a){_.A(this,a,0,-1,null,null)};_.w(tE,_.z);
if(null==_.H(_.ud,tE,20))_.yd.log(Error("eb"));else{var uE;a:{try{if(document.domain==window.top.document.domain){var vE=/google\.(com?\.)?[a-z]{2,3}$/.exec(document.domain);uE=vE&&vE[0];break a}}catch(a){}uE=null}var wE=uE;if(wE){var xE=new Date;_.Sj.set("1P_JAR",[xE.getUTCFullYear(),xE.getUTCMonth()+1,xE.getUTCDate(),xE.getUTCHours()].join("-"),{je:2592E3,path:"/",domain:wE,$j:!0})}}
;
}catch(e){_._DumpException(e)}
try{
var Wq,Yq;_.Xq=function(a,c,d){return Wq(a,c,d).then(function(e){var f=e.responseText;d&&d.uf&&(e=d.uf,_.$d(f,e)&&(f=f.substring(e.length)));return JSON.parse(f)})};
Wq=function(a,c,d){var e=d||{},f=e.uk?e.uk.b():_.Vj.b();return _.Lf(new _.Gf(function(g,h){var l;try{f.open("POST",a,!0)}catch(r){h(new Yq("Error opening XHR: "+r.message,a,f))}f.onreadystatechange=function(){if(4==f.readyState){_.q.clearTimeout(l);var r;!(r=_.Tj(f.status))&&(r=0===f.status)&&(r=_.ik(a),r=!("http"==r||"https"==r||""==r));r?g(f):h(new Zq(f.status,a,f))}};f.onerror=function(){h(new Yq("Network error",a,f))};if(e.headers){for(var m in e.headers){var n=e.headers[m];null!=n&&f.setRequestHeader(m,
n)}n=e.headers["Content-Type"]}m=_.q.FormData&&c instanceof _.q.FormData;void 0!==n||m||f.setRequestHeader("Content-Type","application/x-www-form-urlencoded;charset=utf-8");e.withCredentials&&(f.withCredentials=e.withCredentials);e.responseType&&(f.responseType=e.responseType);e.mimeType&&f.overrideMimeType(e.mimeType);0<e.sf&&(l=_.q.setTimeout(function(){f.onreadystatechange=_.xa;f.abort();h(new $q(a,f))},e.sf));try{f.send(c)}catch(r){f.onreadystatechange=_.xa,_.q.clearTimeout(l),h(new Yq("Error sending XHR: "+
r.message,a,f))}}),function(g){g instanceof _.Mf&&f.abort();throw g;})};Yq=function(a,c){_.Ka.call(this,a+", url="+c);this.url=c};_.w(Yq,_.Ka);Yq.prototype.name="XhrError";var Zq=function(a,c,d){Yq.call(this,"Request Failed, status="+a,c,d);this.status=a};_.w(Zq,Yq);Zq.prototype.name="XhrHttpError";var $q=function(a,c){Yq.call(this,"Request timed out",a,c)};_.w($q,Yq);$q.prototype.name="XhrTimeoutError";
/*

 Copyright The Closure Library Authors.
 SPDX-License-Identifier: Apache-2.0
*/
var ar=function(){};_.w(ar,Error);
_.br=function(){this.b="pending";this.w=[];this.j=this.A=void 0};_.pf(_.br);var cr=function(){_.Ka.call(this,"Multiple attempts to set the state of this Result")};_.w(cr,_.Ka);_.br.prototype.ya=function(){return this.A};_.br.prototype.wait=function(a,c){"pending"==this.b?this.w.push({Mc:a,scope:c||null}):a.call(c,this)};_.br.prototype.o=function(a){if("pending"==this.b)this.A=a,this.b="success",dr(this);else if(!er(this))throw new cr;};
_.br.prototype.f=function(a){if("pending"==this.b)this.j=a,this.b="error",dr(this);else if(!er(this))throw new cr;};var dr=function(a){var c=a.w;a.w=[];for(var d=0;d<c.length;d++){var e=c[d];e.Mc.call(e.scope,a)}};_.br.prototype.cancel=function(){return"pending"==this.b?(this.f(new ar),!0):!1};var er=function(a){return"error"==a.b&&a.j instanceof ar};
_.br.prototype.then=function(a,c,d){var e,f,g=new _.Gf(function(h,l){e=h;f=l});this.wait(function(h){er(h)?g.cancel():"success"==h.b?e(h.ya()):"error"==h.b&&f(h.j)});return g.then(a,c,d)};_.fr=function(a){var c=new _.br;a.then(c.o,c.f,c);return c};
_.gr=function(a){var c=new _.br;c.o(a);return c};_.hr=function(a){var c=new _.br;c.f(a);return c};_.ir=function(a,c,d){a.wait(c,d)};_.jr=function(a,c,d){_.ir(a,function(e){"error"==e.b&&c.call(this,e.j,e)},d)};_.lr=function(a,c){var d=new _.kr([a]);_.ir(a,function(e){"success"==e.b?(e=c.call(void 0,e),d.B.push(e),_.ir(e,function(f){"success"==f.b?d.o(f.ya()):d.f(f.j)})):d.f(e.j)});return d};_.kr=function(a){_.br.call(this);this.B=a};_.w(_.kr,_.br);

}catch(e){_._DumpException(e)}
try{
var Ct=function(a){_.A(this,a,0,-1,null,null)};_.w(Ct,_.z);var Dt=function(a){_.A(this,a,0,-1,null,null)};_.w(Dt,_.z);var Et=function(a,c,d){_.ir(a,function(e){"success"==e.b&&c.call(this,e.ya(),e)},d)},Ft=function(a){_.A(this,a,0,-1,null,null)};_.w(Ft,_.z);
var Gt=function(){this.b={sf:3E3,withCredentials:!0,uf:")]}'\n"}},Ht=function(a,c,d,e){Et(a,c,e);_.jr(a,d,e)};
var It=function(a){_.A(this,a,"og.botreq",-1,null,null)};_.w(It,_.z);
var Kt=function(a){_.A(this,a,"og.botresp",-1,Jt,null)};_.w(Kt,_.z);var Jt=[1];
var Ot=function(){var a=Lt,c=Mt;this.U=parseInt(_.B(Nt,6),10)||0;this.T=_.B(a,9)||_.gk(_.B(a,5),void 0,_.B(a,7),_.B(a,6),_.B(a,3),_.B(a,8));_.B(a,4);this.M=_.B(a,10)||"";this.f=_.B(a,12);this.Lb=Math.max(6E4,_.Mc(_.B(a,1)));1===this.f&&(this.j=2E3);this.Sa=(_.C(a,13)||!1)&&(_.C(a,15)||!1);this.R=_.C(a,14)||!1;this.W=Math.floor(2147483647*Math.random());this.K=_.yd;this.S=new Gt;this.J=new _.wl(407,_.L(_.B(c,5)));this.F={};this.G="";this.b=null;this.A=0;this.D=this.B=!0};Ot.prototype.start=function(){this.O()};
Ot.prototype.O=function(){if(this.B){this.b&&432E5>(0,_.Ha)()-this.A?this.b.invoke((0,_.t)(this.w,this),!0):Pt(this);var a=this.Lb;1===this.f&&(this.j*=2,a=Math.min(this.j,this.Lb));window.setTimeout((0,_.t)(this.O,this),a)}};var Pt=function(a){var c=Qt(a);Ht(c,a.N,function(){},a)};Ot.prototype.o=function(a){a=_.B(a,1)[0];window.botguard&&window.botguard.bg?(this.b=new window.botguard.bg(a,function(){}),this.A=(0,_.Ha)(),this.b.invoke((0,_.t)(this.w,this),!0)):this.K.log(Error("za"))};
Ot.prototype.w=function(a){var c=new Ft;_.F(c,1,this.U);var d=1E3*(0,_.Ha)();_.F(c,2,d);_.F(c,3,a);_.F(c,4,this.W);_.F(c,5,this.Sa);_.F(c,6,this.R);a=new _.el;_.gl(a,c.f());_.fl(a);this.J.log(a);this.J.flush()};
Ot.prototype.N=function(a){if(_.C(a,5))this.B=!1;else if(1>_.B(a,1).length)this.K.log(Error("Aa"));else{var c=_.ze("SCRIPT");c.type="text/javascript";c.charset="UTF-8";if(null!=_.B(a,4)){var d=_.B(a,4);if(d in this.F){this.o(a);return}this.F[d]=!0;this.G=d||""}null!=_.B(a,3)?(d=_.H(a,_.Aj,3),d=_.qb(_.B(d,4)||""),_.je(c,d),c.onload=(0,_.t)(this.o,this,a),_.qe("HEAD")[0].appendChild(c)):null!=_.B(a,2)&&(this.M&&c.setAttribute("nonce",this.M),d=_.H(a,Dt,2),d=_.mb(_.B(d,6)||""),d instanceof _.lb&&d.constructor===
_.lb&&d.f===_.kb?d=d.b:(_.Aa(d),d="type_error:SafeScript"),c.text=d,(d=_.Xd())&&c.setAttribute("nonce",d),_.qe("HEAD")[0].appendChild(c),this.o(a),_.Ae(c))}};
var Qt=function(a){var c=new It;_.F(c,2,a.G);_.F(c,4,a.D);_.F(c,5,a.f);_.F(c,6,a.Sa);var d={"f.req":c.f()};c=Rt;var e=a.S,f=a.T;try{var g=_.ok(d||[]);var h=_.fr(_.Xq(f,g,e.b))}catch(l){h=new _.br,h.f(l)}return c(a,h)},Rt=function(a,c){return _.lr(c,(0,_.t)(function(d){try{var e=d.ya(),f=St(e[0]);if(0==f.length)throw Error("sa");var g=new Kt(f[0]);this.D=!1;return _.gr(g)}catch(h){return _.hr(h)}},a))},St=function(a){return(0,_.Na)(a,function(c){return 0<c.length&&"og.botresp"==c[0]})};
var Nt=_.vd(),Lt=_.H(_.ud,Ct,22),Mt=_.wd();Nt&&Lt&&Mt&&(new Ot).start();

}catch(e){_._DumpException(e)}
try{
var st=[1],tt=function(a){_.A(this,a,0,-1,st,null)};_.w(tt,_.z);
var vt=function(a){_.A(this,a,0,-1,ut,null)};_.w(vt,_.z);var wt=function(a){_.A(this,a,0,-1,null,null)};_.w(wt,_.z);var xt=function(a){_.A(this,a,0,-1,null,null)};_.w(xt,_.z);var ut=[12,24];
var Bt=function(){var a=yt,c=zt,d=At;this.o=_.B(c,1);this.D=Math.max(6E4,_.Mc(_.B(c,2)));this.b=null;this.B=parseInt(_.B(a,6),10)||0;this.G=Math.floor(2147483647*Math.random());this.j=new _.wl(78,_.L(_.B(d,5)));this.A=_.yd;this.f()};Bt.prototype.f=function(){null==this.b&&(this.b=(0,_.Oa)(this.o,function(a){return _.Ch(this.A,document,a,this.w,!0,this)},this))};
Bt.prototype.w=function(){_.Ma(this.b,_.gf);this.b=null;var a=new wt;_.F(a,7,this.B);_.F(a,8,this.G);_.F(a,2,1);var c=new xt;_.F(c,1,screen.width);_.F(c,2,screen.height);var d=new vt;_.tk(d,12,[a]);_.I(d,15,c);a=new _.el;_.gl(a,d.f());_.fl(a);this.j.log(a);this.j.flush();window.setTimeout((0,_.t)(this.f,this),this.D)};
var yt=_.vd(),zt=_.H(_.ud,tt,23),At=_.wd();yt&&zt&&At&&new Bt;

}catch(e){_._DumpException(e)}
try{
var Rp=function(){this.b=_.Xc("dd")};Rp.prototype.f=function(){this.b.w("aw");this.b.w("app")};
_.u("gbar.R",Rp);Rp.prototype.ra=Rp.prototype.f;_.rd(_.sd.ta().j,new Rp);

}catch(e){_._DumpException(e)}
})(this.gbar_);
// Google Inc.

